Principles of Quantum Communication Theory: A Modern Approach

This is a preliminary version of a book in progress on the theory of quantum communication. We adopt an information-theoretic perspective throughout and give a comprehensive account of fundamental results in quantum communication theory from the past decade (and earlier), with an emphasis on the modern one-shot-to-asymptotic approach that underlies much of today's state-of-the-art research in this field. In Part I, we cover mathematical preliminaries and provide a detailed study of quantum mechanics from an information-theoretic perspective. We also provide an extensive and thorough review of quantum entropies, and we devote an entire chapter to the study of entanglement measures. Equipped with these essential tools, in Part II we study classical communication (with and without entanglement assistance), entanglement distillation, quantum communication, secret key distillation, and private communication. In Part III, we cover the latest developments in feedback-assisted communication tasks, such as quantum and classical feedback-assisted communication, LOCC-assisted quantum communication, and secret key agreement.

==> Chapters/QM_overview.tex <==


	This chapter provides an overview of quantum mechanics, placing particular emphasis on those aspects of quantum mechanics that are useful for the communication protocols that we discuss in later chapters. Quantum mechanics is the backbone for quantum information processing, and many aspects of it cannot be explained by classical reasoning. For example, there is no strong classical analogue for pure quantum states or entanglement, and this leads to stark differences between what is possible in the classical and quantum worlds. However, at the same time, it is important to emphasize that all of classical information theory is subsumed by quantum information theory, so that whatever is possible with classical information processing is also possible with quantum information processing. As such, quantum information subsumes classical information while allowing for richer possibilities. 
	
	%We start by stating the axioms of quantum mechanics. After that, we elaborate on the axioms in each section, 
	
	The mathematical description of quantum systems can be summarized by the following axioms. Each of these axioms is elaborated upon in the section indicated.
	\begin{enumerate}
	
		\item \textit{Quantum systems}: A quantum system $A$ is associated with a Hilbert space~$\mathcal{H}_A$. The state of the system $A$ is described by a \textit{density operator}, which is a unit-trace, positive semi-definite linear operator acting on $\mathcal{H}_A$. (See Section \ref{sec-state_meas}.)
		
		\item \textit{Bipartite quantum systems}: For distinct quantum systems $A$ and $B$ with associated Hilbert spaces $\mathcal{H}_A$ and $\mathcal{H}_B$, the composite system $AB$ is associated with the Hilbert space $\mathcal{H}_A\otimes\mathcal{H}_B$. (See Section \ref{subsec-bipartite_state}.)
		
		\item \textit{Measurement}: The measurement of a quantum system $A$ is described by a \textit{positive operator-valued measure (POVM)} $\{M_x\}_{x\in\mathcal{X}}$, which is defined to be a collection of positive semi-definite operators indexed by a finite alphabet satisfying $\sum_{x\in\mathcal{X}} M_x=\mathbbm{1}_{\mathcal{H}_A}$.\footnote{POVMs need not contain a finite number of elements, but we consider POVMs with a finite number of elements exclusively throughout this book.} $\mathcal{X}$ If the system is in the state $\rho$ and the measurement outcome is described by a random variable $X$, then the probability $\Pr[X=x]$ of obtaining the outcome $x$ is given by the \textit{Born rule} as
			\begin{equation}
				\Pr[X=x]=\Tr[M_x\rho].
			\end{equation}
			Furthermore, a physical \textit{observable} $O$ corresponds to a Hermitian operator acting on the underlying Hilbert space. Recall from the spectral theorem (Theorem~\ref{thm-spectral_theorem}) that $O$ has a spectral decomposition as follows:
			\begin{equation}	
			O = \sum_{\lambda\in\text{spec}(O)} \lambda \ \Pi_{\lambda},
			\end{equation}	
			where $\text{spec}(O)$ is the set of distinct eigenvalues of $O$ and $\Pi_\lambda$ is a spectral projection.  
			A measurement of $O$ is described by the POVM $\{\Pi_\lambda\}_{\lambda}$,  which is indexed by the distinct eigenvalues $\lambda$ of $O$.
			The expected value $\left<O\right>_{\rho}$ of the observable $O$ when the state is $\rho$ is given by
			\begin{equation}	
				\left<O\right>_\rho\coloneqq\Tr[O\rho] = \sum_{\lambda\in\text{spec}(O)} \lambda \Tr[\Pi_\lambda\rho].
			\end{equation}
			(See Section \ref{subsec-meas}.)
		\item \textit{Evolution}: The evolution of the state of a quantum system is described by a \textit{quantum channel}, which is a linear, completely positive, and trace-preserving map acting on the state of the system. (See Section \ref{sec-channel}.)
	\end{enumerate}
	
	Note that the second axiom for the description of bipartite quantum systems is sufficient to conclude that the multipartite quantum system $A_1A_2\dotsb\allowbreak A_k$, comprising $k$ distinct quantum systems $A_1,A_2,\dotsc, A_k$, is associated with the Hilbert space $\mathcal{H}_{A_1}\otimes\mathcal{H}_{A_2}\otimes\dotsb\otimes\mathcal{H}_{A_k}$. 
	
	%We briefly summarize these axioms in this chapter, providing the necessary definitions and theorems required for the subsequent chapters.



\section{Quantum Systems, States, and Measurements}\label{sec-state_meas}

	Each quantum system is associated with a Hilbert space. In this book, we consider only finite-dimensional quantum systems, that is, quantum systems described by finite-dimensional Hilbert spaces. In the following, we provide a mathematical description of all possible finite-dimensional quantum systems, along with examples of how these systems can be physically realized. 
	
	\begin{enumerate}
		\item \textit{Qubit systems}: The qubit is perhaps the most fundamental quantum system and is the quantum analogue of the (classical) bit. Every physical system with two distinct degrees of freedom obeying the laws of quantum mechanics can be considered a qubit system. The Hilbert space associated with a qubit system is $\mathbb{C}^2$, whose standard orthonormal basis is  denoted by $\{\ket{0},\ket{1}\}$. Three common ways of physically realizing qubit systems are as follows:
			\begin{enumerate}
				\item The two spin states of a spin-$\frac{1}{2}$ particle.
				\item Two distinct energy levels of an atom, such as the ground state and one of the excited states.
				\item Clockwise and counter-clockwise directions of current flow in a superconducting electronic circuit. 
			\end{enumerate}
		
		\item \textit{Qutrit systems}: A qutrit system is a quantum system consisting of three distinct physical degrees of freedom. The Hilbert space of a qutrit is $\mathbb{C}^3$, with the standard orthonormal basis denoted by $\{\ket{0},\ket{1},\ket{2}\}$. Qutrit systems are less commonly considered than qubit systems for implementations, although one important example of an implementation of a qutrit system occurs in quantum optical systems, which we discuss below. Like qubit systems, qutrit systems can also be physically realized using, for example, the spin states of a spin-1 atom or three distinct energy levels of an atom.
		
		\item \textit{Qudit systems}: A qudit system is a quantum system with $d$ distinct degrees of freedom and is described by the Hilbert space $\mathbb{C}^d$, with the standard orthonormal basis  denoted  by $\{\ket{0},\ket{1},\dotsc,\ket{d-1}\}$. The spin states of every spin-$j$ atom can be used to realize a qudit system with $d=2j+1$. Another physical realization of a qudit system is with the $d$ distinct energy levels of an atom.
		
		\item \textit{Quantum optical systems}: An important quantum system, particularly for the implementation of many quantum communication protocols, is a qu\-antum optical system. By a quantum optical system we mean a physical system, such as an optical cavity or a fiber-optic cable, in which modes of light, with photons as information carriers, propagate. A mode of light has a well defined  momentum, frequency, polarization, and spatial direction. 
			
			Formally, a quantum optical system with $d$ distinct modes is described by the Fock space $\mathcal{F}_{\text{B}}(\mathbb{C}^d)$, which is a Hilbert space equipped with the orthonormal occupation number basis $\{\ket{n_1,\allowbreak\dotsc, n_d}:n_1,\dotsc,n_d\allowbreak \geq 0\}$, where $n_j$, for $1\leq j\leq d$, indicates the number of photons occupied in mode~$j$. See \eqref{eq:math-tools:occupation-num-basis} and the surrounding discussion for a brief review of the occupation number basis and Fock space.
			
			The Fock space is infinite dimensional, but by restricting to particular subspaces, it is possible use photons to physically realize finite-dimensional qua\-ntum systems. The following two realizations of a qubit system are particularly important:
			\begin{enumerate}
				\item A single-mode optical system, with Hilbert space $\mathcal{F}_{\text{B}}(\mathbb{C})$, restricted to the subspace spanned by the states $\{\ket{0},\ket{1}\}$, consisting of either zero or one photon occupied in the mode. The state $\ket{0}$ corresponding to no photons is commonly called the \textit{vacuum state} of the mode.
				\item A two-mode optical system, with Hilbert space $\mathcal{F}_{\text{B}}(\mathbb{C}^2)$, restricted to the subspace span\-ned by the orthogonal states $\{\ket{0,1},\allowbreak\ket{1,0}\}$, consisting of only one photon in total occupying either one of the two modes. This realization of a qubit system is commonly called the \textit{dual-rail encoding} because it makes use of two modes of light. Two distinct polarization degrees of freedom of photons, such as horizontal and vertical polarizations, are commonly used as the two modes in dual-rail encodings of a qubit. One then usually lets $\ket{H}\equiv\ket{0,1}$ and $\ket{V}\equiv\ket{1,0}$ denote a horizontally- and vertically-polarized photon, respectively.
				
					By considering the three-dimensional subspace spanned by $\{\ket{0,0},\ket{0,1},\allowbreak\ket{1,0}\}$, that is, the dual-rail qubit system with the additional orthogonal vacuum state $\ket{0,0}$ of the two modes, we obtain a physical realization of a qutrit system. This particular realization of a qutrit system is relevant for communication protocols in the context of the erasure channel, which is discussed in Section \ref{subsec-qubit_channel}.
			\end{enumerate}
			
	
	\end{enumerate}
	
	Having discussed how a quantum system is mathematically described, let us now move on to the mathematical description of the state of a quantum system.
	
	\begin{definition}{Quantum State}{def-quantum_state}
		The state of a quantum system is described by a density operator acting on the underlying Hilbert space of the quantum system. A density operator is a unit-trace, positive semi-definite linear operator. Throughout the book, we identify a state with its corresponding density operator. We denote the set of density operators on a Hilbert space $\mathcal{H}$ as $\Density(\mathcal{H})$.	
	\end{definition}
	
	We typically use the Greek letters $\rho$, $\sigma$, $\tau$, or $\omega$ to denote quantum states.
	
	\begin{exercise}{exer-QM_states_convex}
		Prove that the set of quantum states is a \textit{convex set}. (Recall the definition of a convex set from Section~\ref{sec-math_tools_convexity}.) In other words, prove that for every alphabet $\mathcal{X}$ and set $\{\rho^x\}_{x\in\mathcal{X}}$ of quantum states, along with every probability distribution $p:\mathcal{X}\rightarrow[0,1]$, the following convex combination is a quantum state:
		\begin{equation}
			\rho=\sum_{x\in\mathcal{X}}p(x)\rho^x.
		\end{equation}
	\end{exercise}
	
	The extremal points in the convex set of quantum states are called \textit{pure states}. A pure state is a unit-rank projection onto a vector in the Hilbert space. Concretely, pure states are of the form $\ket{\psi}\!\bra{\psi}$ for every normalized vector $\ket{\psi}\in\mathcal{H}$. For convenience, we sometimes denote $\ket{\psi}\!\bra{\psi}$ simply as $\psi$ and refer to the vector $\ket{\psi}$ itself as a pure state. Since every element of a convex set can be written as a convex combination of the extremal points in the set, every quantum state $\rho$ that is not a pure state can be written as
	\begin{equation}\label{eq-mixed_state}
		\rho=\sum_k p_k\ket{\psi_k}\!\bra{\psi_k}
	\end{equation}
	for some set $\{\ket{\psi_k}\}_k$ of pure states, where $p_k\geq 0$ and $\sum_k p_k=1$.
	
	States $\rho$ that are not pure are called \textit{mixed states} because they can be thought of as arising from the lack of knowledge of which pure state from the set $\{\ket{\psi_k}\}_k$ the system has been prepared. Note that the decomposition in \eqref{eq-mixed_state} of a quantum state into pure states is generally not unique.
	
	A state $\rho$ is called \textit{maximally mixed} if the set $\{\ket{\psi_k}\}_k$ consists of $d$ orthonormal states and the probabilities $p_k$ are uniform (i.e., $p_k=\frac{1}{d}$ for all $k$). In this case, it follows that
	\begin{equation}\label{eq-max_mixed}
		\rho=\frac{\mathbbm{1}_d}{d}\eqqcolon\pi_d.
	\end{equation}
	To see this, we can expand every unit vector $\ket{\phi}\in\Span\{\ket{\psi_k}:1\leq k\leq d\}$ as $\ket{\phi}=\sum_{k=1}^d c_k\ket{\psi_k}$, with $c_k=\braket{\psi_k}{\phi}$. Writing $\rho = \frac{1}{d} \sum_{k=1}^d \ket{\psi_k}\!\bra{\psi_k}$, we then obtain
	\begin{equation}
		\rho\ket{\phi}=\frac{1}{d}\sum_{k=1}^d\ket{\psi_k}\!\braket{\psi_k}{\phi}=\frac{1}{d}\sum_{k=1}^d c_k\ket{\psi_k}=\frac{1}{d}\ket{\phi}.
	\end{equation}
	The state $\rho$ thus acts as the operator $\frac{\mathbbm{1}_d}{d}$ on the $d$-dimensional Hilbert space spanned by the vectors $\{\ket{\psi_k}:1\leq k\leq d\}$. The state $\pi_d$ is called maximally mixed because it corresponds to having no knowledge about which state from the set $\{\ket{\psi_k}\}_k$ the system is in. This lack of knowledge can be quantified by using quantum entropy, and in Chapter~\ref{chap-entropies}, we find that the maximally mixed state $\pi_d$ has the largest entropy among all states of a finite-dimensional system of dimension~$d$, thus justifying the term ``maximally mixed.''
	
	
\subsection{Bipartite States}\label{subsec-bipartite_state}

	The joint state of two distinct quantum systems $A$ and $B$ is described by a bipartite quantum state $\rho_{AB}\in\Density(\mathcal{H}_A\otimes\mathcal{H}_B)$. For brevity, the joint Hilbert space $\mathcal{H}_A\otimes\mathcal{H}_B$ of the composite system $AB$ is denoted by $\mathcal{H}_{AB}$.
	
	Let $\{\ket{i}_A\}_{i=0}^{d_A-1}$ and $\{\ket{j}_B\}_{j=0}^{d_B-1}$ be orthonormal bases for $\mathcal{H}_A$ and $\mathcal{H}_B$, respectively. Then, 
	\begin{equation}
	\{\ket{i}_A\otimes\ket{j}_B:0\leq i\leq d_A-1,~0\leq j\leq d_B-1\}
	\end{equation}
	 is an orthonormal basis for $\mathcal{H}_{AB}$. For brevity, we often write $\ket{i,j}_{AB}$ instead of $\ket{i}_A\otimes\ket{j}_B$. Every pure state $\ket{\psi}_{AB}\in\mathcal{H}_{AB}$ can thus be written as
	\begin{equation}\label{eq-bipartite_pure_state}
		\ket{\psi}_{AB}=\sum_{i=0}^{d_A-1}\sum_{j=0}^{d_B-1}\alpha_{i,j}\ket{i,j}_{AB},
	\end{equation}
	where $\alpha_{i,j}=\braket{i,j}{\psi}\in\mathbb{C}$ and $\sum_{i=0}^{d_A-1}\sum_{j=0}^{d_B-1}\abs{\alpha_{i,j}}^2=1$. The Schmidt decomposition provides a useful decomposition of every bipartite pure state.
	
	\begin{theorem*}{Schmidt Decomposition}{thm-Schmidt}
		Let $\ket{\psi}_{AB}$ be a pure bipartite state as in \eqref{eq-bipartite_pure_state}. Let $X_{A\to B}$ be the operator with matrix elements $\bra{j}_B X \ket{i}_A =\alpha_{i,j}$, and let $r=\rank(X)$. Then, there exist strictly positive \textit{Schmidt coefficients} $\{\lambda_k > 0 \}_{k=1}^r$ satisfying $\sum_{k=1}^r\lambda_k=1$ and orthonormal vectors $\{\ket{e_k}_A\}_{k=1}^r$ and $\{\ket{f_k}_B\}_{k=1}^r$ such that
		\begin{equation}\label{eq-Schmidt_decomp}
			\ket{\psi}_{AB}=\sum_{k=1}^r \sqrt{\smash[b]{\lambda_k}}\, \ket{e_k}_A\otimes\ket{f_k}_B.
		\end{equation}
		The quantity $r$ is called the \textit{Schmidt rank}, and it holds that $r\leq\min\{d_A,d_B\}$.
	\end{theorem*}
	
	\begin{Proof}
		This is a direct application of the singular value decomposition  (Theorem~\ref{thm-SVD}). Consider the operator $X$ defined in the statement of the theorem, having matrix elements $\bra{j}_B X \ket{i}_A =\alpha_{i,j}$, so that
				\begin{equation}
			X=\sum_{i=0}^{d_A-1}\sum_{j=0}^{d_B-1}\alpha_{i,j}\ket{j}_B \bra{i}_A.
		\end{equation}
		Note that the vector $\ket{\psi}_{AB}$ in \eqref{eq-bipartite_pure_state} is nothing but $\text{vec}(X)$ (see \eqref{eq-vec_operation}).
		Then, by the singular-value decomposition (Theorem~\ref{thm-SVD}), we can write $X$ as
		\begin{equation}
			X=\sum_{k=1}^r s_k \ket{f_k}_B \bra{g_k}_A,
		\end{equation}
		where $s_k$ are strictly positive numbers, $r=\rank(X)\leq \min\{d_A,d_B\}$, and $\{\ket{f_k}_B:1\leq k\leq r\}$ and $\{\ket{g_k}_A:1\leq k\leq r\}$ are sets of orthonormal vectors on $\mathcal{H}_B$ and $\mathcal{H}_A$, respectively. Letting $\lambda_k=s_k^2$, we find that
		\begin{equation}
			X=\sum_{k=1}^r \sqrt{\lambda_k}\ket{f_k}_B\bra{g_k}_A.
		\end{equation}
		Upon vectorizing $X$ as written in this form (see \eqref{eq-vec_operation}), we find that
		\begin{equation}
			\ket{\psi}_{AB}=\text{vec}(X)=\sum_{k=1}^r \sqrt{\lambda_k}
			\ \ \ \conj{\ket{g_k}}_A \otimes
			\ket{f_k}_B.
		\end{equation}
	Letting $\ket{e_k}_A \coloneqq \conj{\ket{g_k}}_A$, the result follows.
	\end{Proof}
	
	A pure state $\ket{\psi}\!\bra{\psi}_{AB}$ is a \textit{product} state if it is  possible to find unit vectors $\ket{\phi}_A$ and $\ket{\varphi}_B$ such that $\ket{\psi}\!\bra{\psi}_{AB} = \ket{\phi}\!\bra{\phi}_{A} \otimes \ket{\varphi}\!\bra{\varphi}_{B}$. A pure state is \textit{entangled} if it is not a product state.
	
	%The Schmidt decomposition gives a simple way to determine if a pure state is entangled. If the Schmidt rank is equal to one, then the state is product. If the Schmidt rank is two or larger, then the state is entangled. Thus, deciding entanglement is easy for pure states, in this sense.
	
	%For more general, mixed states of quantum systems $A$ and $B$, entanglement is a more involved notion, which we develop later in Section~\ref{subsubsec-entanglement}.
	
	
	 
	

\subsubsection{The Partial Trace} 
	
	The trace of a linear operator $X$ acting on a $d$-dimensional Hilbert space can be written as
	\begin{equation}
		\Tr[X]=\sum_{i=0}^{d-1} \bra{i}X\ket{i},
	\end{equation}
	where $\{\ket{i}\}_{i=0}^{d-1}$ is some orthonormal basis.
	We interpret this expression as the sum of the diagonal elements of the matrix representation of $X$ in the basis $\{\ket{i}\}_{i=0}^{d-1}$, although it is straightforward to show that the trace is independent of the choice of basis used to evaluate it.
	
	The trace is known as the \textit{partial trace} when it acts on one subsystem of a bipartite linear operator $X_{AB}$.
	
	\begin{definition}{Partial Trace}{def-partial_trace}%\label{def-partial_trace}
		For every bipartite linear operator $X_{AB}$, the \textit{partial trace over $B$} is denoted by $\Tr_B\equiv \id_A\otimes \Tr_B$ and is defined as
		\begin{equation}\label{eq-partial_trace_B}
			\begin{aligned}
			\Tr_B[X_{AB}]&=(\id_A\otimes \Tr)(X_{AB})\\
			&=\sum_{j=0}^{d_B-1}(\mathbbm{1}_A\otimes\bra{j}_B)X_{AB}(\mathbbm{1}_A\otimes\ket{j}_B).
			\end{aligned}
		\end{equation}
		Similarly, the \textit{partial trace over $A$} is denoted by $\Tr_A\equiv \Tr_A\otimes\id_B$ and is defined as
		\begin{equation}
			\begin{aligned}
			\Tr_A[X_{AB}]&=(\Tr\otimes\id_B)(X_{AB})\\
			&=\sum_{i=0}^{d_A-1}(\bra{i}_A\otimes\mathbbm{1}_B)X_{AB}(\ket{i}_A\otimes\mathbbm{1}_B).
			\end{aligned}
		\end{equation}
	\end{definition}
	
	\begin{remark}
		For every linear operator $X_{AB}$ acting on $\mathcal{H}_{AB}$, we can define the partial trace $\Tr_B[X_{AB}]$ more abstractly as the unique linear operator $X_A$ acting on $\mathcal{H}_A$ such that
		\begin{equation}
			\Tr[(M_A\otimes\mathbbm{1}_B)X_{AB}]=\Tr[M_A X_A]
		\end{equation}
		for every linear operator $M_A$ on $\mathcal{H}_A$. If we let $X_{AB}$ be the state $\rho_{AB}$ and $M_A$ be a Hermitian operator, then we can interpret this equation physically in the following way: in order to determine the expectation value of an observable $M_A$ acting on only one of the subsystems (in this case, the $A$ subsystem), it suffices to know the reduced state $\rho_A$ of the subsystem $A$ rather than the entire joint state $\rho_{AB}$ of the total system. 
	\end{remark}
	
	Given a state $\rho_{AB}$ for the composite system $AB$, we are often interested in determining the state of only one of its subsystems. The partial trace $\Tr_B$ takes a state $\rho_{AB}$ acting on the composite space $\mathcal{H}_{AB}$ and returns a state $\rho_A \equiv \Tr_B[\rho_{AB}]$ acting on the space $\mathcal{H}_A$. The partial trace is therefore the mathematical operation used to determine the state of one of the subsystems given the state of a composite system comprising two or more subsystems, and it can be thought of as the action of ``discarding'' one of the subsystems. The partial trace generalizes the notion of marginalizing a joint probability distribution. Later, in Section~\ref{sec-channel}, we see that partial trace is a particular kind of quantum channel corresponding to this discarding action. 
	
	Now, let us recall from Chapter \ref{chap-math_tools} that, given orthonormal bases $\{\ket{i}_A\}_{i=0}^{d_A-1}$ and $\{\ket{j}_B\}_{j=0}^{d_B-1}$ for $\mathcal{H}_A$ and $\mathcal{H}_B$, respectively, we can define the orthonormal bases
	\begin{equation}
		\{\ket{i}\!\bra{i'}_A:0\leq i,i'\leq d_A - 1\},\quad \{\ket{j}\!\bra{j'}_B:0\leq j,j'\leq d_B - 1\},
	\end{equation}
	for the linear operators on $\mathcal{H}_A$ and $\mathcal{H}_B$, respectively. Then, the set
	\begin{equation}
		\{\ket{i,j}\!\bra{i',j'}_{AB}\equiv\ket{i}\!\bra{i'}_A\otimes\ket{j}\!\bra{j'}_B:0\leq i,i'\leq d_A - 1,~0\leq j,j'\leq d_B - 1\}
	\end{equation}
	forms an orthonormal basis for the linear operators on $\mathcal{H}_{AB}$. Since the action of every linear operator is fully defined by its action on basis elements, we can use the definition above to see that the action of the partial trace $\Tr_B$ on this basis is
	 \begin{equation}
		\Tr_B[\ket{i}\!\bra{i'}_A\otimes\ket{j}\!\bra{j'}_B]=\ket{i}\!\bra{i'}_A\delta_{j,j'}
	\end{equation}
	for all $0\leq i,i'\leq d_A - 1,~0\leq j,j'\leq d_B - 1$. Similarly, for $\Tr_A$, we obtain
	\begin{equation}
		\Tr_A[\ket{i}\!\bra{i'}_A\otimes\ket{j}\!\bra{j'}_B]=\delta_{i,i'}\ket{j}\!\bra{j'}_B
	\end{equation}
	for all $0\leq i,i'\leq d_A - 1,~0\leq j,j'\leq d_B - 1$. Then, by decomposing every linear operator $X_{AB}$ as
	\begin{equation}\label{eq-bipartite_mixed_state}
		\begin{aligned}
		X_{AB}&=\sum_{i,i'=0}^{d_A-1}\sum_{j,j'=0}^{d_B-1}X_{i,j;i',j'}\ket{i}\!\bra{i'}_A\otimes\ket{j}\!\bra{j'}_B\\
		&=\sum_{i,i'=0}^{d_A-1}\sum_{j,j'=0}^{d_B-1}X_{i,j;i',j'}\ket{i,j}\!\bra{i',j'}_{AB},
		\end{aligned}
	\end{equation}
	where $X_{i,j;i',j'}\coloneqq \bra{i,j}X_{AB}\ket{i',j'}$, we find that
	\begin{align}
		\Tr_B[X_{AB}]&=\sum_{i,i'=0}^{d_A-1}\left(\sum_{j=0}^{d_B-1}X_{i,j;i',j}\right)\ket{i}\!\bra{i'}_A,\\
		\Tr_A[X_{AB}]&=\sum_{j,j'=0}^{d_B-1}\left(\sum_{i=0}^{d_A-1}X_{i,j;i,j'}\right)\ket{j}\!\bra{j'}_B.
	\end{align}
	
	For every bipartite linear operator $X_{AB}$, we let
	\begin{equation}
		X_A\equiv\Tr_B[X_{AB}]\text{ and }X_B\equiv\Tr_A[X_{AB}]
	\end{equation}
	denote its partial traces. For states, we also use the terms \textit{marginal states} or \textit{reduced states} to refer to their partial traces.
	
	An immediate consequence of the Schmidt decomposition theorem is that the marginal states $\rho_A\coloneqq\Tr_B[\ket{\psi}\!\bra{\psi}_{AB}]$ and $\rho_B\coloneqq \Tr_A[\ket{\psi}\!\bra{\psi}_{AB}]$ of every pure state $\ket{\psi}_{AB}$ have the same non-zero eigenvalues. Indeed, using \eqref{eq-Schmidt_decomp}, we find that
	 \begin{align}
	 	\rho_A&=\sum_{k,k'=1}^r \sqrt{\lambda_k\lambda_{k'}}\Tr_B[\ket{e_k}\!\bra{e_{k'}}_A\otimes \ket{f_k}\!\bra{f_{k'}}_B]\\
	 		&=\sum_{k,k'=1}^r \sqrt{\lambda_k\lambda_{k'}}\ket{e_k}\!\bra{e_{k'}}_A\delta_{k,k'}\\
	 		&=\sum_{k=1}^r \lambda_k\ket{e_k}\!\bra{e_k}_A, \label{eq-partial-trace-eigenvalues-pure-bistates-1}\\
	 	\text{ and \quad} \rho_B&=\sum_{k,k'=1}^r \sqrt{\lambda_k\lambda_{k'}}\Tr_A[\ket{e_k}\!\bra{e_{k'}}_A\otimes\ket{f_k}\!\bra{f_{k'}}_B]\\
	 		&=\sum_{k,k'=1}^r \sqrt{\lambda_k\lambda_{k'}}\delta_{k,k'}\ket{f_k}\!\bra{f_{k'}}_B\\
	 		&=\sum_{k=1}^r \lambda_k\ket{f_k}\!\bra{f_k}_B,
			\label{eq-partial-trace-eigenvalues-pure-bistates-2}
	 \end{align}
	 in which the equalities in \eqref{eq-partial-trace-eigenvalues-pure-bistates-1} and \eqref{eq-partial-trace-eigenvalues-pure-bistates-2} contain spectral decompositions of $\rho_A$ and $\rho_B$. 


\subsubsection{Purifications and Extensions}
	
	\label{sec:qm:purification-def}
	
	One of the most useful concepts in quantum information is the notion of purification. There is no strong classical analogue of this concept. 
	
	\begin{definition}{Purification}{def-purification}
		Let $\rho_A$ be a state of a system $A$. A \textit{purification} of $\rho_A$ is a pure state $\ket{\psi}\!\bra{\psi}_{RA}$ for a bipartite system $RA$ such that
		\begin{equation}
			\Tr_R[\ket{\psi}\!\bra{\psi}_{RA}]=\rho_A.
		\end{equation}
	\end{definition}
	
	We often call the reference system $R$ the ``purifying system.'' 
	
	The following simple theorem establishes that every state $\rho_A$ has a purification.
	
	\begin{theorem*}{State Purification}{thm-purification}%\label{thm-purification}
		For every state $\rho_A$, there exists a purification $\ket{\psi}\!\bra{\psi}_{RA}$ of $\rho_A$ with $d_R\geq \rank(\rho_A)$. 
	\end{theorem*}
	
	\begin{Proof}
		Consider a spectral decomposition of $\rho_A$
		\begin{equation}
			\rho_A=\sum_{k=1}^r \lambda_k\ket{\phi_k}\!\bra{\phi_k},
		\end{equation}
		where $r=\rank(\rho_A)$. Consider a reference system $R$ with $d_R\geq r$ and an arbitrary set $\{\ket{\varphi_k}_R:1\leq k\leq r\}$ of orthonormal states. The unit vector
		\begin{equation}\label{eq-state_purification}
			\ket{\psi}_{RA}\coloneqq \sum_{k=1}^r\sqrt{\lambda_k}\ket{\varphi_k}_R\otimes\ket{\phi_k}_A
		\end{equation}
		then satisfies
		\begin{align}
			\Tr_R[\ket{\psi}\!\bra{\psi}_{RA}]&=\sum_{k,k'=1}^r \sqrt{\lambda_k\lambda_{k'}}\underbrace{\Tr[\ket{\varphi_k}\!\bra{\varphi_{k'}}_R]}_{\delta_{k,k'}}\ket{\phi_k}\!\bra{\phi_{k'}}_A\\
			&=\sum_{k=1}^r\lambda_k\ket{\phi_k}\!\bra{\phi_k}_A\\
			&=\rho_A,
		\end{align}
		so that $\ket{\psi}\!\bra{\psi}_{RA}$ is a purification of $\rho_A$, as required.
	\end{Proof}
	
	\begin{remark}
		The theorem above states that the condition $d_R\geq\rank(\rho_{A})$ on the dimension of the purifying system $R$ is sufficient to guarantee the existence of a purification. This condition is also necessary, meaning that it is not possible to have a purifying system whose dimension is less than the rank of $\rho_{A}$. 
	\end{remark}
	
	The proof of the theorem above not only tells us that every state has a purification, but it also tells us explicitly how to construct one such purification. We can also construct a purification of every state $\rho_A$ as follows:
	\begin{equation}
		\ket{\psi}_{RA}=(\mathbbm{1}_R\otimes\sqrt{\rho_A})\ket{\Gamma}_{RA}=\text{vec}(\sqrt{\rho_A}),
	\end{equation}
	where $\ket{\Gamma}_{RA}=\sum_{i=0}^{d_A-1}\ket{i,i}_{RA}$ and where the operation $\text{vec}$ is defined in \eqref{eq-vec_operation}. We often call the state $\ket{\psi}\!\bra{\psi}_{RA}$ the \textit{canonical purification} of $\rho_A$. Note that the canonical purification is very closely related to the purification used in the proof of Theorem~\ref{thm-purification}. Indeed, if
	\begin{equation}
		\rho_A=\sum_{k=1}^r \lambda_k\ket{\phi_k}\!\bra{\phi_k}
	\end{equation}
	is a spectral decomposition of $\rho_A$, with $r=\rank(\rho_A)$, then
	\begin{equation}
		\text{vec}(\sqrt{\rho_A})=\sum_{k=1}^r \sqrt{\lambda_k}~\conj{\ket{\phi_k}}_R\otimes \ket{\phi_k}_A,
	\end{equation}
	where we have made use of \eqref{eq-vec_operation_vectors}.
	
	Physically, the fact that every state $\rho_A$ has a purification means that every quantum system $A$ in a mixed state can be viewed as being entangled with \textit{some} system $R$ to which we do not have access, such that the global state is a pure state $\ket{\psi}\!\bra{\psi}_{RA}$. Since we do not have access to $R$, our knowledge of the system has to be described by the partial trace of $\ket{\psi}\!\bra{\psi}_{RA}$ over $R$, i.e., by $\rho_A$. 
	
	Observe that if the state $\rho_A$ is pure, i.e., if $\rho_A=\ket{\phi}\!\bra{\phi}_A$, then the only possible purification of it is of the form $\ket{\psi}\!\bra{\psi}_{RA}=\ket{\varphi}\!\bra{\varphi}_R\otimes\ket{\phi}\!\bra{\phi}_A$, with $\ket{\varphi}\!\bra{\varphi}_R$ a pure state of the system $R$. In other words, purifications of pure states can only be \textit{pure product states}.
	
	Purifications of states are not unique. In fact, given a state $\rho_A$ and a purification $\ket{\psi}\!\bra{\psi}_{RA}$ of $\rho_A$ as in \eqref{eq-state_purification}, let $V_{R\to R'}$ be an isometry (i.e., a linear operator satisfying $V^\dagger V=\mathbbm{1}_R$) acting on the $R$ system. Defining 
	\begin{equation}\label{eq-purif_iso_equiv_1}
		\ket{\psi'}_{R'A}=(V_{R\to R'}\otimes\mathbbm{1}_A)\ket{\psi}_{RA},
	\end{equation}
	we find that
	\begin{align}
		\Tr_{R'}[\ket{\psi'}\!\bra{\psi'}_{R'A}]&=\sum_{k,k'=1}^r \sqrt{\lambda_k\lambda_{k'}}\Tr[V\ket{\varphi_k}\!\bra{\varphi_{k'}}_R V^\dagger]\ket{\phi_k}\!\bra{\phi_k}_A\label{eq-purif_iso_equiv_2}\\
		&=\sum_{k=1}^r\lambda_k\ket{\phi_k}\!\bra{\phi_k}_A\label{eq-purif_iso_equiv_3}\\
		&=\rho_A,\label{eq-purif_iso_equiv_4}
	\end{align}
	where we conclude that $\Tr[V\ket{\varphi_k}\!\bra{\varphi_{k'}}V^\dagger]=\delta_{k,k'}$ from cyclicity of the trace and $V^\dagger V=\mathbbm{1}_R$. So $\ket{\psi'}\!\bra{\psi'}_{R'A}$ is also a purification of $\rho_A$.
	
	A converse statement holds as well by employing the Schmidt decomposition (Theorem~\ref{thm-Schmidt}): if $\ket{\psi}\!\bra{\psi}_{RA}$ and $\ket{\psi'}\!\bra{\psi'}_{R'A}$ are two purifications of the state~$\rho_A$, then they are related by an isometry taking one reference system to the other. By combining this statement and the previous one, we can thus say that purifications are unique ``up to isometries acting on the reference system.''

	We now state a useful fact about purification of states that are permutation invariant. A state $\rho\in\Density(\mathcal{H}^{\otimes n})$ is called \textit{permutation invariant} if
	\begin{equation}\label{eq-state_perm_invar}
		\rho = W^{\pi}\rho W^{\pi\dagger}
	\end{equation}
	for all permutations $\pi\in\mathcal{S}_n$, where the unitary permutation operators $W^{\pi}$ are defined in \eqref{eq-permutation_rep}.
	
	\begin{remark}
		Note that the permutation-invariance condition in \eqref{eq-state_perm_invar} does \textit{not} imply that the state $\rho$ is supported on the symmetric subspace $\text{Sym}_n(\mathcal{H})$ of $\mathcal{H}^{\otimes n}$. In other words, the condition in \eqref{eq-state_perm_invar} does not imply that
		\begin{equation}
			\Pi_{\text{Sym}_n(\mathcal{H})}\rho\Pi_{\text{Sym}_n(\mathcal{H})}=\rho.
		\end{equation}
		As a simple example, suppose that $\mathcal{H}=\mathbb{C}^2$, and let $\rho=\ket{\psi}\!\bra{\psi}\in\Density((\mathbb{C}^2)^{\otimes 2})$, where $\ket{\psi}=\frac{1}{\sqrt{2}}(\ket{0,1}-\ket{1,0})$. Then, it is easy to see that $W^{\pi}\rho W^{\pi\dagger}=\rho$ for all $\pi\in\mathcal{S}_2$, while $\Pi_{\text{Sym}_2(\mathcal{H})}\rho\Pi_{\text{Sym}_2(\mathcal{H})}=0$. The latter is true because $\ket{\psi}$ is an \textit{anti-symmetric state}, i.e., $\ket{\psi}\in\text{ASym}_2(\mathcal{H})$. The state $\rho$ is thus supported on the anti-symmetric subspace, even though it is permutation invariant.
	\end{remark}
	
	
	\begin{Lemma*}{Purification of Permutation-Invariant States}{lem-symm_purif}
		Let $\rho_{A^n}\in\Density(\mathcal{H}_A^{\otimes n})$ be a permutation-invariant state, i.e.,
		\begin{equation}
			\rho_{A^n} = W_{A^n}^{\pi}\rho_{A^n}W_{A^n}^{\pi\dagger}
		\end{equation}
		for all $\pi\in\mathcal{S}_n$, where the unitary operators $\{W_{A^n}^{\pi}\}_{\pi\in\mathcal{S}_n}$ are defined in \eqref{eq-permutation_rep}. Then, there exists a permutation-invariant purification $\ket{\psi^{\rho}}\!\bra{\psi^{\rho}}_{\hat{A}^{n}A^n}$ of $\rho_{A^n}$, such that $\ket{\psi^{\rho}}_{\hat{A}^{n}A^n}\in\text{Sym}_n(\mathcal{H}_{\hat{A}A})$. This means that
		\begin{equation}
			\ket{\psi^{\rho}}_{\hat{A}^{n}A^n} = W_{\hat{A}^{n}}^{\pi}\otimes W_{A^n}^{\pi}\ket{\psi^{\rho}}_{\hat{A}^{n}A^n}
		\end{equation}
		for all $\pi\in\mathcal{S}_n$, where the dimension of $\hat{A}$ is equal to the dimension of $A$.
	\end{Lemma*}
	
	\begin{Proof}
		Let us consider the following spectral decomposition of $\rho_{A^n}$:
		\begin{equation}
			\rho_{A^n}=\sum_{\lambda\in\text{spec}(\rho_{A^n})}\lambda \, \Pi^\lambda_{A^n} ,
		\end{equation}
		where $\text{spec}(\rho_{A^n})$ is the set of (distinct) eigenvalues of $\rho_{A^n}$ and 
		$\Pi^\lambda_{A^n}$ is the spectral projection corresponding to $\lambda$. Let us write $\Pi^\lambda_{A^n}$ as follows:
		\begin{equation}
		\Pi^\lambda_{A^n} = \sum_{k=1}^{d_{\lambda}} \ket{\phi_k^{\lambda}}\!\bra{\phi_k^{\lambda}}_{A^n},
		\end{equation}
		 in terms of an orthonormal basis $\{\ket{\phi_k^{\lambda}}_{A^n}\}_{k=1}^{d_\lambda}$, where  $d_{\lambda} \coloneqq \rank(\Pi^\lambda_{A^n})$. Since $\rho_{A^n}$ is a density operator, it follows that $\sum_{\lambda \in \text{spec}(\rho_{A^n})} \lambda \, d_{\lambda} = 1$.
		Let $E_{\lambda}$ denote the eigenspace corresponding to $\lambda\in\text{spec}(\rho_{A^n})$.
		Define the vectors
		\begin{align}
			\ket{\Gamma_{\lambda}}_{\hat{A}^nA^n}&\coloneqq\sum_{k=1}^{d_\lambda}\conj{\ket{\phi_k^{\lambda}}}_{\hat{A}^n}\otimes\ket{\phi_k^{\lambda}}_{A^n},\\
			\ket{\psi^{\rho}}_{\hat{A}^nA^n}&\coloneqq \sum_{\lambda\in\Lambda}\sqrt{\lambda}\, \ket{\Gamma_{\lambda}}_{\hat{A}^nA^n},
		\end{align}
		where $\conj{\ket{\phi_k^{\lambda}}}$ is the complex conjugate of $\ket{\phi_k^{\lambda}}$ with respect to the standard basis. Observe that
		\begin{equation}
			\Tr_{\hat{A}^n}[\ket{\psi^{\rho}}\!\bra{\psi^{\rho}}_{\hat{A}^nA^n}]=\sum_{\lambda\in\text{spec}(\rho_{A^n})}\sum_{k=1}^{d_\lambda}\lambda\ket{\phi_k^{\lambda}}\!\bra{\phi_k^{\lambda}}_{A^n}=\rho_{A^n},
		\end{equation}
		so that $\ket{\psi^{\rho}}\!\bra{\psi^{\rho}}_{\hat{A}^nA^n}$ is a purification of $\rho_{A^n}$.
		
		Let us now show that $\ket{\psi^{\rho}}_{\hat{A}^nA^n}\in\text{Sym}_n(\mathcal{H}_{\hat{A}A})$.
		Since $\rho_{A^n}$ is permutation invariant, observe that
		\begin{equation}
			W^{\pi\dagger}_{A^n}\rho_{A^n} W_{A^n}^{\pi}\ket{\phi_k^{\lambda}}_{A^n}
			=\rho_{A^n}\ket{\phi_k^{\lambda}}_{A^n}=\lambda\ket{\phi_k^{\lambda}}_{A^n},
		\end{equation}
		for all $\lambda\in\text{spec}(\rho_{A^n})$ and $ k \in \{1, \ldots,  d_{\lambda}\}$. Multiplying both sides on the left by $W_{A^n}^{\pi}$ gives
		\begin{equation}
			\rho_{A^n} W^{\pi}_{A^n}\ket{\phi_k^{\lambda}}_{A^n}=\lambda W^{\pi}_{A^n}\ket{\phi_k^{\lambda}}_{A^n}.
		\end{equation}
		This means that $W_{A^n}\ket{\phi_k^{\lambda}}_{A^n}$ is an eigenvector of $\rho_{A^n}$ with eigenvalue $\lambda$.
		Since both $\ket{\phi_k^{\lambda}}_{A^n}$ and $W_{A^n}\ket{\phi_k^{\lambda}}_{A^n}$ are eigenvectors of $\rho_{A^n}$ with eigenvalue $\lambda$, it follows that the subspaces $E_{\lambda}$ are invariant under all permutation operators~$W^{\pi}_{A^n}$. This implies that the restriction of $W^{\pi}_{A^n}$ to the subspace $E_{\lambda}$ is unitary.
		Observe that the operators $W_{\hat{A}^n}^{\pi}$ are real in the standard basis, meaning that $\conj{W_{\hat{A}^n}^{\pi}}=W_{\hat{A}^n}^{\pi}$ for all $\pi\in\mathcal{S}_n$.
		Then, by applying these two observations, we find that
		\begin{equation}
			  W_{\hat{A}^n}^{\pi}\otimes W_{A^n}^{\pi}\ket{\Gamma_{\lambda}}_{\hat{A}^nA^n}
=			  \conj{W_{\hat{A}^n}^{\pi}} 
			\otimes W_{A^n}^{\pi}\ket{\Gamma_{\lambda}}_{\hat{A}^nA^n}
			  =\ket{\Gamma_{\lambda}}_{\hat{A}^nA^n}
		\end{equation}
		for all $\pi\in\mathcal{S}_n$, where we used \eqref{eq-transpose_trick_unitary} and \eqref{eq:math-tools:Gamma-any-ortho} to establish the last equality. Therefore, by linearity,
		\begin{equation}
			W_{\hat{A}^n}^{\pi}\otimes W_{A^n}^{\pi}\ket{\psi^{\rho}}_{\hat{A}^nA^n}=\ket{\psi^{\rho}}_{\hat{A}^nA^n}
		\end{equation}
		for all $\pi\in\mathcal{S}_n$. By the definition of $\text{Sym}_n(\mathcal{H}_{\hat{A}A})$ in \eqref{eq:math-tools:def-sym-subspace} and the observation in \eqref{eq:math-tools:joint-perms}, we conclude  that
		$\ket{\psi^{\rho}}_{\hat{A}^nA^n}\in\text{Sym}_n(\mathcal{H}_{\hat{A}A})$.
	\end{Proof}



	\begin{definition}{Extension}{def:qm:extension-of-state}
	An extension of a quantum state $\rho_A$ is a state $\omega_{RA}$ satisfying $\Tr_R[\omega_{RA}]=\rho_A$, where $R$ is a reference system. 
	\end{definition}
	
	Thus, a purification $\ket{\psi}\!\bra{\psi}_{RA}$ of a quantum state $\rho_A$ is a particular kind of extension of $\rho_A$. For a purification, it is required that $d_R \geq \rank(\rho_A)$. However, there is no such requirement for an extension.
	
	
	
	Note that if the state $\rho_A$ is pure, i.e., if $\rho_A=\ket{\phi}\!\bra{\phi}_A$, then every extension $\omega_{RA}$ of $\rho_A$ must be a product state, i.e., we must have $\omega_{RA}=\sigma_R\otimes\ket{\phi}\!\bra{\phi}_A$ for some state $\sigma_R$.
	
	

\subsubsection{Ensembles and Classical--Quantum States}

	For a finite alphabet $\mathcal{X}$, an \textit{ensemble} is a collection $\{(p(x),\rho^x)\}_{x\in\mathcal{X}}$ consisting of a probability distribution $p:\mathcal{X}\to[0,1]$ such that each probability $p(x)$ is paired with a quantum state $\rho^x$. Ensembles are used to describe quantum systems that are known to be in one of a given set of states with some probability.
	
	Suppose that Alice is in possession of a quantum system and that she prepares the system in a state $\rho^x$ with probability $p(x)$. The state of the system can thus be described by the ensemble $\{(p(x),\rho^x)\}_{x\in\mathcal{X}}$. If she sends the system to Bob in one of these states without telling him in which of the states the system has been prepared, but Bob knows the ensemble $\{(p(x),\rho^x)\}_{x\in\mathcal{X}}$ describing the system, then from Bob's perspective the state of the system is given by the expected state $\rho$ of the ensemble, which is given by
	\begin{equation}
		\rho=\sum_{x\in\mathcal{X}}p(x)\rho^x.
	\end{equation}
	
	On the other hand, if Alice sends Bob classical information about which state she has prepared, then from Bob's perspective the state of the system can be described by the following \textit{classical--quantum state}:
	\begin{equation}
		\rho_{XB}=\sum_{x\in\mathcal{X}}p(x)\ket{x}\!\bra{x}_X\otimes \rho_B^x,
	\end{equation}
	where $X$ is the $|\mathcal{X}|$-dimensional quantum system corresponding to the register holding the information about which state was sent and $\{\ket{x}\}_{x\in\mathcal{X}}$ is an orthonormal basis for $\mathcal{H}_X$. Classical--quantum states have a block-diagonal structure, in the sense that they can equivalently be written as the following block-diagonal matrix:
	\begin{equation}\label{eq-cq_state_block_diag}
		\rho_{XB}=\begin{pmatrix} p(x_1)\rho^{x_1} & & & \\ & p(x_2)\rho^{x_2} & & \\ & & \ddots & \\ & & & p(x_{|\mathcal{X}|})\rho^{x_{|\mathcal{X}|}} \end{pmatrix}.
	\end{equation}
	We can represent \eqref{eq-cq_state_block_diag} more compactly as
	\begin{equation}
		\rho_{XB} = \bigoplus_{x \in \mathcal{X}} p(x)\rho^x.
	\end{equation}



\subsubsection{Separable and Entangled States}\label{subsubsec-entanglement}

	The concepts of separable and entangled states are at the heart of virtually all of the communication protocols that we consider in this book. Entanglement, in particular, is a key element of private communication and secure key distillation, and the successful distribution of entangled states among several spatially separated parties is a crucial ingredient in the implementation of such protocols over the future quantum internet. If the parties share only separable, unentangled states, then it is not possible for them to distill a key that is secure against a general quantum adversary.
	
	We begin this section by defining separable and entangled states as follows:
	
	\begin{definition}{Separable and Entangled States}{def-sep_ent_state}
		A bipartite state $\sigma_{AB}$ is called \textit{separable} if there exists a finite alphabet $\mathcal{X}$, a probability distribution $p:\mathcal{X}\rightarrow[0,1]$ on $\mathcal{X}$, and sets $\{\omega_A^x\}_{x\in\mathcal{X}}$ and $\{\tau_B^x\}_{x\in\mathcal{X}}$ of states for $A$ and $B$, respectively, such that
		\begin{equation}\label{eq-sep_state}
			\sigma_{AB}=\sum_{x\in\mathcal{X}}p(x)\omega_A^x\otimes\tau_B^x.
		\end{equation}
		In other words, a state is called separable if it can be written as a convex combination of \textit{product states} $\{\omega_A^x\otimes\tau_B^x\}_{x\in\mathcal{X}}$. The set of separable states on $\mathcal{H}_{AB}$ is denoted by $\SEP(A\!:\!B)$.\\[0.1in]
%		\vspace{.1in}
		Any state that is not separable is called \textit{entangled}.
	\end{definition}
	
	\begin{remark}
		Note that a separable state can always be written in the form
		\begin{equation}
			\sigma_{AB}=\sum_{x'\in\mathcal{X}'}q(x')\ket{\psi_{x'}}\!\bra{\psi_{x'}}_A\otimes\ket{\phi_{x'}}\!\bra{\phi_{x'}}_B
	\end{equation}
		for some probability distribution $q:\mathcal{X}'\to[0,1]$ on a finite alphabet $\mathcal{X}'$ and sets of pure states $\{\ket{\psi_{x'}}\!\bra{\psi_{x'}}_A:x'\in\mathcal{X}'\}$, $\{\ket{\phi_{x'}}\!\bra{\phi_{x'}}_B:x'\in\mathcal{X}'\}$. In other words, separable states can always be written as a convex combination of pure product states. Indeed, from \eqref{eq-sep_state}, we can take spectral decompositions of $\omega_A^x$ and $\tau_B^x$,
		\begin{equation}
			\omega_A^x=\sum_{k=1}^{r_A^x} t_k^x\ket{e_k^x}\!\bra{e_k^x}_A,\quad \tau_B^x=\sum_{\ell=1}^{r_B^x}s_\ell^x\ket{f_\ell^x}\!\bra{f_\ell^x}_B,
		\end{equation}
		where $r_A^x=\rank(\omega_A^x)$ and $r_B^x=\rank(\tau_B^x)$, so that
		\begin{equation}\label{eq-sep_state_pure_0}
			\rho_{AB}=\sum_{x\in\mathcal{X}}\sum_{k=1}^{r_A^x}\sum_{\ell=1}^{r_B^x}p(x)t_k^x s_\ell^x \ket{e_k^x}\!\bra{e_k^x}_A\otimes\ket{f_\ell^x}\!\bra{f_\ell^x}_B.
		\end{equation}
		Then, define the alphabet $\mathcal{X}'=\{x'\coloneqq (x,k,\ell):x\in\mathcal{X},~1\leq k\leq r_A^x,~1\leq\ell\leq r_B^x\}$, so that $x'$ is a superindex, and the unit vectors
		\begin{equation}
			\ket{\psi_{x'}}_A\coloneqq \ket{e_k^x}_A,\quad \ket{\phi_{x'}}_B\coloneqq \ket{f_\ell^x}_B.
		\end{equation}
		Also, define the probability distribution $q:\mathcal{X}'\to[0,1]$ by
		\begin{equation}
			q(x,k,\ell)=p(x)t_k^x s_\ell^x.
		\end{equation}
		Therefore, \eqref{eq-sep_state_pure_0} can be written as
		\begin{equation}\label{eq-sep_state_pure}
			\sigma_{AB}=\sum_{x'\in\mathcal{X}'} q(x')\ket{\psi_{x'}}\!\bra{\psi_{x'}}_A\otimes\ket{\phi_{x'}}\!\bra{\phi_{x'}}_B.
		\end{equation}
		From the development above, it follows that the set of separable states is the convex hull of the set of pure product states. By an application of the Fenchel--Eggleston--Carath\'{e}odory Theorem (Theorem~\ref{thm-Caratheodory}), it follows that $\sigma_{AB}$ can be written as a convex combination of no more than $\rank(\sigma_{AB})^2$ pure product states.
	\end{remark}
	
	Bipartite separable states can be thought of as exhibiting purely classical correlations between the two parties, Alice and Bob, in the following sense. Suppose that Alice draws $x$ with  probability $p(x)$, prepares her system in the state $\omega_A^x$, sends $x$ to Bob over a classical channel, who then prepares his system in the state $\tau_B^x$, where $x\in\mathcal{X}$ and $\mathcal{X}$ is a finite alphabet. This procedure corresponds to preparing the ensemble $\{(p(x),\omega_A^x\otimes\tau_B^x)\}_{x\in\mathcal{X}}$, and if Alice and Bob discard the label $x$, then their shared joint state is the separable state $\sigma_{AB}=\sum_{x\in\mathcal{X}}p(x)\omega_A^x\otimes\tau_B^x$.
	
	On the other hand, no such procedure consisting of only local operations by Alice and Bob supplemented by classical communication between them can ever be used to generate an entangled state between Alice and Bob (without some prior  entanglement shared between them). Section~\ref{subsec-LOCC_channels} introduces local operations and classical communication (LOCC) channels and explains this point in more detail. Essentially, two entangled particles are intrinsically linked in such a way that it is insufficient to  describe each particle individually. 
	
	Observe that a pure state $\psi_{AB}$ is separable if and only if it is a product state, i.e., if and only if there exist pure states $\phi_A$ and $\varphi_B$ such that $\psi_{AB}=\phi_A\otimes\varphi_B$. Recalling that every pure state has a Schmidt decomposition (see Theorem~\ref{thm-Schmidt}), we now reiterate what we stated earlier after Theorem~\ref{thm-Schmidt}:
	\begin{specbox}{0.7\textwidth}
		A pure state is entangled if and only if its Schmidt rank is strictly greater than one.
	\end{specbox}
	
	An important example of an entangled pure state is the state $\Phi_{AB}$ on two $d$-dimensional systems $A$ and $B$, defined as
	$\Phi_{AB} \coloneqq \ket{\Phi}\!\bra{\Phi}_{AB}$, where
	\begin{equation}\label{eq-max_ent_state}
		\ket{\Phi}_{AB}\coloneqq\frac{1}{\sqrt{d}}\sum_{i=0}^{d-1}\ket{i}_A\otimes\ket{i}_B=\frac{1}{\sqrt{d}}\ket{\Gamma}_{AB},
	\end{equation}
	and $\ket{\Gamma}_{AB}=\sum_{i=0}^{d-1}\ket{i}_A\otimes\ket{i}_B$ is the vector defined in \eqref{eq-max_ent_vector}. Note that
	\begin{equation}
		\Tr_A[\Phi_{AB}]=\frac{\mathbbm{1}_B}{d},\quad\Tr_B[\Phi_{AB}]=\frac{\mathbbm{1}_A}{d}.
	\end{equation}
	The state $\Phi_{AB}$ is an example of a maximally entangled state. A pure state $\psi_{AB}$, for two systems $A$ and $B$ of the same dimension $d$, is called \textit{maximally entangled} if the Schmidt coefficients of $\ket{\psi}_{AB}$ are all equal to $\frac{1}{\sqrt{d}}$, with $d$ being the Schmidt rank of $\ket{\psi}_{AB}$. In other words, $\psi_{AB}$ is called maximally entangled if $\ket{\psi}_{AB}$ has the Schmidt decomposition
	\begin{equation}
		\ket{\psi}_{AB}=\frac{1}{\sqrt{d}}\sum_{k=1}^d \ket{e_k}_A\otimes\ket{f_k}_B
	\end{equation}
	for some orthonormal sets $\{\ket{e_k}_A:1\leq k\leq d\}$ and $\{\ket{f_k}_B:1\leq k\leq d\}$. Observe then that
	\begin{equation}
		\Tr_A[\ket{\psi}\!\bra{\psi}_{AB}]=\pi_d=\Tr_B[\ket{\psi}\!\bra{\psi}_{AB}].
	\end{equation}
	In other words, like the state $\Phi_{AB}$, the marginal states of every maximally entangled state are maximally mixed on $\mathcal{H}_{A}$ and~$\mathcal{H}_B$.
	
	Maximally entangled states provide a good example of why entangled particles are, in a sense, greater than the sum of their parts. Since maximally entangled states have maximally mixed marginal states, the individual particles in a maximally entangled state can be viewed as being in a completely random state since, as we have seen, maximally mixed states can be written as the expected state of every ensemble of orthonormal pure states with uniform probability distribution. However, intriguingly, the overall composite system is in a pure, definite state.
	
	

\subsubsection{The Partial Transpose and PPT States}\label{subsec-PPT}
	
	As indicated previously in \eqref{eq:math-tools:transpose-superop}, the action of the transpose map $\T$ on a linear operator $X_{A\to A'}$ can be written as
	\begin{equation}
		\T(X)=\sum_{i=0}^{d_A-1}\sum_{j=0}^{d_{A'}-1}\ket{i}_A\bra{j}_{A'} X \ket{i}_A\bra{j}_{A'},
	\end{equation}
	where we have defined the transpose with respect to the orthonormal bases $\{\ket{i}_A:0\leq i\leq d_{A}-1\}$ and $\{\ket{j}_{A'}:0\leq j\leq d_{A'} -1\}$.
	This is consistent with the familiar definition of the transpose of a matrix $X$ as being the matrix $X^{\t}$ with its rows and columns flipped relative to $X$. Indeed, if $X$ has the matrix representation $X=\sum_{j,i}X_{j,i}\ket{j}_{A'}\!\bra{i}_A$, with matrix elements $\{X_{j,i}\}_{j,i}$, then it follows that the transpose map has action
	\begin{equation}
		\T(X)=\sum_{j,i}X_{j,i}\ket{i}_A\bra{j}_{A'},
	\end{equation}
	which, as expected, has $X^{\t}$ as its  matrix representation. Note that, unlike the trace or the conjugate transpose, the transpose depends on the choice of orthonormal bases used to evaluate it. Throughout the rest of this book, we use both $\T(X)$ and $X^{\t}$ to refer to the transpose of $X$.
	
	The transpose map is known as the \textit{partial transpose} when it acts on one subsystem of a bipartite operator $X_{AB}$. 

	\begin{definition}{Partial Transpose}{def-partial_transpose}
		For every bipartite linear operator $X_{AB}$, its \textit{partial transpose on $B$} is denoted by $\T_B\equiv \id_A\otimes \T_B$ and is defined as
		\begin{equation}
			\T_B(X_{AB})\coloneqq\sum_{j,j'=0}^{d_B-1}(\mathbbm{1}_{A}\otimes \ket{j}\!\bra{j'}_{B})X_{AB}(\mathbbm{1}_{A}\otimes\ket{j}\!\bra{j'}_{B}).
		\end{equation}
		Similarly, the \textit{partial transpose on $A$} is denoted by $\T_A\equiv \T_A\otimes\id_B$ and is defined as
		\begin{equation}
			\T_A(X_{AB})\coloneqq\sum_{i,i'=0}^{d_A-1}(\ket{i}\!\bra{i'}_A\otimes\mathbbm{1}_B)X_{AB}(\ket{i}\!\bra{i'}_A\otimes\mathbbm{1}_B).
		\end{equation}
	\end{definition}
	
	Given an expansion of $X_{AB}$ as
	\begin{equation}
		X_{AB}=\sum_{i,j=0}^{d_B-1} X_{A}^{i,j}\otimes\ket{i}\!\bra{j}_{B},
	\end{equation}
	where each $X_{A}^{i,j}$ is a linear operator acting on system $A$, the partial transpose map $\T_{B}$ has the action
	\begin{equation}
		\T_{B}(X_{AB})=
		\sum_{i,j=0}^{d_B-1} X_{A}^{i,j}\otimes\ket{j}\!\bra{i}_{B}
		=\sum_{i,j=0}^{d_B-1} X_{A}^{j,i}\otimes\ket{i}\!\bra{j}_{B}.
	\end{equation}
	
	The partial transpose map is self-inverse, i.e.,%
	\begin{equation}\label{eq:partial-transpose-self-inverse}
		\left(\id_{A}\otimes \T_B\right)\circ\left(\id_{A}\otimes \T_B\right)=\id_{AB},
	\end{equation}
	and it is self-adjoint with respect to the Hilbert--Schmidt inner product, in the sense that
	\begin{equation}\label{eq:partial-transpose-self-adjoint}
		\inner{X_{AB}}{\T_{B}(Y_{AB})}=\inner{\T_{B}(X_{AB})}{Y_{AB}},
	\end{equation}
	for all operators $X_{AB}$ and $Y_{AB}$.
	
	\begin{definition}{PPT State}{def-PPT}%\label{def-PPT}
		A bipartite state $\rho_{AB}$ is called a \textit{positive partial transpose (PPT) state} if the partial transpose $\T_B(\rho_{AB})$ is positive semi-definite.\\[0.1in]
		The set of PPT states is denoted by $\PPT(A\!:\!B)$, so that
		\begin{equation}\label{eq:PPT-states-set}
			\PPT(A\!:\!B)\coloneqq \left\{\sigma_{AB}:\sigma_{AB}\geq 0,~\T_{B}%
(\sigma_{AB})\geq 0,\Tr[\sigma_{AB}]=1\right\}.
		\end{equation}
	\end{definition}
	
	Note that the property of a state being PPT  depends neither on which system the transpose is taken nor on which orthonormal basis is used to define the transpose map. Indeed, to see the first statement, suppose that $\rho_{AB}\in\PPT(A\!:\!B)$. This means that $\T_B(\rho_{AB})\geq 0$. But since the eigenvalues are invariant under a full transpose $\T_A\otimes\T_B$, this means that $(\T_A\otimes\T_B)(\T_B(\rho_{AB}))\geq 0$, the latter being the same as $\T_A(\rho_{AB})\geq 0$ due to the self-inverse property of the partial transpose. So $\T_B(\rho_{AB})\geq 0$ implies $\T_A(\rho_{AB})\geq 0$, and vice versa. 
	
	To see the second statement, let $\T_B(\rho_{AB})\geq 0$, and let $\{ \ket{\phi_\ell}_B \}_{\ell=1}^{d_B}$ be some other orthonormal basis for $B$. The partial transpose with respect to this basis is given by
	\begin{equation}
		\sum_{\ell,\ell'=1}^{d_B}(\mathbbm{1}_A\otimes\ket{\phi_\ell}\!\bra{\phi_{\ell'}}_B)\rho_{AB}(\mathbbm{1}_A\otimes\ket{\phi_{\ell}}\!\bra{\phi_{\ell'}}_{B}).
	\end{equation}
	Now, consider that $\sum_{\ell=1}^{d_B}\ket{\phi_{\ell}}\!\bra{\phi_{\ell}}=\mathbbm{1}_B$, so that
	\begin{align}
	& \T_B(\rho_{AB}) \notag \\&  =
	\sum_{j,j'=0}^{d_B-1}(\mathbbm{1}_{A}\otimes \ket{j}\!\bra{j'}_{B})\rho_{AB}(\mathbbm{1}_{A}\otimes\ket{j}\!\bra{j'}_{B}) \notag\\
	&  =
	\sum_{j,j',\ell, \ell'=1}^{d_B}(\mathbbm{1}_{A}\otimes \ket{j}\braket{j'}{\phi_{\ell}}
	\bra{\phi_{\ell}}_{B})\rho_{AB}(\mathbbm{1}_{A}\otimes\ket{\phi_{\ell'}}\braket{\phi_{\ell'}}{j}\!\bra{j'}_{B}) \notag\\
	&  =
	\sum_{j,j',\ell, \ell'=1}^{d_B}(\mathbbm{1}_{A}\otimes \braket{\phi_{\ell'}}{j} \ket{j}
	\bra{\phi_{\ell}}_{B})\rho_{AB}(\mathbbm{1}_{A}\otimes\ket{\phi_{\ell'}}\!\bra{j'}_{B}\braket{j'}{\phi_{\ell}}) \notag\\
		&  =
	\sum_{\ell, \ell'=1}^{d_B}\left(\mathbbm{1}_{A}\otimes \left(\sum_{j=0}^{d_B-1}\braket{\phi_{\ell'}}{j}\ket{j}\right)
	\bra{\phi_{\ell}}_{B}\right)\rho_{AB}\left(\mathbbm{1}_{A}\otimes\ket{\phi_{\ell'}}
	\left(\sum_{j'=1}^{d_b}\bra{j'}_{B}\braket{j'}{\phi_{\ell}}\right)\right) \notag\\
			&  =
	\sum_{\ell, \ell'=1}^{d_B}\left(\mathbbm{1}_{A}\otimes \conj{\ket{\phi_{\ell'}}}
	\bra{\phi_{\ell}}_{B}\right)\rho_{AB}\left(\mathbbm{1}_{A}\otimes\ket{\phi_{\ell'}}
	\conj{\bra{\phi_{\ell}}}\right) ,
		\end{align}
		where in the last line we defined $\conj{\ket{\phi_{\ell}}} \coloneqq  \sum_{j=0}^{d_B-1}\braket{\phi_{\ell}}{j}\ket{j}$ for $1 \leq \ell \leq d_B$. Note that the set $\{\conj{\ket{\phi_{\ell}}}\}_{\ell=1}^{d_B}$ is orthonormal, so that $U_B \coloneqq  \sum_{\ell=1}^{d_B} \ket{\phi_{\ell}}\!\conj{\bra{\phi_{\ell}}}_B$ is a unitary operator. Then we find that
		\begin{equation}
		\sum_{\ell, \ell'=1}^{d_B}\left(\mathbbm{1}_{A}\otimes \ket{\phi_{\ell'}}
	\bra{\phi_{\ell}}_{B}\right)\rho_{AB}\left(\mathbbm{1}_{A}\otimes\ket{\phi_{\ell'}}
	\bra{\phi_{\ell}}_B\right) = U_B\T_B(\rho_{AB})U_B^\dag \geq 0, 
		\end{equation}
		where the last inequality follows from the condition $\T_B(\rho_{AB}) \geq 0$ and property~1 of Lemma~\ref{prop-operator_ineqs}. We thus conclude that the PPT property  does not depend on which orthonormal basis is used to define the transpose map.
		
	The partial transpose map plays an important role in quantum information theory due to its connection with entanglement. In fact, it leads to a	sufficient condition for a bipartite state to be entangled. To see this, suppose that a state $\sigma_{AB}$ is a separable, unentangled state of the following form:
	\begin{equation}
		\sigma_{AB}=\sum_{x\in\mathcal{X}}p(x)\omega_{A}^{x}\otimes\tau_{B}^{x},
	\end{equation}
	where $p:\mathcal{X}\to[0,1]$ is a probability distribution on a finite alphabet $\mathcal{X}$ and $\{\omega_{A}^{x}\}_{x\in\mathcal{X}}$ and $\{\tau_{B}^{x}\}_{x\in\mathcal{X}}$ are sets of quantum states. Then, the action of the partial transpose map $\T_{B}$ on $\sigma_{AB}$ is as follows:
	\begin{equation}
		\T_{B}(\sigma_{AB})=\sum_{x}p(x)\omega_{A}^{x}\otimes \T(\tau_{B}^{x}),
	\end{equation}
	which is a separable quantum state, being the expected state of the ensemble $\{(p(x),\omega_{A}^{x}\otimes\T(\tau_{B}^{x}))\}_{x\in\mathcal{X}}$. Each element of the ensemble is indeed a quantum state because the transpose is a positive map, i.e., $\T(\tau_{B}^{x})\geq 0$ if $\tau_{B}^{x}\geq 0$. Due to this fact, we conclude that $\T_{B}(\sigma_{AB})\geq 0$, so that $\sigma_{AB}$ is a PPT state. Thus, we conclude the following:
	\begin{specbox}{0.6\textwidth}
		If a state is separable, then it is PPT.
	\end{specbox}
	This is called the \textit{PPT criterion}.
	Equivalently, by taking the contrapositive of this statement, we obtain the following:
	\begin{specbox}{0.6\textwidth}
		If a state is not PPT, then it is entangled.
	\end{specbox}
	So the condition of a state being NPT (non-positive partial transpose) is sufficient for detecting entanglement.
	
	As an example, let us consider applying the partial transpose map $\T_{B}$ to the maximally entangled state $\Phi_{AB}$, as defined in \eqref{eq-max_ent_state}.
	We find that
	\begin{align}
		\T_B(\Phi_{AB})&=\frac{1}{d} \,\T_B\!\left(\sum_{i,i'=1}^d\ket{i}\!\bra{i'}_A\otimes\ket{i}\!\bra{i'}_B\right) \\
		&=\sum_{i,i'=1}^d \ket{i}\!\bra{i'}_A\otimes\ket{i'}\!\bra{i}_B\\
		&\eqqcolon\frac{1}{d}F_{AB},\label{eq-swap_operator}
	\end{align}
	where we have defined the \textit{swap operator} $F_{AB}$ as
	\begin{equation}\label{eq-swap_op_standard}
		F_{AB}\coloneqq \sum_{i,i'=1}^d\ket{i}\!\bra{i'}_A\otimes \ket{i'}\!\bra{i}_B=\sum_{i,i'=1}^d\ket{i,i'}\!\bra{i',i}_{AB}
	\end{equation}
	The swap operator is Hermitian and satisfies $F_{AB}^2=\mathbbm{1}_{AB}$, meaning that it is also unitary and self-inverse. The swap operator has the following spectral decomposition:
	\begin{equation}
	F_{AB} = \Pi^{\mathcal{S}}_{AB} - \Pi^{\mathcal{A}}_{AB},
	\label{eq:qm:spectral-decomp-swap-op}
	\end{equation}
	where
	\begin{equation}
	\Pi^{\mathcal{S}}_{AB}\coloneqq \tfrac{1}{2}\left(\mathbbm{1}_{AB} + F_{AB}\right)
	\end{equation}
	 is the projection onto the symmetric subspace of $\mathbb{C}^d\otimes\mathbb{C}^d$, which has dimension $\Tr[\Pi^{\mathcal{S}}_{AB}] = d(d+1)/2$ (see \eqref{eq-proj_symm_subspace}), and
	 \begin{equation}
	 \Pi^{\mathcal{A}}_{AB}\coloneqq \tfrac{1}{2}\left(\mathbbm{1}_{AB} - F_{AB}\right)
	 \end{equation}
	  is the projection onto the anti-symmetric subspace of $\mathbb{C}^d\otimes\mathbb{C}^d$, with dimension $\Tr[\Pi^{\mathcal{A}}_{AB}] = d(d-1)/2$ (see \eqref{eq-proj_asymm_subspace}). Note that $\Pi^{\mathcal{S}}_{AB} + \Pi^{\mathcal{A}}_{AB} = \mathbbm{1}_{AB}$ and $\Pi^{\mathcal{S}}_{AB} \Pi^{\mathcal{A}}_{AB} = 0$. Thus, the swap operator has negative eigenvalues, which by the PPT criterion means that $\Phi_{AB}$ is an entangled state, as expected.
	
	Although the PPT criterion is generally only a necessary condition for separability of a bipartite state, it is known that the PPT criterion is necessary and sufficient for quantum states $\rho_{AB}$ in which both $A$ and $B$ are qubits or $A$ is a qubit and $B$ is a qutrit; please consult the Bibliographic Notes in Section~\ref{sec:qm:bib-notes}. In particular, therefore, in higher dimensions there are PPT states that are entangled. These PPT entangled states turn out to be useless for the task of entanglement distillation (see Chapter~\ref{chap-ent_distill}), and thus they are called \textit{bound entangled} (although they are entangled, they cannot be used to extract pure maximally entangled states).


%	The basis in which we take the partial transpose map need not be the same as the basis for the maximally entangled state $\Phi_{AB}$, so let us take the partial transpose $\T_{B}$ with respect to the orthonormal basis $\{\ket{\phi_i}\}_{i}$. For every operator $X_{AB}$, we get
%	\begin{equation}
%		\T_{B}(X_{AB})=\sum_{i,j=0}^{d-1}(\mathbbm{1}_{A}\otimes\ket{\phi_i}\!\bra{\phi_j}_{B})X_{AB}(\mathbbm{1}_{A}\otimes\ket{\phi_i}\!\bra{\phi_j}_{B}).
%	\end{equation}
%	Performing this partial transpose on the maximally entangled state $\Phi_{AB}$ gives
%	\begin{align}
%		&\T_{B}(\Phi_{AB})\\
%		&=\sum_{i,j=0}^{d-1}(\mathbbm{1}_{A}\otimes\ket{\phi_i}\!\bra{\phi_j}_{B})\left(\frac{1}{d}\sum_{i',j'=1}^d\ket{i',i'}\!\bra{j',i'}_{AB}\right)(\mathbbm{1}_{A}\otimes\ket{\phi_i}\!\bra{\phi_j}_{B})\label{eq:partial-transpose-max-ent-state-1}\\
%		&=\frac{1}{d}\sum_{i,j,i',j'=1}^d\ket{i'}\!\bra{j'}_{A}\otimes \ket{\phi_i}\braket{\phi_j}{i'}\braket{j'}{\phi_i}\!\bra{\phi_j}_B\\
%		& =\frac{1}{d}\sum_{i,j=0}^{d-1}\left[\sum_{i'=1}^d\braket{\phi_j}{i'}\ket{i'}\right]\left[\sum_{j'=1}^d\bra{j'}_A\braket{j'}{\phi_i}\right] \otimes\ket{\phi_i}\!\bra{\phi_j}_B\\
%		&=\frac{1}{d}\sum_{i,j=0}^{d-1}\ket{\conj{\phi_j}}\!\bra{\conj{\phi_i}}_A\otimes\ket{\phi_i}\!\bra{\phi_j}_{B}\\
%		&  =\frac{1}{d}F_{AB},\label{eq:partial-transpose-max-ent-state-last}
%	\end{align}
%	where in the last two lines we have made use of the definition \textcolor{red}{\textbf{[]}} of the complex conjugate $\ket{\phi_j}=\sum_{i=0}^{d-1}\braket{\phi_j}{i}\ket{i}$ of $\ket{\phi_j}$ with respect to the orthonormal basis $\{\ket{i}\}_{i}$ and we have also defined the swap operator $F_{AB}$ (with respect to the orthonormal basis $\{\ket{\phi_i}\}_i$) as
%	\begin{equation}\label{eq-swap_op_alt}
%		F_{AB}=\sum_{i,j=0}^{d-1}\ket{\conj{\phi_j}}\!\bra{\conj{\phi_i}}\otimes \ket{\phi_i}\!\bra{\phi_j}_{B}.
%	\end{equation}
%	To verify that the operator $F_{AB}$ above is unitary, just like the swap operator $F_{AB}$ defined in \eqref{eq-swap_op_standard} with respect to the standard basis, one can employ the fact that $\{\ket{\conj{\phi_i}}\}_{i}$ is an orthonormal basis as a consequence of $\{\ket{\phi_i}\}_{i}$ being one. Additionally, just like the swap operator in \eqref{eq-swap_op_standard}, the swap operator $F_{AB}$ in \eqref{eq-swap_op_alt} has negative eigenvalues.


\subsection{Measurements}\label{subsec-meas}
	
	Measurements in quantum mechanics are described by \textit{positive operator-valued measures (POVMs)}.
	\begin{definition}{Positive Operator-Valued Measure (POVM)}{def:qm:povm}
	A POVM is a set $\{M_x\}_{x\in\mathcal{X}}$ of operators satisfying
	\begin{equation}
		M_x\geq 0\quad\forall~x\in\mathcal{X},\qquad \sum_{x\in\mathcal{X}}M_x=\mathbbm{1}.
	\end{equation}
	For our purposes, it suffices to consider finite sets of such operators. The elements of the finite alphabet $\mathcal{X}$ are used to label the outcomes of the measurement.
	\end{definition}
	
	The measurement of a quantum system in the state $\rho$ according to the POVM $\{M_x\}_{x\in\mathcal{X}}$ induces a probability distribution $p_X:\mathcal{X}\to[0,1]$. This distribution corresponds to a random variable $X$, which takes values in the alphabet $\mathcal{X}$, and is defined by the \textit{Born rule}:
	\begin{equation}\label{eq-Born_rule}
		p_X(x)=\Pr[X=x]=\Tr[M_x\rho].
	\end{equation}   
	
	If the elements $M_x$ of the POVM are all projections, then the corresponding measurement is called a \textit{projective measurement}. If the POVM of a projective measurement consists solely of rank-one projections, then the measurement is sometimes called a \textit{von Neumann measurement}. Projective measurements, in particular von Neumann measurements, are viewed as the simplest type of measurement that can be performed on a quantum system. However, as it turns out, we can implement every measurement as a von Neumann measurement if we have access to an auxiliary quantum system, and this is the content of \textit{Naimark's theorem}.
	
	\begin{theorem*}{Naimark's Theorem}{thm-naimark}
		For every POVM $\{M_x\}_{x\in\mathcal{X}}$, there exists an isometry $V$ such that
		\begin{equation}
			M_x=V^\dagger (\mathbbm{1}\otimes\ket{x}\!\bra{x})V\quad\forall~x\in\mathcal{X}.
			\label{eq-naimark-ext}
		\end{equation}
	\end{theorem*}
	
	\begin{Proof}
		This follows immediately by defining the isometry $V$ as
		\begin{equation}
			V=\sum_{x\in\mathcal{X}}\sqrt{M_x}\otimes\ket{x}.
			\label{eq-naimark-ext-choice}
		\end{equation}
		This is indeed an isometry because
		\begingroup
		\allowdisplaybreaks[0]
		\begin{align}
			V^\dagger V&=\left(\sum_{x\in\mathcal{X}}\sqrt{M_x}\otimes\bra{x}\right)\left(\sum_{x'\in\mathcal{X}}\sqrt{M_{x'}}\otimes\ket{x'}\right)\\
			&=\sum_{x,x'\in\mathcal{X}}\sqrt{M_x}\sqrt{M_{x'}}\braket{x}{x'}\\
			&=\sum_{x\in\mathcal{X}}M_x\\
			&=\mathbbm{1},
		\end{align}
		\endgroup
		where the last equality holds because $\{M_x\}_{x\in\mathcal{X}}$ is a POVM. It is straightforward to check that \eqref{eq-naimark-ext} is satisfied for the choice of $V$ in \eqref{eq-naimark-ext-choice}.
	\end{Proof}
	
	\begin{figure}
		\centering
		\includegraphics[scale=0.8]{Figures/naimark.pdf}
		\caption{The system-probe model of measurement. In order to measure the system $A$ of interest, we allow it to first interact with a probe system $P$ via an isometry $V_{A\to A'P}$. We then measure the probe with a projective measurement consisting of rank-one elements.}\label{fig-naimark}
	\end{figure}
	
	The physical relevance of Naimark's theorem is illustrated in Figure \ref{fig-naimark}. We model the measurement of the system $A$ of interest as an interaction of the system with a \textit{probe} system $P$ followed by a projective measurement of the probe system described by the POVM $\{\ket{x}\!\bra{x}:x\in\mathcal{X}\}$. The interaction is described by an isometry $V_{A\to A'P}$, and if $\rho_{AP}=V\rho_A V^\dagger$ is the joint state of the system and the probe after the interaction, then the measurement outcome probabilities are
	\begin{align}
		p_X(x)&=\Tr[(\mathbbm{1}_{A'}\otimes\ket{x}\!\bra{x})\rho_{A'P}]\\
		&=\Tr[(\mathbbm{1}_{A'}\otimes\ket{x}\!\bra{x})V\rho_AV^\dagger]\\
		&=\Tr[V^\dagger(\mathbbm{1}_{A'}\otimes\ket{x}\!\bra{x})V\rho_A]\\
		&=\Tr[M_x\rho_A],
	\end{align}
	where we let $M_x\coloneqq V^\dagger(\mathbbm{1}_{A'}\otimes\ket{x}\!\bra{x})V$. This shows us that the system-probe model of measurement, in which the probe is measured after it interacts with the system of interest, can effectively be described by a POVM. Naimark's theorem, on the other hand, tells us the converse: for every measurement described by a POVM, there exists an isometry such that the measurement can be described in the system-probe model, as depicted in Figure \ref{fig-naimark}.
	
	When performing measurements in quantum mechanics, we are typically interested not only in the measurement outcomes and their probabilities but also with the so-called \textit{post-measurement} states of the system being measured. That is, we are interested in knowing the state of the system after we have measured it and observed the outcome.
	
	Since the POVM elements $M_x$ are positive semi-definite, there exist operators $K_x$ such that $M_x=K_x^\dagger K_x$ for all $x\in\mathcal{X}$. For example, we could let $K_x$ be the square root of $M_x$, so that $K_x=\sqrt{M_x}$. Then, the Born rule in \eqref{eq-Born_rule} for the probability of the measurement outcome $x\in\mathcal{X}$ can be written as $p_X(x)=\Tr[K_x\rho K_x^\dagger]$. In this case, the post-measurement state corresponding to the outcome $x\in\mathcal{X}$ is as follows:
	\begin{equation}\label{eq-post_meas}
		\rho^x\coloneqq \frac{K_x\rho K_x^\dagger}{\Tr[K_x\rho K_x^\dagger]}.
	\end{equation}
	The state $\rho^x$ can be understood to capture the experimenter's knowledge of the state of the system given that the measurement outcome was observed to be $x$. 
	
		The post-measurement states $\rho^x$ give rise to the ensemble $\{(p_X(x),\rho^x)\}_{x\in\mathcal{X}}$. The expected density operator of the ensemble is
	\begin{equation}\label{eq-post_meas_avg}
		\rho_{\mathcal{M}}\coloneqq\sum_{x\in\mathcal{X}}p_X(x)\rho^x=\sum_{x\in\mathcal{X}}K_x\rho K_x^\dagger.
	\end{equation}
	This expected density operator is the state of the system after measurement if the measurement outcome is not available. It can be interpreted as the state of the system after measurement if the experimenter has no knowledge of which measurement outcome occurred.
	
	Due to the unitary freedom in the decomposition $M_x=K_x^\dagger K_x$, other choices of $K_x$ are given by $K_x=U_x \sqrt{M_x}$ for some unitary $U_x$, so that there is not a unique way to determine the post-measurement state when starting from a POVM.
	
	Suppose now that we perform a measurement on a subsystem of a composite system. Specifically, consider measuring a system $A$ that is in a joint state $\rho_{RA}$ with a reference system $R$, and let the measurement be described by the POVM $\{M_A^x\}_{x\in\mathcal{X}}$ for some finite alphabet $\mathcal{X}$. If we let $M_A^x=K_A^{x\dagger}K_A^x$, then according to \eqref{eq-post_meas}, the measurement probabilities are given by $p_X(x)=\Tr[(\mathbbm{1}_R\otimes K_A^x)\rho_{RA}(\mathbbm{1}_R\otimes K_A^{x\dagger})]$ and the post-measurement states are as follows:
	\begin{align}
		\rho_{RA}^x&=\frac{(\mathbbm{1}_R\otimes K_A^x)\rho_{RA}(\mathbbm{1}_R\otimes K_A^{x\dagger})}{\Tr[(\mathbbm{1}_R\otimes K_A^x)\rho_{RA}(\mathbbm{1}_R\otimes K_A^{x\dagger})]}\\
		&=\frac{1}{p_X(x)}(\mathbbm{1}_R\otimes K_A^x)\rho_{RA}(\mathbbm{1}_R\otimes K_A^{x\dagger})
	\end{align}
	for all $x\in\mathcal{X}$. The state of the system $R$ conditioned on the measurement outcome $x$ is then
	\begin{align}
		\rho_R^x&\coloneqq\Tr_A[\rho_{RA}^x]\\
		&=\frac{1}{p_X(x)}\Tr_A[(\mathbbm{1}_R\otimes K_A^x)\rho_{RA}(\mathbbm{1}_R\otimes K_A^{x\dagger})]\\
		&=\frac{1}{p_X(x)}\Tr_A[(\mathbbm{1}_R\otimes K_A^{x\dagger}K_A)\rho_{RA}]\\
		&=\frac{1}{p_X(x)}\Tr_A[(\mathbbm{1}_R\otimes M_A^x)\rho_{RA}].\label{eq-post_meas_state_half}
	\end{align}
	We thus see that, although the post-measurement state on the system $A$ being measured is not uniquely defined due to the unitary freedom in the decomposition $M_A^x=K_A^{x\dagger}K_A^x$, as described earlier, the post-measurement state on the reference system $R$ not being measured is uniquely defined because it depends directly on the POVM elements $M_A^x$. If the system $A$ undergoes a measurement for which $M_A^x=\ket{\psi^x}\!\bra{\psi^x}_A$, then \eqref{eq-post_meas_state_half} can be written as
	\begin{equation}\label{eq-post_meas_state_half_proj}
		\rho_R^x=\frac{1}{p_X(x)}\bra{\psi^x}_A\rho_{RA}\ket{\psi^x}_A.
	\end{equation}




\subsection{Quantum State Discrimination}\label{subsec-state_discrimination}

	Having described measurements in quantum mechanics, let us now discuss an important application called \textit{quantum state discrimination}. It is also known as symmetric or Bayesian quantum hypothesis testing.
	
	Suppose that Alice prepares a quantum system in one of two states, $\rho$ or~$\sigma$, the first with probablity $\lambda$ and the second with probability $1-\lambda$, and sends the system to Bob without telling him which state she prepared. Bob's task is to guess the state of the system by performing only one measurement, knowing in advance both the prior probability $\lambda$ and that the state is either $\rho$ or $\sigma$. What is Bob's highest probability of correctly guessing the state, and which measurement can he use to achieve the maximum success probability?
	
	 This scenario is depicted in Figure \ref{fig-state_disc} along with the strategy that Bob can employ, which is the following:
	 \begin{enumerate}
	 	\item He picks a measurement that can be described by the two-element POVM $\{M_\rho,M_\sigma\}$. Note that $M_\rho, M_\sigma \geq 0$ and 
		$M_\rho+M_\sigma=\mathbbm{1}$, by the definition of a POVM, which means that $M_\sigma=\mathbbm{1}-M_\rho$.
	 	\item If the outcome corresponding to $M_\rho$ occurs, then Bob guesses ``$\rho$''; otherwise, if the outcome corresponding to $M_\sigma$ occurs, he guesses ``$\sigma$''.
	 \end{enumerate}
	 
	 \begin{figure}
	 	\centering
	 	\includegraphics[scale=1]{Figures/state_discrimination.pdf}
	 	\caption{Decision tree for the state discrimination problem. Given that Bob receives the state $\rho$ with probability $\lambda$ and the state $\sigma$ with probability $1-\lambda$, he performs a measurement described by the POVM $\{M_\rho,M_\sigma\}$, where $M_\sigma=\mathbbm{1}-M_\rho$. Conditioned on the outcome of his measurement, he guesses the state of the system to be either $\rho$ or $\sigma$.}\label{fig-state_disc}
	 \end{figure}
	 
	 Bob's strategy is successful if his guess is correct; i.e., it is correct when the system is in the state $\rho$ and he guesses ``$\rho$''  or when the system is in the state $\sigma$ and he guesses ``$\sigma$''. By following the decision tree in Figure \ref{fig-state_disc}, we find that the success probability of his strategy is
	 \begin{align}
	 	&\!\!\!\!\!\! p_{\text{succ}}(\{M_\rho,M_\sigma\};\{\lambda,\rho,\sigma\})\nonumber \\
		&\coloneqq \Pr[\text{state is }\rho\text{ and Bob guesses ``$\rho$''}]\nonumber\\
	 	&\qquad +\Pr[\text{state is }\sigma\text{ and Bob guesses ``$\sigma$''}]\nonumber\\
	 	&=\Pr[\text{state is }\rho]\cdot\Pr[\text{Bob guesses ``$\rho$''}~|~\text{state is }\rho]\nonumber\\
	 	&\qquad +\Pr[\text{state is }\sigma]\cdot\Pr[\text{Bob guesses ``$\sigma$''}~|~\text{state is }\sigma]\nonumber\\
	 	&=\lambda\Tr[M_\rho\rho]+(1-\lambda)\Tr[M_\sigma\sigma]\nonumber\\
	 	&=\lambda\Tr[M_\rho\rho]+(1-\lambda)\Tr[(\mathbbm{1}-M_\rho)\sigma]\nonumber\\
	 	&=\Tr[M_\rho(\lambda\rho)]+\Tr[(\mathbbm{1}-M_\rho)((1-\lambda)\sigma)].\label{eq-state_disc_success}
	 \end{align}
 We can manipulate the last line above to find that
 \begin{equation}
 p_{\text{succ}}(\{M_\rho,M_\sigma\};\{\lambda,\rho,\sigma\}) = 1-\lambda + \Tr[M_\rho(\lambda\rho-(1-\lambda)\sigma)],
 \end{equation}
 where we used the fact that $\Tr[\sigma]=1$.
 
 The error probability is then
	 \begin{align}
	 	p_{\text{err}}(\{M_\rho,M_\sigma\};\{\lambda,\rho,\sigma\})&\coloneqq 1-p_{\text{succ}}(\{M_\rho,M_\sigma\};\{\lambda,\rho,\sigma\})\\
	 	&=\lambda-\Tr[M_\rho(\lambda\rho-(1-\lambda)\sigma)]\\
	 	&=\Tr[(\mathbbm{1}-M_{\rho})(\lambda\rho)]+\Tr[M_{\rho}(1-\lambda)\sigma].\label{eq-state_disc_error}
	 \end{align}
	 
	The \textit{optimal} success probability is given by maximizing the success probability in \eqref{eq-state_disc_success} over all two-outcome POVMs. Equivalently, we can optimize over all operators $M$ satisfying $0\leq M\leq\mathbbm{1}$:
	\begin{equation}
	 	p_{\text{succ}}^*(\lambda,\rho,\sigma)\coloneqq\sup_{M:0\leq M\leq \mathbbm{1}}\left\{1-\lambda + \Tr[M(\lambda\rho-(1-\lambda)\sigma)]\right\}.
	\end{equation}
	Similarly, the optimal error probability is given by minimizing the error probability \eqref{eq-state_disc_error} over all operators $M$ satisfying $0\leq M\leq\mathbbm{1}$:
	\begin{equation}\label{eq-state_disc_opt_error_def}
	 	p_{\text{err}}^*(\lambda,\rho,\sigma)\coloneqq\inf_{M:0\leq M\leq\mathbbm{1}}\left\{\Tr[(\mathbbm{1}-M)(\lambda\rho)]+\Tr[M(1-\lambda)\sigma]\right\}.
	\end{equation}
	The solution to this optimization problem is given by Theorem~\ref{thm-Holevo_Helstrom}.
	 
	\begin{theorem*}{Helstrom--Holevo Theorem}{thm-Holevo_Helstrom}
		For every two positive semi-definite operators $A$ and $B$, 
		\begin{multline}\label{eq-Holevo_Helstrom}
			\inf_{M:0\leq M\leq\mathbbm{1}}\left\{\Tr[(\mathbbm{1}-M)A]+\Tr[MB]\right\}\\=\frac{1}{2}\left(\Tr[A+B]-\norm{A-B}_1\right).
		\end{multline}
		A measurement operator $M$ is optimal if and only if $M = \Pi_+ + \Lambda_0$, where $\Pi_+$ is the projection onto the strictly  positive part of $A-B$, the operator $\Pi_0$ is the projection onto the zero eigenspace of $A-B$, and $0 \leq \Lambda_0 \leq \Pi_0$. Furthermore, 
		\begin{equation}\label{eq-Holevo_Helstrom-alt}
			\sup_{M:0\leq M\leq\mathbbm{1}}\Tr[M(A-B)] = \frac{1}{2}\left(\Tr[A-B] + \norm{A-B}_1\right),
		\end{equation}
		and the conditions for an optimal $M$ are the same as given above.
	\end{theorem*}
	
	Letting $A=\lambda\rho$ and $B=(1-\lambda)\sigma$ in \eqref{eq-Holevo_Helstrom}, we recognize that the objective function on the left-hand side of \eqref{eq-Holevo_Helstrom} is equal to $p_{\text{err}}(\{M,\mathbbm{1}-M\};\{\lambda,\rho,\sigma\})$ as defined in \eqref{eq-state_disc_error}. We thus obtain
	\begin{equation}\label{eq-state_disc_opt_error}
		p_{\text{err}}^*(\lambda,\rho,\sigma)=\frac{1}{2}\left(1-\norm{\lambda\rho-(1-\lambda)\sigma}_1\right).
	\end{equation}
	Note that Theorem~\ref{thm-Holevo_Helstrom} also gives us a measurement that achieves the minimal error probability.
	
	\begin{Proof}[Proof of Theorem~\ref{thm-Holevo_Helstrom}]
		Let $M$ satisfying $0\leq M\leq\mathbbm{1}$ be arbitrary. Let $\Delta \coloneqq A-B$ and let $\Delta_+$ and $\Delta_-$ be the positive and negative parts, respectively, of $\Delta$, so that $A-B=\Delta_+-\Delta_-$ and $\Delta_+\Delta_-=0$ (recall \eqref{eq-operator_pos_neg_decomp}). We can then write the objective function in \eqref{eq-Holevo_Helstrom} as
		\begin{equation}
			\Tr[(\mathbbm{1}-M)A]+\Tr[MB] = \Tr[A]-\left(\Tr[M\Delta_+]-\Tr[M\Delta_-]\right).
			\label{eq-Holevo_Helstrom-rewrite}
		\end{equation}
		Now, since $\Tr[M\Delta_-]\geq 0$, on account of both $M$ and $\Delta_-$ being positive semi-definite, we find that
		\begin{align}
			\Tr[M\Delta_+]-\Tr[M\Delta_-] \leq \Tr[M\Delta_+] \leq \Tr[\Delta_+],
			\label{eq-up-bnd-trace-norm-1}
		\end{align}
		where  the last inequality follows because $M\leq\mathbbm{1}$.
		However, since
		\begin{equation}
			\norm{A-B}_1=\Tr[|A-B|]=\Tr[\Delta_+]+\Tr[\Delta_-]
		\end{equation}
		and
		\begin{equation}
			\Delta_-=\Delta_++B-A,
		\end{equation}
		we can write $\Tr[\Delta_+]$ as
		\begin{equation}\label{eq-state_disc_pf}
			\Tr[\Delta_+]=\frac{1}{2}\left(\norm{A-B}_1-\Tr[B-A]\right),
		\end{equation}
		which means that the objective function on the left-hand side of \eqref{eq-Holevo_Helstrom-rewrite} can be bounded from below by $\frac{1}{2}\left(\Tr[A\allowbreak+B]-\norm{A-B}_1\right)$. We have thus shown that
		\begin{equation}\label{eq-state_disc_pf2}
			\Tr[(\mathbbm{1}-M)A]+\Tr[MB]\geq \frac{1}{2}\left(\Tr[A+B]-\norm{A-B}_1\right).
		\end{equation}
		for all $M$ such that $0\leq M\leq \mathbbm{1}$, which implies that
		\begin{equation}
			\inf_{M:0\leq M\leq\mathbbm{1}}\Tr[(\mathbbm{1}-M)A]+\Tr[MB]
			\geq \frac{1}{2}\left(\Tr[A+B]-\norm{A-B}_1\right).
			\end{equation}
		
		To see the reverse inequality, let $M = \Pi_+ + \Lambda_0$, where $\Pi_+$ is the projection onto the strictly positive part of $A-B$ and $\Lambda_0$ satisfies $0 \leq \Lambda_0 \leq \Pi_0$, with $\Pi_0$ the projection onto the zero eigenspace of $A-B$. Then,
		\begin{align}
			\Tr[M(A-B)]&=\Tr[(\Pi_+ + \Lambda_0)(\Delta_+-\Delta_-)] \label{eq-up-bnd-trace-norm-2}\\
			&=\Tr[(\Pi_+ + \Lambda_0)\Delta_+]-\Tr[(\Pi_+ + \Lambda_0)\Delta_-]\\
			&=\Tr[\Delta_+] \label{eq-up-bnd-trace-norm-3},
		\end{align}
		where  the last equality follows because $\Tr[\Pi_+\Delta_+]=\Tr[\Delta_+]$ and $\Tr[\Pi_+\Delta_-]=0$, since $\Pi_+$ and $\Delta_-$ are by definition orthogonal. We also used $\Tr[\Lambda_0 \Delta_+] = \Tr[\Lambda_0 \Delta_-]=0$, with these latter equalities following because $0 \leq \Tr[\Lambda_0 \Delta_{\pm}] \leq \Tr[\Pi_0 \Delta_{\pm}] = 0$. Therefore, using \eqref{eq-state_disc_pf}, we find that
		\begin{equation}
			\Tr[A]-\Tr[(\Pi_+ + \Lambda_0)(A-B)]=\frac{1}{2}\left(\Tr[A+B]-\norm{A-B}_1\right).
		\end{equation}
		The operator $\Pi_+ + \Lambda_0$ thus achieves the bound in \eqref{eq-state_disc_pf2}, which means that
		\begin{equation}
			\inf_{M:0\leq M\leq \mathbbm{1}}\Tr[(\mathbbm{1}-M)A]+\Tr[MB]=\frac{1}{2}\left(\Tr[A+B]-\norm{A-B}_1\right),
		\end{equation}
		so that \eqref{eq-Holevo_Helstrom} is established.
		
		To see that $\Pi_+ + \Lambda_0$ is the only form for an optimal measurement operator, suppose that $M$ is optimal, i.e., satisfies $0 \leq M \leq \mathbbm{1}$ and saturates \eqref{eq-Holevo_Helstrom} with equality. Then it follows that the two inequalities in \eqref{eq-up-bnd-trace-norm-1} are saturated with equality, so that
		\begin{equation}
		 \Tr[M(\Delta_+ - \Delta_-)] = \Tr[M \Delta_+] = \Tr[ \Delta_+]= \Tr[\Pi_+ \Delta_+].
		\end{equation}
		This implies that $\Tr[M \Delta_-] = 0$, where $\Delta_-$ is the  strictly negative part of $A-B$. Since both $M$ and $\Delta_-$ are positive semi-definite and $\Pi_-$ is the projection onto the strictly negative part of $\Delta_-$, we conclude that $M \Pi_- =  \Pi_- M = 0$. This in turn implies that
		\begin{equation}
		M (\Pi_+ + \Pi_0)= (\Pi_+ + \Pi_0) M = M,
		\end{equation}
		which, after sandwiching $M \leq \mathbbm{1}$ on the left and right by $\Pi_+ + \Pi_0$, implies that $M \leq \Pi_+ + \Pi_0$.
		Since
		\begin{align}
		0 & = \Tr[\Delta_+ (\Pi_+  - M)] \\
		& =
		\Tr[\Delta_+ (\Pi_+  - \Pi_+ M \Pi_+ )] \\
		& =\Tr[\Delta_+ \Pi_+ (\mathbbm{1}  -  M  )\Pi_+],
		\end{align}
		we find that $\Pi_+ (\mathbbm{1}  -  M  )\Pi_+ = 0$. Now consider that $\Pi_- (\mathbbm{1}  -  M  )\Pi_+ = 0$ because $\Pi_- \Pi_+ =0 $ and $\Pi_- M  \Pi_+ = \Pi_- (\Pi_+ + \Pi_0) M  \Pi_+ = 0$. So then $\Pi_+ (\mathbbm{1}  -  M  )\Pi_+ = 0$ and $\Pi_- (\mathbbm{1}  -  M  )\Pi_+ = 0$ imply that $(\mathbbm{1}  -  M  )\Pi_+ = 0$. From this equation, we conclude that $\Pi_+  = \Pi_+ M = M \Pi_+$. By sandwiching $\Pi_+ \leq \mathbbm{1}$ by $M$ and applying operator monotonicity of the square-root function (see Section~\ref{sec:math-tools:functions-herm-ops}), we conclude that $\Pi_+ \leq M$. Combining this operator inequality with the previous one, we conclude that an optimal $M$ satisfies $\Pi_+ \leq M \leq \Pi_+ + \Pi_0$, which is equivalent to $M$ decomposing as $M = \Pi_+ + \Lambda_0$ for $0 \leq \Lambda_0 \leq \Pi_0$.
		
		The equality in \eqref{eq-Holevo_Helstrom-alt} follows as a rewrite of \eqref{eq-Holevo_Helstrom}:
		\begin{align}
		\frac{1}{2}\norm{A-B}_1 & = \frac{1}{2}\Tr[A+B] - \inf_{M:0\leq M\leq\mathbbm{1}}\Tr[(\mathbbm{1}-M)A]+\Tr[MB] \\
		&  = \sup_{M:0\leq M\leq\mathbbm{1}}\frac{1}{2}\Tr[A+B] - (\Tr[(\mathbbm{1}-M)A]+\Tr[MB]) \\
		&  = \sup_{M:0\leq M\leq\mathbbm{1}}\frac{1}{2}\Tr[B-A] + \Tr[M(A-B)] \\
		&  = \frac{1}{2}\Tr[B-A] + \sup_{M:0\leq M\leq\mathbbm{1}} \Tr[M(A-B)].
		\end{align}
Rearranging this equality, we arrive at \eqref{eq-Holevo_Helstrom-alt}.
		An optimal $M$ having the form $\Pi_+ + \Lambda_0$  again follows from \eqref{eq-up-bnd-trace-norm-1}, \eqref{eq-up-bnd-trace-norm-2}--\eqref{eq-up-bnd-trace-norm-3}, and the reasoning given above. 
	\end{Proof}	
	
	The Helstrom--Holevo theorem gives us the lowest possible error probability in distinguishing between two states $\rho$ and $\sigma$, given just one copy of either state. Suppose now that, instead of just one copy, Alice sends Bob $n$~copies of either $\rho$ or $\sigma$. Bob's task is then to discriminate between the states $\rho^{\otimes n}$ and $\sigma^{\otimes n}$. The Helstrom--Holevo theorem still applies in this case, so that
	\begin{equation}
		p_{\text{err}}^*(\lambda\rho^{\otimes n},\bar{\lambda}\sigma^{\otimes n})=\frac{1}{2}\left(1-\norm{\lambda\rho^{\otimes n}-(1-\lambda)\sigma^{\otimes n}}_1\right)
	\end{equation}
	is the lowest possible error probability. However, because Bob now has $n$ copies of either $\rho$ or $\sigma$, he can perform a  discrimination strategy that involves a collective measurement acting on the $n$ copies of the state. This means that the optimal \textit{error exponent} can generally be lower with $n\geq 2$ copies than with just one copy. In other words, it is possible to have $p_{\text{err}}^*(\lambda\rho^{\otimes n},\bar{\lambda}\sigma^{\otimes n})<(p_{\text{err}}^*(\lambda,\rho,\sigma))^n$. If we allow for an arbitrary number $n$ of copies of either state, then we are interested in the lowest possible error exponent that can be achieved. Specifically, we are interested in the optimal asymptotic error exponents, defined as follows:
	\begin{align}
		\underline{\xi}(\rho,\sigma) & \coloneqq \liminf_{n\to \infty}-\frac{1}{n}\log_2 p_{\text{err}}^*(\lambda\rho^{\otimes n},\bar{\lambda}\sigma^{\otimes n}),
		\label{eq:qm-over:chernoff-def-lower}\\
		\overline{\xi}(\rho,\sigma) & \coloneqq \limsup_{n\to \infty}-\frac{1}{n}\log_2 p_{\text{err}}^*(\lambda\rho^{\otimes n},\bar{\lambda}\sigma^{\otimes n}).
		\label{eq:qm-over:chernoff-def-upper}
	\end{align}
	In defining these exponents, we have suppressed the dependence on the prior probability $\lambda$ because, as we will see, they do not depend on them when taking the limit.
	We define the two asymptotic quantities separately, mainly because the limit $\lim_{n \to \infty}$ need not exist \textit{a priori} (see Section~\ref{sec:math-tools:cont-inf-sup}).
	The \textit{quantum Chernoff divergence} of states $\rho$ and $\sigma$ is defined as follows:
	\begin{equation}
		C(\rho\Vert\sigma) \coloneqq \sup_{s\in(0,1)} \left( -\log_2\Tr[\rho^s\sigma^{1-s}]\right),
		\label{eq:qm:chern-divergence}
		\end{equation}
		and finds its operational meaning in the following theorem:
		
	\begin{theorem*}{Quantum Chernoff Bound}{thm-quantum_Chernoff}
		For every  two quantum states $\rho$ and $\sigma$, the optimal asymptotic error exponents are equal to the quantum Chernoff divergence:
		\begin{equation}\label{eq-quantum_Chernoff_bound}
			\underline{\xi}(\rho,\sigma) = \overline{\xi}(\rho,\sigma) = C(\rho\Vert\sigma).
		\end{equation}
	\end{theorem*}
	
	\begin{Proof}
		See Appendix~\ref{app-Chernoff}. An important element of the proof is Lemma~\ref{lemma:spectral-ineq} below, which provides us with a lower bound on $\underline{\xi}(\rho,\sigma)$.
	\end{Proof}
	
	Since Theorem~\ref{thm-quantum_Chernoff} establishes that the equality $\underline{\xi}(\rho,\sigma) = \overline{\xi}(\rho,\sigma)$ holds, this means that the limit exists and we can simply define
	\begin{equation}
	\xi(\{\rho,\sigma\}) \coloneqq 
	\lim_{n\to \infty}-\frac{1}{n}\log_2 p_{\text{err}}^*(\lambda\rho^{\otimes n},\bar{\lambda}\sigma^{\otimes n}).
	\end{equation}
	
	\begin{remark}
		Theorem~\ref{thm-quantum_Chernoff} tells us that, as $n$ becomes large, the following approximation holds
		\begin{equation}
			p_{\text{err}}^*(\{\lambda\rho^{\otimes n},\bar{\lambda}\sigma^{\otimes }\}) \approx 2^{-n\, \xi(\{\rho,\sigma\})}.
		\end{equation}
		We can thus think of $\xi(\{\rho,\sigma\})$ as the \textit{optimal error exponent} for the decay of the error probability as the number $n$ of copies increases.
		
		Note that the optimal error exponent in \eqref{eq-quantum_Chernoff_bound} is independent of the prior probability distribution. This means that, in the asymptotic limit (i.e., in the limit $n\to\infty$), the prior probability distribution is irrelevant for the optimal error exponent.
	
		We call Theorem~\ref{thm-quantum_Chernoff} the quantum Chernoff bound because it is analogous to the Chernoff bound from (classical) symmetric hypothesis testing, which is the task of discriminating between two hypotheses, each of which has a corresponding probability distribution (please consult the Bibliographic Notes in Section~\ref{sec:qm:bib-notes} for details).
	\end{remark}

	\begin{Lemma}{lemma:spectral-ineq}%\label{lemma:spectral-ineq}
		Let $A$ and $B$ be positive semi-definite operators. Then, for all $s\in\left(0,1\right)$,
		\begin{equation}
			\frac{1}{2}\left(\Tr[A+B]-\norm{A-B}_1\right)  \leq\Tr[A^{s}B^{1-s}].
		\end{equation}
	\end{Lemma}

	\begin{Proof}
		Let $\Delta\coloneqq A-B$, and let $\Delta_+$ and $\Delta_-$ be the positive and negative parts, respectively, of $\Delta$, so that $\Delta=\Delta_+-\Delta_-$ (recall \eqref{eq-operator_pos_neg_decomp}). Then,
		\begin{equation}
			|\Delta|=|\Delta_+-\Delta_-|=\Delta_++\Delta_-.
		\end{equation}
		Therefore,
		\begin{equation}
			\norm{A-B}_1 = \norm{\Delta}_1=\Tr[|\Delta|]=\Tr[\Delta_+]+\Tr[\Delta_-].
		\end{equation}
		In addition, we write
		\begin{equation}
			A+B=A-B+2B=\Delta_+-\Delta_-+2B,
		\end{equation}
		so that
		\begin{align}
			&\frac{1}{2}\left(\Tr[A+B]-\norm{A-B}_1\right)\nonumber\\
			&=\frac{1}{2}\left(\Tr[\Delta_+]-\Tr[\Delta_-]+2\Tr[B]-\Tr[\Delta_+]-\Tr[\Delta_-]\right)\\
			&=\Tr[B]-\Tr[\Delta_-].
		\end{align}
		So it suffices to prove that the following inequality holds for all $s\in(0,1)$:
		\begin{equation}\label{eq-lem_spec_ineq_pf_0}
			\Tr[B]-\Tr[\Delta_-]\leq\Tr[A^sB^{1-s}].
		\end{equation}
		Using the fact that $\Delta_+\geq 0$, by definition of the positive part of $\Delta$, we obtain
		\begin{equation}\label{eq-lem_spec_ineq_pf_1}
			B+\Delta_+\geq B.
		\end{equation}
		Similarly, using $A-B=\Delta_+-\Delta_-$, we obtain
		\begin{equation}\label{eq-lem_spec_ineq_pf_2}
			A+\Delta_-=B+\Delta_+\geq B.
		\end{equation}
		By the operator monotonicity of $x\mapsto x^s$ for $s\in(0,1)$ (recall Definition~\ref{def-op_conv_conc_mono} and thereafter), the inequality in \eqref{eq-lem_spec_ineq_pf_2} implies that
		\begin{equation}
			B^s\leq (A+\Delta_-)^s.
		\end{equation}
		Using this, along with the fact that $\Tr[B]=\Tr[B^sB^{1-s}]$, we find that
		\begin{align}
			\Tr[B]-\Tr[A^sB^{1-s}]&=\Tr[(B^s-A^s)B^{1-s}]\\
			&\leq \Tr[((A+\Delta_-)^s-A^s)B^{1-s}]\\
			&\leq \Tr[((A+\Delta_-)^s-A^s)(A+\Delta_-)^{1-s}]\\
			&=\Tr[A]+\Tr[\Delta_-]-\Tr[A^s(A+\Delta_-)^{1-s}] \label{eq-lem_spec_ineq_pf_3}.
		\end{align}
		Finally, observe that
		\begin{align}
			&A\leq A+\Delta_-\\
			\Rightarrow \quad &A^{\frac{s}{2}}A^{1-s}A^{\frac{s}{2}}\leq A^{\frac{s}{2}}(A+\Delta_-)^{1-s}A^{\frac{s}{2}}\\
			\Rightarrow \quad &A\leq A^{\frac{s}{2}}(A+\Delta_-)^{1-s}A^{\frac{s}{2}}\\
			\Rightarrow \quad  &\Tr[A]\leq \Tr[A^s(A+\Delta_-)^{1-s}].
		\end{align}
		Therefore, continuing from \eqref{eq-lem_spec_ineq_pf_3}, we find that
		\begin{align}
			\Tr[B]-\Tr[A^sB^{1-s}]&\leq \Tr[A]+\Tr[\Delta_-]-\Tr[A^s(A+\Delta_-)^{1-s}]\\
			&\leq \Tr[\Delta_-],
		\end{align}
		establishing \eqref{eq-lem_spec_ineq_pf_0}, as required.
	\end{Proof}
	


\subsubsection{Multiple State Discrimination}
	
	\label{sec:QM-over:multiple-state-disc}
	
	We now briefly consider state discrimination with more than two states. Suppose that Alice prepares a quantum system in a state chosen randomly from a set $\{\rho^x\}_{x\in\mathcal{X}}$ of states. We assume that $\mathcal{X}$ is some finite alphabet with size $|\mathcal{X}|\geq 2$ and that the state $\rho^x$ is chosen with probability $p(x)$, where $p:\mathcal{X}\to[0,1]$ is a probability distribution. Alice sends her chosen state to Bob, whose task is to guess the value of $x$, i.e., which state Alice sent. Bob's knowledge of the system can be described by the ensemble $\{(p(x),\rho_B^x)\}_{x\in\mathcal{X}}$, which has the following associated classical--quantum state:
	\begin{equation}\label{eq-state_disc_cq_state}
		\rho_{X_A B}\coloneqq \sum_{x\in\mathcal{X}}p(x)\ket{x}\!\bra{x}_{X_A}\otimes\rho_B^x,
	\end{equation}
	where $X_A$ is a classical $|\mathcal{X}|$-dimensional register that contains Alice's choice of state. Note that while Bob knows both the prior probability distribution $p$ and the association $x\leftrightarrow\rho^x$ between the labels $x$ and the states $\rho^x$, he does not have access to the register $X_A$. (If Bob did have access to the classical register $X_A$, he could simply measure it in the basis $\{\ket{x}\}_{x\in\mathcal{X}}$ and figure out what state Alice sent.) Therefore, as before, Bob must make a measurement. His strategy is to choose a POVM $\{M_B^x\}_{x\in\mathcal{X}}$ with elements indexed by the elements of~$\mathcal{X}$. If he obtains the outcome corresponding to $x\in\mathcal{X}$, then he guesses that the state sent was $\rho^x$. The probability of success, given that the state $\rho^x$ was selected, is thus $\Tr[M_B^x \rho^x_B]$, according to the Born rule. It then follows that the expected success probability is
	\begin{equation}
	p_{\text{succ}}(\{M^x\}_x;\{(p(x),\rho^x)\}_x) = \sum_{x\in\mathcal{X}}p(x)\Tr[M^x\rho^x].
	\end{equation}
	and furthermore that the optimal success probability is
	\begin{multline}
	\label{eq-opt_guessing_prob}
		p_{\text{succ}}^*(\{(p(x),\rho^x)\}_{x})\\=\sup_{\{M^x\}_x}\left\{\sum_{x\in\mathcal{X}}p(x)\Tr[M^x\rho^x]:0\leq M^x\leq\mathbbm{1}\ \forall x,\sum_{x\in\mathcal{X}}M^x=\mathbbm{1}\right\}.
	\end{multline}
	
	We can also arrive at the conclusion in \eqref{eq-opt_guessing_prob} by using the notion of a measurement channel, which is a concept introduced later in Definition~\ref{def-qc_channel}.
	Let $\mathcal{M}_{B\to X_B}(\cdot)\coloneqq \sum_{x\in\mathcal{X}}\Tr[M_B^x(\cdot)]\ket{x}\!\bra{x}_{X_B}$ be the measurement channel corresponding to the POVM $\{M_B^x\}_{x\in\mathcal{X}}$, where $X_B$ is a $|\mathcal{X}|$-dimensional classical register. After the measurement, the classical--quantum state in \eqref{eq-state_disc_cq_state} transforms to
	\begin{align}
		\omega_{X_AX_B}&\coloneqq\mathcal{M}_{B\to X_B}(\rho_{X_AB})\\
		&=\sum_{x,x'\in\mathcal{X}}p(x)\Tr[M_B^{x'}\rho_B^x]\ket{x}\!\bra{x}_{X_A}\otimes\ket{x'}\!\bra{x'}_{X_B}.
	\end{align}
	Let
	\begin{equation}
		\Pi_{X_AX_B}^{\text{succ}}\coloneqq\sum_{x\in\mathcal{X}}\ket{x}\!\bra{x}_{X_A}\otimes\ket{x}\!\bra{x}_{X_B},
	\end{equation}
	which is a projector corresponding to the registers $X_A$ and $X_B$ having the same value; this is what we want for state discrimination to be successful. The success probability of the strategy given by the POVM $\{M^x\}_{x\in\mathcal{X}}$ is thus
	\begin{align}
		p_{\text{succ}}(\{M^x\}_x;\{(p(x),\rho^x)\}_x)&=\Tr[\Pi_{X_AX_B}\omega_{X_AX_B}]\\
		&=\sum_{x\in\mathcal{X}}p(x)\Tr[M^x\rho^x],
	\end{align}
	and the optimal success probability is as given in \eqref{eq-opt_guessing_prob}.
%	\begin{multline}\label{eq-opt_guessing_prob}
%		p_{\text{succ}}^*(\{(p(x),\rho^x)\}_{x})\\=\sup_{\{M^x\}_x}\left\{\sum_{x\in\mathcal{X}}p(x)\Tr[M^x\rho^x]:0\leq M^x\leq\mathbbm{1}~\forall x,\sum_{x\in\mathcal{X}}M^x=\mathbbm{1}\right\}.
%	\end{multline}

The scenario of multiple state discrimination is very similar to the task of classical communication over a quantum channel $\mathcal{N}$ that we consider in Chapter~\ref{chap-classical_capacity}. The classical messages to be sent correspond to the labels $x\in\mathcal{X}$, while the states $\rho^x$ correspond to an encoding of the messages into quantum states, which are then sent through the quantum channel, and $p$ corresponds to the prior probability over the set of messages. The measurement performed in order to guess the state corresponds to a decoding channel that is applied at the receiving end of the quantum channel in order to determine the message that was sent. The quantity in \eqref{eq-opt_guessing_prob}, evaluated for the ensemble $\{(p(x),\mathcal{N}(\rho^x))\}_{x \in \mathcal{X}}$, is then the optimal average probability of correctly guessing the message sent, where the optimization is over all POVMs indexed by the messages.


	The optimal success probability in \eqref{eq-opt_guessing_prob} can be computed by means of a semi-definite program (recall Section~\ref{sec-SDPs}), giving us a good opportunity to practice semi-definite programming with a well motivated physical example. The semi-definite program for \eqref{eq-opt_guessing_prob} is as follows:
	\begin{equation}
	p^*_{\text{succ}}  = \sup_{ M_{XB}\geq 0 }\left\{\Tr[M_{XB}\rho_{XB}] : \Tr_X[M_{XB}] = \mathbbm{1}_B \right\},
	\end{equation} 
	where we have employed the shorthand $p^*_{\text{succ}} \equiv p_{\text{succ}}^*(\{(p(x),\rho^x)\}_{x})$ and $\rho_{XB}$ is the classical--quantum state in \eqref{eq-state_disc_cq_state}, with the shorthand $X\equiv X_A$. This is equal to \eqref{eq-opt_guessing_prob} because the objective function $\Tr[M_{XB}\rho_{XB}]$ reduces to that in \eqref{eq-opt_guessing_prob} with $M^x_B = \bra{x}_X M_{XB}\ket{x}_X$, due to the classical--quantum structure of $\rho_{XB}$. The constraint $\Tr_X[M_{XB}] = \mathbbm{1}_B$ is then the same as the constraint in \eqref{eq-opt_guessing_prob}. The SDP above is equivalent to the following one with a relaxed constraint:
		\begin{equation}
	p^*_{\text{succ}}  = \sup_{ M_{XB}\geq 0 }\left\{\Tr[M_{XB}\rho_{XB}] : \Tr_X[M_{XB}] \leq \mathbbm{1}_B \right\}, \label{eq:qm:modified-sdp-mult-state-disc}
	\end{equation}
	which follows because we can add in $\ket{0}\!\bra{0}_X \otimes (\mathbbm{1}_B - \Tr_X[M_{XB}])$ as an additional term to $M_{XB}$ if we do not have equality in the constraint in \eqref{eq:qm:modified-sdp-mult-state-disc}. Furthermore, the objective function in \eqref{eq:qm:modified-sdp-mult-state-disc} only increases under this addition. The SDP in \eqref{eq:qm:modified-sdp-mult-state-disc} is now in the standard primal form from Definition~\ref{def-SDPs}, with $A = \rho_{XB}$, $X = M_{XB}$, $B = \mathbbm{1}_B$, and $\Phi(X) =\Tr_X[M_{XB}]$. Since the dual map $\Phi^\dag$ of the partial trace is tensoring with the identity, it follows from Definition~\ref{def-SDPs} that the dual SDP is given by
	\begin{equation}
	\widehat{p}^*_{\text{succ}} = 
	\inf_{Y_B \geq 0} \{\Tr[Y_B] : \mathbbm{1}_X \otimes Y_B \geq \rho_{XB}\},
	\label{eq:QM-over:multiple-state-disc-dual-SDP}
	\end{equation} which is equivalent to
	\begin{equation}
	\widehat{p}^*_{\text{succ}} = 
	\inf_{Y_B \geq 0} \{\Tr[Y_B] :   Y_B \geq p(x) \rho^x_{B} \ \ \forall x \in \mathcal{X}\}.
	\end{equation}
	Strong duality holds because the operator $M_{XB} = \mathbbm{1}_{XB} / |\mathcal{X}|$ is feasible for the primal, while $Y_B = \sum_{x \in \mathcal{X}} p(x) \rho^x_B + \mathbbm{1}_B$ is strictly feasible for the dual. So we conclude that $\widehat{p}_{\text{succ}} = \widehat{p}^*_{\text{succ}}$. The complementary slackness conditions from Proposition~\ref{prop:math-tools:comp-slack} reduce to the following for this case: $Y_B =\Tr_X[M_{XB}] Y_B$ and $\rho_{XB} M_{XB}  = (I_X \otimes Y_B) M_{XB}$. Taking a partial trace over the second condition gives $\Tr_X[\rho_{XB} M_{XB}] = Y_B \Tr_X[M_{XB}] = Y_B$, where we used the first condition to arrive at the last equality. This final equality becomes  $Y_B = \sum_{x \in \mathcal{X}} p(x) \rho^x_B M^x_B$. Thus, we find that an optimal dual operator $Y_B$ is a direct function of an optimal measurement
	$\{M^x_B\}_{x \in \mathcal{X}}$.

	
		
	
	



\section{Quantum Channels}\label{sec-channel}


	The evolution of a quantum system is described mathematically by a \textit{quantum channel}, which is a linear, \textit{completely positive}, and \textit{trace-preserving} (CPTP) map acting on the quantum states of the underlying Hilbert space of the system. The main idea behind the formalism of quantum channels is that every admissible quantum physical evolution should accept a quantum state as input and output a legitimate quantum state. Furthermore, if such an evolution acts on a mixture of quantum states, then the output state should be equal to the mixture of the individual outputs. This latter requirement is called convex linearity on density operators, and for each convex linear map acting on the convex set of density operators, it is possible to define a unique linear map acting on the space of all linear operators. The latter is the mathematical object that we employ. The fact that this linear map should map quantum states to quantum states means that it should be a trace-preserving and positive map. However, it is furthermore reasonable to demand that if the channel acts on one share $A$ of a bipartite quantum state $\rho_{RA}$, then the output should be a legitimate bipartite quantum state. So we demand additionally that a quantum channel should be not simply positive, but in fact completely positive. Thus, a quantum channel is a linear, completely positive, and trace-preserving map.
	
	In detail, consider a map $\mathcal{N}:\Lin(\mathcal{H})\to\Lin(\mathcal{H}')$ (also called ``superoperator,'' as discussed previously in Section~\ref{sec:math-tools:super-ops}).
	\begin{enumerate}
		\item $\mathcal{N}$ is called \textit{positive} if it maps positive semi-definite operators to positive semi-definite operators, i.e., $\mathcal{N}(X)\geq 0$ for all $X\geq 0$. A map $\mathcal{N}$ is called \textit{completely positive} if the map $\id_k\otimes\mathcal{N}$ is positive for all integers $k\geq 1$. Note that if $\mathcal{N}$ is a map acting on linear operators in $\Lin(\mathbb{C}^{d})$, then the map $\id_k\otimes\mathcal{N}$ acts on linear operators in $\Lin(\mathbb{C}^{kd})$. In other words, for every linear operator $X$ acting on a $kd$-dimensional Hilbert space, which we can decompose as the block matrix
			\begin{equation}
				X=\begin{pmatrix} X_{0,0} & \dotsb & X_{0,k-1} \\ \vdots & \ddots & \vdots \\ X_{k-1,0} & \dotsb & X_{k-1,k-1} \end{pmatrix},
			\end{equation}
			such that $X_{i,j}$ is a $d\times d$ matrix for all $0\leq i,j\leq k-1$, the action of the map $\id_k\otimes\mathcal{N}$ is defined as
			\begin{equation}
				(\id_k\otimes\mathcal{N})(X)=\begin{pmatrix}\mathcal{N}(X_{0,0}) & \dotsb & \mathcal{N}(X_{0,k-1}) \\ \vdots & \ddots & \vdots \\ \mathcal{N}(X_{k-1,0}) & \hdots & \mathcal{N}(X_{k-1,k-1}) \end{pmatrix}.
			\end{equation}
			We can write this more compactly as follows. Noting that $\Lin(\mathbb{C}^{kd}) $ is isomorphic to $\Lin(\mathbb{C}^{k})\otimes \Lin(\mathbb{C}^{d}) $, we can write $X \in \Lin(\mathbb{C}^{kd})$ as
			\begin{equation}
			X = \sum_{i,j=0}^{k-1} \ket{i}\!\bra{j} \otimes X_{i,j}.
			\end{equation}
			Then the action of $\id_k \otimes \mathcal{N}$ is defined as
			\begin{equation}
			(\id_k \otimes \mathcal{N})(X) = \sum_{i,j=0}^{k-1} \ket{i}\!\bra{j} \otimes \mathcal{N}(X_{i,j}).
			\end{equation}
			
			Physically, the complete positivity of $\mathcal{N}$ takes into account the fact that the system of interest might be entangled with another system that is outside of our control, so that simply letting $\mathcal{N}$ be positive is not sufficient to ensure that all positive semi-definite operators get mapped to positive semi-definite operators. Letting $\mathcal{N}$ be completely positive means that positive semi-definite operators are mapped to positive semi-definite operators even in this more general setting.
		\item $\mathcal{N}$ is called \textit{trace preserving} if $\Tr[\mathcal{N}(X)]=\Tr[X]$ for all linear operators $X$.
	\end{enumerate}
	
	The defining properties of complete positivity and trace preservation for quantum channels together ensure that quantum states for the systems of interest get mapped to quantum states, even if they happen to be entangled with other external systems outside of our control. 
	
	Thoughout this book, we write $\mathcal{N}_{A\to B}$ to denote a map $\mathcal{N}:\Lin(\mathcal{H}_A)\to\Lin(\mathcal{H}_B)$ taking a quantum system $A$ to a quantum system $B$. We sometimes write $\mathcal{N}_A$ if the input and output systems of the channel have the same dimension. We drop the subscript indicating the input and output systems if they are not important in the context being considered.
	
\subsection{Choi Representation}
	
	The Choi representation of a quantum channel gives a way to represent a quantum channel as a bipartite operator and is an essential concept in quantum information theory.
	
	\begin{definition}{Choi Representation}{def-Choi_rep}
		For every quantum channel $\mathcal{N}_{A\to B}$, its \textit{Choi representation}, or \textit{Choi operator}, is defined as
		\begin{equation}\label{eq-Choi_rep}
			\Gamma^{\mathcal{N}}_{AB}\coloneqq\mathcal{N}_{A'\to B}(\ket{\Gamma}\!\bra{\Gamma}_{AA'})=\sum_{i,j=0}^{d_A-1}\ket{i}\!\bra{j}_A\otimes\mathcal{N}(\ket{i}\!\bra{j}_{A'}),
		\end{equation}
		where $\mathcal{H}_{A'}$ is isomorphic to the Hilbert space $\mathcal{H}_{A}$ corresponding to the channel input system $A$.
		The \textit{Choi state} $\Phi_{AB}^{\mathcal{N}}$ of $\mathcal{N}$ is defined as
		\begin{equation}
			\Phi_{AB}^{\mathcal{N}}\coloneqq\frac{1}{d_A}\Gamma_{AB}^{\mathcal{N}}=\mathcal{N}_{A'\to B}(\Phi_{AA'}),
		\end{equation}
		where $\Phi_{AA'}=\ket{\Phi}\!\bra{\Phi}_{AA'}$ is the maximally entangled state defined in~\eqref{eq-max_ent_state}.
	\end{definition}
	
	The Choi representation $\Gamma_{AB}^{\mathcal{N}}$ of the channel $\mathcal{N}_{A\to B}$ is an operator acting on $\mathcal{H}_{AB}$ and uniquely characterizes the channel because it specifies the action of $\mathcal{N}$ on the basis $\{\ket{i}\!\bra{j}_A:0\leq i,j\leq d_A - 1\}$ of linear operators acting on~$\mathcal{H}_A$. The Choi state $\Phi_{AB}^{\mathcal{N}}$ is simply the Choi representation normalized by the dimension $d_A$ of the input system $A$ of the channel $\mathcal{N}$, and it is the state resulting from sending one share of a maximally entangled state through $\mathcal{N}$; see Figure~\ref{fig-Choi_state}.
	
	\begin{figure}
		\centering
		\includegraphics[scale=0.9]{Figures/Choi_state.pdf}
		\caption{The Choi state $\Phi_{AB}^{\mathcal{N}}$ of a quantum channel $\mathcal{N}_{A\to B}$ is the state resulting from sending one share of the maximally entangled state $\Phi_{AA'}$, defined in \eqref{eq-max_ent_state}, through $\mathcal{N}$.}\label{fig-Choi_state}
	\end{figure}
	
	\begin{proposition*}{Quantum Dynamics from Choi Operator}{prop:qm:dyn-from-choi}
	Let $\mathcal{N}_{A\to B}$ be a quantum channel, and let $X_{RA}$ be a bipartite operator, with $R$ an arbitrary reference system. Then the action of the channel $\id_R\otimes \mathcal{N}_{A\to B}$ on $X_{RA}$ can be expressed in terms of the Choi operator $\Gamma_{AB}^{\mathcal{N}}$ as follows:
		\begin{align}
	(\id_R\otimes\mathcal{N}_{A\to B})(X_{RA}) & =
	\Tr_A[(\T_A(X_{RA}) \otimes\mathbbm{1}_B)(\mathbbm{1}_R \otimes \Gamma_{AB}^{\mathcal{N}})], 	\label{eq-Choi_rep_action}\\
		(\id_R\otimes\mathcal{N}_{A\to B})(X_{RA}) & =\bra{\Gamma}_{A'A}(X_{RA'}\otimes\Gamma_{AB}^{\mathcal{N}})\ket{\Gamma}_{A'A},
		\label{eq-QM:post-selected-TP-Choi-op}
	\end{align}
	where $\T_A$ denotes the partial transpose from Definition~\ref{def-partial_transpose}.
	\end{proposition*}
	
	\begin{Proof}
	Observe that \eqref{eq-Choi_rep} implies that
	\begin{equation}
		\mathcal{N}_{A\to B}(\ket{i}\!\bra{j}_A)=(\bra{i}_A\otimes\mathbbm{1}_B)\Gamma_{AB}^{\mathcal{N}}(\ket{j}_A\otimes\mathbbm{1}_B)
	\end{equation}
	for all $0\leq i,j\leq d_A - 1$. We extend this by linearity to apply to every input operator $X_A$ by the following reasoning. Expanding $X_A$ as $X_A = \sum_{i,j=0}^{d_A-1} X_{i,j} \ket{i}\!\bra{j}_A$, we find that
	\begin{align}
	\mathcal{N}_{A\to B}(X_A) & = \sum_{i,j=0}^{d_A-1} X_{i,j}	\mathcal{N}_{A\to B}(\ket{i}\!\bra{j}_A)\\
	& =
	\sum_{i,j=0}^{d_A-1} X_{i,j}
	(\bra{i}_A\otimes\mathbbm{1}_B)\Gamma_{AB}^{\mathcal{N}}(\ket{j}_A\otimes\mathbbm{1}_B) \\
 &  = \sum_{i,j=0}^{d_A-1} X_{i,j}
	\Tr_A[ (\ket{j}\!\bra{i}_A\otimes\mathbbm{1}_B)\Gamma_{AB}^{\mathcal{N}}]\\
	& = \Tr_A[(X_A^{\t}\otimes\mathbbm{1}_B)\Gamma_{AB}^{\mathcal{N}}].
	\end{align}
	So we conclude that the action of $\mathcal{N}_{A\to B}$ on every linear operator $X_A$ can be expressed using the Choi representation as
	\begin{equation}
		\mathcal{N}_{A\to B}(X_A)=\Tr_A[(X_A^{\t}\otimes\mathbbm{1}_B)\Gamma_{AB}^{\mathcal{N}}].
	\end{equation}
	Now employing \eqref{eq-trace_identity} and \eqref{eq-transpose_trick}, we conclude that the action of $\mathcal{N}_{A\to B}$ on every linear operator $X_A$ can be expressed alternatively as
	\begin{equation}
		\mathcal{N}_{A\to B}(X_{A})=\bra{\Gamma}_{A'A}(X_{A'}\otimes\Gamma_{AB}^{\mathcal{N}})\ket{\Gamma}_{A'A}.
		\label{eq-QM:post-selected-TP-Choi-op-simple-1}
	\end{equation}
The identities in \eqref{eq-Choi_rep_action} and \eqref{eq-QM:post-selected-TP-Choi-op-simple-1} extend more generally to the case of the channel $\id_R \otimes \mathcal{N}_{A\to B}$ acting on a bipartite operator $X_{RA}$ by expanding $X_{RA}$ as $X_{RA} = \sum_{i,j=0}^{d_R-1} \ket{i}\!\bra{j}_R \otimes X^{i,j}_A$ and using linearity. We thus conclude \eqref{eq-Choi_rep_action} and \eqref{eq-QM:post-selected-TP-Choi-op}.
\end{Proof}

	
	
	Using the definition of the Choi state and the maximally entangled state~$\Phi_{A'A}$, we can write \eqref{eq-QM:post-selected-TP-Choi-op} as
	\begin{equation}\label{eq-Choi_state_post_selected_teleportation}
		\bra{\Phi}_{A'A}(X_{RA'}\otimes\Phi_{AB}^{\mathcal{N}})\ket{\Phi}_{A'A}=\frac{1}{d_A^2}\mathcal{N}_{A'\to B}(X_{RA'}).
	\end{equation}
	Comparing this equation with \eqref{eq-post_meas_state_half_proj}, we see that it has the following physical interpretation: if we start with the systems $R$, $A'$, $A$ and $B$ in the state $\rho_{RA'}\otimes\Phi_{AB}^{\mathcal{N}}$ and we measure $A'$ and $A$ according to the POVM $\{\ket{\Phi}\!\bra{\Phi}_{A'A},\mathbbm{1}_{A'A}\allowbreak-\ket{\Phi}\!\bra{\Phi}_{A'A}\}$, then the outcome corresponding to $\ket{\Phi}\!\bra{\Phi}_{A'A}$ occurs with probability $\frac{1}{d_A^2}$ and the post-measurement state on systems $R$ and $B$ is $\mathcal{N}_{A'\to B}(\rho_{RA'})$. The Choi state $\Phi_{AB}^{\mathcal{N}}$ can thus be viewed as a \textit{resource state} for the probabilistic implementation of the channel $\mathcal{N}$. We return to this point in Section~\ref{sec-teleportation} when we discuss post-selected quantum teleportation.
	
	The concept of the Choi state allows us to associate to each quantum channel $\mathcal{N}_{A\to B}$ a bipartite quantum state. Conversely, given a bipartite state $\rho_{AB}$, we can associate a map given by
	\begin{equation}
		X_A\mapsto d_A\Tr_A[(X_A^{\t}\otimes\mathbbm{1}_B)\rho_{AB}].
	\end{equation}
	It is straightforward to see that this map is completely positive; however, it is trace preserving if and only if $\Tr_B[\rho_{AB}]=\pi_A$. On the other hand, the map $\mathcal{N}_{A\to B}^{\rho}$ defined as
	\begin{equation}\label{eq-state_to_channel}
		\mathcal{N}_{A\to B}^{\rho}(X_A)\coloneqq\Tr_A\!\left[(X_A^{\t}\otimes\mathbbm{1}_B)\rho_A^{-\frac{1}{2}}\rho_{AB}\rho_A^{-\frac{1}{2}}\right]
	\end{equation}
	is a quantum channel whenever $\rho_A$ is positive definite, where $\rho_A=\Tr_B[\rho_{AB}]$. The operator $\rho_A^{-\frac{1}{2}}\rho_{AB}\rho_A^{-\frac{1}{2}}$ is sometimes called a ``conditional state,'' motivated by the fact that it reduces to a conditional probability distribution when $\rho_{AB}$ is a fully classical state, so that it can be written as $\rho_{AB} = \sum_{x,y} p(x,y) \ket{x}\!\bra{x}_A \otimes \ket{y}\!\bra{y}_B$ where $p(x,y)$ is a probability distribution. Note that if $\rho_A$ is not invertible, then the inverse in \eqref{eq-state_to_channel} should be taken on the support of $\rho_A$ (as in \eqref{eq-Herm_op_neg_power}), in which case the channel $\mathcal{N}_{A\to B}^{\rho}$ is defined as in \eqref{eq-state_to_channel} only on the support of $\rho_A$.

	
	Given two quantum channels $(\mathcal{N}_1)_{A_1\to B_1}$ and $(\mathcal{N}_2)_{A_2\to B_2}$, the Choi representation of the tensor product channel $\mathcal{N}_1\otimes\mathcal{N}_2$ is given by
	\begin{equation}\label{eq-Choi_rep_tensor_prod}
		\Gamma_{A_1A_2B_1B_2}^{\mathcal{N}_1\otimes\mathcal{N}_2}=\Gamma_{A_1B_1}^{\mathcal{N}_1}\otimes\Gamma_{A_2B_2}^{\mathcal{N}_2}.
	\end{equation}
	This is due to the fact that the operator $\Gamma_{A_1A_2A_1'A_2'}=\ket{\Gamma}\!\bra{\Gamma}_{A_1A_2A_1'A_2'}$ splits into a tensor product as
	\begin{equation}
		\Gamma_{A_1A_2A_1'A_2'}=\Gamma_{A_1A_1'}\otimes\Gamma_{A_2A_2'}.
	\end{equation}
	
	Given two quantum channels $\mathcal{N}_{A\to B}$ and $\mathcal{M}_{B\to C}$, the Choi representation of the composition $(\mathcal{M}\circ\mathcal{N})_{A\to C}$ is given by
	\begin{align}
		\Gamma_{AC}^{\mathcal{M}\circ\mathcal{N}} & = \mathcal{M}_{B\to C}(\Gamma_{AB}^{\mathcal{N}}) \\
		& = \Tr_B[ \T_B(\Gamma_{AB}^{\mathcal{N}}) \Gamma_{BC}^{\mathcal{M}}] \\
		& = \bra{\Gamma}_{BB'}
		\Gamma_{AB}^{\mathcal{N}} \otimes 
		\Gamma_{B'C}^{\mathcal{M}}
		\ket{\Gamma}_{BB'}.	
		\label{eq-QM:serial-comp-choi}	
	\end{align}
	The first equality follows  from the definition of the Choi representation, the second follows from \eqref{eq-Choi_rep_action}, and the third from \eqref{eq-QM:post-selected-TP-Choi-op}.




\subsection{Characterizations of Quantum Channels: Choi, Kraus, Stinespring}

	The following theorem provides three useful ways to characterize quantum channels, and as such, it is one of the most important theorems in quantum information theory.
	
	\begin{theorem*}{Quantum Channels}{thm-q_channels}%\label{thm-q_channels}
		Let $\mathcal{N}_{A\to B}$ be a linear map from $\Lin(\mathcal{H}_A)$ to $\Lin(\mathcal{H}_B)$. Then the following are equivalent:
		\begin{enumerate}
			\item $\mathcal{N}$ is a quantum channel.
			\item \textit{Choi}: The Choi representation $\Gamma_{AB}^{\mathcal{N}}$ is positive semi-definite and satisfies $\Tr_B[\Gamma_{AB}^{\mathcal{N}}]=\mathbbm{1}_A$.
			\item \textit{Kraus}: There exists a set $\{K_i\}_{i=1}^r$ of operators such that
				\begin{equation}\label{eq-q_channel_Kraus}
					\mathcal{N}(X_A)=\sum_{i=1}^r K_iX_AK_i^\dagger
				\end{equation}
				for all linear operators $X_A$, where $K_i\in\Lin(\mathcal{H}_A,\mathcal{H}_B)$ for all $i\in \{1,\dotsc, r\}$, $r\geq\rank(\Gamma_{AB}^{\mathcal{N}})$, and $\sum_{i=1}^r K_i^\dagger K_i=\mathbbm{1}_A$.
			\item \textit{Stinespring}: There exists an isometry $V_{A\to BE}$, with $d_E\geq\rank(\Gamma_{AB}^{\mathcal{N}})$, such that
				\begin{equation}\label{eq-q_channel_Stinespring}
					\mathcal{N}(X_A)=\Tr_E[VX_AV^\dagger]
				\end{equation}
				for all linear operators $X_A$.
		\end{enumerate}
	\end{theorem*}
	

	
	Please consult the Bibliographic Notes in  Section~\ref{sec:qm:bib-notes} for references containing a proof of this theorem. 

	The operators $K_i$ in \eqref{eq-q_channel_Kraus} are called \textit{Kraus operators}. They have an interpretation in quantum error correction as ``error operators'' that characterize various errors that a quantum system undergoes. Kraus operators for a given quantum channel are, however, not unique in general. If $\{K_i\}_{i=1}^r$ is a set of Kraus operators for the channel $\mathcal{N}$, then, given an $s\times r$ isometric matrix $V$ with elements $\{V_{i,j}: 1\leq i\leq s,~1\leq j\leq r\}$, the operators $\{K_i'\}_{i=1}^s$ defined as
	\begin{equation}
		K_i'=\sum_{j=1}^r V_{i,j}K_j
		\label{eq:qm:isometry-between-kraus-ops}
	\end{equation}
	are also Kraus operators for $\mathcal{N}$. Indeed, for every linear operator $X$, the following equality holds
	\begin{align}
		\sum_{i=1}^s K_i' X (K_i')^\dagger&=\sum_{i=1}^s\sum_{j,j'=1}^r V_{i,j}\conj{V_{i,j'}}K_j X K_{j'}^\dagger\\
		&=\sum_{j,j'=1}^r \underbrace{\left(\sum_{i=1}^s (V^\dagger)_{j',i} V_{i,j}\right)}_{(V^\dagger V)_{j',j}=\delta_{j',j}} K_j X K_{j'}^\dagger\\
		&=\sum_{j=1}^r K_j X K_j^\dagger\\
		&=\mathcal{N}(X),
	\end{align}
	where  the second equality follows because $\conj{V_{i,j'}}=(V^\dagger)_{j',i}$. We note also that a converse statement holds: if $\{K_i\}_{i=1}^r$ and $\{K_i'\}_{i=1}^s$ are two sets of Kraus operators that realize the same quantum channel, then they are related by an isometry as in \eqref{eq:qm:isometry-between-kraus-ops}. This is a dynamical version of the statement made earlier in Section~\ref{sec:qm:purification-def}, the statement there being that all purification of a state are related by an isometry acting on the purifying system.
	
		

	The isometry $V_{A\to BE}$ in \eqref{eq-q_channel_Stinespring} is called an \textit{isometric extension} of $\mathcal{N}$. Physically, the isometry can be thought of as modeling the interaction of the quantum system of interest with its \textit{environment}, i.e., anything external to the quantum system that is not under our control. Stinespring's theorem then tells us that the evolution of every quantum system can be thought of as first an interaction of the system with its environment, followed by discarding the environment; see Figure \ref{fig-stinespring}. Given a set $\{K_i\}_{i=1}^{r}$ of Kraus operators for $\mathcal{N}$, we can let the environment $E$ correspond to a space of dimension $r$ and define the isometry $V_{A\to BE}$ as
	\begin{equation}\label{eq-Kraus_to_Stinespring}
		V_{A\to BE}=\sum_{j=1}^{r} K_j\otimes\ket{j-1}_E.
	\end{equation}
	It is straightforward to show that this is indeed an isometric extension of $\mathcal{N}$ since $\Tr_E[VXV^\dagger]=\sum_{j=1}^{r} K_j X K_j^\dagger=\mathcal{N}(X)$.
	
	\begin{figure}
		\centering
		\includegraphics[scale=0.8]{Figures/stinespring1.pdf}\qquad
		\includegraphics[scale=0.8]{Figures/stinespring2.pdf}
		\caption{(Left) According to Stinespring's theorem, the evolution of every quantum system $A$ via a quantum channel $\mathcal{N}_{A\to B}$ can be described as an interaction of the system $A$ with its environment $E$ via an isometry $V_{A\to BE}$, followed by discarding the environment. (Right) The isometry $V_{A\to BE}$ can be extended to a unitary $U_{AE'\to BE''}$ using, e.g., the construction in \eqref{eq-chan_iso_ext_to_unitary}, such that $A$ and $E'$ are initially in a product state, with $E'$ starting in a pure state. The two systems then interact accoring to $U$, and after discarding the environment $E''$ the resulting state is the output of the channel.}\label{fig-stinespring}
	\end{figure}
	
	\subsubsection{Unitary Extensions of Quantum Channels from Isometric Extensions}
	
	We can always extend every isometric extension $V_{A\to BE}$ of a channel $\mathcal{N}_{A\to B}$ to a unitary $U_{AE'\to BE''}$ in a way similar to what we used in \eqref{eq:math-tools:op-Jensen-unitary-from-iso} in the proof of the operator Jensen inequality (Theorem~\ref{thm-Jensen}). Let the unitary $U_{AE'\to BE''}$ be defined as the following block matrix:
	\begin{equation}\label{eq-chan_iso_ext_to_unitary}
		U=\begin{pmatrix}
		V & \mathbbm{1}-VV^\dagger & 0_{d_B d_E \times d'} \\
		0_{d_A \times d_A} & V^\dagger & 0_{d_A \times d'} \\
		0_{d' \times d_A} & 0_{d' \times d_B d_E} & \mathbbm{1}_{d'}\end{pmatrix},
	\end{equation}
	where we set $d'\coloneqq (d_B-1)d_A$.  Without the various dimensions indicated, $U$ is more simply expressed as
		\begin{equation}
		U=\begin{pmatrix}
		V & \mathbbm{1}-VV^\dagger & 0 \\
		0 & V^\dagger & 0 \\
		0 & 0 & \mathbbm{1}\end{pmatrix}.
	\end{equation}
	Note that $V$ is a $d_Bd_E\times d_A$ matrix and $VV^\dagger$ is a $d_Bd_E\times d_Bd_E$ matrix. Furthermore, let us suppose that $d_E=d_Ad_B$. Note that, by the Stinespring theorem, it is always possible to pick this as the dimension of $\mathcal{H}_E$ since $0<\rank(\Gamma_{AB}^{\mathcal{N}})\leq d_Ad_B$. Then 
	\begin{equation}
	d_Bd_E+d_A+d' = d_A d_B (d_B+1),
	\end{equation}
	and we conclude that $U$ is a $(d_A d_B (d_B+1))\times (d_A d_B (d_B+1))$ matrix. It is also indeed a unitary because
	\begin{align}
		UU^\dagger&=
		\begin{pmatrix}
		V & \mathbbm{1}-VV^\dagger & 0  \\
		0 & V^\dagger & 0 \\
		0 & 0 & \mathbbm{1}
		\end{pmatrix}
		\begin{pmatrix}
		V^\dagger & 0 & 0 \\
		\mathbbm{1}-VV^\dagger & V & 0 \\
		0 & 0 & \mathbbm{1}
		\end{pmatrix}\\
		&=\begin{pmatrix}
		VV^\dagger + (\mathbbm{1}-VV^\dagger)(\mathbbm{1}-VV^\dagger) & (\mathbbm{1}-VV^\dagger)V & 0 \\
		V^\dagger(\mathbbm{1}-VV^\dagger) & V^\dagger V & 0 \\
		0 & 0 & \mathbbm{1}
		\end{pmatrix}\\
		&=\begin{pmatrix}
		\mathbbm{1} & 0 & 0 \\
		0 & \mathbbm{1} & 0 \\
		0 & 0 & \mathbbm{1}
		\end{pmatrix}.
	\end{align}
	Similarly, it can be shown that $U^\dagger U=\mathbbm{1}$.
	%This means that $U$ is a $d_A(d_B^2+1)\times d_A(d_B^2+1)$ matrix.
	By defining the system $E'$ with dimension $d_{E'}=d_B(d_B+1)$, we can think of $U$ as acting on the input tensor-product space $\mathcal{H}_{E'}\otimes\mathcal{H}_{A}$. Then, we can embed the state $\rho_A$ into this larger space as
	\begin{equation}
		\ket{0}\!\bra{0}_{E'}\otimes\rho_{A}=
		\begin{pmatrix}
		\rho_A & 0 & 0 \\
		0 & 0 & 0\\
		0 & 0 & 0
		\end{pmatrix},
	\end{equation}
	so that
	\begin{equation}
		U\begin{pmatrix}
		\rho_A & 0 & 0 \\
		0&0 & 0\\
		0&0 & 0
		\end{pmatrix}U^\dagger=
		\begin{pmatrix}
		V\rho V^\dagger & 0 & 0 \\
		0 & 0 & 0 \\
		0 & 0 & 0 
		\end{pmatrix}.
	\end{equation}
	By defining the system $E''$ with dimension $d_{E''}=d_A(d_B+1)$, we can think of the output space of $U$ as the tensor-product space $\mathcal{H}_B\otimes\mathcal{H}_{E''}$, so that 
	\begin{equation}
		\mathcal{N}(\rho_A)=\Tr_E[V\rho V]=\Tr_{E''}[U(\ket{0}\!\bra{0}_{E'}\otimes\rho_A)U^\dagger].
	\end{equation}
	
	The above construction is not necessarily an efficient construction (using as few extra degrees of freedom as possible), but it illustrates the principle that every quantum channel can be thought of as arising from
	\begin{enumerate}
	\item adjoining an environment state $\ket{0}\!\bra{0}_{E'}$ to the input system $A$,
	\item performing a unitary interaction $U$, and then
	\item  tracing over an output environment system $E''$,
	\end{enumerate}
	thus assigning a strong physical meaning to the notion of isometric extension of a quantum channel; see Figure \ref{fig-stinespring}.
	
	Another construction of a unitary operator that is less explicit but more efficient is as follows. Let $V_{A\to BE}$ be the isometric extension from \eqref{eq-Kraus_to_Stinespring}, and let $r=\rank(\Gamma_{AB}^{\mathcal{N}})$. Since $r \leq d_A d_B$, without loss of generality, we can take the output environment system $E$ to have dimension $d_E = d_A d_B$. Let $\{\ket{k}_A \otimes \ket{\ell}_{E'}\}_{k,\ell}$ be an orthonormal basis for the input system $A$ and an input environment system $E'$, with $d_{E'}=d_B^2$, where $0 \leq k \leq d_A-1$ and $0 \leq \ell \leq d_{E'}-1$. Then define the orthonormal vectors $\ket{\phi_{k,1}}_{BE}$ for $0 \leq k \leq d_A-1$ as follows:
	\begin{align}
		\ket{\phi_{k,0}}_{BE} & \coloneqq \left(\sum_{j=1}^{d_E} K_j\otimes\ket{j-1}_E\bra{0}_{E'} \right) \ket{k}_A \otimes \ket{0}_{E'} \\
	 & = V_{A\to BE} \ket{k}_A.
	\end{align}
	The fact that these vectors form an orthonormal set is a consequence of the facts that $V^\dag V = \mathbbm{1}_A$ and $\{\ket{k}_A \}_{k=0}^{d_A-1}$ is an orthonormal set. We then define the action of the unitary $U_{AE'\to BE}$ on these vectors $\ket{k}_A \otimes \ket{0}_{E'}$ as follows:
	\begin{equation}
	U_{AE'\to BE} \ket{k}_A \otimes \ket{0}_{E'} = \ket{\phi_{k,0}}_{BE},
	\end{equation}
	for $0 \leq k \leq d_A-1$.
	By construction, we have that
	\begin{equation}
	\sum_{k=0}^{d_A-1} \ket{\phi_{k,0}}\!\bra{\phi_{k,0}}_{BE} = VV^\dag.
	\end{equation}
	Now let a spectral decomposition of the projection $\mathbbm{1}_{BE} - VV^\dag$ of dimension $d_B d_E - d_A = (d_B^2-1)d_A$ be given by
	\begin{equation}
	\mathbbm{1}_{BE} - VV^\dag = \sum_{k=0}^{d_A-1}\sum_{\ell = 1}^{d_B^2-1} \ket{\phi_{k,\ell}}\!\bra{\phi_{k,\ell}}_{BE}.
	\end{equation}
	We can thus complete the action of the unitary $U_{AE'\to BE}$ on the remaining vectors as follows:
		\begin{equation}
	U_{AE'\to BE}\ket{k}_A \otimes \ket{\ell}_{E'} = \ket{\phi_{k,\ell}}_{BE},
	\end{equation}
	for $0 \leq k \leq d_A-1$ and $1 \leq \ell \leq d_B^2-1$. Thus, the full unitary $U_{AE'\to BE}$ is specified as
	\begin{equation}
	U_{AE'\to BE} \coloneqq \sum_{k=0}^{d_A-1}\sum_{\ell = 0}^{d_B^2-1} \ket{\phi_{k,\ell}}_{BE}\bra{k}_A \otimes \bra{\ell}_{E'}.
	\end{equation}
	By construction, the following identity holds for every input state $\rho_A$:
	\begin{equation}
	U_{AE'\to BE} \left(\rho_A \otimes \ket{0}\!\bra{0}_{E'}\right) (U_{AE'\to BE})^\dag = V \rho_A V^\dag,
	\end{equation}
	so that we can realize the isometric channel $\rho_A \mapsto V \rho_A V^\dag$ by tensoring in an environment state $\ket{0}\!\bra{0}_{E'}$ and applying the unitary  $U_{AE'\to BE}$. We then realize the original channel $\mathcal{N}_{A\to B}$ by applying a final partial trace over the environment system $E$:
	\begin{equation}
	\mathcal{N}_{A\to B}(\rho_A) = \Tr_E[U_{AE'\to BE} \left(\rho_A \otimes \ket{0}\!\bra{0}_{E'}\right) (U_{AE'\to BE})^\dag].
	\end{equation}

\subsubsection{Relating Extensions and Purifications by Quantum Channels}

We can now establish a fundamental relationship between a purification $\psi_{RA}$ of a state $\rho_A$ and an extension $\omega_{R'A}$ of $\rho_A$.

\begin{proposition}{prop-extension_purif}
		Let $\rho_A$ be a quantum state with purification $\psi_{RA}$. For every extension $\omega_{R'A}$ of $\rho_A$, there exists a quantum channel $\mathcal{N}_{R\to R'}$ such that
		\begin{equation}
			\mathcal{N}_{R\to R'}(\psi_{RA})=\omega_{R'A}.
		\end{equation}
	\end{proposition}
	
	\begin{Proof}
		Consider a purification $\phi_{R''R'A}$ of $\omega_{R'A}$, with purifying system $R''$ satisfying $d_{R''}\geq\rank(\omega_{R'A})$. Since $\omega_{R'A}$ is an extension of $\rho_A$, we have that
		\begin{equation}
			\Tr_{R''R'}[\phi_{R''R'A}]=\rho_A,
		\end{equation}
		which means that $\phi_{R''R'A}$ is a purification of $\rho_A$. The state $\psi_{RA}$ is also a purification of $\rho_A$, which means that, by the isometric equivalence of purifications (see \eqref{eq-purif_iso_equiv_1}--\eqref{eq-purif_iso_equiv_4} and the paragraph thereafter), there exists an isometry $V_{R\to R''R'}$ such that
		\begin{equation}
			V_{R\to R''R'}\ket{\psi}_{RA}=\ket{\phi}_{R''R'A}.
		\end{equation}
		Now, let us use this isometry to define the channel $\mathcal{N}_{R\to R'}$:
		\begin{equation}
			\mathcal{N}_{R\to R'}(\cdot)=\Tr_{R''}[V_{R\to R''R'}(\cdot)V_{R\to R''R'}^\dagger].
		\end{equation}
		It then follows that
		\begin{equation}
			\mathcal{N}_{R\to R'}(\psi_{RA})=\Tr_{R''}[V_{R\to R''R'}\psi_{RA}V_{R\to R''R'}^\dagger]=\Tr_{R''}[\phi_{R''R'A}]=\omega_{R'A},
		\end{equation}
		as required.
	\end{Proof}
	
	Proposition~\ref{prop-extension_purif} tells us that an extension of a quantum state can be ``reached'' via a quantum channel acting on a purification of the state. In this sense, a purification can be viewed as the ``strongest'' extension of a state.


\subsection{Unital Maps and Adjoint Maps}

	\begin{definition}{Unital Map}{def-unital_map}
		A map $\mathcal{N}_{A\to B}$ is called \textit{unital} if it preserves the identity operator $\mathbbm{1}_A$, i.e.,
		\begin{equation}\label{eq-unital_def}
			\mathcal{N}(\mathbbm{1}_A)=\mathbbm{1}_B.
		\end{equation}
	\end{definition}
	
	\begin{remark}
		Observe that if $\mathcal{N}$ is trace preserving and $A$ and $B$ are finite dimensional, then by taking the trace on both sides of \eqref{eq-unital_def} we find that $d_A=d_B$. This means that, in finite dimensions, it is necessary for unital channels to have the same input and output dimensions.
	\end{remark}
	
	Unital channels thus have the maximally mixed state $\pi_A$ as a fixed point.
	
	Given that the set $\Lin(\mathcal{H}_A,\mathcal{H}_B)$ of linear operators between the Hilbert spac\-es $\mathcal{H}_A$ and $\mathcal{H}_B$ is itself a Hilbert space under the Hilbert--Schmidt inner product defined in \eqref{eq-Hilbert_Schmidt_inner_prod}, it is possible to define the adjoint of a map $\mathcal{N}:\Lin(\mathcal{H}_A)\allowbreak\to\Lin(\mathcal{H}_B)$ as follows.
	
	\begin{definition}{Adjoint Map}{def-adjoint_map}
		For a map $\mathcal{N}:\Lin(\mathcal{H}_A)\to\Lin(\mathcal{H}_B)$, its \textit{adjoint map} $(\mathcal{N}^\dagger)_{B\to A}$ is defined as the unique linear map from $\Lin(\mathcal{H}_B)$ to $\Lin(\mathcal{H}_A)$ satisfying
		\begin{equation}\label{eq-adjoint}
			\inner{Y_B}{\mathcal{N}(X_A)}=\langle \mathcal{N}^\dagger(Y_B), X_A\rangle
		\end{equation}
		for all $X\in\Lin(\mathcal{H}_A)$ and $Y\in\Lin(\mathcal{H}_B)$.
	\end{definition}

	Given a channel $\mathcal{N}_{A\to B}$ with Kraus representation
	\begin{equation}
		\mathcal{N}(X)=\sum_{i=1}^r K_i X K_i^\dagger
	\end{equation}
	and Stinespring representation $V$ satisfying
	\begin{equation}
		\mathcal{N}(X)=\Tr_E[VXV^\dagger],
	\end{equation}
	it is straightforward to verify using \eqref{eq-adjoint} that the adjoint map $\mathcal{N}^\dagger$ can be represented in the following two ways:
	\begin{align}
		\mathcal{N}^\dagger(Y) & =\sum_{i=1}^r K_i^\dagger Y K_i\\
		& = V^\dagger(Y\otimes\mathbbm{1}_E)V.
	\end{align}
	From this, the following facts are straightforward to verify:
	\begin{enumerate}
		\item The adjoint of a completely positive map is completely positive.
		\item The adjoint of a trace preserving map is a unital map.
		\item The adjoint of a unital map is trace preserving.
	\end{enumerate}
	
	
	
\subsection{Appending, Replacement, Partial Trace, Isometric, Complementary, and Degradable Channels}
	
	We now detail a variety of quantum channels that tend to come up often in quantum information theory.
	
	

\subsubsection{Preparation, Appending, and Replacement Channels}

	The preparation of a quantum system in a given (fixed) state, as well as taking the tensor product of a state with a given (fixed) state, can both be viewed as quantum channels.
	
	\begin{definition}{Preparation and Appending Channels}{def-prep_app_channel}
		For a quantum system $A$ and a state $\rho_A$, the \textit{preparation channel}  $\mathcal{P}_{\rho_A}$ is defined for $\alpha\in\mathbb{C}$ as
		\begin{equation}
			\mathcal{P}_{\rho_A}(\alpha)\coloneqq \alpha\rho_A.
		\end{equation}
		When acting in parallel with the identity channel on a linear operator~$Y_B$ of another quantum system $B$, the preparation channel $\mathcal{P}_{\rho_A}$ is called the \textit{appending channel} $\mathcal{P}_{\rho_A}$ and is defined as
		\begin{equation}
			\mathcal{P}_{\rho_A}(Y_B)\equiv (\mathcal{P}_{\rho_A}\otimes\id_B)(Y_B)=\rho_A\otimes Y_B.
		\end{equation}
		In other words, the appending channel $\mathcal{P}_{\rho_A} \otimes\id_B$ takes the tensor product of its argument with $\rho_A$.
	\end{definition}
	
	One way to determine whether a map $\mathcal{N}$ on quantum states is completely positive is to find a Kraus representation for it, i.e., a set $\{K_i\}_i$ of operators such that $\mathcal{N}(X)=\sum_i K_i XK_i^\dagger$ for all operators $X$, for then by Theorem \ref{thm-q_channels} we get that $\mathcal{N}$ is completely positive. If in addition the Kraus operators satisfy $\sum_i K_i^\dagger K_i=\mathbbm{1}$, then $\mathcal{N}$ is also trace preserving and therefore a quantum channel.
	
	Supposing that $\rho_A$ has a spectral decomposition of the form
	\begin{equation}
		\rho_A=\sum_k \lambda_k \ket{\phi_k}\!\bra{\phi_k}_A,
	\end{equation}
	one set of Kraus operators for the preparation channel $\mathcal{P}_{\rho_A}$ is $\{\sqrt{\lambda_k}\ket{\phi_k}_A\}_k$. A set of Kraus operators for the appending channel $\mathcal{P}_{\rho_A}\otimes\id_B$ is then $\{\sqrt{\lambda_k}\ket{\phi_k}\otimes\mathbbm{1}_B\}_k$.
	
	\begin{definition}{Replacement Channel}{def-replace_channel}
		For a state $\sigma_B$, the \textit{replacement channel}  $\mathcal{R}_{A\to B}^{\sigma_B}$ is defined as the channel that traces out its input and replaces it with the state $\sigma_B$, i.e.,
		\begin{equation}\label{eq-replacement_channel}
			\mathcal{R}_{A\to B}^{\sigma_B}(X_A)=\Tr[X_A]\sigma_B.
		\end{equation}
		for all linear operators $X_A$. When acting on one share of a bipartite state $\rho_{RA}$, the replacement channel $\mathcal{R}_{A\to B}^{\sigma_B}$ has the following action:
		\begin{equation}
			\mathcal{R}_{A\to B}^{\sigma_B}(\rho_{RA})=\Tr_A[\rho_{RA}]\otimes\sigma_B=\rho_R\otimes\sigma_B.
		\end{equation}
	\end{definition}
	
	Observe that we can write the replacement channel $\mathcal{R}_{A\to B}^{\sigma_B}$  as the composition of the partial trace over $A$ followed by the preparation/append\-ing channel $\mathcal{P}_{\sigma_B}$:
	\begin{equation}
		\mathcal{R}_{A\to B}^{\sigma_B}=\mathcal{P}_{\sigma_B}\circ\Tr_A.
	\end{equation}
	We often omit the superscript on $\mathcal{R}_{A\to B}^{\sigma_B}$  when it is clear from the context that the replacement state is  $\sigma_B$.


\subsubsection{Trace and Partial-Trace Channels}

	Recall the trace and partial trace of a linear operator from Definition \ref{def-partial_trace}. As a map acting on linear operators, one can ask whether the partial trace is a channel. The answer, perhaps not surprisingly, is ``yes.'' In fact, observe that the definition in \eqref{eq-partial_trace_B} of the partial trace $\Tr_B$ over $B$ is already in Kraus form, with Kraus operators $K_j=\mathbbm{1}_A\otimes\bra{j}_B$. This means that $\Tr_B$ is completely positive. It is also trace preserving because
	\begin{equation}
		\sum_{j=0}^{d_B-1}K_j^\dagger K_j=\sum_{j=0}^{d_B-1}(\mathbbm{1}_A\otimes\ket{j}_B)(\mathbbm{1}_A\otimes\bra{j}_B)=\mathbbm{1}_A\otimes\sum_{j=0}^{d_B-1}\ket{j}\!\bra{j}_B=\mathbbm{1}_{AB},
	\end{equation}
	where we used the fact that $\sum_{j=0}^{d_B-1}\ket{j}\!\bra{j}_B=\mathbbm{1}_B$.
	
	Unlike the trace and partial trace, the transpose and partial transpose are trace-preserving maps but \textit{not} completely positive. Indeed, for the latter, recall from \eqref{eq-swap_operator} that $\T_B(\Phi_{AB})=\frac{1}{d}F_{AB}$, so that its Choi representation is $\Gamma_{AB}^{\T_B}=F_{AB}$, which we know has negative eigenvalues, as shown in \eqref{eq:qm:spectral-decomp-swap-op}. So by Theorem \ref{thm-q_channels}, the transpose map $\T_B$ is not completely positive. 
	
\subsubsection{Isometric and Unitary Channels}	

\label{sec:OM-over:iso-unitary-chs}

	Two more simple examples of quantum channels are \textit{isometric} and \textit{unitary channels}. An isometric channel conjugates  the channel input by an isometry, and a unitary channel conjugates the channel input by a unitary. Specifically, the isometric channel $\mathcal{V}$ corresponding to an isometry $V$ is
	\begin{equation}
		\mathcal{V}(X)\coloneqq VXV^\dagger.
	\end{equation}
	Similarly, the unitary channel $\mathcal{U}$ corresponding to a unitary $U$ is
	\begin{equation}
		\mathcal{U}(X)\coloneqq UXU^\dagger.
	\end{equation}
	Since every unitary is also an isometry, it follows that every unitary channel is an isometric channel.
	Isometric channels are completely positive because they can be described using only one Kraus operator, the isometry $V$. In fact, a quantum channel is isometric if and only if it has a single Kraus operator.
	
	Observe that by the unitarity of $U$, the map
	\begin{equation}
		\mathcal{U}^\dagger(Y)\coloneqq U^\dagger Y U,
	\end{equation}
	i.e., the conjugation by $U^\dagger$, is also a channel. In particular,
	\begin{equation}
		\mathcal{U}^\dagger\circ\mathcal{U}=\mathcal{U}\circ\mathcal{U}^\dagger=\id,
	\end{equation}
	so that $\mathcal{U}^\dagger$ is the inverse channel of $\mathcal{U}$. 
	
	On the other hand, for an isometry $V$, conjugation by $V^\dagger$ is \textit{not} necessarily a channel: although the map $\mathcal{V}^\dagger(Y)\coloneqq V^\dagger YV$ is completely positive, it is not necessarily trace preserving because $VV^\dagger\neq\mathbbm{1}$ in general. However, by defining the reversal channel $\mathcal{R}_V$ as
	\begin{equation}\label{eq-isometry_recover}
		\mathcal{R}_V(Y)\coloneqq \mathcal{V}^\dagger(Y)+\Tr[(\mathbbm{1}-VV^\dagger)Y]\sigma,
	\end{equation}
	where $\sigma$ is an arbitrary (but fixed) state, we find that $\mathcal{R}_V$ is trace preserving:
	\begin{align}
		\Tr[\mathcal{R}_V(Y)]&=\Tr\!\left[\mathcal{V}^\dagger(Y)+\Tr[(\mathbbm{1}-VV^\dagger)Y]\sigma\right]\\
		&=\Tr[V^\dagger Y V]+\Tr[Y]-\Tr[VV^\dagger Y]\\
		&=\Tr[Y].
	\end{align}
	Since it is also completely positive, being the sum of completely positive maps, the map $\mathcal{R}_V$ is indeed a quantum channel. Like $\mathcal{U}^\dagger$, the reversal channel~$\mathcal{R}_V$ reverses the action of $\mathcal{V}$:
	\begin{align}
		(\mathcal{R}_V\circ\mathcal{V})(X)&=\mathcal{V}^\dagger(\mathcal{V}(X))+\Tr[(\mathbbm{1}-VV^\dagger)\mathcal{V}(X)]\sigma\\
		&=V^\dagger V XV^\dagger V+\Tr[(\mathbbm{1}-VV^\dagger)VXV^\dagger]\sigma\\
		&=X+(\Tr[VXV^\dagger]-\Tr[VV^\dagger VXV^\dagger])\sigma\\
		&=X.
	\end{align}
	In the above sense, $\mathcal{R}_V$ is a left inverse of $\mathcal{V}$. Unlike~$\mathcal{U}^\dagger$, however, $\mathcal{R}_V$ is not the right inverse of $\mathcal{V}$ because the equality $(\mathcal{V}\circ\mathcal{R}_V)(Y)\allowbreak=Y$ need not hold.
	

\subsubsection{Complementary Channels}
	
	\label{sec-QM:complementary-chs}
	
	As stated earlier, the Stinespring representation $\mathcal{N}_{A\to B}(X_A)=\Tr_E[VXV^\dagger]$ of a quantum channel $\mathcal{N}_{A\to B}$, where $V_{A\to BE}$ is an isometry, can be interpreted as an interaction of the quantum system $A$ of interest with its environment $E$ followed by discarding $E$. If instead we discard the system $B$ of the isometric channel $\mathcal{V}_{A\to BE}(X_A) = VXV^\dagger$, then we obtain the state of the environment after the interaction with $A$. This defines a channel complementary to $\mathcal{N}_{A \to B}$.
	
	\begin{definition}{Complementary Channel}{def-complementary_chan}
		Let $V_{A\to BE}$ be an isometry and  $\mathcal{N}_{A\to B}$ a quantum channel defined as
		\begin{equation}
			\mathcal{N}_{A\to B}(X_A)=\Tr_E[VXV^\dagger].
		\end{equation}
		The \textit{complementary channel} for $\mathcal{N}_{A\to B}$ associated with the isometric extension $V_{A\to BE}$ is denoted by $\mathcal{N}^c_{A\to E}$ and is defined as
		\begin{equation}
			\mathcal{N}^c_{A\to E}(X_A)\coloneqq\Tr_B[VXV^\dagger].
		\end{equation}
		Related to the above, the channel $\mathcal{M}^c_{A\to E}$ is a complementary channel for the channel $\mathcal{M}_{A\to B}$ if there exists an isometric channel $\mathcal{W}_{A \to BE}$ such that
		\begin{align}
		\mathcal{M}_{A\to B} & = \Tr_E \circ \mathcal{W}_{A \to BE} \\
		\mathcal{M}^c_{A\to E} & = \Tr_B \circ 
		\mathcal{W}_{A \to BE}.
		\end{align}
	\end{definition}
	
	Given a channel $\mathcal{N}_{A\to B}$, it does not have a unique complementary channel, just as it does not have a unique Kraus representation, nor does a given quantum state $\rho_A$ have a unique purification. Similar to the latter scenarios, however, it is possible to show that all complementary channels for $\mathcal{N}_{A\to B}$ are related by an isometric channel acting on their output. That is, let us suppose that $(\mathcal{N}_1)^c_{A\to E}$ and $(\mathcal{N}_2)^c_{A\to E'}$ are complementary channels for $\mathcal{N}_{A\to B}$. Then there exists an isometric channel $\mathcal{S}_{E \to E'}$ such that
	\begin{equation}
	(\mathcal{N}_2)^c_{A\to E'} = \mathcal{S}_{E \to E'} \circ (\mathcal{N}_1)^c_{A\to E}.
	\end{equation}	
	

	
	The notion of a complementary channel arises in the scenario  in which two parties, Alice and Bob, wish to communicate to each other using a channel~$\mathcal{N}_{A \to B}$ in the presence of an eavesdropper Eve. In this scenario, we can naturally identify Alice and Bob with the quantum systems $A$ and $B$ and Eve with the system $E$, where $E$ is as given in Definition~\ref{def-complementary_chan}. Any signals sent through the quantum channel by Alice are received by Bob via the action of $\mathcal{N}_{A \to B}$, while Eve receives a signal via the action of $\mathcal{N}^c_{A \to E}$. These concepts are important for private communication over quantum channels, which is the topic of Chapter~\ref{chap-private_capacity}. Two important classes of channels are relevant in this context.
	
	\begin{definition}{Degradable and Anti-Degradable Channels}{def-deg_antideg_chan}
		A channel $\mathcal{N}_{A \to B}$ is called \textit{degradable} if there exists a channel $\mathcal{D}_{B \to E}$, called a \textit{degrading channel}, such that
		\begin{equation}
			\mathcal{D}_{B \to E}\circ\mathcal{N}_{A \to B}=\mathcal{N}^c_{A \to E},
		\end{equation}
		where $\mathcal{N}^c_{A \to E}$ is a complementary channel of $\mathcal{N}_{A \to B}$.
		The channel $\mathcal{N}_{A \to B}$ is called \textit{anti-degradable} if a  complementary channel $\mathcal{N}^c_{A \to E}$ of it is degradable, i.e., if there exists a channel $\mathcal{A}_{E \to B}$, called an \textit{anti-degrading channel}, such that
		\begin{equation}
			\mathcal{A}_{E \to B}\circ\mathcal{N}^c_{A\to E}=\mathcal{N}_{A\to B}.
		\end{equation}
	\end{definition}
	
	See Figure \ref{fig-degradable_antidegradable} for a schematic depiction of degradable and anti-degradable channels. A degradable channel is one whose complement can be simulated (via $\mathcal{D}$) using the output of $\mathcal{N}$. This means that Bob can simulate Eve's received signal. On the other hand, an anti-degradable channel is such that $\mathcal{N}$ can be simulated (via $\mathcal{A}$) using the output of $\mathcal{N}^c$, which means that Eve can simulate Bob's received signal. 
	
		\begin{figure}
		\centering
		\begin{subfigure}{0.49\textwidth}
			\centering\includegraphics[scale=1]{Figures/degradable.pdf}\caption{$\mathcal{N}$ degradable.}\label{subfig-degradable}
		\end{subfigure}~
		\begin{subfigure}{0.49\textwidth}
			\centering\includegraphics[scale=1]{Figures/antidegradable.pdf}\caption{$\mathcal{N}$ anti-degradable.}\label{subfig-antidegradable}
		\end{subfigure}
		\caption{Degradable and anti-degradable channels. In \subref{subfig-degradable}, the channel $\mathcal{N}$ is degradable, meaning that there exists a channel $\mathcal{D}$ that Bob can apply to the output he receives via $\mathcal{N}$ that can be used to simulate what Eve receives via $\mathcal{N}^c$. In \subref{subfig-antidegradable} on the other hand, $\mathcal{N}$ is anti-degradable since Eve can simulate, using the channel $\mathcal{E}$, what Bob receives.}\label{fig-degradable_antidegradable}
	\end{figure}



\subsection{Amplitude Damping, Erasure, Pauli, and Depolarizing Channels}

\label{subsec-qubit_channel}

	Let us now go through some common quantum channels of interest in quantum communication. 


\subsubsection{(Generalized) Amplitude Damping Channel}

\label{sec:QM-over:amp-damp-ch}

	The \textit{amplitude damping channel with decay parameter $\gamma\in[0,1]$} is the channel $\mathcal{A}_\gamma$ given by $\mathcal{A}_{\gamma}(\rho)=A_1\rho A_1^\dagger+A_2\rho A_2^\dagger$, with the two Kraus operators $A_1$ and $A_2$ defined as
	\begin{equation}\label{eq-amplitude_damping_channel}
		A_1=\sqrt{\gamma}\ket{0}\!\bra{1},\quad A_2=\ket{0}\!\bra{0}+\sqrt{1-\gamma}\ket{1}\!\bra{1}.
	\end{equation}
	It is straightforward to verify that $A_1^\dagger A_1+A_2^\dagger A_2=\mathbbm{1}$, so that $\mathcal{A}_\gamma$ is indeed trace preserving. 
	
	Let $\rho$ be a state with a matrix representation in the standard basis $\{\ket{0},\ket{1}\}$ as
	\begin{equation}\label{eq-qubit_state}
		\rho=\begin{pmatrix} 1-\lambda & \alpha \\ \conj{\alpha} & \lambda \end{pmatrix}.
	\end{equation}
	In order for $\rho$ to be a state (positive semi-definite with unit trace),
the conditions $0\leq \lambda\leq 1$ and  $\lambda(1-\lambda)\geq\abs{\alpha}^2$ should hold, where $\alpha\in\mathbb{C}$. The output state $\mathcal{A}_\gamma(\rho)$ has the matrix representation
	\begin{equation}
		\mathcal{A}_\gamma(\rho)=\begin{pmatrix} 1-(1-\gamma)\lambda & \sqrt{1-\gamma}\alpha \\ \sqrt{1-\gamma}\conj{\alpha} & (1-\gamma)\lambda  \end{pmatrix}.
	\end{equation}
	
	To obtain a physical interpretation of the amplitude damping channel, consider that it can written in the Stinespring form as
	\begin{equation}\label{eq-amp_damp_Stinespring}
		\mathcal{A}_\gamma(\rho)=\Tr_E[U^\eta(\rho\otimes\ket{0}\!\bra{0}_E)(U^{\eta})^\dagger],
	\end{equation}
	where $E$ is a qubit environment system, $\eta\coloneqq 1-\gamma$, and
	\begin{equation}\label{eq-amp_damp_BS}
		U^{\eta}=\begin{pmatrix}1&0&0&0\\0&\sqrt{\eta}&\I\sqrt{1-\eta}&0\\0&\I\sqrt{1-\eta}&\sqrt{\eta}&0\\0&0&0&1\end{pmatrix}
	\end{equation}
	is unitary. Note that the action of $\mathcal{A}_\gamma$ on the pure states $\ket{0}$ and $\ket{1}$ is, respectively,
	\begin{equation}\label{eq-amp_damp_receiver}
		\begin{aligned}
		\mathcal{A}_{1-\eta}(\ket{0}\!\bra{0}_A)&=\ket{0}\!\bra{0}_B,\\
		\mathcal{A}_{1-\eta}(\ket{1}\!\bra{1}_A)&=(1-\eta)\ket{0}\!\bra{0}_B+\eta\ket{1}\!\bra{1}_B.
		\end{aligned}
	\end{equation}
	A complementary channel $\mathcal{A}_{1-\eta}^c$ for $\mathcal{A}_\gamma$ is defined from
	\begin{equation}
	\mathcal{A}_{1-\eta}^c(\rho) \coloneqq 
	\Tr_B[U^\eta(\rho\otimes\ket{0}\!\bra{0}_E)(U^{\eta})^\dagger].
	\end{equation}
	Note that the action of the complementary channel $\mathcal{A}_{1-\eta}^c$ on these states is
	\begin{equation}\label{eq-amp_damp_env}
		\begin{aligned}
		\mathcal{A}_{1-\eta}^c(\ket{0}\!\bra{0}_A)&=\ket{0}\!\bra{0}_E,\\
		\mathcal{A}_{1-\eta}^c(\ket{1}\!\bra{1}_A)&=\eta\ket{0}\!\bra{0}_E+(1-\eta)\ket{1}\!\bra{1}_E.
		\end{aligned}
	\end{equation}
	We see that whenever the state $\ket{0}\!\bra{0}$ is input to the channel, the output systems $B$ and $E$ are both in the state $\ket{0}\!\bra{0}$. On the other hand, if the input state is $\ket{1}\!\bra{1}$, then $B$ receives a mixed state: with probability $1-\eta$, the state is $\ket{0}\!\bra{0}$, and with probability $\eta$, the state is $\ket{1}\!\bra{1}$. The situation for $E$ is reversed, receiving $\ket{0}\!\bra{0}$ with probability $\eta$ and $\ket{1}\!\bra{1}$ with probability $1-\eta$. The unitary $U^\eta$ can thus be viewed as a qubit analogue of a \textit{beamsplitter}, and the amplitude damping channel $\mathcal{A}_{1-\eta}$ can be viewed as a qubit analogue of the \textit{pure-loss bosonic channel}; see Figure \ref{fig-amp_damp}. 
	
	\begin{figure}
		\centering
		\includegraphics[scale=0.8]{Figures/AD.pdf}
		\caption{The amplitude damping channel $\mathcal{A}_{1-\eta}$ can be interpreted, using \eqref{eq-amp_damp_Stinespring}, as an interaction with a qubit analogue of a bosonic beamsplitter unitary $U^\eta$, followed by discarding the output state of the environment. The channel from the sender to the receiver is from the left to the right, while the input and output environment systems are at the top and the bottom, respectively. In the bosonic case, the state $\ket{0}\!\bra{0}$ of the environmental input arm of the beamsplitter corresponds to the vacuum state, which contains no photons, and the channel to the receiver's end is called the pure-loss bosonic channel.}\label{fig-amp_damp}
	\end{figure}
	
	A beamsplitter is an optical device that takes two beams of light as input and splits them into two separate output beams, with one of the output beams containing a fraction $\eta$ of the intensity of the incoming beam and the other output beam containing the remaining fraction $1-\eta$ of the incoming intensity. When one of the input ports of the beamsplitter is empty, i.e., is in the vacuum state, the output to the receiver is by definition the pure-loss bosonic channel. In the case of a single incoming photon, the pure-loss channel either transmits the photon with probability $\eta$ (allowing it to go to the receiver) or reflects it with probability $1-\eta$ (sending it to the environment). 
	
	To draw the correspondence between the qubit amplitude damping channel and the pure-loss bosonic channel described above, we can think of the qubit state $\ket{0}$ as the vacuum state and the qubit state $\ket{1}$ as the state of a single photon. It is possible to show that the output states of the amplitude damping channel in \eqref{eq-amp_damp_receiver} and \eqref{eq-amp_damp_env} for the receiver and environment, respectively, then exactly match the action of the bosonic pure-loss channel on the subspace spanned by $\ket{0}$ and $\ket{1}$ (please consult the Bibliographic Notes in Section~\ref{sec:qm:bib-notes} for further references on this connection). The amplitude damping channel can indeed, therefore, be viewed as the qubit analogue of the bosonic pure-loss channel.
	
	By replacing the initial state $\ket{0}\!\bra{0}$ of the environment in \eqref{eq-amp_damp_Stinespring} with the state
	\begin{equation}
		\theta_{N_B}\coloneqq (1-N_B)\ket{0}\!\bra{0}+N_B\ket{1}\!\bra{1},\quad N_B\in[0,1],
	\end{equation}
	we define the \textit{generalized amplitude damping channel} $\mathcal{A}_{1-\eta,N_B}$ as
	\begin{equation}\label{eq-gen_amp_damp}
		\mathcal{A}_{\gamma,N_B}(\rho) \equiv \mathcal{A}_{1-\eta,N_B}(\rho)\coloneqq\Tr_E[U^\eta(\rho\otimes\theta_{N_B})(U^\eta)^\dagger],
	\end{equation}
	where we again use the relation $\gamma=1-\eta$.
	This channel has the following four Kraus operators:
	\begin{align}
		A_1=\sqrt{1-N_B}\begin{pmatrix}1&0\\0&\sqrt{1-\gamma}\end{pmatrix},&\quad A_2=\sqrt{1-N_B}\begin{pmatrix}0&\sqrt{\gamma}\\0&0\end{pmatrix},\label{eq-gen_amp_damp_Kraus1}\\
		A_3=\sqrt{N_B}\begin{pmatrix}\sqrt{1-\gamma}&0\\0&1\end{pmatrix},&\quad A_4=\sqrt{N_B}\begin{pmatrix}0&0\\\sqrt{\gamma}&0\end{pmatrix},\label{eq-gen_amp_damp_Kraus2}.
	\end{align}
 Note that the amplitude damping channel is a special case of the generalized amplitude damping channel in which the thermal noise $N_B = 0$, so that $\mathcal{A}_{1-\eta}=\mathcal{A}_{1-\eta,0}$.
	
	The state $\theta_{N_B}$ is a qubit thermal state and can be regarded as a qubit analogue of the bosonic thermal state. The latter is a state corresponding to a heat bath with an average number of photons equal to $N_B$. The generalized amplitude damping channel can then be seen as a qubit analogue of the bosonic thermal noise channel.



\subsubsection{Erasure Channel}

\label{sec:QM-over:qudit-erasure}

	The qubit \textit{erasure channel} $\mathcal{E}_{p}$ with \textit{erasure probability} $p\in[0,1]$ has the following action on an  input qubit state $\rho$:
	\begin{equation}\label{eq-erasure_channel}
		\mathcal{E}_{p}(\rho)=(1-p)\rho+p\Tr[\rho]\ket{e}\!\bra{e},
	\end{equation}
	where $\ket{e}$ is some unit vector that is orthogonal to all states in the input qubit Hilbert space and $\ket{e}\!\bra{e}$ is called the \textit{erasure state}.
	%That is, the channel input space is $\Lin(\mathbb{C}^2)$, and  the channel output space expands the input space by one dimension to $\Lin(\mathbb{C}^2)\oplus \ket{e}\!\bra{e}$.
	For example, if the input qubit Hilbert space is spanned by the standard basis $\{\ket{0},\ket{1}\}$ and the output qutrit Hilbert space is spanned by the standard basis $\{\ket{0},\ket{1},\ket{2}\}$, then we can set~$\ket{e}=\ket{2}$. 
	
	It is straightforward to verify that a set of Kraus operators for $\mathcal{E}_p$ is
	\begin{equation}
		\left\{\sqrt{1-p}(\ket{0}\!\bra{0}+\ket{1}\!\bra{1}),\sqrt{p}\ket{e}\!\bra{0},\sqrt{p}\ket{e}\!\bra{1}\right\}.
	\end{equation}
	
	The qudit erasure channel is a simple generalization of the qubit erasure channel. In fact, it is defined by \eqref{eq-erasure_channel}, with the main exception being that the input state $\rho$ is a  qudit input state. A set of Kraus operators for the qudit erasure channel is
		\begin{equation}
		\left\{\sqrt{1-p}(\ket{0}\!\bra{0}+\cdots + \ket{d-1}\!\bra{d-1}),\sqrt{p}\ket{e}\!\bra{0},\ldots, \sqrt{p}\ket{e}\!\bra{d-1}\right\}.
	\end{equation}

	
	We now discuss how the pure-loss bosonic channel restricted to acting on dual-rail single-photon inputs, an important model for transmission of single photons thro\-ugh an optical fiber, corresponds to a qubit erasure channel. The correspondence is illustrated in Figure \ref{fig-pure_loss_DR}.
	
	Consider a dual-rail optical system, i.e., a quantum optical system with two distinct optical modes $A_1$ and $A_2$ representing the input to the channel. As described at the beginning of Section~\ref{sec-state_meas}, the two-dimensional subspace spanned by the states $\{\ket{0,1}_{A_1,A_2},\ket{1,0}_{A_1,A_2}\}$, consisting of a total of one photon in either one of the two modes, constitutes a qubit system. We also let~$E_1$ and $E_2$ be two distinct optical modes constituting a dual-rail qubit system representing the environment of the channel. Finally, let $B_1$ and $B_2$ be two distinct optical modes spanned by the states $\{\ket{0,0}_{B_1,B_2},\ket{0,1}_{B_1,B_2},\ket{1,0}_{B_1,B_2}\}$, so that together $B_1$ and $B_2$ constitute a qutrit system.
	
	\begin{figure}
		\centering
		\includegraphics[scale=0.8]{Figures/pure_loss_DR.pdf}
		\caption{The qubit erasure channel $\mathcal{E}_{1-\eta}$, for $\eta\in[0,1]$, can be physically realized by using a photonic dual-rail qubit system and passing each of the two modes through a beamsplitter, modeled by the unitary $U^\eta$ in \eqref{eq-pure_loss_BS}, such that the input from the environment is the vacuum state. }\label{fig-pure_loss_DR}
	\end{figure}
	
	When the unitary corresponding to a quantum-optical beamsplitter acts on the space spanned by $\{\ket{0,0},\ket{0,1},\ket{1,0}\}$, it is equivalent to the upper left $3\times 3$ matrix in \eqref{eq-amp_damp_BS}. We can thus make use of this fact because the environment state for the bosonic pure-loss channel is prepared in the state $\ket{0}\!\bra{0}$. Let $U_{A_iE_i\to B_iE_i}^\eta$ then denote the beamsplitter unitary, for $i\in\{1,2\}$, with the following action on the basis $\{\ket{0,0},\ket{0,1},\ket{1,0}\}$ of the input and output modes (in that order):
	\begin{equation}\label{eq-pure_loss_BS}
		U_{A_iE_i\to B_iE_i}^\eta=\begin{pmatrix} 1&0&0
		\\
		0&\sqrt{\eta}&\I\sqrt{1-\eta}
		\\
		0&\I\sqrt{1-\eta}&\sqrt{\eta}
\end{pmatrix}.
	\end{equation}
	Letting $\rho_{A_1A_2}$ be an arbitrary qubit state on the two modes $A_1$ and $A_2$ defined by
	\begin{equation}\label{eq-pure_loss_input}
		\begin{aligned}
		\rho_{A_1,A_2}&=(1-\lambda)\ket{0,1}\!\bra{0,1}_{A_1,A_2}+\alpha\ket{0,1}\!\bra{1,0}_{A_1,A_2}+\conj{\alpha}\ket{1,0}\!\bra{0,1}_{A_1,A_2}\\
		&\qquad\qquad+\lambda\ket{1,0}\!\bra{1,0}_{A_1,A_2},
		\end{aligned}
	\end{equation}
	the pure-loss bosonic channel on the dual-rail qubit system $A_1A_2$ is given by
	\begin{equation}
		\begin{aligned}
		&\Tr_{E_1,E_2}\!\left[(U_{A_1E_1\to B_1E_1}^\eta\otimes U_{A_2E_2\to B_2E_2}^\eta)(\rho_{A_1,A_2}\otimes\ket{0,0}\!\bra{0,0}_{E_1,E_2})\right.\\
		&\qquad\qquad \left.\times (U_{A_1E_1\to B_1E_1}^\eta\otimes U_{A_2E_2\to B_2E_2}^\eta)^\dagger\right].
		\end{aligned}
	\end{equation}
	Although this has a similar form to \eqref{eq-amp_damp_Stinespring}, which defines the amplitude damping channel, our particular realization of the qubit system in terms of dual-rail single photons results in a completely different output from that of the amplitude damping channel. In particular, using \eqref{eq-pure_loss_input} along with \eqref{eq-pure_loss_BS}, it is straightforward to show that
	\begin{align}
		&\Tr_{E_1,E_2}\!\left[(U_{A_1E_1\to B_1E_1}^\eta\otimes U_{A_2E_2\to B_2E_2}^\eta)(\rho_{A_1,A_2}\otimes\ket{0,0}\!\bra{0,0}_{E_1,E_2})\right. \nonumber \\
		&\qquad\qquad \left. \times(U_{A_1E_1\to B_1E_1}^\eta\otimes U_{A_2E_2\to B_2E_2}^\eta)^\dagger\right]\nonumber\\
		&=\eta\rho_{B_1,B_2}+(1-\eta)\ket{0,0}\!\bra{0,0}_{B_1,B_2}\nonumber\\
		&=\mathcal{E}_{1-\eta}(\rho_{A_1,A_2}).
	\end{align}
	In other words, the pure-loss bosonic channel on a dual-rail qubit system is simply the qubit erasure channel $\mathcal{E}_{1-\eta}$ with erasure probability $1-\eta$ and erasure state $\ket{0,0}\!\bra{0,0}_{B_1,B_2}$. This means that a dual-rail single-photonic qubit sent through a pure-loss bosonic channel is transmitted to the receiver unchanged with probability $\eta$, or it is lost, and replaced by the vacuum state $\ket{0,0}\!\bra{0,0}$, with probability $1-\eta$. 
	

\subsubsection{Pauli Channels}

	The \textit{Pauli channels} constitute an important class of channels on qubit  systems. They are based on the qubit \textit{Pauli operators} $X$, $Y$, $Z$, which have the following matrix representation in the standard basis $\{\ket{0},\ket{1}\}$:
	\begin{equation}\label{eq-Pauli_operators}
		X=\begin{pmatrix} 0&1\\1&0\end{pmatrix},\quad Y=\begin{pmatrix} 0&-\I\\\I &0\end{pmatrix},\quad Z=\begin{pmatrix} 1&0\\0&-1\end{pmatrix}.
	\end{equation}
	The Pauli operators are Hermitian, satisfy $X^2=Y^2=Z^2=\mathbbm{1}$, and mutually anti-commute.
	
	A general Pauli channel is one whose Kraus operators are proportional to the Pauli operators, i.e.,
	\begin{equation}
		\rho\mapsto p_I\rho+p_X X\rho X +p_Y Y\rho Y +p_Z Z\rho Z,
	\end{equation}
	where $p_I,p_X,p_Y,p_Z\geq 0$, $p_I+p_X+p_Y+p_Z=1$.
	
	Here we highlight two particular Pauli channels of interest.
	\begin{enumerate}
		\item \textit{Dephasing channel}: We let $p_I=1-p$ and $p_Z=p$ for $0\leq p\leq 1,$ and $p_X=p_Y=0$. The action of the dephasing channel is thus
			\begin{equation}
				\rho\mapsto (1-p)\rho+pZ\rho Z.
			\end{equation}
			To see why this is called the dephasing channel, consider again a general state $\rho$ of the form \eqref{eq-qubit_state} and let $p=\frac{1}{2}$. In this case, we call the channel the \textit{completely dephasing channel}, and it is straightforward to see that
			\begin{equation}\label{eq-completely_dephasing_channel}
				\rho=\begin{pmatrix} 1-\lambda & \alpha \\ \conj{\alpha} & \lambda \end{pmatrix}\mapsto \frac{1}{2}\rho+\frac{1}{2}Z\rho Z=\begin{pmatrix} 1-\lambda & 0\\ 0 & \lambda \end{pmatrix}.
			\end{equation}
			In other words, the completely dephasing channel eliminates the off-diagonal elements of the input state (when represented in the standard basis, which is the same basis in which $Z$ is diagonal), so that the relative phase between the $\ket{0}$ state and the $\ket{1}$ state vanishes and the state becomes effectively classical.
			
			In the more general case when $p\neq\frac{1}{2}$, the effect of the dephasing channel is to reduce the magnitude of the off-diagonal elements:
			\begin{align}
				\rho  =\begin{pmatrix} 1-\lambda & \alpha \\ \conj{\alpha} & \lambda \end{pmatrix}
				& \mapsto (1-p)\rho+p Z\rho Z\\
				& =\begin{pmatrix}
				1-\lambda & (1-2p)\alpha  
				\\ (1-2p)\conj{\alpha} & \lambda \end{pmatrix}.
			\end{align}
		
		\item \textit{Depolarizing Channel}: For $p\in[0,1]$, the depolarizing channel is defined by letting $p_I=1-p$ and $p_X=p_Y=p_Z=\frac{p}{3}$, so that
			\begin{equation}\label{eq-qubit_depolarizing_channel}
				\rho\mapsto (1-p)\rho +\frac{p}{3}(X\rho X+Y\rho Y+Z\rho Z).
			\end{equation}
			By using the identity
			\begin{equation}\label{eq-Pauli_twirl}
				\frac{1}{4}\rho+\frac{1}{4}X\rho X+\frac{1}{4}Y\rho Y+\frac{1}{4}Z\rho Z=\Tr[\rho]\pi,
			\end{equation}
			we can equivalently write the action of the depolarizing channel as
			\begin{equation}
				\rho\mapsto \left(1-\frac{4p}{3}\right)\rho+\frac{4p}{3}\Tr[\rho]\pi,
			\end{equation}
			which has the interpretation that the state of the system is replaced by the maximally mixed state $\pi$ with probability $\frac{4p}{3}$. Observe, however, that $\frac{4p}{3}$ can be interpreted as a probability only for $0\leq p\leq\frac{3}{4}$.	
	\end{enumerate}
	
\subsubsection{Generalized Pauli Channels}\label{sec:QM-over:gen-pauli-chs}
	
	
	The qubit Pauli channels have a generalization to the qudit case also. Before defining the generalized Pauli channels, we first generalize the qubit Pauli operators to the Heisenberg--Weyl operators. The latter are defined as
	\begin{align}
		W_{z,x} & =Z(z)X(x), \label{eq-Heisenberg_Weyl_operators}\\
		Z(z) & \coloneqq\sum_{k=0}^{d-1}\e^{\frac{2\pi\I kz}{d}}\ket{k}\!\bra{k},\label{eq-gen_Z_Pauli}\\
		 X(x) & \coloneqq\sum_{k=0}^{d-1}\ket{k+x}\!\bra{k},\label{eq-gen_X_pauli}
	\end{align}
	for all $0\leq z,x\leq d-1$. When the dimension $d=2$, these operators reduce to the Pauli operators. The addition operation in the definition of $X(x)$ is performed modulo $d$. The operators $X(x)$ and $Z(z)$ satisfy the commutation relation
	\begin{equation}\label{eq-Heisenberg_Weyl_prop1}
		Z(z)X(x)=\e^{\frac{2\pi\I xz}{d}}X(x)Z(z).
	\end{equation}
	The Heisenberg--Weyl operators are unitary, just like the Pauli operators; however, unlike the Pauli operators, they are \textit{not} Hermitian. In particular,
	\begin{equation}\label{eq-Heisenberg_Weyl_prop2}
		W_{z,x}^\dagger =\e^{-\frac{2\pi\I xz}{d}}W_{-z,-x}.
	\end{equation}
	It is also straightforward to show that
	\begin{equation}\label{eq-Heisenberg_Weyl_prop3}
		W_{z_1,x_1}W_{z_2,x_2}=\e^{-\frac{2\pi\I x_1z_2}{d}}W_{z_1+z_2,x_1+x_2}.
	\end{equation}
	Furthermore, the Heisenberg--Weyl operators are orthogonal with respect to the Hilbert--Schmidt inner product, meaning that
	\begin{equation}
		\inner{W_{z_1,x_1}}{W_{z_2,x_2}}=\Tr[W_{z_1,x_1}^\dagger W_{z_2,x_2}]=d\delta_{z_1,z_2}\delta_{x_1,x_2}
		\label{eq:QM-over:HW-orthogonal}
	\end{equation}
	for all $0\leq z_1,z_2,x_1,x_2\leq d-1$. 
	The following identity, called a ``Heisenberg--Weyl twirl,'' plays an important role here and throughout this book:

	\begin{Lemma*}{Heisenberg--Weyl Twirl}{lem:QM-over:HW-twirl}
	Let $M$ be a linear operator, and set $\pi_d\coloneqq \frac{\mathbbm{1}}{d}$. Then
		\begin{equation}\label{eq-HW_twirl}
			\frac{1}{d^2}\sum_{z,x=0}^{d-1}W_{z,x}M W_{z,x}^\dagger=\Tr[M] \pi_d . 
		\end{equation}
	\end{Lemma*}
	
\begin{Proof}
The Heisenberg--Weyl operators form an irreducible projective unitary representation of the group $\mathbb{Z}_d\times\mathbb{Z}_d$. This fact can be used to prove \eqref{eq-HW_twirl} (see Bibliographic Notes in Section~\ref{sec:qm:bib-notes}).

Here we give a direct proof. To see the identity in \eqref{eq-HW_twirl}, consider that
\begin{equation}
\frac{1}{d^{2}}\sum_{z,x}W_{z,x}MW_{z,x}^{\dag}=(\overline{\Delta}_{X}%
\circ\overline{\Delta}_{Z})(M),
\end{equation}
where%
\begin{equation}
\overline{\Delta}_{Z}(M)\coloneqq \frac{1}{d}\sum_{z=0}^{d-1}Z(z)MZ(z)^{\dag}%
,\qquad\overline{\Delta}_{X}(M)\coloneqq \frac{1}{d}\sum_{x=0}^{d-1}X(x)MX(x)^{\dag}.
\end{equation}
We prove \eqref{eq-HW_twirl} by showing that $(\overline{\Delta}_{X}\circ\overline{\Delta}%
_{Z})(|\ell\rangle\!\langle m|)=\delta_{\ell,m}\mathbbm{1}/d$, from which the statement in
\ref{eq-HW_twirl} follows by linearity because%
\begin{align}
(\overline{\Delta}_{X}\circ\overline{\Delta}_{Z})(M)  & =(\overline{\Delta
}_{X}\circ\overline{\Delta}_{Z})\left(  \sum_{\ell,m}M_{\ell,m}|\ell
\rangle\!\langle m|\right)  \\
& =\sum_{\ell,m}M_{\ell,m}(\overline{\Delta}_{X}\circ\overline{\Delta}%
_{Z})\left(  |\ell\rangle\!\langle m|\right)  \\
& =\sum_{\ell,m}M_{\ell,m}\delta_{\ell,m}\frac{\mathbbm{1}}{d}\\
& =\operatorname{Tr}[M]\frac{\mathbbm{1}}{d}.
\end{align}
Consider that%
\begin{align}
\overline{\Delta}_{Z}(|\ell\rangle\!\langle m|)  & =\frac{1}{d}\sum_{z=0}%
^{d-1}Z(z)|\ell\rangle\!\langle m|Z(z)^{\dag}\\
& =\frac{1}{d}\sum_{z=0}^{d-1}\e^{2\pi \I\ell z/d}|\ell\rangle\!\langle m|\e^{-2\pi
\I mz/d}\\
& =|\ell\rangle\!\langle m|\left(  \frac{1}{d}\sum_{z=0}^{d-1}\e^{2\pi \I \left(
\ell-m\right)  z/d}\right)  \\
& =|\ell\rangle\!\langle m|\delta_{\ell,m}.
\end{align}
Now consider that%
\begin{align}
\overline{\Delta}_{X}(|\ell\rangle\!\langle\ell|)  & =\frac{1}{d}\sum
_{x=0}^{d-1}X(x)|\ell\rangle\!\langle\ell|X(x)^{\dag}\\
& =\frac{1}{d}\sum_{x=0}^{d-1}|\ell+x\rangle\!\langle\ell+x|\\
& =\frac{\mathbbm{1}}{d}.
\end{align}
This concludes the proof.
\end{Proof}

	
	A generalized Pauli channel is then defined as
	\begin{equation}
	\rho \mapsto \sum_{z,x=0}^{d-1} p_{z,x} W_{z,x} \rho W_{z,x}^{\dag},
	\end{equation}
	where $\{p_{z,x}\}_{z,x} $ is a probability distribution satisfying $p_{z,x} \geq 0$ for all $0\leq z,x\leq d-1$ and $\sum_{z,x}p_{z,x}=1$. Thus, this channel randomly applies one of the Heisenber--Weyl operators in \eqref{eq-Heisenberg_Weyl_operators} to the input.
	
	A special case of a generalized Pauli channel is a $d$-dimensional dephasing channel
	\begin{equation}
	\rho \mapsto \sum_{z=0}^{d-1} p_{z} Z(z) \rho Z(z)^{\dag},
	\label{eq:QM-over:d-dim-dephase}
	\end{equation}
	where $\{p_z\}_z$ is a probability distribution. For this special case, only the phase operators $Z(z)$ are applied randomly to the input $\rho$, with the effect being to modify only the off-diagonal elements of $\rho$ (with respect to the standard basis).
	
	The depolarizing channel on qubits can be generalized using the Heisen\-berg--Weyl operators, as defined in \eqref{eq-Heisenberg_Weyl_operators}.
	%as the set $\{W_{z,x}:0\leq x,z\leq d-1\}$ with
	%\begin{align}
%		W_{z,x}&=Z(z)X(x),\\
%		Z(z)&=\sum_{k=0}^{d-1}\e^{\frac{2\pi\I kz}{d}}\ket{k}\!\bra{k},\\
%		X(x)&=\sum_{k=0}^{d-1}\ket{k+x}\!\bra{k},
%	\end{align}
%	where the addition in the definition of $X(x)$ is performed modulo $d$.
	The \textit{qudit depolarizing channel} is then defined as
	\begin{equation}
		\mathcal{D}_{p}^{(d)}(\rho)\coloneqq (1-p)\rho+\frac{p}{d^2-1}\sum_{(z,x)\neq (0,0)}W_{z,x}\rho W_{z,x}^\dagger,\quad 0\leq p\leq 1.
		\label{eq:QM-over:qudit-depolarizing}
	\end{equation}
	Setting%
\begin{equation}
q\equiv q(p)\coloneqq \frac{pd^{2}}{d^{2}-1}%
\end{equation}
the depolarizing channel can alternatively be written in terms of this reparameterization as%
\begin{equation}
\mathcal{D}_{p}^{(d)}(\rho)=\left(  1-q\right)  \rho+q\operatorname{Tr}%
[\rho]\frac{\mathbbm{1}}{d},
\label{eq:QM-over:qudit-depol-reparam}
\end{equation}
because%
\begin{align}
\mathcal{D}_{p}^{(d)}(\rho)  & =\left(  1-p\right)  \rho+\frac{p}{d^{2}-1}%
\sum_{\left(  z,x\right)  \neq\left(  0,0\right)  }W_{z,x}\rho W_{z,x}^{\dag
}\\
& =\left(  1-p-\frac{p}{d^{2}-1}\right)  \rho+\frac{p}{d^{2}-1}\sum
_{z,x}W_{z,x}\rho W_{z,x}^{\dag}\\
& =\left(  1-q\right)  \rho+q\frac{1}{d^{2}}\sum_{z,x}W_{z,x}\rho
W_{z,x}^{\dag}\\
& =\left(  1-q\right)  \rho+q\operatorname{Tr}[\rho]\frac{\mathbbm{1}}{d}\ ,
\end{align}
where the last equality follows from \eqref{eq-HW_twirl}.



\subsection{Classical--Quantum and Quantum--Classical Channels}

	Any classical probability distribution $p:\mathcal{X}\to[0,1]$ over a finite alphabet $\mathcal{X}$ can be represented as a quantum state of a $|\mathcal{X}|$-dimensional system $X$ that is diagonal in an orthonormal basis $\{\ket{x}\}_{x\in\mathcal{X}}$ of $X$. Specifically, the probability distribution can be represented as the state
	\begin{equation}
		\rho_X=\sum_{x\in\mathcal{X}}p(x)\ket{x}\!\bra{x}_X.
	\end{equation}
	States that are diagonal in a preferred basis as in the above equation are typically called \textit{classical states}. In addition to being in one-to-one correspondence with classical probability distributions, classical states do not exhibit the quantum properties of coherence and entanglement.
	
	In Chapter~\ref{chap-classical_capacity}, however, we are interested in classical communication over quantum channels. We are then interested in so-called \textit{classical--quantum channels}, which we discuss in this section, that take a classical state as input and output a quantum state. 
	
	\begin{definition}{Classical--Quantum Channel}{def-cq_channel}
		A \textit{classical--quantum channel} is a map from a system $X$ with alphabet $\mathcal{X}$ and orthonormal basis $\{\ket{x}:x\in\mathcal{X}\}$ to a quantum system $A$ with a specified set $\{\sigma_A^x:x\in\mathcal{X}\}$ of states such that
		\begin{equation}
			\ket{x}\!\bra{x'}\mapsto \delta_{x,x'}\sigma_A^x\quad\forall~ x,x'\in\mathcal{X}.
		\end{equation}
	\end{definition}
	
	If $\mathcal{N}^{\text{cq}}$ is a classical--quantum channel, then for every classical state $\rho_X\allowbreak=\sum_{x\in\mathcal{X}}p(x)\ket{x}\!\bra{x}$, we have that
	\begin{equation}
		\mathcal{N}^{\text{cq}}(\rho_X)=\sum_{x\in\mathcal{X}}p(x)\sigma_A^x.
	\end{equation}
	More generally, for every $|\mathcal{X}|$-dimensional system $A$ and every state $\rho_{A}$ that is not necessarily classical and is expressed in the computational basis as $\rho_{A}=\sum_{x,x'\in\mathcal{X}}\bra{x}\rho_A\ket{x'}\ket{x}\!\bra{x'}$, we find that
	\begin{equation}
		\mathcal{N}^{\text{cq}}(\rho_A)=\sum_{x,x'\in\mathcal{X}}\bra{x}\rho_A\ket{x'}\delta_{x,x'}\sigma_A^x=\sum_{x\in\mathcal{X}}\bra{x}\rho_A\ket{x}\sigma_A^x.
	\end{equation}
	Therefore, for every quantum state, the classical--quantum channel $\mathcal{N}^{\text{cq}}$ takes the input state, measures it in the computational basis $\{\ket{x}\}_{x\in\mathcal{X}}$, and with the corresponding outcome probability $\bra{x}\rho_A\ket{x}$, outputs the state $\sigma_A^x$. 
	
	The Choi state $\Phi^{\mathcal{N}^{\text{cq}}}$ of a classical--quantum channel is
	\begin{equation}
		\Phi_{XA}^{\mathcal{N}^{\text{cq}}}=\frac{1}{|\mathcal{X}|}\sum_{x,x'\in\mathcal{X}}\ket{x}\!\bra{x'}_X\otimes\mathcal{N}(\ket{x}\!\bra{x'}_X)=\sum_{x\in\mathcal{X}}\frac{1}{|\mathcal{X}|}\ket{x}\!\bra{x}_X\otimes\sigma_A^x.
	\end{equation}
	In other words, the Choi state of a classical--quantum channel is a classical--quantum state.
	
	If the states $\sigma_A^x$ have spectral decomposition
	\begin{equation}
		\sigma_A^x=\sum_{j=1}^{r_x}\lambda_j^x\ket{\varphi_j^x}\!\bra{\varphi_j^x},
	\end{equation}
	where $r_x=\rank(\sigma_A^x)$, then $\{K_j^x:x\in\mathcal{X},~1\leq j\leq r_x\}$ is a set of Kraus operators for $\mathcal{N}^{\text{cq}}$, where $K_j^x=\sqrt{\smash[b]{\lambda_j^x}}\ket{\varphi_j^x}_A\bra{x}_X$. Indeed, for all $x,x'\in\mathcal{X}$,
	\begin{align}
		&\sum_{x''\in\mathcal{X}}\sum_{j=1}^{r_{x''}}K_j^{x''}\ket{x}\!\bra{x'}(K_j^{x''})^\dagger \notag\\
		&=\sum_{x''\in\mathcal{X}}\sum_{j=1}^{r_{x''}}\sqrt{\smash[b]{\lambda_j^{x''}}}\ket{\varphi_j^{x''}}\braket{x''}{x}\braket{x'}{x''}\!\bra{\varphi_j^{x''}}\sqrt{\smash[b]{\lambda_j^{x''}}}\\
		&=\delta_{x,x'}\sum_{j=1}^{r_x}\lambda_k^x\ket{\varphi_j^x}\!\bra{\varphi_j^x}\\
		&=\delta_{x,x'}\sigma_A^x\\
		&=\mathcal{N}^{\text{cq}}(\ket{x}\!\bra{x'}),
	\end{align}
	and
	\begin{align}
		\sum_{x\in\mathcal{X}}\sum_{j=1}^{r_x}(K_j^x)^\dagger K_j^x&=\sum_{x\in\mathcal{X}}\sum_{j=1}^{r_x}\lambda_j^x\ket{x}\underbrace{\braket{\smash[b]{\varphi_j^x}}{\smash[b]{\varphi_j^x}}}_{=1}\bra{x}\\
		&=\sum_{x\in\mathcal{X}}\underbrace{\sum_{j=1}^{r_x}\lambda_j^x}_{=1~\forall~x}\ket{x}\!\bra{x}\\
		&=\mathbbm{1}_X.
	\end{align}
	Also, observe from the  construction above that every classical--quantum channel has a Kraus representation with unit-rank Kraus operators.
	
	Having described classical--quantum channels, let us now describe channels for which the situation is opposite, such that they accept quantum inputs and provide classical outputs.

	\begin{definition}{Quantum--Classical Channel}{def-qc_channel}
		Given a quantum system $A$ and a measurement on $A$ with corresponding POVM $\{M_x\}_{x\in\mathcal{X}}$ indexed by elements of a finite alphabet $\mathcal{X}$, a \textit{quantum--classical channel}, or \textit{measurement channel}, is a map from the quantum system $A$ to a classical system $X$ with alphabet $\mathcal{X}$ such that
		\begin{equation}\label{eq-measurement_channel}
			\rho_A\mapsto \sum_{x\in\mathcal{X}}\Tr[M_x\rho_A]\ket{x}\!\bra{x}_X
		\end{equation}
		for every state $\rho_A$ on $A$, where $\{\ket{x}:x\in\mathcal{X}\}$ is an orthonormal basis for $X$.
	\end{definition}
	
	A measurement channel thus takes the measurement outcome probabilities $\Tr[M_x\rho_A]$ and arranges them into a classical state.
	
	Denoting the measurement channel in Definition~\ref{def-qc_channel} as $\mathcal{M}_{A\to X}$, its Choi state $\Phi^{\mathcal{M}}_{AX}$ is as follows:
	\begin{align}
	\Phi^{\mathcal{M}}_{AX} & = 
	\frac{1}{d_A} \sum_{i,j=0}^{d_A-1} \ket{i}\!\bra{j}_A \otimes \sum_{x \in \mathcal{X}} \Tr[M_x \ket{i}\!\bra{j}] \ket{x}\!\bra{x}_X \\
		& = \frac{1}{d_A} \sum_{x\in \mathcal{X}} \sum_{i,j=0}^{d_A-1} \ket{i}\!\bra{j}_A \otimes  \bra{j} M_x \ket{i} \ket{x}\!\bra{x}_X \\
		& = \frac{1}{d_A} \sum_{x\in \mathcal{X}} \sum_{i,j=0}^{d_A-1} \ket{i}\bra{j} M_x \ket{i} \bra{j}_A \otimes   \ket{x}\!\bra{x}_X \\
		& = \frac{1}{d_A} \sum_{x\in \mathcal{X}}  (M_x^{\t})_A  \otimes   \ket{x}\!\bra{x}_X ,
	\end{align}
	where we applied Definition~\ref{def-partial_transpose} to arrive at the last equality.
	
	
	By writing a spectral decomposition of $M_x$ as
	\begin{equation}
		M_x=\sum_{j=1}^{r_x}\mu_{j}^x\ket{\phi_j^{x}}\!\bra{\phi_j^{x}},
	\end{equation}
	where $r_x=\rank(M_x)$, we can write
	\begin{equation}
		\Tr[M_x\rho]=\sum_{j=1}^{r_x}\mu_{j}^x\bra{\phi_{j}^x}\rho\ket{\phi_{j}^x}.
	\end{equation}
	Therefore, the action of a quantum--classical channel $\mathcal{N}^{\text{qc}}$ can be written as
	\begin{align}
		\mathcal{N}^{\text{qc}}(\rho)&=\sum_{x\in\mathcal{X}}\Tr[M_x\rho]\ket{x}\!\bra{x}\\
		&=\sum_{x\in\mathcal{X}}\sum_{j=1}^{r_x}\mu_j^x\bra{\phi_{j}^x}\rho\ket{\phi_{j}^x}\ket{x}\!\bra{x}\\
		&=\sum_{x\in\mathcal{X}}\sum_{j=1}^{r_x}\sqrt{\smash[b]{\mu_j^x}}\ket{x}\!\bra{\phi_{j}^x}\rho\ket{\phi_{j}^x}\!\bra{x}\sqrt{\smash[b]{\mu_j^x}}\\
		&=\sum_{x\in\mathcal{X}}\sum_{j=1}^{r_x}K_j^x\rho(K_j^x)^\dagger,
	\end{align}
	where
	\begin{equation}
		K_j^x\coloneqq\sqrt{\smash[b]{\mu_j^x}}\ket{x}\!\bra{\phi_{j}^x}\quad\forall ~x\in\mathcal{X},~1\leq j\leq r_x.
	\end{equation}
	Since
	\begin{align}
		\sum_{x\in\mathcal{X}}\sum_{j=1}^{r_x}(K_j^x)^\dagger K_j^x&=\sum_{x\in\mathcal{X}}\sum_{j=1}^{r_x}\mu_j^x\ket{\phi_{j}^x}\braket{x}{x}\!\bra{\phi_{j}^x}\\
		&=\sum_{x\in\mathcal{X}}\underbrace{\sum_{j=1}^{r_x}\mu_j^x\ket{\phi_{j}^x}\!\bra{\phi_{j}^x}}_{M_x}\\
		&=\sum_{x\in\mathcal{X}}M_x\\
		&=\mathbbm{1}_A,
	\end{align}
	it holds that $\{K_j^x:x\in\mathcal{X},~1\leq j\leq r_x\}$ is a set of Kraus operators for $\mathcal{N}^{\text{qc}}$. This means that all quantum--classical channels have a Kraus representation with unit-rank Kraus operators.
	
	
	
	%By concatenating a quantum--classical channel followed by a classical--quantum channel, we can obtain the following 
	
	%Note that if the classical system $X$ in the definition of the classical--quantum channel arises from measurement of a quantum system, i.e., as the output of a quantum--classical channel, then 



\subsection{Quantum Instruments}
	
	Recall from Section~\ref{subsec-meas} that, for an arbitrary POVM $\{M_x\}_{x\in\mathcal{X}}$, a set of post-measure\-ment states corresponding to an initial state $\rho$ can be given by \eqref{eq-post_meas},
	\begin{equation}
		\rho^x=\frac{K_x\rho K_x^\dagger}{\Tr[K_x\rho K_x^\dagger]}\quad\forall~x\in\mathcal{X},
	\end{equation}
	where $\{K_x\}_{x\in\mathcal{X}}$ is a set of operators such that $M_x=K_x^\dagger K_x$ for all $x\in\mathcal{X}$. Also recall that the expected density operator of the measurement is given by~\eqref{eq-post_meas_avg},
	\begin{equation}
		\sum_{x\in\mathcal{X}}K_x\rho K_x^\dagger.
	\end{equation}
	This expected state can be seen as arising from a quantum channel with Kraus operators $\{K_x\}_{x\in\mathcal{X}}$. Note that this map is indeed a channel since $\sum_{x\in\mathcal{X}} K_x^\dagger K_x=\sum_{x\in\mathcal{X}} M_x=\mathbbm{1}$. We can view the channel as being the sum of the completely positive and trace-non-increasing maps $\mathcal{M}_x$ defined as
	\begin{equation}
		\mathcal{M}_x(\rho)=K_x \rho K_x^\dagger.
	\end{equation}
	
	A quantum instrument generalizes this notion to maps $\mathcal{M}_x$ that are completely positive and trace non-increasing with an arbitrary number of Kraus operators, not just one.
	
	\begin{definition}{Quantum Instrument}{def-q_instrument}
		A \textit{quantum instrument} is a collection $\{\mathcal{M}_x\}_{x\in\mathcal{X}}$ of completely positive and trace-non-increasing maps indexed by elements of a finite alphabet $\mathcal{X}$, such that the sum map $\sum_{x\in\mathcal{X}} \mathcal{M}_x$ is a quantum channel.
	\end{definition}
	
	A quantum instrument corresponds to a more general notion of a measurement in which, as before, the elements of the alphabet $\mathcal{X}$ correspond to the measurement outcomes. If the initial state of the system is $\rho$, then the corresponding measurement outcome probabilities $p(x)$ are given by
	\begin{equation}
		p(x)=\Tr[\mathcal{M}_x(\rho)],
	\end{equation}
	and the corresponding post-measurement state is
	\begin{equation}
		\rho^x=\frac{\mathcal{M}_x(\rho)}{\Tr[\mathcal{M}_x(\rho)]}.
	\end{equation}
	The expected state of the ensemble $\{(p(x),\rho^x)\}_{x\in\mathcal{X}}$ is then
	\begin{equation}\label{eq-post_meas_avg2}
		\sum_{x\in\mathcal{X}}\mathcal{M}_x(\rho).
	\end{equation}
	
	It is customary to define the output of a quantum instrument $\{\mathcal{M}_x\}_{x\in\mathcal{X}}$ as the channel $\mathcal{M}$ defined by
	\begin{equation}\label{eq-instrument_output}
		\mathcal{M}(\rho)=\sum_{x\in\mathcal{X}}
		\ket{x}\!\bra{x}_X \otimes
		\mathcal{M}_x(\rho).
	\end{equation}
	That is, the output of a quantum instrument is a classical--quantum state such that the classical register $X$ stores the outcome of the measurement. This is unlike the expected state in \eqref{eq-post_meas_avg2}, which represents a lack of knowledge of which measurement outcome occurred.
	
	Note that the channel in \eqref{eq-instrument_output} corresponding to a quantum instrument reduces to the measurement channel defined in \eqref{eq-measurement_channel} if we consider a measurement with POVM $\{M_x\}_{x\in\mathcal{X}}$ and we define the maps $\mathcal{M}_x$ as $\mathcal{M}_x(\rho)=\Tr[M_x\rho]$ for all $x\in\mathcal{X}$. In this case, the channel in \eqref{eq-instrument_output} becomes,
	\begin{equation}
		\mathcal{M}(\rho)=\sum_{x\in\mathcal{X}}\Tr[M_x\rho]\ket{x}\!\bra{x}_X,
	\end{equation}
	which is precisely the measurement channel in \eqref{eq-measurement_channel}.



\subsection{Entanglement-Breaking Channels}\label{subsec-ent_break_channels}

	An important class of channels in quantum communication consists of those that, when acting on one share of a bipartite state, eliminate any entanglement between the two systems. Such channels are called \textit{entanglement breaking}, and we define them as follows.
	
	\begin{definition}{Entanglement-Breaking Channel}{def-ent_break_chan}
		A channel $\mathcal{N}_{A\to B}$ is called \textit{entanglement breaking} if $(\id_R\otimes\mathcal{N}_{A\to B})(\rho_{RA})$ is a separable state for every state $\rho_{RA}$, where $R$ is an arbitrary reference system.
	\end{definition}
	
	Although Definition~\ref{def-ent_break_chan} suggests that it is necessary to check an infinite number of input states to determine whether a channel is entanglement breaking, the following proposition states that it is only necessary to check the output of the channel on the maximally entangled state.
	
		\begin{proposition}{prop:qm-over:EB-Choi-sep}
		A channel $\mathcal{N}$ is entanglement breaking if and only if  its Choi state $\Phi_{AB}^{\mathcal{N}}$ is separable.
	\end{proposition}
	
	\begin{Proof}
	Observe that if $\mathcal{N}_{A\to B}$ is entanglement breaking, then its Choi state $\Phi_{AB}^{\mathcal{N}}$ is separable. On the other hand, if the Choi state $\Phi_{AB}^{\mathcal{N}}$ of a given channel $\mathcal{N}$ is separable, then it is of the form
	\begin{equation}
		\Phi_{AB}^{\mathcal{N}}=\sum_{x\in\mathcal{X}}p(x)\sigma_A^x\otimes\tau_B^x
	\end{equation}
	for some probability distribution $p:\mathcal{X}\to[0,1]$ on a finite alphabet $\mathcal{X}$ and sets of states $\{\sigma_A^x:x\in\mathcal{X}\}$, $\{\tau_B^x:x\in\mathcal{X}\}$. We note that the property $\Tr_B[\Phi_{AB}^{\mathcal{N}}]=\pi_A$ of the Choi state translates to
	\begin{equation}\label{eq-choi_state_sep_partrace}
		\pi_A = \frac{\mathbbm{1}_A}{d_A}=\sum_{x\in\mathcal{X}} p(x)\sigma_A^x.
	\end{equation}
	Then, for every reference $R$ and state $\xi_{RA}$ on $\mathcal{H}_{RA}$, we find by using \eqref{eq-Choi_rep_action}
	\begin{align}
		(\id_R\otimes\mathcal{N})(\xi_{RA})&=d_A\Tr_A[(\T_A(\xi_{RA})\otimes\mathbbm{1}_B)(\mathbbm{1}_R\otimes\Phi_{AB}^{\mathcal{N}})]\\
		&=\sum_{x\in\mathcal{X}}q(x)\omega_R^x\otimes\tau_B^x,
	\end{align}
	where
	\begin{align}
		\omega_R^x & \coloneqq\frac{\Tr_A[\T_A(\xi_{RA})(\mathbbm{1}_R\otimes d_Ap(x)\sigma_A^x)]}{q(x)},\\
		 q(x) & \coloneqq p(x)d_A\Tr[\xi_A^{\t}\sigma_A^x].
	\end{align}
	Now, the map $x\mapsto q(x)$ is a probability distribution on $\mathcal{X}$ since $q(x)\geq 0$ for all $x\in\mathcal{X}$ and
	\begin{align}
		\sum_{x\in\mathcal{X}}q(x)&=d_A\Tr\!\left[\xi_A^{\t}\left(\sum_{x\in\mathcal{X}} p(x)\sigma_A^x\right)\right]\\
		&=d_A\Tr[\xi_A^{\t}\pi_A]\\
		&=\Tr[\xi_A]\\
		&=1,
	\end{align}
	where we have made use of \eqref{eq-choi_state_sep_partrace}. So $(\id_R\otimes\mathcal{N})(\xi_{RA})$ is a separable state.
	\end{Proof}

	
	Another useful characterization of entanglement breaking channels is thr\-ough their Kraus representations, as shown in the following proposition:
	
	\begin{proposition}{prop-ent_break_Kraus}%\label{prop-ent_break_Kraus}
		A channel $\mathcal{N}$ is entanglement breaking if and only if there exists a set of Kraus operators for $\mathcal{N}$, with each Kraus operator having unit rank.
	\end{proposition}
	
	\begin{Proof}
		First suppose that the Kraus operators of $\mathcal{N}$ have unit rank. They are therefore of the form $\ket{\phi_j}_B\bra{\psi_j}_A\eqqcolon K_j$ for $1\leq j\leq r$. Without loss of generality, we can let each vector in the set $\{\ket{\phi_j}\}_{j=1}^r$ be normalized. Then, since $\mathcal{N}$ is trace preserving, it holds that
		\begin{equation}\label{eq-ent_break_proof}
			\mathbbm{1}_A=\sum_{j=1}^r K_j^\dagger K_j=\sum_{j=1}^r\ket{\psi_j}_A\braket{\phi_j}{\phi_j}\!\bra{\psi_j}_A=\sum_{j=1}^r\ket{\psi_j}\!\bra{\psi_j}_A.
		\end{equation}
		
		Now, for every reference system $R$ of arbitrary dimension and every state $\rho_{RA}$, we find that
		\begin{align}
			(\id_R\otimes\mathcal{N})(\rho_{RA})&=\sum_{j=1}^r (\mathbbm{1}_R\otimes K_j)\rho_{RA}(\mathbbm{1}_R\otimes K_j^\dagger)\\
			&=\sum_{j=1}^r (\mathbbm{1}_R\otimes \ket{\phi_j}_B\bra{\psi_j}_A)\rho_{RA}(\mathbbm{1}_R\otimes \ket{\psi_j}_A\bra{\phi_j}_B)\\
			&=\sum_{j=1}^r (\mathbbm{1}_R\otimes\bra{\psi_j}_A)(\rho_{RA})(\mathbbm{1}_R\otimes\ket{\psi_j}_A)\otimes\ket{\phi_j}\!\bra{\phi_j}_B\\
			&=\sum_{j=1}^r p(j)\sigma_R^j\otimes\ket{\phi_j}\!\bra{\phi_j}_B,
		\end{align}
		where
		\begin{equation}
			\sigma_R^j\coloneqq \frac{(\mathbbm{1}_R\otimes\bra{\psi_j}_A)(\rho_{RA})(\mathbbm{1}_R\otimes\ket{\psi_j}_A)}{p(j)},\quad p(j)\coloneqq\bra{\psi_j}_A\rho_A\ket{\psi_j}_A.
		\end{equation}
		Note that $j\mapsto p(j)$ is a probability distribution since $p(j)\geq 0$ for all $j$, and
		\begin{align}
			\sum_{j=1}^r p(j)&=\sum_{j=1}^r\bra{\psi_j}_A\rho_A\ket{\psi_j}_A\\
			&=\sum_{j=1}^r\Tr[\ket{\psi_j}\!\bra{\psi_j}\rho_A]\\
			&=\Tr\!\left[\left(\sum_{j=1}^r \ket{\psi_j}\!\bra{\psi_j}_A\right)\rho_A\right]\\
			&=\Tr[\rho_A]\\
			&=1,
		\end{align}
		where we have made use of \eqref{eq-ent_break_proof}. Therefore, $(\id_R\otimes\mathcal{N})(\rho_{RA})$ is a separable state, so that $\mathcal{N}$ is entanglement breaking.
		
		Now, suppose that $\mathcal{N}$ is entanglement breaking. This means that its Choi state $\Phi_{AB}^{\mathcal{N}}$ is a separable state, which means that it can be written as
		\begin{equation}
			\Phi_{AB}^{\mathcal{N}}=\sum_{x\in\mathcal{X}}p(x)\ket{\psi_x}\!\bra{\psi_x}_A\otimes\ket{\phi_x}\!\bra{\phi_x}_B
		\end{equation}
		for some probability distribution $p:\mathcal{X}\to[0,1]$ on a finite alphabet $\mathcal{X}$ and sets of pure states $\{\ket{\psi_x}_A:x\in\mathcal{X}\}$, $\{\ket{\phi_x}_B:x\in\mathcal{X}\}$. Now, define the unit-rank operators
		\begin{equation}
			K_x\coloneqq \sqrt{\smash[b]{d_Ap(x)}}\ket{\phi_x}_B\bra{\conj{\psi_x}}_A,\quad x\in\mathcal{X}.
		\end{equation}
		Then, for every orthonormal basis state $\ket{i}_A$ on $A$, we have
		\begin{align}
			K_x\ket{i}_A&=\sqrt{\smash[b]{d_Ap(x)}}\ket{\phi_x}_B\braket{\conj{\psi_x}}{i}\\
			&=\sqrt{\smash[b]{d_Ap(x)}}\braket{i}{\psi_x}\ket{\phi_x}_B\\
			&=\sqrt{\smash[b]{d_Ap(x)}}(\bra{i}_A\otimes\mathbbm{1}_B)(\ket{\psi_x}_A\otimes\ket{\phi_x}_B).
		\end{align}
		Using this, we find that
		\begin{align}
			\mathcal{N}(\ket{i}\!\bra{i'}_A)&=d_A(\bra{i}_A\otimes\mathbbm{1}_B)\Phi_{AB}^{\mathcal{N}}(\ket{i'}_A\otimes\mathbbm{1}_B)\nonumber\\
			&=\sum_{x\in\mathcal{X}}\sqrt{\smash[b]{d_Ap(x)}}(\bra{i}_A\otimes\mathbbm{1}_B)(\ket{\psi_x}_A\otimes\ket{\phi_x}_B)\nonumber\\
			&\qquad\qquad\qquad\times(\bra{\psi_x}_A\otimes\bra{\phi_x}_B)(\ket{i'}_A\otimes\mathbbm{1}_B)\sqrt{\smash[b]{d_Ap(x)}}\nonumber\\
			&=\sum_{x\in\mathcal{X}}K_x\ket{i}\!\bra{i'}_A K_x^\dagger.
		\end{align}
		This holds for all $0\leq i,i'\leq d_A - 1$, which means that $\{K_x\}_{x\in\mathcal{X}}$ is a set of Kraus operators for $\mathcal{N}$, each of which has unit rank.
	\end{Proof}

	From this proposition, we immediately see that both quantum--class\-ical and classical--quantum channels are entanglement breaking, because each one has a Kraus representation with unit-rank Kraus operators. This implies that a composition of a quantum--classical channel followed by a classical-quan\-tum channel is also entanglement-breaking, for every such map can be written as
	\begin{equation}\label{eq-cq_qc_comp}
		\rho\mapsto \sum_{x\in\mathcal{X}}\Tr[M_x\rho] \sigma^x,
	\end{equation}
	where $\mathcal{X}$ is a finite alphabet, $\{\sigma^x\}_{x\in\mathcal{X}}$ is a set of quantum states, and $\{M_x\}_{x\in\mathcal{X}}$ is a POVM. If each POVM element $M_x$ has a spectral decomposition of the form
	\begin{equation}
		M_x=\sum_{k=1}^{r_x}\lambda_k^x\ket{\psi_k^x}\!\bra{\psi_k^x},
	\end{equation}
	where $r_x=\rank(M_x)$, and each state $\sigma^x$ has a spectral decomposition of the form
	\begin{equation}
		\sigma^x=\sum_{\ell=1}^{s_x}\alpha_\ell^x\ket{\phi_\ell^x}\!\bra{\phi_\ell^x},
	\end{equation}
	where $s_x=\rank(\sigma^x)$, then \eqref{eq-cq_qc_comp} can be written as
	\begin{align}
		\rho&\mapsto\sum_{x\in\mathcal{X}}\sum_{k=1}^{r_x}\sum_{\ell=1}^{s_x}\lambda_k^x\alpha_\ell^x\ket{\phi_\ell^x}\!\bra{\phi_\ell^x}\!\bra{\psi_k^x}\rho\ket{\psi_k^x}\\
		&=\sum_{x\in\mathcal{X}}\sum_{k=1}^{r_x}\sum_{\ell=1}^{s_x}\sqrt{\lambda_k^\ell\alpha_\ell^x}\ket{\phi_\ell^x}\!\bra{\psi_k^x}\rho\ket{\psi_k^x}\!\bra{\phi_\ell^x}\sqrt{\lambda_k^x\alpha_\ell^x}\\
		&=\sum_{x\in\mathcal{X}}\sum_{k=1}^{r_x}\sum_{\ell=1}^{s_x}K_{k,\ell}^x \rho (K_{k,\ell}^x)^\dagger,
	\end{align}
	where $K_{k,\ell}^x\coloneqq\sqrt{\lambda_k^x\alpha_\ell^x}\ket{\phi_\ell^x}\!\bra{\psi_k^x}$. Since $\{K_{k,\ell}^x:x\in\mathcal{X},~1\leq k\leq r_x,~1\leq\ell\leq s_x\}$ is a set of Kraus operators for the map, with each Kraus operator having unit rank, it holds by Proposition \ref{prop-ent_break_Kraus} that the map in \eqref{eq-cq_qc_comp} is entanglement breaking.
	
	A channel of the form \eqref{eq-cq_qc_comp} is sometimes called a ``measure-and-prepare channel'' or an ``inter\-cept-resend channel'' since the input to the channel is first measured then replaced by a new state conditioned on the measurement outcome. Remarkably, \textit{any} entanglement breaking channel can be written in the form \eqref{eq-cq_qc_comp}, as we now show.
	
	\begin{theorem}{thm-ent_break_meas_reprepare}%\label{thm-ent_break_meas_reprepare}
		For every entanglement-breaking channel $\mathcal{N}$, there exists a finite alphabet $\mathcal{X}$, a set $\{\sigma^x\}_{x\in\mathcal{X}}$ of states, and a POVM $\{M_x\}_{x\in\mathcal{X}}$ such that the action of $\mathcal{N}$ can be written as
		\begin{equation}\label{eq-meas_reprep_map_2}
			\mathcal{N}(\rho)=\sum_{x\in\mathcal{X}}\Tr[M_x\rho]\sigma^x
		\end{equation}
		for every state $\rho$.
	\end{theorem}
	
	\begin{Proof}
		By Proposition \ref{prop-ent_break_Kraus}, the action of $\mathcal{N}$ can be written as
		\begin{equation}
			\mathcal{N}(\rho)=\sum_{j=1}^r K_j\rho K_j^\dagger,
		\end{equation}
		where $r=\rank(\Gamma^{\mathcal{N}})$ and $\{K_j\}_{j=1}^r$ is a set of Kraus operators for $\mathcal{N}$, with each Kraus operator having unit rank. Since each Kraus operator has unit rank, it holds that $K_j=\ket{\phi_j}\!\bra{\psi_j}$ for all $1\leq j\leq r$, where $\{\ket{\phi_j}\}_{j=1}^r$ and $\{\ket{\psi_j}\}_{j=1}^r$ are sets of pure states. Since $\mathcal{N}$ is trace preserving, it holds that
		\begin{equation}
			\sum_{j=1}^r K_j^\dagger K_j=\sum_{j=1}^r \ket{\psi_j}\!\braket{\phi_j}{\phi_j}\!\bra{\psi_j}=\sum_{j=1}^r\ket{\psi_j}\!\bra{\psi_j}=\mathbbm{1}.
		\end{equation}
		This implies that $\{\ket{\psi_j}\!\bra{\psi_j}\}_{j=1}^r$ is a POVM. Therefore, defining the alphabet $\mathcal{X}=\{1,2,\dotsc,r\}$, the POVM elements $M_x\coloneqq \ket{\psi_x}\!\bra{\psi_x}$ and states $\sigma^x\coloneqq\ket{\phi_x}\!\bra{\phi_x}$, we have that
		\begin{equation}
			\mathcal{N}(\rho)=\sum_{x\in\mathcal{X}}\Tr[M_x\rho] \sigma^x,
		\end{equation}
		as required.
	\end{Proof}
	
	An extreme example of a measure-and-prepare channel, as in \eqref{eq-meas_reprep_map_2}, is one in which the output is a fixed state $\sigma$ for every outcome of the measurement described by the POVM $\{M_x\}_{x\in\mathcal{X}}$. In this case, the channel in \eqref{eq-meas_reprep_map_2} takes the form
	\begin{equation}
		\mathcal{N}(\rho)=\sum_{x\in\mathcal{X}}\Tr[M_x\rho]\sigma=\Tr[\rho]\sigma=\mathcal{R}^{\sigma}(\rho),
	\end{equation}
	where  the second equality follows because $\sum_{x\in\mathcal{X}}M_x=\mathbbm{1}$, and for the last equality we used the definition of the replacement channel for $\sigma$ in Definition~\ref{def-replace_channel}. This means that every replacement channel is a measure-and-prepare channel, and in particular an entanglement-breaking channel.
	
	The development above Proposition~\ref{prop-ent_break_Kraus} tells us that to every entanglement breaking channel there is associated a separable state, namely, the Choi state. Conversely, given a separable state $\rho_{AB}=\sum_{x\in\mathcal{X}}p(x)\omega_A^x\otimes\tau_B^x$, the channel $\mathcal{N}_{A\to B}^{\rho}$ defined in \eqref{eq-state_to_channel} has the form
	\begin{equation}
		\mathcal{N}_{A\to B}^{\rho}(X_A)=\sum_{x\in\mathcal{X}}\Tr[X_AM_A^x]\tau_B^x,
	\end{equation}
	where
	\begin{equation}
	M_A^x=p(x)\left(\rho_A^{-\frac{1}{2}}\omega_A^x\rho_A^{-\frac{1}{2}}\right)^{\t}
	\end{equation}
	 for all $x\in\mathcal{X}$. In other words, by Theorem~\ref{thm-ent_break_meas_reprepare}, every separable state can be associated with an entanglement-breaking channel.
		
	

\subsection{Hadamard Channels}\label{subsec-Hadamard_chan}

	It turns out that every entanglement-breaking channel can be regarded as the complement of what is called a \textit{Hadamard channel}, which we now define.
	
	\begin{definition}{Hadamard Channel}{def-Hadamard_chan}
		A channel $\mathcal{N}$ is called a \textit{Hadamard channel} or a \textit{Schur channel} if there exists a positive semi-definite operator $N$ with unit diagonal elements (in the standard basis) and an isometry $V$ such that
		\begin{equation}\label{eq-Hadamard_channel}
			\mathcal{N}(X)=N\ast VXV^\dagger
		\end{equation}
		for all linear operators $X$, where $N\ast VXV^\dagger$ is the \textit{Hadamard product}, also called the \textit{Schur product}, which is defined as the element-wise product of the operators $N$ and $VXV^\dagger$ when represented as matrices with respect to the standard basis.
	\end{definition}
	
	Given linear operators $X$ and $Y$ acting on a $d$-dimensional Hilbert space, with matrix representations in the standard basis as
	\begin{equation}
		X=\sum_{i,j=0}^{d-1} X_{i,j}\ket{i}\!\bra{j},\quad Y=\sum_{i,j=0}^{d-1} Y_{i,j}\ket{i}\!\bra{j},
	\end{equation}
	the Hadamard product $X\ast Y$ is the operator with matrix representation in the standard basis given by the product of the matrix elements of $X$ and $Y$:
	\begin{equation}\label{eq-Hadamard_product}
		X\ast Y=\sum_{i,j=0}^{d-1} X_{i,j}Y_{i,j}\ket{i}\!\bra{j}.
	\end{equation}
	Note that the Hadamard product can be defined as the element-wise product with respect to an arbitrary orthonormal basis; however, in this book, we only consider the Hadamard product with respect to the standard basis.
	%It can be shown that a Hadamard channel $\mathcal{N}$ is completely positive if and only if its corresponding operator $N$ is positive semi-definite.
	
	The positive semi-definiteness of $N$ in the definition of a Hadamard channel is necessary and sufficient for the map $\mathcal{N}$ defined in \eqref{eq-Hadamard_channel} to be completely positive, while the fact that $N$ has unit diagonal elements in the standard basis and that $V$ is an isometry ensures that $\mathcal{N}$ is trace preserving.
	
%\begin{comment}
%	Given a Hadamard channel $\mathcal{N}$ on a $d$-dimensional system with associated operator $N$, its Choi representation is
%	\begin{equation}\label{eq-Hadamard_Choi}
%		C(\mathcal{N})=\sum_{i,i'=1}^d \ket{i}\!\bra{i'}\otimes\mathcal{N}(\ket{i}\!\bra{i'})=\sum_{i,i'=1}^d N_{i,i'}\ket{i,i}\!\bra{i',i'}=WNW^\dagger,
%	\end{equation}
%	where we have used the fact that $\mathcal{N}(\ket{i}\!\bra{i'})=N\ast\ket{i}\!\bra{i'}=N_{i,i'}\ket{i}\!\bra{i'}$, and
%	\begin{equation}
%		W\coloneqq \sum_{i=0}^{d-1}\ket{i,i}\!\bra{i}.
%	\end{equation}
%\end{comment}
	
	The following fact about complements of Hadamard channels provides an important characterization of Hadamard channels:
		
	\begin{proposition}{prop-Hadamard_chan_comp}%\label{prop-Hadamard_chan_comp}
		Any complement of a Hadamard channel is entanglement breaking.
	\end{proposition}
	
	\begin{Proof}
		Suppose $\mathcal{N}_{A\to B}$ is a Hadamard channel between $d$-dimensional systems $A$ and $B$ with associated positive semi-definite operator $N$ having unit diagonal elements in the standard basis and with associated isometry $V$. Since $N$ is positive semi-definite and it has unit diagonal elements, it can be expressed as the Gram matrix of some set $\{\ket{\psi_i}:1\leq i\leq d\}$ of normalized vectors, so that
		\begin{equation}
			N=\sum_{i,j=0}^{d-1} \braket{\psi_i}{\psi_j}\ket{i}\!\bra{j}.
		\end{equation}
		Therefore, using \eqref{eq-Hadamard_product} and Definition~\ref{def-Hadamard_chan}, the action of $\mathcal{N}$ can be written as
		\begin{equation}
			\mathcal{N}(X)=\sum_{i,j=0}^{d-1} \braket{\psi_i}{\psi_j}\!\bra{i}VXV^\dagger\ket{j}\ket{i}\!\bra{j}_B.
		\end{equation}
		Now, set
		\begin{equation}
			\ket{\phi_i}\coloneqq V^\dagger\ket{i}\Rightarrow \bra{\phi_i}=\bra{i}V,
		\end{equation}
		so that
		\begin{equation}
			\mathcal{N}(X)=\sum_{i,j=0}^{d-1}\braket{\psi_i}{\psi_j}\!\bra{\phi_i}X\ket{\phi_j}\ket{i}\!\bra{j}_B.
		\end{equation}
		Consider the operator $(U^{\mathcal{N}})_{A\to BE}$ defined as
		\begin{equation}\label{eq-Hadamard_chan_iso_ext}
			U^{\mathcal{N}}\coloneqq \sum_{i=0}^{d-1} \ket{i}_B\bra{\phi_i}_A\otimes\ket{\psi_i}_E.
		\end{equation}
		Since $V$ is an isometry, and the vectors $\{\ket{\psi_i}:1\leq i\leq d\}$ are normalized, it follows that
		\begin{equation}
			(U^{\mathcal{N}})^\dagger U^{\mathcal{N}}=\sum_{i=0}^{d-1} \ket{\phi_i}\!\bra{\phi_i}=\sum_{i=0}^{d-1} V^\dagger\ket{i}\!\bra{i}V=V^\dagger V=\mathbbm{1}.
		\end{equation}
		This means that $U^{\mathcal{N}}$ is an isometry. Furthermore,
		\begin{equation}\label{eq-Hadamard_comp_pf}
			U^{\mathcal{N}} X (U^{\mathcal{N}})^\dagger =\sum_{i,j=0}^{d-1} \bra{\phi_i}X\ket{\phi_j}\ket{\psi_i}\!\bra{\psi_j}_E\otimes\ket{i}\!\bra{j}_B,
		\end{equation}
		so that $\Tr_E[U^{\mathcal{N}}X(U^{\mathcal{N}})^\dagger]=\mathcal{N}(X)$. The operator $U^{\mathcal{N}}$ is therefore an isometric extension of $\mathcal{N}$. A complementary channel then results from tracing out $B$ in \eqref{eq-Hadamard_comp_pf}, i.e.,
		\begin{align}
			\mathcal{N}^c(X)&=\Tr_B[U^{\mathcal{N}}X(U^{\mathcal{N}})^\dagger]\\
			&=\sum_{i=0}^{d-1} \bra{\phi_i}X\ket{\phi_i}\ket{\psi_i}\!\bra{\psi_i}_E\\
			&=\sum_{i=0}^{d-1} \ket{\psi_i}\!\bra{\phi_i}X\ket{\phi_i}\!\bra{\psi_i}\\
			&=\sum_{i=0}^{d-1} K_i X K_i^\dagger,
		\end{align}
		where $K_i\coloneqq \ket{\psi_i}\!\bra{\phi_i}$. So $\mathcal{N}^c$ has a Kraus representation with unit-rank Kraus operators, which means, by Proposition \ref{prop-ent_break_Kraus}, that $\mathcal{N}^c$ is entanglement breaking. Every complement of a channel is related to another complement by an isometric channel acting on the output of the complement, and this does not change the entanglement-breaking property. 
	\end{Proof}
	
	By following the proof above  backwards, we find that every entangle\-ment-breaking channel is the complement of some Hadamard channel.
	

\subsection{Petz Recovery Map}\label{subsec-Petz_channel}

	The following channel plays an important role in variations of the data-processing inequality for the quantum relative entropy and other entropic quantities that we define in the next chapter.
	
	\begin{definition}{Petz Recovery Map}{def-Petz_recovery}
		Let $\sigma\in\Lin(\mathcal{H})$ be a positive semi-definite operator and let $\mathcal{N}:\Lin(\mathcal{H})\to\Lin(\mathcal{H}')$ be a quantum channel. The \textit{Petz recovery map for $\sigma$ and $\mathcal{N}$} is the completely positive and trace-non-increasing map $\mathcal{P}_{\sigma,\mathcal{N}}:\Lin(\mathcal{H}')\to\Lin(\mathcal{H'})$ defined as
		\begin{equation}\label{eq-Petz_chan_def}
			\mathcal{P}_{\sigma,\mathcal{N}}(X)\coloneqq\sigma^{\frac{1}{2}}\mathcal{N}^\dagger\!\left(\mathcal{N}(\sigma)^{-\frac{1}{2}}X\mathcal{N}(\sigma)^{-\frac{1}{2}}\right)\sigma^{\frac{1}{2}}
		\end{equation}
		for all $X\in\Lin(\mathcal{H}')$.
	\end{definition}
	
	\begin{remark}
		If the operator $\mathcal{N}(\sigma)$ is invertible, then the Petz recovery map $\mathcal{P}_{\sigma,\mathcal{N}}$ is a channel. If the operator $\mathcal{N}(\sigma)$ is not invertible, then  the inverse $\mathcal{N}(\sigma)^{-\frac{1}{2}}$ is taken on the support on $\mathcal{N}(\sigma)$, following the convention from Section~\ref{sec:math-tools:functions-herm-ops}. In this latter case, the Petz recovery map $\mathcal{P}_{\sigma,\mathcal{N}}$ is a trace non-increasing map. %The action of $\mathcal{P}_{\sigma,\mathcal{N}}$ as per \eqref{eq-Petz_chan_def} then only holds when the input $X$ is on the support of $\mathcal{N}(\sigma)$.
	\end{remark}
	
	The Petz recovery map is indeed completely positive because it is the composition of the following completely positive maps:
	\begin{enumerate}
		\item Sandwiching by the positive semi-definite operator $\mathcal{N}(\sigma)^{-\frac{1}{2}}$.
		\item The adjoint $\mathcal{N}^\dagger$ of $\mathcal{N}$.
		\item Sandwiching by the positive semi-definite operator $\sigma^{\frac{1}{2}}$. 
	\end{enumerate}
	The Petz recovery map is also trace non-increasing, as we can readily verify. For all positive semi-definite operators $X$, the following holds
	\begin{align}
		\Tr[\mathcal{P}_{\sigma,\mathcal{N}}(X)]&=\Tr\!\left[\sigma^{\frac{1}{2}}\mathcal{N}^\dagger\!\left(\mathcal{N}(\sigma)^{-\frac{1}{2}}X\mathcal{N}(\sigma)^{-\frac{1}{2}}\right)\sigma^{\frac{1}{2}}\right]\\
		&=\Tr\!\left[\sigma\mathcal{N}^\dagger\!\left(\mathcal{N}(\sigma)^{-\frac{1}{2}}X\mathcal{N}(\sigma)^{-\frac{1}{2}}\right)\right]\\
		&=\Tr\!\left[\mathcal{N}(\sigma)\mathcal{N}(\sigma)^{-\frac{1}{2}}X\mathcal{N}(\sigma)^{-\frac{1}{2}}\right]\\
		&=\Tr\!\left[\mathcal{N}(\sigma)^{-\frac{1}{2}}\mathcal{N}(\sigma)\mathcal{N}(\sigma)^{-\frac{1}{2}}X\right]\\
		&=\Tr[\Pi_{\mathcal{N}(\sigma)}X]\\
		&\leq\Tr[X],
	\end{align}
	where $\Pi_{\mathcal{N}(\sigma)}$ is the projection onto the support of $\mathcal{N}(\sigma)$, which arises because $\mathcal{N}(\sigma)$ need not be invertible. If $X$ is contained in the support of $\mathcal{N}(\sigma)$, then $\Tr[\Pi_{\mathcal{N}(\sigma)}X]=\Tr[X]$, which means that the Petz recovery channel is trace-preserving for all inputs with support contained in the support of $\mathcal{N}(\sigma)$.
	
	One of the important properties of the Petz recovery channel $\mathcal{P}_{\sigma,\mathcal{N}}$ is that it reverses the action of $\mathcal{N}$ on $\sigma$ whenever $\mathcal{N}(\sigma)$ is invertible. In particular,
	\begin{align}
		\mathcal{P}_{\sigma,\mathcal{N}}(\mathcal{N}(\sigma))&=\sigma^{\frac{1}{2}}\mathcal{N}^\dagger\!\left(\mathcal{N}(\sigma)^{-\frac{1}{2}}\mathcal{N}(\sigma)\mathcal{N}(\sigma)^{-\frac{1}{2}}\right)\sigma^{\frac{1}{2}}\\
		&=\sigma^{\frac{1}{2}}\mathcal{N}^\dagger(\mathbbm{1}_{\mathcal{H}'})\sigma^{\frac{1}{2}}\\
		&=\sigma,\label{eq-Petz_recovery_sigma}
	\end{align}
	where we have used the fact that $\mathcal{N}(\sigma)$ is invertible, so that
	\begin{equation}
		\mathcal{N}(\sigma)^{-\frac{1}{2}}\mathcal{N}(\sigma)\mathcal{N}(\sigma)^{-\frac{1}{2}}=\mathbbm{1}_{\mathcal{H}'}.
	\end{equation}
	Then, since $\mathcal{N}$ is a channel, its adjoint is unital, which leads to the final equality.
	
	\begin{remark}
		The equality in \eqref{eq-Petz_recovery_sigma} holds more generally; i.e., it holds even when $\mathcal{N}(\sigma)$ is not invertible. To see this, we use the fact that the projection $\Pi_{\mathcal{N}(\sigma)}$ onto the support of $\mathcal{N}(\sigma)$ satisfies $\Pi_{\mathcal{N}(\sigma)}\leq\mathbbm{1}_{\mathcal{H}'}$. Then, we find that
		\begin{align}
			\mathcal{P}_{\sigma,\mathcal{N}}(\mathcal{N}(\sigma))&=\sigma^{\frac{1}{2}}\mathcal{N}^\dagger\!\left(\mathcal{N}(\sigma)^{-\frac{1}{2}}\mathcal{N}(\sigma)\mathcal{N}(\sigma)^{-\frac{1}{2}}\right)\sigma^{\frac{1}{2}}\\
			&=\sigma^{\frac{1}{2}}\mathcal{N}^\dagger(\Pi_{\mathcal{N}(\sigma)})\sigma^{\frac{1}{2}}\\
			&\leq\sigma^{\frac{1}{2}}\mathcal{N}^\dagger(\mathbbm{1}_{\mathcal{H}'})\sigma^{\frac{1}{2}}\\
			&=\sigma.
		\end{align}
		On the other hand, if we let $U:\mathcal{H}\to\mathcal{H}'\otimes\mathcal{H}_E$ be an isometric extension of $\mathcal{N}$, then we can use Lemma~\ref{lem-app:support-1} from Appendix~\ref{app:QM-over:support-lemmas}, which implies that $\supp(U\sigma U^\dagger) \subseteq\supp(\mathcal{N}(\sigma)\otimes\mathbbm{1}_E)$, and in turn implies that $\Pi_{U\sigma U^\dagger}\leq\Pi_{\mathcal{N}(\sigma)\otimes\mathbbm{1}_E}$. Then, for every vector $\ket{\psi}\in\mathcal{H}$, we obtain
		\begin{align}
			\bra{\psi}\Pi_{\sigma}\ket{\psi}&=\bra{\psi}U^\dagger\Pi_{U\sigma U^\dagger}U\ket{\psi}\\
			&\leq \bra{\psi}U^\dagger(\Pi_{\mathcal{N}(\sigma)}\otimes\mathbbm{1}_E)U\ket{\psi}\\
			&=\Tr[U\ket{\psi}\!\bra{\psi}U^\dagger(\Pi_{\mathcal{N}(\sigma)}\otimes\mathbbm{1}_E)]\\
			&=\Tr[\Tr_E[U\ket{\psi}\!\bra{\psi}U^\dagger]\Pi_{\mathcal{N}(\sigma)}]\\
			&=\Tr[\mathcal{N}(\ket{\psi}\!\bra{\psi})\Pi_{\mathcal{N}(\sigma)}]\\
			&=\Tr[\ket{\psi}\!\bra{\psi}\mathcal{N}^\dagger(\Pi_{\mathcal{N}(\sigma)})]\\
			&=\bra{\psi}\mathcal{N}^\dagger(\Pi_{\mathcal{N}(\sigma)})\ket{\psi}.
		\end{align}
		Since $\ket{\psi}$ is arbitrary, it holds that $\Pi_\sigma\leq\mathcal{N}^\dagger(\Pi_{\mathcal{N}(\sigma)})$. Using this, we find that
		\begin{equation}
			\mathcal{P}_{\sigma,\mathcal{N}}(\mathcal{N}(\sigma))=\sigma^{\frac{1}{2}}\mathcal{N}^\dagger(\Pi_{\mathcal{N}(\sigma)})\sigma^{\frac{1}{2}}\geq\sigma^{\frac{1}{2}}\Pi_\sigma\sigma^{\frac{1}{2}}=\sigma.
		\end{equation}
		Having shown that $\mathcal{P}_{\sigma,\mathcal{N}}(\mathcal{N}(\sigma))\leq\sigma$ and $\mathcal{P}_{\sigma,\mathcal{N}}(\mathcal{N}(\sigma))\geq \sigma$, we conclude that
		\begin{equation}
			\mathcal{P}_{\sigma,\mathcal{N}}(\mathcal{N}(\sigma))=\sigma,
		\end{equation}
		even when $\mathcal{N}(\sigma)$ is not invertible.
	\end{remark}


\subsubsection{Petz Recovery Channel for Partial Trace}

\label{sec:petz-recovery-partial-trace}

	Let the input Hilbert space to the channel $\mathcal{N}$ in the definition of the Petz recovery map be $\mathcal{H}=\mathcal{H}_{AB}$. Then, let $\mathcal{N}=\Tr_B$ be the partial trace over $B$, and note that
	\begin{equation}
		\mathcal{N}^\dagger(\sigma_B)=\sigma_A\otimes\mathbbm{1}_B.
	\end{equation}
	Indeed, using the definition of the adjoint of a superoperator, we have
	\begin{align}
		\langle\mathcal{N}^\dagger(\sigma_A),\sigma_{AB}\rangle&=\inner{\sigma_A\otimes\mathbbm{1}_B}{\sigma_{AB}}\\
		&=\Tr[(\sigma_A\otimes\mathbbm{1}_B)^\dagger\sigma_{AB}]\\
		&=\Tr[\sigma_A^\dagger\Tr_B(\sigma_{AB})]\\
		&=\inner{\sigma_A}{\mathcal{N}(\sigma_{AB})}.
	\end{align}
	Therefore, the Petz recovery map corresponding to the partial trace over $B$ is
	\begin{equation}\label{eq-Petz_channel_partrace}
		\mathcal{P}_{\sigma_{AB},\Tr_B}(X_A)=\sigma_{AB}^{\frac{1}{2}}\left(\sigma_A^{-\frac{1}{2}}X_A\sigma_A^{-\frac{1}{2}}\otimes\mathbbm{1}_B\right)\sigma_{AB}^{\frac{1}{2}}.
	\end{equation}
	By writing the identity on $B$ as $\mathbbm{1}_B=\sum_{j=0}^{d_B-1}\ket{j}\!\bra{j}_B$, we can write the action $\mathcal{P}_{\sigma_{AB},\Tr_B}$ as
	\begin{align}
		\mathcal{P}_{\sigma_{AB},\Tr_B}(X_A)&=\sigma_{AB}^{\frac{1}{2}}\left(\sigma_A^{-\frac{1}{2}}X_A\sigma_A^{-\frac{1}{2}}\otimes\mathbbm{1}_B\right)\sigma_{AB}^{\frac{1}{2}}\\
		&=\sum_{j=0}^{d_B-1}\sigma_{AB}^{\frac{1}{2}}\left(\sigma_A^{-\frac{1}{2}}X_A\sigma_A^{-\frac{1}{2}}\otimes\ket{j}\!\bra{j}_B\right)\sigma_{AB}^{\frac{1}{2}}\\
		&=\sum_{j=0}^{d_B-1}\sigma_{AB}^{\frac{1}{2}}\left(\sigma_A^{-\frac{1}{2}}\otimes\ket{j}_B\right)X_A\left(\sigma_A^{-\frac{1}{2}}\otimes\bra{j}_B\right)\sigma_{AB}^{\frac{1}{2}}\\
		&=\sum_{j=0}^{d_B-1} K_jX_A K_j^\dagger,
	\end{align}
	where
	\begin{equation}
		K_j\coloneqq \sigma_{AB}^{\frac{1}{2}}\left(\sigma_A^{-\frac{1}{2}}\otimes\ket{j}_B\right).
	\end{equation}
	The operators $K_j$, for $0\leq j\leq d_B-1$, are thus Kraus operators for the Petz recovery map for the partial trace. Using \eqref{eq-Kraus_to_Stinespring}, and letting the environment $E$ be denoted by $\hat{B}$ (since the dimension of the environment in the construction \eqref{eq-Kraus_to_Stinespring} is the same as the number of Kraus operators, which in this case is equal to the dimension of $B$), we find that
	\begin{align}
		V_{A\to B\hat{B}} &= \sum_{j=0}^{d_B-1}\sigma_{AB}^{\frac{1}{2}}(\sigma_A^{-\frac{1}{2}}\otimes\ket{j}_B)\otimes\ket{j}_{\hat{B}}\\
		&=\sum_{j=0}^{d_B-1}\sigma_{AB}^{\frac{1}{2}}(\sigma_A^{-\frac{1}{2}}\otimes\ket{j}_B\otimes\ket{j}_{\hat{B}})\\
		&=(\sigma_{AB}^{\frac{1}{2}}\otimes\mathbbm{1}_{\hat{B}})(\sigma_A^{-\frac{1}{2}}\otimes\mathbbm{1}_B\otimes\mathbbm{1}_{\hat{B}})\left(\mathbbm{1}_A\otimes\sum_{j=0}^{d_B-1}\ket{j,j}_{B\hat{B}}\right)\\
		&= (\sigma_{AB}^{\frac{1}{2}}\otimes\mathbbm{1}_{\hat{B}})(\sigma_A^{-\frac{1}{2}}\otimes\mathbbm{1}_{B\hat{B}})(\mathbbm{1}_A\otimes\ket{\Gamma}_{B\hat{B}}),\label{eq-Petz_PT_iso_ext}
	\end{align}
	which is an isometric extension of the Petz recovery map $\mathcal{P}_{\sigma_{AB},\Tr_B}$. Omitting identity operators, this can be written more simply as follows:
	\begin{equation}
	V_{A\to B\hat{B}} = \sigma_{AB}^{\frac{1}{2}}\sigma_A^{-\frac{1}{2}}\ket{\Gamma}_{B\hat{B}}.
	\end{equation}



\subsection{LOCC Channels}

\label{subsec-LOCC_channels}
	
	A very common physical scenario encountered in quantum information theory is one in which two parties, Alice and Bob, who are distantly separated, perform local quantum operations (consisting of channels and/or measurements) at their respective locations and communicate classically with each other in order to transform some initially shared state to some final desired state. This sequence of \textit{local operations and classical communication} is abbreviated \textit{LOCC} and is an important element of many quantum communication protocols, such as entanglement distillation and secret key distillation.
	
	As with every other transformation in quantum theory, an LOCC operation corresponds mathematically to a channel, which we call an \textit{LOCC channel}. Formally, an LOCC channel is defined as follows:
	
	\begin{definition}{LOCC Channel}{def-LOCC}
		Let $\mathcal{X}$ be a finite alphabet, let $\{\mathcal{M}^x\}_{x\in\mathcal{X}}$ be a quantum instrument (a set of completely positive trace-non-increasing maps such that $\sum_{x\in\mathcal{X}}\mathcal{M}^x$ is a channel), and let $\{\mathcal{N}^x\}_{x\in\mathcal{X}}$ be a set of quantum channels. Then, a \textit{one-way LOCC channel from Alice to Bob} is the channel $\mathcal{L}_{AB\to A'B'}^{\rightarrow}$ from Alice's initial and final systems $A$ and $A'$ to Bob's initial and final systems $B$ and $B'$, defined as
		\begin{equation}\label{eq-LOCC_A_to_B}
			\mathcal{L}_{AB\to A'B'}^{\rightarrow}=\sum_{x\in\mathcal{X}}\mathcal{M}_{A\to A'}^x\otimes\mathcal{N}_{B\to B'}^x.
		\end{equation}
		
		A \textit{one-way LOCC channel from Bob to Alice} is the channel $\mathcal{L}_{AB\to A'B'}^{\leftarrow}$ defined as
		\begin{equation}
			\mathcal{L}_{AB\to A'B'}^{\leftarrow}=\sum_{x\in\mathcal{X}}\mathcal{N}_{A\to A'}^x\otimes\mathcal{M}_{B\to B'}^x.
			\label{eq-QM:one-way-LOCC-from-B-to-A}
		\end{equation}
		
		An \textit{LOCC channel} is a composition of a finite, but arbitrarily large number of one-way LOCC channels from Alice to Bob and from Bob to Alice and can be written as
		\begin{equation}
		\label{eq-LOCC_chan_gen}
			\mathcal{L}_{AB\to A'B'}^{\leftrightarrow}=\sum_{y\in\mathcal{Y}}\mathcal{S}_A^y\otimes\mathcal{W}_B^y
		\end{equation}
		for some finite alphabet $\mathcal{Y}$ and sets $\{\mathcal{S}^y\}_{y\in\mathcal{Y}}$, $\{\mathcal{W}^y\}_{y\in\mathcal{Y}}$ of completely positive trace-non-increasing maps such that $\sum_{y\in\mathcal{Y}}\mathcal{S}^y\otimes\mathcal{W}^y$ is trace preserving.
	\end{definition}
	
	Consider the one-way LOCC channel $\mathcal{L}_{AB\to A'B'}^{\rightarrow}$ from Alice to Bob defined as in \eqref{eq-LOCC_A_to_B}. The values $x\in\mathcal{X}$ form the possible messages that might be communicated from Alice to Bob and constitute the ``classical communication'' part of LOCC. The set $\{\mathcal{M}^x\}_{x\in\mathcal{X}}$ of completely positive trace-non-increasing maps and the set $\{\mathcal{N}^x\}_{x\in\mathcal{X}}$ of quantum channels specify the actions of Alice and Bob for each value $x\in\mathcal{X}$ and constitute the ``local operations'' part of LOCC. The set $\{\mathcal{M}^x\}_{x\in\mathcal{X}}$ of completely positive trace-non-increasing maps that sum to a channel essentially specifies a quantum instrument. The operations corresponding to these maps can thus be considered probabilisitic since the maps are not trace preserving. In general, the party that performs the quantum instrument determines the direction of classical communication and thus the direction of the LOCC channel. In this case, Alice performs the classical communication since she performs the quantum instrument. The values $x$ specify the outcomes of the instrument, and Alice communicates the outcome to Bob, who performs the corresponding channel selected from his set $\{\mathcal{N}^x\}_{x\in\mathcal{X}}$ of channels.
	
	In more detail, let $\rho_{AB}$ be the initial state shared by Alice and Bob. Using the definition in \eqref{eq-instrument_output} for the channel corresponding to the quantum instrument $\{\mathcal{M}^x\}_{x\in\mathcal{X}}$, the state after applying the quantum instrument is
	\begin{equation}\label{eq-1wayLOCC_step1}
		\sum_{x\in\mathcal{X}}\mathcal{M}_{A\to A'}^x(\rho_{AB})\otimes\ket{x}\!\bra{x}_{X_A},
	\end{equation}
	where the system $X_A$ stores the classical information corresponding to the outcome of the instrument. Alice then communicates the outcome of the instrument to Bob. This classical communication can be understood via the noiseless classical channel from $X_A$ to $X_B$ defined by
	\begin{equation}\label{eq-classical_channel_action}
		\theta_{X_A}\mapsto \sum_{x\in\mathcal{X}}\!\bra{x}_{X_A}\theta_{X_A} \ket{x}_{X_A} \ket{x}\!\bra{x}_{X_B}.
	\end{equation}
	The state in \eqref{eq-1wayLOCC_step1} thus gets transformed to
	\begin{equation}
		\sum_{x\in\mathcal{X}}\mathcal{M}_{A\to A'}^x(\rho_{AB})\otimes\ket{x}\!\bra{x}_{X_B}.
	\end{equation}
	Finally, Bob applies the channel specified by
	\begin{equation}\label{eq-1wayLOCC_last_step}
		\tau_B\otimes\omega_{X_B}\mapsto \sum_{x\in\mathcal{X}}\mathcal{N}_{B\to B'}^x(\tau_B)\otimes \bra{x}_{X_B}\omega_{X_B}\ket{x}_{X_B},
	\end{equation}
	which corresponds to Bob measuring his system $X_B$ in the basis $\{\ket{x}_{X_B}\}_{x\in\mathcal{X}}$ and applying a quantum channel from the set $\{\mathcal{N}_{B\to B'}^x\}_{x\in\mathcal{X}}$ to the system $B$ based on the outcome. The final state is then
	\begin{equation}
		\sum_{x\in\mathcal{X}}(\mathcal{M}_{A\to A'}^x\otimes\mathcal{N}_{B\to B'}^x)(\rho_{AB}),
	\end{equation}
	which is precisely the output of the one-way LOCC channel $\mathcal{L}_{AB\to A'B'}^{\rightarrow}$ defined in \eqref{eq-LOCC_A_to_B}. We can succinctly write the steps in \eqref{eq-1wayLOCC_step1}--\eqref{eq-1wayLOCC_last_step} as
	\begin{equation}\label{eq-1wayLOCC_decomp}
		\mathcal{L}_{AB\to A'B'}(\rho_{AB})=(\mathcal{N}_{X_B B\to B'}\circ\mathcal{C}_{X_A \to X_B}\circ\mathcal{M}_{A\to A'X_A})(\rho_{AB}),
	\end{equation}
	where the channel $\mathcal{M}_{A\to A'X_A}$ is defined as
	\begin{equation}
		\mathcal{M}_{A\to A'X_A}(\xi_A)\coloneqq\sum_{x\in\mathcal{X}}\mathcal{M}_{A\to A'}^x(\xi_A)\otimes\ket{x}\!\bra{x}_{X_A},
	\end{equation}
	and the channel $\mathcal{N}_{B X_B\to B'}$ is defined as
	\begin{equation}
		\mathcal{N}_{B X_B\to B'}(\tau_B\otimes\ket{x}\!\bra{x}_{X_B})\coloneqq \mathcal{N}_{B\to B'}^x(\tau_B)
	\end{equation}
	for all $x\in\mathcal{X}$. As indicated above, the channel $\mathcal{C}_{X_A\to X_B}$, defined in \eqref{eq-classical_channel_action}, is a noiseless classical channel that transforms the classical register $X_A$, held by Alice, to the classical register $X_B$ (which is simply a copy of $X$), held by Bob.
	
	\begin{figure}
		\centering
		\includegraphics[scale=0.65]{Figures/LOCC.pdf}
		\caption{Illustration of an LOCC channel with $k$ rounds of alternating one-way LOCC channels from Alice to Bob and from Bob to Alice. In each round $i$, there is a finite alphabet $\mathcal{X}_i$, a set $\{\mathcal{M}_i^x\}_{x\in\mathcal{X}_i}$ of completely positive trace-non-increasing maps that sum to a channel, and a set $\{\mathcal{N}_i^x\}_{x\in\mathcal{X}_i}$ of quantum channels.}\label{fig-LOCC}
	\end{figure}
	
	An example of an LOCC channel is illustrated in Figure \ref{fig-LOCC}. This is an LOCC channel consisting of $k$ rounds of alternating Alice-to-Bob and Bob-to-Alice one-way LOCC channels and is of the form
	\begin{equation}
		\begin{aligned}
		\mathcal{L}_{A_0B_0\to A_kB_k}^{\leftrightarrow}=\mathcal{L}_{A_{k-1}B_{k-1}\to A_kB_k}^{k,\rightarrow}&\circ\mathcal{L}_{A_{k-2}B_{k-2}\to A_{k-1}B_{k-1}}^{k-1,\leftarrow}\circ\dotsb\\
		&\qquad\circ\mathcal{L}_{A_1B_1\to A_2B_2}^{2,\leftarrow}\circ\mathcal{L}_{A_0B_0\to A_1B_1}^{1,\rightarrow}.
		\end{aligned}
	\end{equation}
	For each round $i$, there is a finite alphabet $\mathcal{X}_i$ consisting of the messages communicated in the round, along with a set $\{\mathcal{M}_i^x\}_{x\in\mathcal{X}_i}$ of completely positive trace-non-increasing maps that sum to a quantum channel and a set $\{\mathcal{N}_i^x\}_{x\in\mathcal{X}_i}$ of quantum channels. In a multi-round LOCC channel such as this one, it possible for the operation sets $\{\mathcal{M}_i^x\}_{x\in\mathcal{X}_i}$ and $\{\mathcal{N}_i^x\}_{x\in\mathcal{X}_i}$ on the $i$th round to depend on the outcomes and actions taken in previous rounds. The quantum teleportation protocol in Section \ref{sec-teleportation} below provides a concrete example of a one-way LOCC protocol from Alice to Bob.

	 \begin{definition}{Separable Channel}{def:QM-over:separable-channel}
	 A \textit{separable channel}  is a quantum channel $\mathcal{S}_{AB\to A'B'}$ such that
	\begin{equation}
	\label{eq-separable_map}
		\mathcal{S}_{AB\to A'B'}=\sum_{x\in\mathcal{X}}\mathcal{C}_{A\to A'}^x\otimes\mathcal{D}_{B\to B'}^x
	\end{equation}
	for some finite alphabet $\mathcal{X}$ and sets of completely positive and trace-non-increasing maps $\{\mathcal{C}^x\}_{x\in\mathcal{X}}$ and $\{\mathcal{D}^x\}_{x\in\mathcal{X}}$ such that $\mathcal{S}$ is trace preserving.
	\end{definition}
	
	Every separable channel has a set of Kraus operators in product form; i.e., for every separable channel $\mathcal{S}_{AB\to A'B'}$ as in \eqref{eq-separable_map} there exists a finite alphabet $\mathcal{Y}$ and sets $\{C^y_{A\to A'}\}_{y\in\mathcal{Y}}$ and $\{D^y_{B\to B'}\}_{y\in\mathcal{Y}}$ such that
	\begin{equation}
		\mathcal{S}_{AB\to A'B'}(\rho_{AB})=\sum_{y\in\mathcal{Y}} (C^y_{A\to A'}\otimes D^y_{B\to B'})\rho_{AB}(C^y_{A\to A'}\otimes D^y_{B\to B'})^\dagger
		\label{eq:QM-over:kraus-form-sep-ch}
	\end{equation}
	for all $\rho_{AB}$.
	
	
	
	A key property of a separable channel is that it outputs a separable state if the input state is separable. To see this, consider the separable state $\sigma_{AB} = \sum_{z\in \mathcal{Z}} p(z) \tau^z_A \otimes \omega^z_B$. Then the output state $\mathcal{S}_{AB\to A'B'}(\sigma_{AB})$ is given by
	\begin{align}
	& \mathcal{S}_{AB\to A'B'}(\sigma_{AB}) \notag \\& = \sum_{y\in\mathcal{Y}} (C^y_{A\to A'}\otimes D^y_{B\to B'})
	\left(\sum_{z\in \mathcal{Z}} p(z) \tau^z_A \otimes \omega^z_B\right)(C^y_{A\to A'}\otimes D^y_{B\to B'})^\dagger
		 \label{eq:QM-over:sep-preserves-sep-1}
		 \\
	& = \sum_{y\in\mathcal{Y},z\in \mathcal{Z}} p(z) C^y_{A\to A'} 
	 \tau^z_A (C^y_{A\to A'})^\dagger \otimes D^y_{B\to B'} \omega^z_B (D^y_{B\to B'})^\dagger,
	 \label{eq:QM-over:sep-preserves-sep-2}
	\end{align}
	and is manifestly separable.
	
	\begin{proposition*}{LOCC Channels are Separable Channels}{prop:QM-over:sep-ch-contains-LOCC}
	From \eqref{eq-LOCC_chan_gen} and \eqref{eq-separable_map}, we conclude that every LOCC channel is a separable channel.
	\end{proposition*}
	
	 The converse of Proposition~\ref{prop:QM-over:sep-ch-contains-LOCC} is not true. For example, let us define the following operators:
	\begin{align}
		K_1&\coloneqq\frac{1}{\sqrt{2}}\ket{0}\!\bra{0}+\ket{1}\!\bra{1},\quad K_2\coloneqq\ket{0}\!\bra{0},\quad K_3\coloneqq\ket{1}\!\bra{1}.
	\end{align}
	Then, following the notation in \eqref{eq-separable_map}, let
	\begin{align}
		\mathcal{C}^1_{A\to A'}(\cdot)&=K_1(\cdot)K_1^\dagger,\\
		\mathcal{C}^2_{A\to A'}(\cdot)&=K_2(\cdot)K_2^\dagger,\\
		\mathcal{C}^3_{A\to A'}(\cdot)&=K_3(\cdot)K_3^\dagger,
	\end{align}
	and
	\begin{align}
		\mathcal{D}^1_{B\to B'}(\cdot)&=K_2(\cdot)K_2^\dagger,\\
		\mathcal{D}^2_{B\to B'}(\cdot)&=K_1(\cdot)K_1^\dagger,\\
		\mathcal{D}^3_{B\to B'}(\cdot)&=K_3(\cdot)K_3^\dagger.
	\end{align}
	Then, the map
	\begin{align}
		\mathcal{S}_{AB\to A'B'}(\cdot)&\coloneqq\sum_{x=1}^3 (\mathcal{C}_{A\to A'}^x\otimes\mathcal{D}_{B\to B'}^x)(\cdot)\\
		&=(K_1\otimes K_2)(\cdot)(K_1\otimes K_2)^\dagger+(K_2\otimes K_1)(\cdot)(K_2\otimes K_1)^\dagger\\
		&\qquad +(K_3\otimes K_3)(\cdot)(K_3\otimes K_3)^\dagger
	\end{align}
	is a separable channel, but it can be shown that it is not an LOCC channel; please consult the Bibliographic Notes in Section~\ref{sec:qm:bib-notes}.


\subsubsection{LOCC and Separable Simulation of Channels}

	Given a quantum channel $\mathcal{N}_{AB\to A'B'}$, an important question related to the physical realization of the channel is whether the channel is an LOCC channel. This amounts to determining whether the channel can be decomposed as in \eqref{eq-LOCC_chan_gen}. More generally, one can ask whether a given channel $\mathcal{N}_{A\to B}$ can be \textit{simulated} by an LOCC channel acting on the input and a resource state, a notion that is illustrated in Figure \ref{fig-LOCC_sim} and defined below.
	
	\begin{definition}{LOCC-Simulable Channel}{def-LOCC_sim_chan}
		A channel $\mathcal{N}_{A\to B}$ is called \textit{LOCC-simulable} with associated resource state $\omega_{RB'}$ if there exists an auxiliary system $R$ and an LOCC channel $\mathcal{L}^{\leftrightarrow}_{RAB'\to B}$ such that for every state $\rho_A$
		\begin{equation}
			\mathcal{N}(\rho_A)=\mathcal{L}^{\leftrightarrow}_{RAB'\to B}(\rho_A\otimes\omega_{RB'}).
		\end{equation}
		For the LOCC channel $\mathcal{L}^{\leftrightarrow}_{RAB'\to B}$, the input systems $RA$ are Alice's, the input system $B'$ is Bob's, Alice's output system is trivial, and Bob's output system is $B$.
	\end{definition}
	
	\begin{figure}
		\centering
		\includegraphics[scale=0.8]{Figures/LOCC_sim_gen.pdf}
		\caption{Depiction of an LOCC-simulable channel $\mathcal{N}_{A\to B}$ with associated resource state $\omega_{RB'}$. The channel $\mathcal{N}_{A\to B}$ can be realized via the LOCC channel $\mathcal{L}_{RAB'\to B}^{\leftrightarrow}$ and the resource state $\omega_{RB'}$, for some auxiliary system $R$. The LOCC channel $\mathcal{L}_{RAB'\to B}^{\leftrightarrow}$ could in principle consist of a sequence of several rounds of one-way LOCC channels, as depicted in Figure \ref{fig-LOCC}.}\label{fig-LOCC_sim}
	\end{figure}
	
	If a channel $\mathcal{N}_{A\to B}$ is LOCC-simulable with associated resource state $\omega_{RB'}$, it means that Alice and Bob, the sender and receiver of the channel, respectively, can execute an LOCC channel of the form as depicted in Figure \ref{fig-LOCC}, with the assistance of the auxiliary system $R$, such that the output on Bob's system at the end is $\mathcal{N}(\rho_A)$. The resource state $\omega_{RB'}$ is fixed, being such that the same resource state can be used for all input states $\rho_A$ on Alice's system. A concrete example of an LOCC simulation of a channel is shown in the context of quantum teleportation in Section~\ref{sec-teleportation} below. 

Due to the fact that separable channels strictly contain LOCC channels, it is sensible to generalize the notion of teleportation simulation even further to this case:
	\begin{definition}{Separable-Simulable Channel}{def-SEP_sim_chan}
		A channel $\mathcal{N}_{A\to B}$ is called \textit{separable-simulable} with associated resource state $\omega_{RB'}$ if there exists an auxiliary system $R$ and a separable channel $\mathcal{S}_{RAB'\to B}$ such that for every state $\rho_A$
		\begin{equation}
			\mathcal{N}(\rho_A)=\mathcal{S}_{RAB'\to B}(\rho_A\otimes\omega_{RB'}).
		\end{equation}
		For the separable channel $\mathcal{S}^{\leftrightarrow}_{RAB'\to B}$, the input systems $RA$ are Alice's, the input system $B'$ is Bob's, Alice's output system is trivial, and Bob's output system is $B$.
	\end{definition}



\subsection{Completely PPT-Preserving Channels}

\label{sec-QM:C-PPT-P-chs}

	In Definition \ref{def-PPT}, we introduced PPT states as bipartite states $\rho_{AB}$ such that the partial transpose $\T_B(\rho_{AB})$  is positive semi-definite. The class of channels that preserve PPT states are called \textit{completely PPT-preserving channels}, abbreviated as C-PPT-P channels, and we define them formally as follows.

	\begin{definition}{Completely PPT-Preserving Channel}{def-PPT_pres_chan}
		A channel $\mathcal{P}_{AB\to A'B'}$ is called \textit{completely PPT-preserving} if the map $\T_{B'}\circ\mathcal{P}_{AB\to A'B'}\circ\T_B$ is a channel.
	\end{definition}
	
	\begin{proposition}{prop:QM:C-PPT-P-preserves-PPT}
	Completely PPT-preserving channels preserve the set of PPT states.
	\end{proposition}
	
	\begin{Proof}
		Suppose that $\rho_{AB}$ is a PPT state and that $\mathcal{P}_{AB\to A'B'}$ is a completely PPT-preserving channel. If we take the partial transpose $\T_{B'}$ on the output state $\sigma_{A'B'}=\mathcal{P}_{AB\to A'B'}(\rho_{AB})$, then we find that
		\begin{align}
			\T_{B'}(\sigma_{A'B'})&=(\T_{B'}\circ\mathcal{P}_{AB\to A'B'})(\rho_{AB})\\
			&=(\T_B\circ\mathcal{P}_{AB\to A'B'}\circ\T_{B})(\T_B(\rho_{AB})).
		\end{align}
		Since $\mathcal{P}_{AB\to A'B'}$ is completely PPT-preserving, by definition $\T_{B'}\circ\mathcal{P}_{AB\to A'B'}\circ\T_B$ is completely positive. Since $\T_B(\rho_{AB})$ is positive, this implies that $\T_{B'}(\sigma_{A'B'})$ is positive, which means that the output state is a PPT state.
	\end{Proof}
	
	
	\begin{proposition}{prop-LOCC_PPT_preserving}
		Every separable channel is a completely PPT-preserving channel.
	\end{proposition}
	
	\begin{Proof}
		Let $\mathcal{S}_{AB\to A'B'}$ be a separable channel. By definition, it has the form
		\begin{equation}
			\mathcal{S}_{AB\to A'B'}=\sum_{x\in\mathcal{X}}\mathcal{R}^x_{A\to A'}\otimes\mathcal{W}_{B\to B'}^x,
		\end{equation}
		where $\mathcal{X}$ is a finite alphabet and $\{\mathcal{R}^x\}_{x\in\mathcal{X}}$ and $\{\mathcal{W}^x\}_{x\in\mathcal{X}}$ are sets of completely positive trace non-increasing maps such that $\sum_{x\in\mathcal{X}}\mathcal{R}^x \otimes \mathcal{W}^x$ is trace preserving. Then,
		\begin{equation}
			\T_{B'}\circ\mathcal{S}_{AB\to A'B'}\circ\T_B=\sum_{x\in\mathcal{X}}\mathcal{R}_{A\to A'}^x\otimes (\T_{B'}\circ\mathcal{W}^x_{B\to B'}\circ \T_B).
		\end{equation}
		By applying Lemma~\ref{lemma-transpose-CPTP} below, we conclude that the maps $\T_{B'}\circ\mathcal{W}_{B\to B'}^x\circ\T_B$ are completely positive for all $x\in\mathcal{X}$, which means that $\T_{B'}\circ\mathcal{S}_{AB\to A'B'}\circ\T_B$ is completely positive. Therefore,  $\mathcal{S}_{AB\to A'B'}$ is completely PPT-preserving.
	\end{Proof}
	
	As a consequence of Proposition~\ref{prop-LOCC_PPT_preserving}, it follows that every LOCC channel is a completely PPT-preserving channel, because every LOCC channel is a separable channel.
	

The next lemma applies to channels that do not have a bipartite structure, i.e., there is no input or output system for Alice.
	\begin{Lemma}{lemma-transpose-CPTP}
		Let $\mathcal{N}_{B\to B'}$ be a completely positive map. Then the map $ \T_{B'} \circ \mathcal{N}_{B\to B'} \circ \T_B$ is completely positive, and its Choi operator is given by the full transpose of the Choi operator for $\mathcal{N}_{B\to B'}$, i.e.,
		\begin{equation}
			\Gamma_{BB'}^{\T_{B'}\circ\mathcal{N}_{B\to B'}\circ\T_{B}}=\T(\Gamma_{BB'}^{\mathcal{N}}).
		\end{equation}
	\end{Lemma}
	
	\begin{Proof}
		Let $\Gamma_{B\hat{B}}=\ket{\Gamma}\!\bra{\Gamma}_{B\hat{B}}$, where $\ket{\Gamma}$ is defined in \eqref{eq-max_ent_vector} and $d_{\hat{B}}=d_B$. Observe that $\T_B(\Gamma_{\hat{B}B}) = \T_{\hat{B}}(\Gamma_{\hat{B}B})$, since
		\begin{align}
		\label{eq:QM-over:transpose-on-ME-1}
		\T_B(\Gamma_{\hat{B}B}) & = \sum_{i,j=0}^{d_B-1}\ket{i}\!\bra{j}_{\hat{B}}\otimes(\ket{i}\!\bra{j}_B)^{\t} \\
		& = \sum_{i,j=0}^{d_B-1}\ket{i}\!\bra{j}_{\hat{B}}\otimes \ket{j}\!\bra{i}_B \\
		& = \sum_{i,j=0}^{d_B-1}(\ket{j}\!\bra{i}_{\hat{B}})^{\t}\otimes\ket{j}\!\bra{i}_B \\
		& = \T_{\hat{B}}(\Gamma_{\hat{B}B}).
		\end{align}
		Then the following holds for the Choi representation of $\T_{B'}\circ\mathcal{N}_{B\to B'}\circ \T_B$:
		\begin{align}
			\Gamma_{BB'}^{\T_{B'}\circ\mathcal{N}_{B\to B'}\circ\T_{B}}&=(\T_{B'}\circ\mathcal{N}_{B\to B'}\circ\T_{B})(\Gamma_{\hat{B}B})\\
			& = ((\T_{\hat{B}} \otimes \T_{B'})\circ\mathcal{N}_{B\to B'})(\Gamma_{\hat{B}B}) \\
			&  = \T(\Gamma_{BB'}^{\mathcal{N}}).
			\label{eq:QM-over:transpose-on-ME-last}
		\end{align}
		Since the map $\mathcal{N}_{B\to B'}$ is completely positive, its Choi representation $\Gamma_{BB'}^{\mathcal{N}}$ is positive semi-definite. Since positive semi-definiteness is preserved under transposition, we find that $\T(\Gamma_{BB'}^{\mathcal{N}})$ is positive semi-definite, which means that the map $\T_{B'}\circ\mathcal{N}_{B\to B'}\circ\T_B$ is completely positive. 
	\end{Proof}

As a generalization of the lemma above, we have the following:

\begin{proposition*}{Choi States of C-PPT-P Channels}{prop:QM-over:Choi-C-PPT-P-chs}
Let $\mathcal{N}_{AB \to A'B'}$ be a bipartite channel. The channel $\mathcal{N}_{AB \to A'B'}$ is completely PPT-preserving if and only if its Choi state $\Phi^{\mathcal{N}}_{AB A'B'}$ is a PPT state with respect to the bipartite cut $AA'|BB'$. 
\end{proposition*}

\begin{Proof}
We begin by proving the only-if part. Suppose that $\mathcal{N}_{AB \to A'B'}$ is completely PPT-preserving. By definition, this implies that $\T_{B'} \circ \mathcal{N}_{AB \to A'B'} \circ \T_B$ is completely positive. By  the definition of complete positivity, we conclude that $(\T_{B'} \circ \mathcal{N}_{AB \to A'B'} \circ \T_B)(\Phi_{\bar{A}\bar{B}AB})$ is a positive semi-definite operator, where systems $\bar{A}$ and $\bar{B}$ are isomorphic to the input systems $A$ and $B$, respectively. By employing a calculation similar to that in \eqref{eq:QM-over:transpose-on-ME-1}--\eqref{eq:QM-over:transpose-on-ME-last}, we conclude that
\begin{equation}
(\T_{B'} \circ \mathcal{N}_{AB \to A'B'} \circ \T_B)(\Phi_{\bar{A}\bar{B}A'B'}) = 
((\T_{\bar{B}} \otimes \T_{B'}  )\circ \mathcal{N}_{AB \to A'B'} )(\Phi_{\bar{A}\bar{B}AB}),
\end{equation}
which implies that the Choi state $\mathcal{N}_{AB \to A'B'} )(\Phi_{\bar{A}\bar{B}AB})$ is a PPT state with respect to the bipartite cut $AA'|BB'$. Running this calculation backwards and making use of Theorem~\ref{thm-q_channels} establishes the if-part of the proposition.
\end{Proof}

\subsubsection{PPT Simulation of Channels}

	Just as we asked whether a given channel $\mathcal{N}_{A\to B}$ can be simulated by an LOCC channel, we can ask whether the channel $\mathcal{N}_{A\to B}$ can be simulated by a completely PPT-preserving channel. This leads to the following definition:
	
	\begin{definition}{PPT-Simulable Channel}{def-PPT_sim_chan}
		A channel $\mathcal{N}_{A\to B}$ is called \textit{PPT-simulable} with associated resource state $\omega_{RB'}$ if there exists an auxiliary system $R$ and a completely PPT-preserving channel $\mathcal{P}_{RAB'\to B}$ such that for every state $\rho_A$
		\begin{equation}
			\mathcal{N}(\rho_A)=\mathcal{P}_{RAB'\to B}(\rho_A\otimes\omega_{RB'}).
		\end{equation}
		For the C-PPT-P channel $\mathcal{P}_{RAB'\to B}$, the input systems $RA$ are Alice's, the input system $B'$ is Bob's, Alice's output system is trivial, and Bob's output system is $B$.
	\end{definition}
	
	The definition of a PPT-simulable channel is illustrated in Figure \ref{fig-PPT_sim}.
	
	\begin{figure}
		\centering
		\includegraphics[scale=0.8]{Figures/PPT_sim_gen.pdf}
		\caption{Depiction of a PPT-simulable channel $\mathcal{N}_{A\to B}$ with associated resource state $\omega_{RB'}$. The channel $\mathcal{N}_{A\to B}$ can be realized via the completely PPT-preserving channel $\mathcal{P}_{RAB'\to B}$ and the resource state $\omega_{RB'}$, for some auxiliary system $R$.}\label{fig-PPT_sim}
	\end{figure}

\subsection{Non-Signaling Channels}

\label{sec-QM:non-sig-chs}

One of the main applications considered in this book is communication and, more specifically, when communication is possible or impossible. To this end, suppose that Alice and Bob are connected by means of a bipartite channel $\mathcal{N}_{AB\rightarrow A^{\prime}B^{\prime}}$. Such a channel is said to be non-signaling from Alice to Bob if it is impossible for Alice and Bob to make use of it for the purpose of Alice to communicate a message to Bob. We give a precise definition as follows: 

\begin{definition}{Non-Signaling Channel}{def-QM:non-sig-channel}
A bipartite channel $\mathcal{N}_{AB\rightarrow A^{\prime}B^{\prime}}$ is
non-signaling from Alice to Bob  if the following condition
holds 
\begin{equation}
\operatorname{Tr}_{A^{\prime}}\circ\mathcal{N}_{AB\rightarrow A^{\prime
}B^{\prime}}=\operatorname{Tr}_{A^{\prime}}\circ\mathcal{N}_{AB\rightarrow
A^{\prime}B^{\prime}}\circ\mathcal{R}_{A}^{\pi},\label{eq:NS-A-to-B-cond}%
\end{equation}
where $\mathcal{R}_{A}^{\pi}$ is a replacer channel, defined as $\mathcal{R}%
_{A}^{\pi}(\cdot)\coloneqq \operatorname{Tr}_{A}[\cdot]\pi_{A}$, with $\pi_{A}%
\coloneqq \mathbbm{1}_{A}/d_{A}$ the maximally mixed state on system $A$.
\end{definition}

To interpret the
condition in \eqref{eq:NS-A-to-B-cond}, consider the following. For Bob, the reduced state of his output
system $B^{\prime}$ is obtained by tracing out Alice's output system
$A^{\prime}$. Note that the reduced state on $B^{\prime}$ is all that Bob can
access at the output in this scenario. If the condition in
\eqref{eq:NS-A-to-B-cond} holds, then the reduced state on Bob's output system
$B^{\prime}$ has no dependence on Alice's input system. Thus, if
\eqref{eq:NS-A-to-B-cond} holds, then Alice cannot use $\mathcal{N}%
_{AB\rightarrow A^{\prime}B^{\prime}}$ to send a signal to Bob.

\begin{proposition*}{Choi Operator of a Non-Signaling Channel}{prop:QM-over:Choi-non-sig-chs}
Let $\mathcal{N}_{AB\rightarrow A^{\prime}B^{\prime}}$ be a bipartite channel. Let
\begin{equation}
\Gamma^{\mathcal{N}}_{AB A^{\prime}B^{\prime}} \coloneqq
\mathcal{N}_{\bar{A}\bar{B}\rightarrow A^{\prime}B^{\prime}}(\Gamma_{A\bar{A}} \otimes \Gamma_{B\bar{B}})
\end{equation}
be the Choi operator of $\mathcal{N}_{AB\rightarrow A^{\prime}B^{\prime}}$, where $\bar{A}$ is isomorphic to $A$ and $\bar{B}$ is isomorphic to $B$.
The channel $\mathcal{N}_{AB\rightarrow A^{\prime}B^{\prime}}$ is non-signaling from Alice to Bob if and only if its Choi operator $\Gamma^{\mathcal{N}}_{AB A^{\prime}B^{\prime}}$
 satisfies the following condition:
\begin{equation}
\Tr_{A'}[\Gamma^{\mathcal{N}}_{AB A^{\prime}B^{\prime}}] = 
\pi_A \otimes \Tr_{A'A}[\Gamma^{\mathcal{N}}_{AB A^{\prime}B^{\prime}}].
\label{eq-QM:non-sig-Choi}
\end{equation}
\end{proposition*}
\begin{Proof}
We begin by proving the if-part. Consider that
\begin{equation}
\operatorname{Tr}_{A^{\prime}}\circ\mathcal{N}_{\bar{A}\bar{B}\rightarrow A^{\prime
}B^{\prime}}(\Gamma_{A\bar{A}} \otimes \Gamma_{B\bar{B}}) = 
\operatorname{Tr}_{A^{\prime}}[\Gamma^{\mathcal{N}}_{AB A^{\prime}B^{\prime}}]
\end{equation}
Also, consider that
\begin{align}
& (\operatorname{Tr}_{A^{\prime}}\circ\mathcal{N}_{\bar{A}\bar{B}\rightarrow
A^{\prime}B^{\prime}}\circ\mathcal{R}_{\bar{A}}^{\pi})(\Gamma_{A\bar{A}} \otimes \Gamma_{B\bar{B}}) \notag \\
& = 
(\operatorname{Tr}_{A^{\prime}}\circ\mathcal{N}_{\bar{A}\bar{B}\rightarrow
A^{\prime}B^{\prime}})(\mathbbm{1}_{A} \otimes \pi_{\bar{A}}\otimes \Gamma_{B\bar{B}}) \\
& = 
(\operatorname{Tr}_{A^{\prime}}\circ\mathcal{N}_{\bar{A}\bar{B}\rightarrow
A^{\prime}B^{\prime}})(\pi_{A} \otimes \mathbbm{1}_{\bar{A}}\otimes \Gamma_{B\bar{B}}) \\
& = 
\pi_{A} \otimes (\operatorname{Tr}_{A^{\prime}}\circ\mathcal{N}_{\bar{A}\bar{B}\rightarrow
A^{\prime}B^{\prime}})( \mathbbm{1}_{\bar{A}}\otimes \Gamma_{B\bar{B}}) \\
& = 
\pi_{A} \otimes (\operatorname{Tr}_{AA^{\prime}}\circ\mathcal{N}_{\bar{A}\bar{B}\rightarrow
A^{\prime}B^{\prime}})( \Gamma_{A\bar{A}}\otimes \Gamma_{B\bar{B}}) \\
& = \pi_{A} \otimes  \Tr_{A'A}[\Gamma^{\mathcal{N}}_{AB A^{\prime}B^{\prime}}].
\end{align}
Thus, we conclude that \eqref{eq:NS-A-to-B-cond} implies \eqref{eq-QM:non-sig-Choi}.

To see the other implication, we simply run the reasoning given above backwards and note that two channels are equal if and only if their Choi operators are equal (see Theorem~\ref{thm-q_channels}).
\end{Proof}

A one-way LOCC channel from Bob to Alice is an interesting example of a bipartite channel that is non-signaling from Alice to Bob. Indeed, consider a bipartite channel of the form in \eqref{eq-QM:one-way-LOCC-from-B-to-A}, and let us check that the condition in \eqref{eq:NS-A-to-B-cond} holds for such a channel. By tracing over the output system $A'$, we find that
\begin{align}
 \operatorname{Tr}_{A'}[\mathcal{L}_{AB\to A'B'}^{\leftarrow}(\rho_{AB})] & = 
\sum_{x\in\mathcal{X}} \operatorname{Tr}_{A'}[(\mathcal{N}_{A\to A'}^x\otimes\mathcal{M}_{B\to B'}^x)(\rho_{AB})] \\
& = \sum_{x\in\mathcal{X}} \mathcal{M}_{B\to B'}^x(\operatorname{Tr}_{A}[\rho_{AB}]) \\
& = \sum_{x\in\mathcal{X}} \mathcal{M}_{B\to B'}^x(\rho_{B}).
\end{align}
The second equality follows because $\mathcal{N}_{A\to A'}^x$ is trace preserving for all $x$.
Also, consider that
\begin{align}
& \!\!\!\!\!(\operatorname{Tr}_{A'} \circ\mathcal{L}_{AB\to A'B'}^{\leftarrow}\circ \mathcal{R}_{A}^{\pi})(\rho_{AB}) \notag \\
& = 
(\operatorname{Tr}_{A'} \circ\mathcal{L}_{AB\to A'B'}^{\leftarrow})(\pi_A \otimes \rho_{B})\\
& = \sum_{x\in\mathcal{X}} \operatorname{Tr}_{A'}[(\mathcal{N}_{A\to A'}^x\otimes\mathcal{M}_{B\to B'}^x)(\pi_A \otimes \rho_{B})] \\
& = \sum_{x\in\mathcal{X}} \mathcal{M}_{B\to B'}^x(\operatorname{Tr}_{A}[\pi_A \otimes \rho_{B}]) \\
& = \sum_{x\in\mathcal{X}} \mathcal{M}_{B\to B'}^x (\rho_{B}).
\end{align}
Thus, the condition in \eqref{eq:NS-A-to-B-cond} holds, and as expected, $\mathcal{L}_{AB\to A'B'}^{\leftarrow}$ is non-signaling from Alice to Bob.




\section{Quantum Teleportation}\label{sec-teleportation}

	Quantum teleportation is a remarkable and fundamental protocol in quantum information theory. The simplest version of the protocol allows two parties, say Alice and Bob, to transfer the state of a qubit from Alice to Bob while making use of one shared pair of qubits in a maximally entangled state.
	
	\subsection{Qubit Teleportation Protocol}
	
	Before stating the basic teleportation protocol, let us start by introducing a key element of the protocol, the \textit{Bell measurement}. 

	The Bell measurement is a measurement on two qubits defined by the POVM $\{\ket{\Phi^+}\!\bra{\Phi^+},\allowbreak\ket{\Phi^-}\!\bra{\Phi^-},\ket{\Psi^+}\!\bra{\Psi^+},\ket{\Psi^-}\!\bra{\Psi^-}\}$, where
	\begin{align}
		\ket{\Phi^+}&\coloneqq \frac{1}{\sqrt{2}}(\ket{0,0}+\ket{1,1}),\\
		\ket{\Phi^-}&\coloneqq \frac{1}{\sqrt{2}}(\ket{0,0}-\ket{1,1}),\\
		\ket{\Psi^+}&\coloneqq \frac{1}{\sqrt{2}}(\ket{0,1}+\ket{1,0}),\\
		\ket{\Psi^-}&\coloneqq \frac{1}{\sqrt{2}}(\ket{0,1}-\ket{1,0})
	\end{align}
	are the two-qubit \textit{Bell states}. They are all maximally entangled, and they form an orthonormal basis for the Hilbert space $\mathbb{C}^2\otimes\mathbb{C}^2$ of two qubits. As such, we have that $\ket{\Phi^+}\!\bra{\Phi^+}+\ket{\Phi^-}\!\bra{\Phi^-}+\ket{\Psi^+}\!\bra{\Psi^+}+\ket{\Psi^-}\!\bra{\Psi^-}=\mathbbm{1}$, so that the set $\{\ket{\Phi^+}\!\bra{\Phi^+},\ket{\Phi^-}\!\bra{\Phi^-},\ket{\Psi^+}\!\bra{\Psi^+},\ket{\Psi^-}\!\bra{\Psi^-}\}$ is indeed a POVM.
	
	We can write the usual computational basis states for two qubits in terms of the Bell states as
	\begin{align}
		\ket{0,0}&=\frac{1}{\sqrt{2}}(\ket{\Phi^+}+\ket{\Phi^-}),\label{eq-Bell_to_comp_1}\\
		\ket{0,1}&=\frac{1}{\sqrt{2}}(\ket{\Psi^+}+\ket{\Psi^-}),\\
		\ket{1,0}&=\frac{1}{\sqrt{2}}(\ket{\Psi^+}-\ket{\Psi^-}),\\
		\ket{1,1}&=\frac{1}{\sqrt{2}}(\ket{\Phi^+}-\ket{\Phi^-}).\label{eq-Bell_to_comp_4}
	\end{align}
	
	Observe that we can write the Bell states compactly as
	\begin{equation}\label{eq-qubit_Bell_compact}
		\ket{\Phi_{x,z}}_{AB}\coloneqq (\mathbbm{1}_A\otimes X_B^x Z_B^z)\ket{\Phi^+}_{AB}=(Z_A^zX_A^x\otimes\mathbbm{1}_B)\ket{\Phi^+}_{AB}
	\end{equation}
	for all $x,z\in\{0,1\}$. In other words, all four two-qubit Bell states can be obtained from each other using only local operations on either $A$ or $B$. Furthermore, the Bell measurement POVM can be written as $\{\ket{\Phi_{x,z}}\!\bra{\Phi_{x,z}}:x,z\in\{0,1\}\}$, so that the classical bits $x$ and $z$ can be viewed as being the outcomes of the measurement. 

	\begin{figure}
		\centering
		\includegraphics[scale=0.8]{Figures/teleportation.pdf}
		\caption{Circuit diagram for the teleportation protocol. Conditioned on the outcomes $(x,z)$ of Alice's Bell measurement on her qubits $A$ and $A'$, Bob performs the operation $Z^zX^x$ on his qubit to transform it to~$\ket{\psi}$.}\label{fig-teleportation}
	\end{figure}
	
	We now detail the teleportation protocol; see Figure \ref{fig-teleportation} for a circuit diagram depicting the protocol. The protocol starts with Alice and Bob sharing two qubits in the state $\ket{\Phi^+}_{AB}$. Alice has an additional qubit, which is in the state $\ket{\psi}_{A'}$, that she wishes to teleport to Bob, where
	\begin{equation}
		\ket{\psi}_{A'}=\alpha\ket{0}_{A'}+\beta\ket{1}_{A'},\quad\alpha,\beta\in\mathbb{C},\quad \abs{\alpha}^2+\abs{\beta}^2=1.
	\end{equation}
	The state $\ket{\psi}_{A'}$ is arbitrary and need not be known to either Alice or Bob. The total joint state between Alice and Bob at the start of the protocol is therefore
	\begin{equation}\label{eq-teleport_state_start}
		\begin{aligned}
		\ket{\psi}_{A'}\otimes\ket{\Phi^+}_{AB}&=\frac{1}{\sqrt{2}}(\alpha\ket{0,0,0}_{A'AB}+\alpha\ket{0,1,1}_{A'AB}\\
		&\qquad\qquad+\beta\ket{1,0,0}_{A'AB}+\beta\ket{1,1,1}_{A'AB}).
		\end{aligned}
	\end{equation}
	Alice and Bob then proceed as follows.
	\begin{enumerate}
		\item Alice performs a Bell measurement on her two qubits $A'$ and $A$. To easily determine the measurement outcomes and their probabilities, it is helpful to write down the initial state \eqref{eq-teleport_state_start} in the Bell basis on Alice's systems. Using \eqref{eq-Bell_to_comp_1}--\eqref{eq-Bell_to_comp_4}, we find that
			\begin{align}
				& \ket{\psi}_{A'}\otimes\ket{\Phi^+}_{AB}\notag\\
				&=\frac{1}{2}\left(\ket{\Phi^+}_{A'A}\otimes(\alpha\ket{0}_B+\beta\ket{1}_B)\right.
				\left.+\ket{\Phi^-}_{A'A}\otimes (\alpha\ket{0}_B-\beta\ket{1}_B)\right.\nonumber\\
				&\qquad\quad\left.+\ket{\Psi^+}_{A'A}\otimes(\alpha\ket{1}_B+\beta\ket{0}_B)\right.
				\left.+\ket{\Psi^-}_{A'A}\otimes (\alpha\ket{1}_B-\beta\ket{0})\right)
				\notag \\
				&=\frac{1}{2}\left(\ket{\Phi^+}_{A'A}\otimes\ket{\psi}_B\right.\left.+\ket{\Phi^-}_{A'A}\otimes Z_B\ket{\psi}_B\right.\nonumber\\
				&\qquad\qquad\left.+\ket{\Psi^+}_{A'A}\otimes X_B\ket{\psi}_B\right.\left.+\ket{\Psi^-}_{A'A}\otimes X_BZ_B\ket{\psi}_B\right).
			\end{align}
			From this, it is clear that each outcome $(x,z)\in\{0,1\}^2$ of the Bell measurement occurs with equal probablity $\frac{1}{4}$ and that the state of Bob's qubit after the measurement is $X_B^xZ_B^z\ket{\psi}_B$.
		\item Alice communicates to Bob the two classical bits $x$ and $z$ resulting from the Bell measurement.
		\item Upon receiving the measurement outcomes, Bob performs $X^x$ and then~$Z^z$ on his qubit. The resulting state of Bob's qubit is $\ket{\psi}$. 
		
	\end{enumerate}
	
	Although we have described the teleportation protocol using a pure state~$\ket{\psi}_{A'}$ as the state being teleported, the protocol applies just as well if the state to be teleported is a mixed state $\rho_{A'}$.
	
	
\subsection{Qudit Teleportation Protocol}

	The teleportation protocol for qubits described above can be easily generalized to qudits using the Heisenberg--Weyl operators $\{W_{z,x}:0\leq z,x\leq d-1\}$, as defined in Section~\ref{sec:QM-over:gen-pauli-chs}.
	
	We begin by defining the \textit{qudit Bell states} in terms of the Heisenberg--Weyl operators as
	\begin{equation}\label{eq-qudit_Bell}
		\ket{\Phi_{z,x}}\coloneqq (W_{z,x}\otimes \mathbbm{1})\ket{\Phi},
	\end{equation}
	which is a direct generalization of \eqref{eq-qubit_Bell_compact}, where $\ket{\Phi}=\frac{1}{\sqrt{d}}\sum_{i=0}^{d-1}\ket{i,i}$. Just like the qubit Bell states, the qudit Bell states are orthonormal because
	\begin{align}
		\braket{\Phi_{z_1,x_1}}{\Phi_{z_2,x_2}}&=\bra{\Phi}(W_{z_1,x_1}^\dagger\otimes\mathbbm{1})(W_{z_2,x_2}\otimes\mathbbm{1})\ket{\Phi}\\
		&=\bra{\Phi}(W_{z_1,x_1}^\dagger W_{z_2,x_2}\otimes\mathbbm{1})\ket{\Phi}\\
		&=\frac{1}{d}\Tr[W_{z_1,x_1}^\dagger W_{z_2,x_2}]\\
		&=\delta_{z_1,z_2}\delta_{x_1,x_2}
	\end{align}
	for all $0\leq z_1,z_2,x_1,x_2\leq d-1$. The last equality follows from \eqref{eq:QM-over:HW-orthogonal}. This means that the set of operators
	\begin{equation}
	\{\ket{\Phi_{z,x}}\!\bra{\Phi_{z,x}}:0\leq z,x\leq d-1\}
	\end{equation}
	 constitutes a POVM, which is the POVM corresponding to the Bell measurement on two qudits.
	
	Now we start, like before, with Alice holding two qudits, one shared with Bob and in the joint state $\ket{\Phi}_{AB}$, and the other in the state $\ket{\psi}_{A'}$, where
	\begin{equation}
		\ket{\psi}_{A'}=\sum_{i=0}^{d-1}c_i\ket{i},\quad\sum_{i=0}^{d-1}\abs{c_i}^2=1.
	\end{equation}
	The state $\ket{\psi}_{A'}$ is the one to be teleported to Bob's system. The starting joint state on the three qudits $A'$, $A$, and $B$ is
	\begin{equation}
		\ket{\psi}_{A'}\otimes\ket{\Phi}_{AB}=\frac{1}{\sqrt{d}}\sum_{i,j=0}^{d-1} c_i\ket{i,j,j}_{A'AB}.
	\end{equation}
	Alice then performs a Bell measurement on her two qudits. By writing the Bell states $\ket{\Phi_{z,x}}_{A'A}$ as
	\begin{equation}
		\ket{\Phi_{z,x}}_{A'A}=\frac{1}{\sqrt{d}}\sum_{k=0}^{d-1}\e^{\frac{2\pi\I(k+x)z}{d}}\ket{k+x,k}_{A'A},
	\end{equation}
	for each outcome $(z,x)\in\{0,\dotsc,d-1\}^2$, we use \eqref{eq-post_meas_state_half_proj} to find that the corresponding (unnormalized) post-measurement state on Bob's qudit is
	\begin{align}
		&(\bra{\Phi_{z,x}}_{A'A}\otimes\mathbbm{1}_B)(\ket{\psi}_{A'}\otimes\ket{\Phi}_{AB})\nonumber\\
		&\qquad=\frac{1}{d}\sum_{j,k,\ell=0}^{d-1}c_{\ell}\e^{-\frac{2\pi\I(k+x)z}{d}}\braket{k+x}{\ell}\braket{k}{j}\ket{j}_B\\
		&\qquad=\frac{1}{d}\sum_{k=0}^{d-1}c_{k+x}\e^{-\frac{2\pi\I(k+x)z}{d}}\ket{k}_B\\
		&\qquad=\frac{1}{d}\sum_{k'=0}^{d-1}c_{k'}\e^{-\frac{2\pi\I k'z}{d}}\ket{k'-x}_B\\
		&\qquad=\frac{1}{d}\sum_{k=0}^{d-1}c_{k'} X(-x)Z(-z)\ket{k'}_B\\
		&\qquad=\frac{1}{d}X(-x)Z(-z)\ket{\psi}_B.
	\end{align}
	Therefore, each outcome occurs with probability $\frac{1}{d^2}$ and the corresponding post-measurement state on Bob's qudit is $X(-x)Z(-z)\ket{\psi}_B$. This means that Bob, upon receving the two classical values corresponding to the outcome of the Bell measurement, can perform $Z(z)X(x)=W_{z,x}$ in order to transform the state of his qudit to $\ket{\psi}_B$, completing the teleportation protocol.
	
	\begin{figure}
		\centering
		\includegraphics[scale=0.8]{Figures/teleportation_chan.pdf}
		\caption{The qudit teleportation protocol, depicted on the left, can be regarded as an LOCC channel $\mathcal{T}_{A'AB\to B}$ with the input states $\rho_{A'}$ and $\ket{\Phi}\!\bra{\Phi}_{AB}$ and the output state $\rho_B$, as shown on the right.}\label{fig-teleportation_chan}
	\end{figure}
	
	Of course, the teleportation protocol works just as well if the state to be teleported is mixed. Also, as shown in Figure \ref{fig-teleportation_chan}, we can write down the entire teleportation protocol as a one-way LOCC channel $\mathcal{T}_{A'AB\to B}$ from Alice to Bob, with the state $\rho_{A'}$ to be teleported and the state $\ket{\Phi}\!\bra{\Phi}_{AB}$ as the inputs. By the analysis above, the output state received by Bob is exactly the same as the original input state:
	\begin{equation}\label{eq-teleportation_channel}
		\mathcal{T}_{A'AB\to B}(\rho_{A'}\otimes\ket{\Phi}\!\bra{\Phi}_{AB})=\rho_B.
	\end{equation}
	This equation can also be interpreted as follows:
	\begin{equation}\label{eq-teleportation_sim_id}
		\mathcal{T}_{A'AB\to B}((\cdot)_{A'}\otimes \ket{\Phi}\!\bra{\Phi}_{AB})=\id_{A'\to B}(\cdot),
	\end{equation}
	i.e., that the teleportation protocol simulates the identity channel.
	
	To see that the teleportation protocol can indeed be viewed as a one-way LOCC channel from Alice to Bob, let us explicitly write down the quantum channel $\mathcal{T}_{A'AB\to B}$ defined above in the form of \eqref{eq-1wayLOCC_decomp}, i.e.,
	\begin{equation}\label{eq-teleportation_LOCC_chan}
		\mathcal{T}_{A'AB\to B}=\mathcal{D}_{BY_1Y_2\to B}\circ\mathcal{C}_{X_1X_2\to Y_1Y_2}\circ\mathcal{E}_{A'A\to X_1X_2}
	\end{equation}
	which we recall is equivalent to the form in \eqref{eq-LOCC_A_to_B}. We have,
	\begin{align}
		\mathcal{E}_{A'A\to X_1X_2}&=\sum_{z,x=0}^{d-1}\mathcal{E}_{A'A\to\varnothing}^{z,x}\otimes\ket{z,x}\!\bra{z,x}_{X_1X_2},\\
		\mathcal{E}_{A'A\to\varnothing}^{z,x}(\cdot)&\coloneqq \Tr_{A'A}[\ket{\Phi_{z,x}}\!\bra{\Phi_{z,x}}_{A'A}(\cdot)],\\
		\mathcal{C}_{X_1X_2\to Y_1Y_2}(\ket{z,x}\!\bra{z,x}_{X_1X_2})&=\ket{z,x}\!\bra{z,x}_{Y_1Y_2},\\
		\mathcal{D}_{BY_1Y_2\to B}((\cdot)_B\otimes\ket{z,x}\!\bra{z,x}_{Y_1Y_2})&=\mathcal{D}_{B\to B}^{z,x}(\cdot),\\
		\mathcal{D}_{B\to B}^{z,x}(\cdot)&\coloneqq W_{z,x}(\cdot)W_{z,x}^\dagger.
	\end{align}
	
	We can also connect with the previously defined notion of LOCC simulation of a quantum channel (Definition~\ref{def-LOCC_sim_chan}). That is, we can understand the teleportation protocol and \eqref{eq-teleportation_channel} as demonstrating that the identity channel is LOCC simulable with associated resource state given by the maximally entangled state. Now, by using the teleportation protocol in conjunction with a quantum channel $\mathcal{N}_{A\to B}$, we find that every quantum channel $\mathcal{N}_{A\to B}$ is LOCC simulable with associated resource state given by the maximally entangled state of an appropriate Schmidt rank. To see this, observe that the channel $\mathcal{N}_{A\to B}$ can be trivially written as $\mathcal{N}_{A\to B}=\mathcal{N}_{B'\to B}\circ\id_{A\to B'}$, where $B'$ is an auxiliary system with the same dimension as $A$. Then, by \eqref{eq-teleportation_sim_id}, we can simulate the identity channel $\id_{A\to B'}$ using the usual teleportation protocol, so that the overall LOCC channel $\mathcal{L}$ is $\mathcal{N}_{B'\to B}\circ\mathcal{T}_{AA'B'\to B'}$ and the resource state is $\ket{\Phi}\!\bra{\Phi}_{A'B'}$, with the dimension of $A'$ equal to the dimension of $A$. This is illustrated in Figure \ref{fig-teleportation_sim_arbitrary}. We can also simulate $\mathcal{N}$ via teleportation in a different manner, in which Alice locally applies the channel $\mathcal{N}$ to her input state $\rho_A$, then teleports the resulting state to Bob. Mathematically, we write this as $\mathcal{N}_{A\to B}=\id_{\hat{A}\to B}\circ\mathcal{N}_{A\to\hat{A}}=\mathcal{T}_{\hat{A}\tilde{A}B\to B}\circ\mathcal{N}_{A\to\hat{A}}$, where $\hat{A},\tilde{A}$ are auxiliary systems with the same dimension as $B$. We thus have have the following two ways to represent the action of the channel $\mathcal{N}$ using teleportation:
	\begin{align}
		\mathcal{N}_{A\to B}(\rho_A)&=\mathcal{N}_{B'\to B}\left(\mathcal{T}_{AA'B'\to B'}(\rho_{A}\otimes\ket{\Phi}\!\bra{\Phi}_{A'B'})\right)\label{eq-chan_tele_sim_1}\\
		&=\mathcal{T}_{\hat{A}\tilde{A}B\to B}\left(\mathcal{N}_{A\to\hat{A}}(\rho_A)\otimes\ket{\Phi}\!\bra{\Phi}_{\tilde{A}B}\right).\label{eq-chan_tele_sim_2}
	\end{align}
	
	\begin{figure}
		\centering
		\includegraphics[scale=0.8]{Figures/teleportation_sim_arb.pdf}
		\caption{Any channel $\mathcal{N}$ is teleportation simulable, since Alice and Bob can first perform the usual teleportation protocol, after which Bob can apply the channel $\mathcal{N}$ to the state teleported by Alice. The combination of these two steps can be taken as the LOCC channel $\mathcal{L}_{A'AB'\to B}^{\rightarrow}$.}\label{fig-teleportation_sim_arbitrary}
	\end{figure}
	
	Depending on whether the input dimension is smaller than the output dimension of the channel, there can be a more economical way to perform the simulation. If the channel's output dimension is smaller than its input dimension, then the more economical way to simulate the channel is for Alice to first apply $\mathcal{N}_{A\to B}$ and then for Alice and Bob to perform the teleportation protocol. In this way, they exploit a maximally entangled state of Schmidt rank $d_B$ in order to accomplish the simulation. If the channel's input dimension is smaller than its output dimension, then the more economical way to simulate the channel is for Alice and Bob to first perform the teleportation protocol, and then for Bob to apply the channel locally. In this way, they exploit a maximally entangled state of Schmidt rank $d_A$ in order to accomplish the simulation. As we see in Section~\ref{subsec-tele_sim}, depending on the channel and its symmetries, there can be even more economical methods to simulate a quantum channel via teleportation.
	
	
\subsection{Qudit Teleportation Protocol With Respect to a Finite Group}
	
	The qudit teleportation protocol outlined above is based on the Heisenberg--Weyl operators $\{W_{z,x}:0\leq z,x\leq d-1\}$ acting on a $d$-dimensional system, which are used to form the qudit Bell states and thus the Bell measurement. %They satisfy the identity
%	\begin{equation}\label{eq-HW_twirl}
%		\frac{1}{d^2}\sum_{z,x=0}^{d-1}W_{z,x}\rho W_{z,x}^\dagger=\Tr[\rho] \pi_d
%	\end{equation}
%	for every state $\rho$, where $\pi_d=\frac{\mathbbm{1}}{d}$, 
%	and they also form an irreducible projective unitary representation of the group $\mathbb{Z}_d\times\mathbb{Z}_d$. This fact can actually be used to prove \eqref{eq-HW_twirl} (see Bibliographic Notes in Section~\ref{sec:qm:bib-notes}).
	
	More generally, we can consider an arbitrary finite group $G$ and an irreducible unitary representation $\{U^g\}_{g\in G}$ of $G$ acting on a $d$-dimensional Hilbert space. It then follows from Schur's lemma (see Bibliographic Notes in Section~\ref{sec:qm:bib-notes}) that
	\begin{equation}
		\frac{1}{|G|}\sum_{g\in G}U^g \rho U^{g\dagger}=\Tr[\rho]\pi_{|G|}
	\end{equation}
	for every state $\rho$. In particular, for bipartite states $\rho_{AB}$ in which the systems $A$ and $B$ are both $d$-dimensional, we find that
	\begin{equation}\label{eq-twirl_G_tensor}
		\frac{1}{|G|}\sum_{g\in G}(U_A^g\otimes \mathbbm{1}_B) \rho_{AB} (U_A^{g\dagger}\otimes\mathbbm{1}_B)=\pi_A\otimes\Tr_A[\rho_{AB}].
	\end{equation}
	
	Now, let us take the maximally entangled state $\ket{\Phi}_{AB}$ and define the states
	\begin{equation}\label{eq-qudit_Bell_G}
		\ket{\Phi^g}_{AB}\coloneqq (U_A^g\otimes \mathbbm{1}_B)\ket{\Phi}_{AB}.
	\end{equation}
	We call these states the \textit{generalized Bell states}. We see that these states are a direct generalization of the usual qudit Bell states in \eqref{eq-qudit_Bell}. Then, by substituting $\ket{\Phi}\!\bra{\Phi}_{AB}$ for $\rho_{AB}$ in \eqref{eq-twirl_G_tensor}, we find that
	\begin{equation}
		\frac{1}{|G|}\sum_{g\in G}\ket{\Phi^g}\!\bra{\Phi^g}_{AB}= \pi_{AB} = \frac{\mathbbm{1}_{AB}}{d^2}.
	\end{equation}
	By defining the operators
	\begin{equation}\label{eq-G_Bell_meas}
		\Pi_{AB}^g\coloneqq \frac{d^2}{|G|}\ket{\Phi^g}\!\bra{\Phi^g}_{AB},
	\end{equation}
	we find that
	\begin{equation}
		\sum_{g\in G}\Pi_{AB}^g=\mathbbm{1}_{AB}.
	\end{equation}
	Since the operators $\Pi^g_{AB}$ are also positive semi-definite, we conclude that the set $\{\Pi^g_{AB}\}_{g\in G}$ constitutes a POVM. This POVM corresponds, by definition, to the \textit{$G$-Bell measurement}. Note that $\frac{d^2}{|G|} \leq 1$, which follows as a consequence of the facts that $\sum_{g \in G}\Pi^g = \mathbbm{1}$ and each $\ket{\Phi^g}$ is a unit vector (were it not so, then the sum $\sum_{g \in G}\Pi^g$ would exceed the identity). Indeed, consider that the identity $\sum_{g \in G}\Pi^g = \mathbbm{1}$ and the fact that $\Pi^g\geq 0$ for all $g \in G$ implies that $\Pi^g \leq \mathbbm{1}$ for all $g\in G$. Then decomposing $\mathbbm{1}_{AB} = \ket{\Phi_g}\!\bra{\Phi_g} + \ket{\Phi^g}\!\bra{\Phi^g}^{\perp}$, where $\ket{\Phi^g}\!\bra{\Phi^g}^{\perp} \coloneqq \mathbbm{1} - \ket{\Phi^g}\!\bra{\Phi^g}$, we see that the only way the operator inequality $\Pi^g \leq \mathbbm{1}$ can be satisfied is if $\frac{d^2}{|G|} \leq 1$.
	
	We use the $G$-Bell measurement given by the POVM $\{\Pi^g\}_{g\in G}$ to construct our generalized teleportation protocol. The protocol proceeds as follows. As before, Alice and Bob start by sharing two qudits in the state $\ket{\Phi}_{AB}$, with Alice holding an extra qudit in the state $\ket{\psi}_{A'}$ to be teleported to Bob. 
	\begin{enumerate}
		\item Alice performs, on her qudits $A$ and $A'$, the generalized Bell measurement given by the POVM $\{\Pi_{AA'}^g\}_{g\in G}$. For each outcome $g\in G$ of the measurement, according to \eqref{eq-post_meas_state_half_proj} the (unnormalized) post-measurement state of Bob's qudit is
			\begin{align}
				&\left(\frac{d}{\sqrt{|G|}}\bra{\Phi_g}_{A'A}\otimes\mathbbm{1}_B\right)(\ket{\psi}_{A'}\otimes\ket{\Phi}_{AB})\nonumber\\
				&\qquad=\frac{d}{\sqrt{|G|}}\left(\bra{\Phi}_{A'A}(U_{A'}^{g\dagger}\otimes\mathbbm{1}_A)\otimes\mathbbm{1}_B\right)(\ket{\psi}_{A'}\otimes\ket{\Phi}_{AB})\\
				&\qquad=\frac{d}{\sqrt{|G|}}\left(\frac{1}{\sqrt{d}}\sum_{k=1}^d\bra{k,k}_{A'A}(U_{A'}^{g\dagger}\otimes\mathbbm{1}_A)\otimes\mathbbm{1}_B\right)\nonumber\\
				&\qquad\qquad\qquad\qquad\qquad\times \left(\ket{\psi}_{A'}\otimes\frac{1}{\sqrt{d}}\sum_{k'=1}^d\ket{k',k'}_{AB}\right)\\
				&\qquad=\frac{1}{\sqrt{|G|}}\sum_{k,k'=1}^d\bra{k}_{A'}U_{A'}^{g\dagger}\ket{\psi}_{A'}\ket{k}_B\braket{k}{k'}\\
				&\qquad=\frac{1}{\sqrt{|G|}}\sum_{k=1}^d\bra{k}_{A'}U_{A'}^{g\dagger}\ket{\psi}_{A'}\ket{k}_B\\
				&\qquad=\frac{1}{\sqrt{|G|}}U_{B}^{g\dagger}\ket{\psi}_B
			\end{align}
			We see that each outcome occurs with probability $\frac{1}{|G|}$, and the post-meas\-urement state of Bob's qudit is $U_{B}^{g\dagger}\ket{\psi}_B$.
		\item Alice communicates the outcome $g$ resulting from the measurement to Bob.
		\item Upon receiving the measurement outcome, Bob applies $U^g$ on his qudit. The resulting state of Bob's qudit is $\ket{\psi}_{B}$.	
	\end{enumerate}
	
	Observe that the original qudit teleportation protocol is a special case of the generalized teleportation protocol outlined above, in which the group $G$ is $\mathbb{Z}_d\times\mathbb{Z}_d$ and its irreducible projective unitary representation $\{U^g\}_{g\in G}$ is taken to be the set of Heisenberg--Weyl operators. Then, the generalized Bell states $\ket{\Phi^g}$ are precisely the qudit Bell states $\ket{\Phi_{z,x}}$ defined in \eqref{eq-qudit_Bell}. Furthermore, since $|G|=d^2$, the POVM elements $\Pi^g=\frac{d^2}{|G|}\ket{\Phi^g}\!\bra{\Phi^g}$ are the projections onto the qudit Bell states, exactly as in the qudit teleportation protocol.
	
	
\subsection{Post-Selected Teleportation}

	Throughout this section, we have described teleportation protocols that involve performing a particular kind of Bell measurement between a system $A'$, whose state is to be teleported, and a system $A$ that forms half of a bipartite system $AB$ that is in the joint resource state $\ket{\Phi}\!\bra{\Phi}_{AB}$. Based on the Bell measurement outcome on $A'A$, Bob applies a particular correction operation in order to obtain the initial state of $A'$ in his system $B$. Thus, although the individual measurement outcomes of the Bell measurement occur with some probability, due to the correction operations the overall teleportation protocol is deterministic, i.e., it succeeds with probability one.
	
	If Bob does not have the ability to apply correction operations to his system based on the Bell measurement outcomes, then Alice and Bob can perform what is called \textit{post-selected teleportation}. Post-selected teleportation is based on the fact that, in the teleportation protocols that we have considered, Bob does not need to apply a correction operation on his system if the outcome corresponding to $\ket{\Phi}\!\bra{\Phi}_{A'A}$ occurs in the Bell measurement on $A'A$. This is due to the fact that the post-measurement state on Bob's system, conditioned on the $\ket{\Phi}_{A'A}$ outcome, is precisely the initial state $\rho_{A'}$ to be teleported:
	\begin{equation}\label{eq-post_selected_teleportation}
		\bra{\Phi}_{A'A}(\rho_{A'}\otimes\ket{\Phi}\!\bra{\Phi}_{AB})\ket{\Phi}_{A'A}=\frac{1}{d^2}\,\rho_B,
	\end{equation}
	where $d=d_A=d_B$. This is a special case of \eqref{eq-Choi_state_post_selected_teleportation} in which $\mathcal{N}_{A'\to B}=\id_{A'\to B}$ and $X_{RA'}=\rho_{A'}$. If we thus modify the teleportation protocol such that we consider the $\ket{\Phi}_{A'A}$ outcome of the Bell measurement as a ``success'' and the rest of the outcomes as a ``failure'', then we obtain post-selected teleportation. Post-selected teleportation is probabilistic by definition. In particular, from \eqref{eq-post_selected_teleportation}, we see that it succeeds with probability $\frac{1}{d^2}$. 
	
	

\subsection{Teleportation-Simulable Channels}\label{subsec-tele_sim}

	

	Let us now consider the even more general protocol depicted in Figure \ref{fig-teleportation_gen}. Let $G$ be a finite group. As before, Alice and Bob start with a shared pair of qudits in the state $\ket{\Phi}_{AB}$, while Alice holds an extra qudit in the state $\rho_{A'}$ to be teleported to Bob's qudit. Unlike the teleportation protocol above, however, Bob applies the channel $\mathcal{N}$ to his qudit before he receives the results of the Bell measurement. Once he receives the measurement results, he applies the unitary operation $V^{g}$ from the set $\{V^{g}:g\in G\}$ of pre-determined unitary operators constituting a projective unitary representation of $G$. 
	
	\begin{figure}
		\centering
		\includegraphics[scale=0.8]{Figures/teleportation_gen.pdf}
		\caption{Circuit diagram of a modified teleportation protocol in which Bob applies a channel $\mathcal{N}$ to his qudit before performing a correction operation $V^g$, which is a unitary operation from the set $\{V^g:g\in G\}$ of unitary operators.}\label{fig-teleportation_gen}
	\end{figure}
	
	The initial tripartite joint state of the protocol is 
	\begin{equation}\label{eq-teleport_gen}
		\rho_{A'}\otimes(\mathbbm{1}_A\otimes\mathcal{N}_B)(\ket{\Phi}\!\bra{\Phi}_{AB}).
	\end{equation}
	Alice performs the same generalized Bell measurement as before on $A$ and $A'$, which we recall has the POVM $\{\Pi_{AA'}^g\}_{g\in G}$ with elements $\Pi_{AA'}^g$ defined in \eqref{eq-G_Bell_meas}. Recall that this POVM corresponds to an irreducible projective unitary representation of $G$ given by $\{U^g\}_{g\in G}$. Since the Bell measurement operates only on the systems $A'$ and $A$, we can bring them inside the action of $\mathcal{N}$ on Bob's share of the state $\ket{\Phi}_{AB}$. This means that the analysis for the qudit teleportation from above carries over exactly in this case. In other words, each outcome $g\in G$ occurs with an equal probability of $\frac{1}{|G|}$, and the post-measurement state on Bob's qudit corresponding to the outcome $g$ is
	\begin{equation}
		\mathcal{N}(U^{g\dagger}\rho U^g).
	\end{equation}
	After Bob applies the unitary $V^g$, the state of Bob's qudit at the end of the protocol is
	\begin{equation}
		V^g\mathcal{N}(U^{g\dagger}\rho U^g)V^{g\dagger}.
	\end{equation}
	This occurs with probability $\frac{1}{|G|}$ for all $g\in G$.
	

	\begin{figure}
		\centering
		\includegraphics[scale=0.8]{Figures/teleportation_gen2.pdf}
		\caption{A mathematically equivalent way of describing the protocol in Figure \ref{fig-teleportation_gen}. In this case, Alice and Bob start with the Choi state $\Phi_{AB}^{\mathcal{N}}$ of the channel $\mathcal{N}$ instead of the maximally entangled state $\ket{\Phi}\!\bra{\Phi}_{AB}$.}\label{fig-teleportation_gen2}
	\end{figure}
	
	Now, observe that the state \eqref{eq-teleport_gen} can be written as
	\begin{equation}
		\rho_{A'}\otimes\Phi_{AB}^{\mathcal{N}},
	\end{equation}
	where we recall that $\Phi_{AB}^{\mathcal{N}}=(\id_A\otimes\mathcal{N}_B)(\ket{\Phi}\!\bra{\Phi}_{AB})$ is the Choi state of the channel $\mathcal{N}$. In other words, the protocol depicted in Figure \ref{fig-teleportation_gen} is mathematically equivalent to the teleportation protocol over a group $G$ outlined above except that instead of starting with the shared maximally entangled state $\ket{\Phi}_{AB}$, Alice and Bob start with the shared state $\Phi_{AB}^{\mathcal{N}}$. This equivalent protocol is depicted in Figure \ref{fig-teleportation_gen2}.
	
		If at the end of the protocol Bob discards the classical message $g$, then the state of his system is given by
	\begin{equation}\label{eq-twirled-channel}
	   \overline{\mathcal{N}}(\rho) \coloneqq \frac{1}{|G|} \sum_{g \in G} V^g\mathcal{N}(U^{g\dagger}\rho U^g)V^{g\dagger}.
	\end{equation}
	This transformation of the channel $\mathcal{N}$ in \eqref{eq-twirled-channel} is known as a \textit{channel twirl} with respect to the unitary representations $\{U^g\}_{g\in G}$ and $\{V^g\}_{g\in G}$, because the twirled channel $\overline{\mathcal{N}}$ is a symmetrized version of the original channel $\mathcal{N}$. Thus, the generalized teleportation protocol gives an explicit procedure for implementing a channel twirl by implementing the teleportation protocol using the Choi state of the channel as the resource state.

	Suppose now that the channel $\mathcal{N}$ satisfies the following property called \textit{group-covariance}:
	
	\begin{definition}{Group-Covariant Channel}{def-group_cov_chan}%\label{def-group_cov_chan}
		Let $G$ be a group. A channel $\mathcal{N}_{A\to B}$ is called \textit{covariant with respect to $G$}, \textit{group-covariant}, \textit{$G$-covariant}, or simply \textit{covariant}, if there exist (projective) unitary representations $\{U_A^g\}_{g\in G}$ and $\{V_B^g\}_{g\in G}$ of $G$ such that for all $\rho_A$,
		\begin{equation}\label{eq-tele_covariant}
			\mathcal{N}_{A\to B}(U_A^g\rho_A U_A^{g\dagger})=V_B^g\mathcal{N}_{A\to B}(\rho_A)V_B^{g\dagger}
		\end{equation}
		for all $g\in G$.
	\end{definition}
	
	\begin{figure}
		\centering
		\includegraphics[scale=0.8]{Figures/teleportation_sim.pdf}
		\caption{Teleportation simulation of a $G$-covariant channel $\mathcal{N}$, where the operators $\{V^g:g\in G\}$ form a unitary representation of $G$ on the output space of $\mathcal{N}$.}\label{fig-teleportation_sim_covariant}
	\end{figure}
	
	We thus see that if $\mathcal{N}$ is $G$-covariant, with the associated unitary representation $\{V^g\}_{g\in G}$ of $G$ at the output of the channel, then for all outcomes $g$ of Alice's generalized Bell measurement we have $\mathcal{N}(U^{g\dagger}\rho U^g)=V^{g\dagger}\mathcal{N}(\rho)V^g$. Therefore, after Bob applies $V^g$, the state of his qudit is $\mathcal{N}(\rho)$. This generalized teleportation protocol therefore effectively applies the channel $\mathcal{N}$ to the state $\rho_{A'}$ and transfers the resulting state to Bob's qudit; see Figure \ref{fig-teleportation_sim_covariant}. We say that the teleportation protocol \textit{simulates} the action of the channel $\mathcal{N}$ on the input state $\rho_{A'}$. As stated earlier, in this sense, the original teleportation protocol can be regarded as a way to simulate the identity channel.
	
	The notion of simulation of a channel by a teleportation protocol can be extended to a one-way LOCC channel $\mathcal{L}^{\rightarrow}$, as introduced in Definition \ref{def-LOCC}, to obtain the following definition.
	
	\begin{figure}
		\centering
		\includegraphics[scale=0.8]{Figures/teleportation_sim_gen.pdf}
		\caption{Depiction of a teleportation-simulable channel with associated resource state $\omega_{RB'}$. The teleportation-simulable channel $\mathcal{N}_{A\to B}$ can be realized via the interaction LOCC channel $\mathcal{L}^{\rightarrow}_{RAB\to B}$ and the resource state $\omega_{RB'}$.}\label{fig-teleportation_sim_gen}
	\end{figure}
	
	\begin{definition}{Teleportation-Simulable Channel}{def-teleportation_sim}%\label{def-teleportation_sim}
		A channel $\mathcal{N}_{A\to B}$ is called \textit{teleportation-simulable} with associated resource state $\omega_{RB}$ if there exists a one-way LOCC channel $\mathcal{L}_{RAB'\to B}^{\rightarrow}$  such that for all input states $\rho_A$
		\begin{equation}\label{eq-teleportation_sim}
			\mathcal{N}(\rho_A)=\mathcal{L}_{RAB'\to B}^{\rightarrow}(\rho_A\otimes \omega_{RB'}).
		\end{equation}
	\end{definition}
	
	Figure \ref{fig-teleportation_sim_gen} illustrates the concept of a teleportation-simulable channel. Note that in \eqref{eq-teleportation_sim} the resource state $\omega_{RB'}$ is fixed, as well as the LOCC channel $\mathcal{L}^{\rightarrow}$. Both sides of the equation should thus be regarded as functions of $\rho_A$. 

	From the discussions above, we conclude that every group-covariant channel is teleportation-simulable, where the one-way LOCC channel $\mathcal{L}$ is simply the teleportation protocol with respect to the group, and the resource state is the Choi state of the channel.
	



\section{Quantum Super-Dense Coding}\label{sec-super_dense_coding}

	We now discuss the quantum super-dense coding protocol. This protocol can be viewed as a ``dual'' to the quantum teleportation protocol in the following sense: while in the basic quantum teleportation protocol, Alice and Bob make use of two qubits in the entangled state $\ket{\Phi^+}=\frac{1}{\sqrt{2}}(\ket{0,0}+\ket{1,1})$ and two bits of classical information to simulate a noiseless qubit channel, in quantum super-dense coding they make use of the shared entangled state $\ket{\Phi^+}$ along with one use of a noiseless qubit channel to communicate \textit{two} bits of classical information. This is remarkable because, without the shared entanglement and only one use of the noiseless qubit channel, they can communicate at most only one bit of classical information. The quantum super-dense coding protocol thus represents one of the simplest examples in which prior shared entanglement provides an advantage for classical communication.
	
	\begin{figure}
		\centering
		\includegraphics[scale=0.8]{Figures/super_dense_coding.pdf}
		\caption{Circuit diagram for the quantum super-dense coding protocol. Using the bits $(z,x)$ that she wishes to send, Alice applies the appropriate Pauli $X$ and/or $Z$ operators to her share of the maximally entangled qubits that are in the state $\ket{\Phi^+}_{AB}$ and sends it through a noiseless qubit channel to Bob. Bob then performs a Bell measurement on the two qubits to recover the encoded bits $(z,x)$.}\label{fig-super_dense_coding}
	\end{figure}
	
	Let us now go through the quantum super-dense coding protocol. See Figure \ref{fig-super_dense_coding} for a depiction of the protocol. Alice wishes to send two classical bits $(z,x)\in\{0,1\}^2$ to Bob by making use of a shared pair of qubits in the maximally entangled state $\ket{\Phi^+}_{AB}$ and one use of a noiseless qubit channel. Depending on the bits she wishes to send, she performs the following operations on her share of the entangled qubits:
	\begin{itemize}
		\item To send the bits $(0,0)$, she does nothing.
		\item To send the bits $(0,1)$, she applies the Pauli $X$ operator to her qubit, transforming the joint state $\ket{\Phi^+}_{AB}$ to $\ket{\Psi^+}_{AB}$.
		\item To send the bits $(1,0)$, she applies the Pauli $Z$ operator to her qubit, transforming the joint state $\ket{\Phi^+}_{AB}$ to $\ket{\Phi^-}_{AB}$.
		\item To send the bits $(1,1)$, she applies the $X$ operator followed by the $Z$ operator, so that the joint state becomes $\ket{\Psi^-}_{AB}$.
	\end{itemize}
	After applying the appropriate operation, Alice sends her qubit to Bob with the one allowed use of a noiseless qubit channel.
	
	Bob now holds both qubits, and they are in one of the four Bell states
	\begin{equation}
		\ket{\Phi_{z,x}}_{AB}=(Z_A^zX_A^x\otimes\mathbbm{1}_B)\ket{\Phi^+}_{AB}
	\end{equation}
	depending on the bits $(z,x)$ Alice sent. Bob then performs a Bell measurement on his two qubits, and the outcome of this measurement consists precisely of the bits $(z,x)$ that Alice wished to send. 
	
	The super-dense coding protocol has a simple generalization to the qudit case. In this case, Alice and Bob share the qudit Bell state $\ket{\Phi}_{AB}$ before communication begins, and by applying one of the $d^2$ Heisenberg--Weyl operators $W_{z,x}$ from \eqref{eq-Heisenberg_Weyl_operators} on her share of the state, Alice can rotate the global state to one of the $d^2$ qudit Bell states in \eqref{eq-qudit_Bell}. After Alice sends her share of the encoded state over a noiseless qudit channel to Bob, Bob can then perform the qudit Bell measurement to decode which of the $d^2$ messages Alice transmitted.


\section{Distinguishability Measures for Quantum States and Channels}\label{sec-dist_measures}

	We conclude this chapter with a discussion of distinguishability measures for quantum states and channels. These measures are important for assessing the quality of performance of various quantum communication protocols. The primary measures for states on which we focus are the trace distance and fidelity, which have compelling operational interpretations.

\subsection{Trace Distance}\label{sec-QM-trace-distance}
	
	The trace distance is based on the trace norm. For two states $\rho$ and $\sigma$, we define the \textit{trace distance between $\rho$ and $\sigma$} as $\frac{1}{2}\norm{\rho-\sigma}_1$. Note that the trace distance between pure states $\ket{\psi}\!\bra{\psi}$ and $\ket{\phi}\!\bra{\phi}$ is given by
	\begin{equation}\label{eq-trace_dist_pure_states}
		\frac{1}{2}\norm{\ket{\psi}\!\bra{\psi}-\ket{\phi}\!\bra{\phi}}_1=\sqrt{1-\abs{\braket{\psi}{\phi}}^2}.
	\end{equation}
	This follows in a straightforward manner by writing $\ket{\phi}$ as
	\begin{equation}
		\ket{\phi}=\alpha\ket{\psi}+\beta\ket{\psi^{\perp}},
	\end{equation}
	where $\ket{\psi^{\perp}}$ is a pure state orthogonal to $\ket{\psi}$, $\alpha=\braket{\psi}{\phi}$, and $|\alpha|^2+|\beta|^2=1$. Then, as a matrix in the basis $\{\ket{\psi},\ket{\psi^{\perp}}\}$, we have that
	\begin{equation}
		\ket{\psi}\!\bra{\psi}-\ket{\phi}\!\bra{\phi}=
		\begin{pmatrix}
		1-|\alpha|^2 & - \alpha \conj{\beta} \\
		-\conj{\alpha}\beta & -|\beta|^2
		\end{pmatrix},
	\end{equation}
	which has eigenvalues $\pm|\beta|=\pm\sqrt{1-|\alpha|^2}$. Therefore, recalling that the trace norm of a Hermitian operator is the sum of the absolute value of its eigenvalues, we conclude \eqref{eq-trace_dist_pure_states}.
	
	
	The trace distance provides a natural way to measure the distance between two quantum states $\rho$ and $\sigma$, and to assess the performance of a quantum information processing protocol in which the ideal state to be generated is $\rho$ but the actual state generated is $\sigma$. To see that this is the case, suppose that a third party is trying to assess how distinguishable the actual state $\sigma$ is from the ideal state $\rho$. Such an individual can do so by performing a quantum measurement described by the POVM $\{\Lambda_{x}\}_{x}$. The probability of obtaining a particular outcome $x$ is given by the Born rule. In the case that $\rho$ was prepared, this probability is $\Tr[\Lambda_{x}\rho]$, and in the case that $\sigma$ was prepared, this probability is $\Tr[\Lambda_{x}\sigma]$. What we demand is that the absolute deviation between the actual probability $\Tr[\Lambda_{x}\sigma]$ and the ideal probability $\Tr[\Lambda_{x}\rho]$ be no larger than some tolerance $\varepsilon$. Since this should be the case for every possible measurement outcome, what we demand mathematically is that
	\begin{equation}
		\sup_{0\leq\Lambda\leq \mathbbm{1}}\left\vert \operatorname{Tr}[\Lambda\rho] - \operatorname{Tr}[\Lambda\sigma]\right\vert \leq\varepsilon.
	\end{equation}
	As stated in Theorem~\ref{thm-trace_dist_meas} below, the following identity holds
	\begin{equation}\label{eq-trace_dist_variational1}
		\sup_{0\leq\Lambda\leq \mathbbm{1}}\left\vert \Tr[\Lambda\rho]-\operatorname{Tr}[\Lambda\sigma]\right\vert =\frac{1}{2}\left\Vert \rho-\sigma\right\Vert _{1},
	\end{equation}
	indicating that if $\frac{1}{2}\left\Vert \rho-\sigma\right\Vert _{1}\leq \varepsilon$, then the deviation between probabilities for every possible measurement operator never exceeds $\varepsilon$, so that the approximation between states $\rho$ and $\sigma$ is naturally quantified by the trace distance $\frac{1}{2}\norm{\rho-\sigma}_{1}$.
	
	Let us now prove the variational characterization of the trace distance stated in \eqref{eq-trace_dist_variational1}.
	
	\begin{theorem*}{Trace Distance via Measurement}{thm-trace_dist_meas}
		For two states $\rho$ and $\sigma$, the following equality holds
		\begin{equation}\label{eq-trace_dist_meas}
			\frac{1}{2}\norm{\rho-\sigma}_1=\sup_{0\leq\Lambda\leq\mathbbm{1}}\left|\Tr\!\left[\Lambda(\rho-\sigma)\right]\right|.
		\end{equation}
		An optimal measurement operator $\Lambda$ is equal to $\Pi_+ + \Lambda_0$, where $\Pi_+$ is the projection onto the strictly positive part of $\rho-\sigma$ and $\Lambda_0$ is an operator satisfying $0 \leq \Lambda_0 \leq \Pi_0$, with $\Pi_0$ the projection onto the zero eigenspace of $\rho-\sigma$.
	\end{theorem*}
	
	\begin{Proof}
	Consider that
	\begin{equation}
	\sup_{0\leq\Lambda\leq\mathbbm{1}}\left|\Tr\!\left[\Lambda(\rho-\sigma)\right]\right|
	= \sup_{0\leq\Lambda\leq\mathbbm{1}}\Tr\!\left[\Lambda(\rho-\sigma)\right],
	\end{equation}
	because there are always choices for $\Lambda$ such that $\Tr\!\left[\Lambda(\rho-\sigma)\right]\geq 0$.
	Then the equality follows as a direct application of \eqref{eq-Holevo_Helstrom-alt} and the optimality statement following it, with $A=\rho$ and $B=\sigma$.
	\end{Proof}
	
	From the expression in \eqref{eq-trace_dist_meas}, it is clear that the trace distance can be computed via a semi-definite program (SDP). The following proposition states this fact formally and also states the dual optimization problem. Appendix~\ref{app-trace_dist_fidelity_SDP} provides a proof.
	
		\begin{proposition*}{SDPs for Normalized Trace Distance}{prop-trace_dist_SDP}
		The trace distance between any two quantum states $\rho$ and $\sigma$ can be written as the following semi-definite programs:
		\begin{align}
			\frac{1}{2}\norm{\rho-\sigma}_1&=\sup_{\Lambda\geq 0}\{\Tr[\Lambda(\rho-\sigma)]:\Lambda\leq\mathbbm{1}\}\label{eq-trace_dist_SDP_primal}\\
			&=\inf_{Z\geq 0}\{\Tr[Z]:Z\geq \rho-\sigma\}.\label{eq-trace_dist_SDP_dual}
		\end{align}
	\end{proposition*}

	
	The trace distance is non-increasing under the action of a  quantum channel (and more generally, positive, trace-preserving maps).
	
	\begin{theorem*}{Data-Processing Inequality for Trace Distance}{thm-trace_dist_monotone}
		Let $\rho$ and $\sigma$ be states, and let $\mathcal{N}$ be a positive, trace-preserving map. Then,
		\begin{equation}\label{eq-trace_dist_monotone-PTNI}
			\norm{\rho-\sigma}_1\geq \norm{\mathcal{N}(\rho)-\mathcal{N}(\sigma)}_1.
		\end{equation}
	\end{theorem*}
	
	\begin{Proof}
		Using the definition of the adjoint $\mathcal{N}^\dagger$ of $\mathcal{N}$, for every measurement operator $0\leq\Lambda'\leq\mathbbm{1}$, we find that
		\begin{equation}
			\Tr[\Lambda'(\mathcal{N}(\rho)-\mathcal{N}(\sigma))]=\Tr[\mathcal{N}^\dagger(\Lambda')(\rho-\sigma)].
		\end{equation}
		Now, since $\mathcal{N}$ is a positive map, so is $\mathcal{N}^{\dagger}$, which means that $\mathcal{N}^\dagger(\Lambda')\geq 0$. Furthermore, since $\mathcal{N}$ is trace preserving, the adjoint $\mathcal{N}^\dagger$ is unital. This, along with $\Lambda'\leq\mathbbm{1}$, means that 
		\begin{equation}
			\mathcal{N}^\dagger(\mathbbm{1}-\Lambda')\geq 0\Rightarrow \mathcal{N}^\dagger(\Lambda')\leq\mathcal{N}^\dagger(\mathbbm{1})=\mathbbm{1}.
		\end{equation}
		In other words, $0\leq\mathcal{N}^\dagger(\Lambda')\leq\mathbbm{1}$. Therefore,
		\begin{equation}
			\Tr[\mathcal{N}^\dagger(\Lambda')(\rho-\sigma)]\leq\sup_{0\leq\Lambda\leq\mathbbm{1}}\Tr[\Lambda(\rho-\sigma)]=\frac{1}{2}\norm{\rho-\sigma}_1,
		\end{equation}
		where  the equality follows from Theorem~\ref{thm-trace_dist_meas}. Since $\Lambda'$ was arbitrary, we find that
		\begin{equation}
			\sup_{0\leq\Lambda'\leq\mathbbm{1}}\Tr[\Lambda'(\mathcal{N}(\rho)-\mathcal{N}(\sigma))]\leq\frac{1}{2}\norm{\rho-\sigma}_1,
		\end{equation}
		from which the result follows since the left-hand side of the inequality is equal to $\frac{1}{2}\norm{\mathcal{N}(\rho)-\mathcal{N}(\sigma)}_1$ by Theorem~\ref{thm-trace_dist_meas}.
	\end{Proof}
	
	The data-processing inequality for the trace distance tells us that for the task of state discrimination (see Section \ref{subsec-state_discrimination}), applying a channel to the states $\rho$ and $\sigma$ before performing the measurement can never exceed the performance (as quantified by the success probability) of measuring $\rho$ and $\sigma$ directly.
	
	More general than Proposition~\ref{prop-trace_dist_SDP} and Theorem~\ref{thm-trace_dist_monotone}, the following proposition holds, which we state here without proof:
	
	\begin{proposition*}{Trace Norm for Hermitian Operators}{prop:QM-over:trace-norm-herm-ops}
	Let $A$ be a Hermitian operator. Then
	\begin{align}
	\norm{A}_1 & = \sup_{\Lambda_1,\Lambda_2 \geq 0} \{\Tr[(\Lambda_1 - \Lambda_2) A] : \Lambda_1,\Lambda_2 \leq \mathbbm{1} \}\\
	& = \inf_{Y_1, Y_2 \geq 0} \{ \Tr[Y_1+Y_2] : Y_1\geq A, Y_2 \geq -A\}.
	\label{eq:MT:trace-norm-herm-op-dual}
	\end{align}
	Let $\mathcal{N}$ be a positive, trace-preserving map. Then
	\begin{equation}
	\norm{A}_1 \geq \norm{\mathcal{N}(A)}_1.
	\end{equation}
	\end{proposition*}
	
	
	
	By combining the results of Theorems~\ref{thm-trace_dist_meas} and \ref{thm-trace_dist_monotone}, we find that the trace distance is achieved by a measurement channel:
	
	\begin{theorem*}{Trace Distance Achieved by Measurement Channel}{thm-trace_dist_ach_by_meas_channel}
		For two states $\rho$ and $\sigma$, the following equality holds
		\begin{equation}
			\norm{\rho-\sigma}_1=\max_{\{\Lambda_x\}_x}\sum_{x\in\mathcal{X}}\abs{\Tr[\Lambda_x\rho]-\Tr[\Lambda_x\sigma]},
		\end{equation}
		where the optimization is performed over POVMs $\{\Lambda_x\}_{x\in\mathcal{X}}$ defined with respect to a finite alphabet $\mathcal{X}$, and an optimal POVM is given by $\{\Lambda^*, \mathbbm{1} - \Lambda^*\}$, where $\Lambda^* = \Pi_+ + \Lambda_0$, the projection $\Pi_+$ is the projection onto the strictly positive part of $\rho-\sigma$, and $\Lambda_0$ satisfies $0 \leq \Lambda_0 \leq \Pi_0$, with $\Pi_0$ the projection onto the zero eigenspace of $\rho-\sigma$.
	\end{theorem*}
	
	\begin{Proof}
	The inequality
	\begin{equation}
	\norm{\rho-\sigma}_1 \geq\max_{\{\Lambda_x\}_x}\sum_{x\in\mathcal{X}}\abs{\Tr[\Lambda_x\rho]-\Tr[\Lambda_x\sigma]}
	\end{equation}
	follows from Theorem~\ref{thm-trace_dist_monotone} by taking the channel $\mathcal{N}$ to be the quantum--classical channel defined as $\mathcal{N}(\omega)= \sum_{x \in \mathcal{X}} \Tr[\Lambda_x \omega] \ket{x}\!\bra{x}$. Then, from Theorem~\ref{thm-trace_dist_meas}, we have the equality
	\begin{equation}
	\frac{1}{2} \norm{\rho-\sigma}_1 = |\Tr[\Lambda^*(\rho -\sigma)]|.
	\end{equation}
	Since $|\Tr[\Lambda^*(\rho -\sigma)]|=|\Tr[(\mathbbm{1}-\Lambda^*)(\rho -\sigma)]|$, we conclude that
	\begin{equation}
	\norm{\rho-\sigma}_1 = |\Tr[\Lambda^*(\rho -\sigma)]| + |\Tr[(\mathbbm{1}-\Lambda^*)(\rho -\sigma)]|,
	\end{equation}
	so that an optimal POVM is given by $\{\Lambda^*, \mathbbm{1} - \Lambda^*\}$.
	\end{Proof}
	
	

\subsection{Fidelity}\label{subsec-fidelity}

	In addition to the trace distance, another distinguishability measure for states that we consider in this book is the fidelity (also called Uhlmann fidelity).
	
	\begin{definition}{Fidelity}{def-fidelity}
		For two quantum states $\rho$ and $\sigma$, the \textit{fidelity between $\rho$ and $\sigma$}, denoted by $F(\rho,\sigma)$, is defined as
		\begin{equation}
			F(\rho,\sigma)\coloneqq \norm{\sqrt{\rho}\sqrt{\sigma}}_1^2=\left(\Tr\!\left[\sqrt{\smash[b]{\sqrt{\smash[b]{\sigma}}\rho\sqrt{\smash[b]{\sigma}}}}\right]\right)^2.
		\end{equation}
	\end{definition}
	
	Observe that the fidelity is symmetric in its arguments. We also have that $F(\rho,\sigma)\in[0,1]$ for all states $\rho$ and $\sigma$, a fact that we prove below. 
	
	For a pure state $\ket{\psi}$ and mixed state $\rho$, the fidelity between them is equal to
	\begin{equation}\label{eq-fidelity_pure_mixed}
		F(\rho,\ket{\psi}\!\bra{\psi})=\bra{\psi}\rho\ket{\psi}=\Tr[\ket{\psi}\!\bra{\psi}\rho].
	\end{equation}
	Also, for two pure states $\ket{\psi}$ and $\ket{\phi}$, the fidelity is simply 
	\begin{equation}\label{eq-fidelity_pure_pure}
		F(\ket{\psi}\!\bra{\psi},\ket{\phi}\!\bra{\phi})=\abs{\braket{\psi}{\phi}}^2.
	\end{equation}
	
	The formula in \eqref{eq-fidelity_pure_mixed} gives the fidelity an operational meaning that we employ in later chapters. Suppose that the goal of a quantum information processing protocol is to produce the pure state $\ket{\psi}\!\bra{\psi}$, but it instead produces a mixed state $\rho$. Then the fidelity $F(\rho,\ket{\psi}\!\bra{\psi})$ is equal to the probability that the actual state $\rho$ passes a test for being the ideal state $\ket{\psi}\!\bra{\psi}$, with the test being given by the POVM $\{\ket{\psi}\!\bra{\psi}, \mathbbm{1} -\ket{\psi}\!\bra{\psi}\}$. That is, the probability of obtaining the first outcome of the measurement (i.e., ``success'') is equal to $F(\rho,\ket{\psi}\!\bra{\psi})$. In this way, the fidelity provides another natural way for assessing the performance of quantum information processing protocols.
	
	Like the trace distance, the fidelity can  be computed via a semi-definite program, as stated in the following proposition:
	\begin{proposition*}{SDPs for Root Fidelity of States}{prop:QM-over:SDP-fidelity-states}
	The root fidelity $\sqrt{F}(\rho
,\sigma)=\left\Vert \sqrt{\rho}\sqrt{\sigma}\right\Vert _{1}$\ of quantum
states $\rho$ and $\sigma$ is characterized by the following primal and dual
semi-definite programs:%
\begin{align}
\sqrt{F}(\rho,\sigma)  & =\frac{1}{2}\sup_{X\in\mathcal{L}(\mathcal{H}%
)}\left\{  \operatorname{Tr}[X]+\operatorname{Tr}[X^{\dag}]:%
\begin{pmatrix}
\rho & X\\
X^{\dag} & \sigma
\end{pmatrix}
\geq0\right\}  \label{eq:QM-over:fidelity-primal-SDP}\\
& =\frac{1}{2}\inf_{Y,Z\geq 0}\left\{  \operatorname{Tr}[Y\rho]+\operatorname{Tr}%
[Z\sigma]:%
\begin{pmatrix}
Y & \mathbbm{1}\\
\mathbbm{1} & Z
\end{pmatrix}
\geq0\right\}  \label{eq:QM-over:fidelity-dual-SDP}%
\end{align}
	\end{proposition*}
	
	\begin{Proof}
	See Appendix \ref{app:QM-over:SDP-fid-states}.
	\end{Proof}
	
	\begin{theorem*}{Basic Properties of Fidelity}{thm-fidelity_properties}
		\begin{enumerate}
			\item For two states $\rho$ and $\sigma$, the inequalities $0\leq F(\rho,\sigma)\leq 1$ hold. Furthermore, $F(\rho,\sigma)=1$ if and only if $\rho=\sigma$, and $F(\rho,\sigma)=0$ if and only if $\rho$ and $\sigma$ are supported on orthogonal subspaces.
			
			\item\textit{Isometric invariance}: For all states $\rho$ and $\sigma$, and for every isometry~$V$,
				\begin{equation}
					F(\rho,\sigma)=F(V\rho V^\dagger,V\sigma V^\dagger).
				\end{equation}
			
			\item\textit{Multiplicativity}: The fidelity is multiplicative with respect to tensor-product states, meaning that for all states $\rho_1,\sigma_1,\rho_2,\sigma_2$, we have
				\begin{equation}\label{eq-fidelity_multiplicative}
					F(\rho_1\otimes\rho_2,\sigma_1\otimes\sigma_2)=F(\rho_1,\sigma_1)F(\rho_2,\sigma_2).
				\end{equation}
	
			%\item\textit{Direct-sum property}: Let $p,q:\mathcal{X}\to[0,1]$ be probability distributions on a finite alphabet $\mathcal{X}$ with associated $|\mathcal{X}|$-dimensional system $X$, and let $\{\rho_A^x:x\in\mathcal{X}\}$ and $\{\sigma_A^x:x\in\mathcal{X}\}$ be sets of states. Then,
			%	\begin{multline}
			%		\sqrt{F}\!\left(\sum_{x\in\mathcal{X}}p(x)\ket{x}\!\bra{x}_X\otimes\rho_A^x,\sum_{x\in\mathcal{X}}q(x)\ket{x}\!\bra{x}_X\otimes\sigma_A^x\right)\\
			%		=\sum_{x\in\mathcal{X}}\sqrt{p(x)q(x)}\sqrt{F}(\rho_A^x,\sigma_A^x).
			%	\end{multline}
		\end{enumerate}
	\end{theorem*}
	
	\begin{Proof}
		\hfill\begin{enumerate}
			\item The fact that $F(\rho,\sigma)\geq 0$ for all states $\rho$ and $\sigma$ follows from the definition of the fidelity as the squared trace norm and the fact that the trace norm is always non-negative. If $\rho$ and $\sigma$ are supported on orthogonal subspaces, then $\sqrt{\rho}\sqrt{\sigma}=0$, which means that $F(\rho,\sigma)=0$. Conversely, if $F(\rho,\sigma)=0$, then $\norm{\sqrt{\rho}\sqrt{\sigma}}_1=0$, which implies (by definition of a norm) that $\sqrt{\rho}\sqrt{\sigma}=0$, which in turn implies that $\rho$ and $\sigma$ are supported on orthogonal subspaces.
			
			Now, using \eqref{eq-trace_norm_variational}, there exists a unitary $U$ such that
			\begin{equation}
				F(\rho,\sigma)=\norm{\sqrt{\rho}\sqrt{\sigma}}_1^2=\abs{\Tr[U\sqrt{\rho}\sqrt{\sigma}]}^2.
			\end{equation}
			Then, using the Cauchy--Schwarz inequality for the Hilbert--Schmidt inner product (see \eqref{eq-Cauchy_Schwarz_HS}), we find that
			\begin{align}
				F(\rho,\sigma)&=\abs{\Tr[U\sqrt{\rho}\sqrt{\sigma}]}^2\\
				&\leq \Tr[U\sqrt{\rho}\sqrt{\rho}U^\dagger]\Tr[\sqrt{\sigma}\sqrt{\sigma}]\\
				&=\Tr[\sqrt{\rho}\sqrt{\rho}]\Tr[\sqrt{\sigma}\sqrt{\sigma}]\\
				&=\Tr[\rho]\Tr[\sigma]\\
				&=1.
			\end{align}
			If $\rho=\sigma$, then $F(\rho,\sigma)=\norm{\rho}_1^2=\Tr[\rho]^2=1$. On the other hand, if $F(\rho,\sigma)=1$, then the inequality in the Cauchy--Schwarz inquality is saturated. The Cauchy--Schwarz inequality is saturated if and only if the two operators involved are proportional to each other. This means that $\rho=\alpha\sigma$ for some $\alpha>0$. But since both $\rho$ and $\sigma$ are states, it must be the case that $\alpha=1$, which means that $\rho=\sigma$.
			
			\item \textit{Proof of isometric invariance}: For every isometry $V$ and every two states $\rho$ and $\sigma$, since the action of an isometry does not change the eigenvalues, we have that $\sqrt{V\rho V^\dagger}=V\sqrt{\rho}V^\dagger$ and $\sqrt{V\sigma V^\dagger}=V\sqrt{\sigma}V^\dagger$. Therefore,
				\begin{align}
					F(V\rho V^\dagger,V\sigma V^\dagger)&=\norm{\sqrt{V\rho V^\dagger}\sqrt{V\sigma V^\dagger}}_1^2\\
					&=\norm{V\sqrt{\rho}V^\dagger V\sqrt{\sigma}V^\dagger}_1^2\\
					&=\norm{V\sqrt{\rho}\sqrt{\sigma}V^\dagger}_1^2\\
					&=\norm{\sqrt{\rho}\sqrt{\sigma}}_1^2,
				\end{align}
				as required, where the last line is due to the isometric invariance of the Schatten norms, as stated in \eqref{eq-Schatten_norm_iso_invar}.
				
			\item\textit{Proof of multiplicativity}: Using the fact that $\sqrt{\rho_1\otimes\rho_2}=\sqrt{\rho_1}\otimes\sqrt{\rho_2}$, and similarly for $\sqrt{\sigma_1\otimes\sigma_2}$, and using the multiplicativity of the trace norm with respect to the tensor product (see \eqref{eq-Schatten_norm_mult}), we find that
				\begin{align}
					F(\rho_1\otimes\rho_2,\sigma_1\otimes\sigma_2)&=\norm{\sqrt{\rho_1\otimes\rho_2}\sqrt{\sigma_1\otimes\sigma_2}}_1^2\\
					&=\norm{(\sqrt{\rho_1}\otimes\sqrt{\rho_2})(\sqrt{\sigma_1}\otimes\sqrt{\sigma_2})}_1^2\\
					&=\norm{\sqrt{\rho_1}\sqrt{\sigma_1}\otimes\sqrt{\rho_2}\sqrt{\sigma_2}}_1^2\\
					&=\norm{\sqrt{\rho_1}\sqrt{\sigma_1}}_1^2\norm{\sqrt{\rho_2}\sqrt{\sigma_2}}_1^2\\
					&=F(\rho_1,\sigma_1)F(\rho_2,\sigma_2),
				\end{align}
				as required. \qedhere 
		\end{enumerate}
	\end{Proof}
	
%\begin{comment}
%\item\textit{Proof of the direct-sum property}: It holds that
%				\begin{equation}
%					\sqrt{\sum_{x\in\mathcal{X}}p(x)\ket{x}\!\bra{x}_X\otimes\rho_A^x}=\sum_{x\in\mathcal{X}}\sqrt{p(x)}\ket{x}\!\bra{x}_X\otimes\sqrt{\rho_A^x},
%				\end{equation}
%				and similarly for $\sqrt{\sum_{x\in\mathcal{X}}q(x)\ket{x}\!\bra{x}_X\otimes\sigma_A^X}$. This is due to the fact that a classical--quantum state can be viewed as a block-diagonal matrix, as shown in \eqref{eq-cq_state_block_diag}, and the square root of any such matrix is given by the block-diagonal matrix composed of the square roots of the blocks of the original matrix. Therefore,
%				\begin{align}
%					&\sqrt{F}\!\left(\sum_{x\in\mathcal{X}}p(x)\ket{x}\!\bra{x}_X\otimes\rho_A^x,\sum_{x\in\mathcal{X}}q(x)\ket{x}\!\bra{x}_X\otimes\sigma_A^x\right)\nonumber\\
%					&\quad =\norm{\sqrt{\sum_{x\in\mathcal{X}}p(x)\ket{x}\!\bra{x}_X\otimes\rho_A^x}\sqrt{\sum_{x\in\mathcal{X}}q(x)\ket{x}\!\bra{x}_X\otimes\sigma_A^x}}_1\\
%					&\quad =\norm{\left(\sum_{x\in\mathcal{X}}\sqrt{p(x)}\ket{x}\!\bra{x}_X\otimes\sqrt{\rho_A^x}\right)\left(\sum_{x\in\mathcal{X}}\sqrt{q(x)}\ket{x}\!\bra{x}_X\otimes\sqrt{\sigma_A^x}\right)}_1\\
%					&\quad =\norm{\sum_{x\in\mathcal{X}}\sqrt{p(x)q(x)}\ket{x}\!\bra{x}_X\otimes\sqrt{\rho_A^x}\sqrt{\sigma_A^x}}_1.
%				\end{align}
%				Now, we use the property in \eqref{eq-trace_norm_blkdiag}, which, like before, tells us that the trace norm of a block-diagonal matrix is simply the sum of the trace norm of the individual blocks. Therefore,
%				\begin{multline}
%					\sqrt{F}\!\left(\sum_{x\in\mathcal{X}}p(x)\ket{x}\!\bra{x}_X\otimes\rho_A^x,\sum_{x\in\mathcal{X}}q(x)\ket{x}\!\bra{x}_X\otimes\sigma_A^x\right)\\
%					\sum_{x\in\mathcal{X}}\sqrt{p(x)}\sqrt{q(x)}\sqrt{F}(\rho_A^x,\sigma_A^x),
%				\end{multline}
%				as required.
%\end{comment}	


	\begin{theorem*}{Uhlmann's Theorem}{thm-Uhlmann_fidelity}
		For two quantum states $\rho_A$ and $\sigma_A$, let $\ket{\psi^{\rho}}\coloneqq(\mathbbm{1}_R\otimes\sqrt{\rho}_A)\ket{\Gamma}_{RA}$ and $\ket{\psi^{\sigma}}\coloneqq(\mathbbm{1}_R\otimes\sqrt{\sigma_A})\ket{\Gamma}_{RA}$ be purifications of $\rho$ and $\sigma$, respectively, with the dimension of $R$ equal to the dimension of $A$. Then,
		\begin{equation}\label{eq-Uhlmann_fidelity}
			F(\rho,\sigma)=\max_{U_R}\abs{\bra{\psi^{\rho}}_{RA}(U_R\otimes\mathbbm{1}_A)\ket{\psi^{\sigma}}_{RA}}^2,
		\end{equation}
		where the optimization is over unitaries on $R$.
	\end{theorem*}
	
	\begin{remark}
		Since all purifications are related to each other by isometries on the purifying system (which is the system $R$ as in the statement of the theorem), Uhlmann's theorem tells us that the fidelity between two quantum states is equal to the maximum overlap between their purifications.
		
		Furthermore, it is straightforward to show that it suffices to take the dimension of $R$ the same as the dimension of $A$, as we have done in the statement of the theorem. In other words, performing an optimization over the dimension of $R$ leads to the same result as in \eqref{eq-Uhlmann_fidelity}.
	\end{remark}
	
	\begin{Proof}
		Using the definitions of $\ket{\psi^{\rho}}_{RA}$ and $\ket{\psi^{\sigma}}_{RA}$, we find for every unitary $U_R$ that
		\begin{align}
			&\abs{\bra{\psi^{\rho}}_{RA}(U_R\otimes\mathbbm{1}_A)\ket{\psi^{\sigma}}_{RA}}^2\nonumber\\
			&\quad=\abs{\bra{\Gamma}_{RA}(\mathbbm{1}_R\otimes\sqrt{\rho_A})(U_R\otimes\mathbbm{1}_A)(\mathbbm{1}_R\otimes\sqrt{\sigma_A})\ket{\Gamma}_{RA}}^2\\
			&\quad=\abs{\bra{\Gamma}_{RA}(U_R\otimes\sqrt{\rho_A}\sqrt{\sigma_A})\ket{\Gamma}_{RA}}^2\\
			&\quad=\abs{\bra{\Gamma}_{RA}(\mathbbm{1}_R\otimes\sqrt{\rho_A}\sqrt{\sigma_A}U_A^{\t})\ket{\Gamma_{RA}}}^2,
		\end{align}
		where  the last line follows from the transpose trick in \eqref{eq-transpose_trick}. Then, using \eqref{eq-trace_identity}, we find that
		\begin{equation}
			\abs{\bra{\psi^{\rho}}_{RA}(U_R\otimes\mathbbm{1}_A)\ket{\psi^{\sigma}}_{RA}}^2=\abs{\Tr[\sqrt{\rho_A}\sqrt{\sigma_A}U_A^{\t}]}^2.
		\end{equation}
		Since $U_A$ is arbitrary, and $U_A^{\t}$ is also a unitary, we use \eqref{eq-trace_norm_variational} to obtain
		\begin{align}
			\max_U\abs{\bra{\psi^{\rho}}_{RA}(U_R\otimes\mathbbm{1}_A)\ket{\psi^{\sigma}}_{RA}}^2&=\max_U\abs{\Tr[\sqrt{\rho_A}\sqrt{\sigma_A}U_A^{\t}]}^2\\
			&=\max_U\abs{\Tr[\sqrt{\rho_A}\sqrt{\sigma_A}U_A]}^2\\
			&=\norm{\sqrt{\rho_A}\sqrt{\sigma_A}}_1^2
		\end{align}
		as required.
	\end{Proof}
	
	\begin{theorem*}{Data-Processing Inequality for Fidelity}{thm-fidelity_monotone}
		Let $\rho$ and $\sigma$ be states, and let $\mathcal{N}$ be a quantum channel. Then,
		\begin{equation}
			F(\rho,\sigma)\leq F(\mathcal{N}(\rho),\mathcal{N}(\sigma)).
		\end{equation}
	\end{theorem*}
	
	\begin{Proof}
		Recall that every quantum channel $\mathcal{N}_{A\to B}$ can be written in the Stinespring form as $\mathcal{N}_{A\to B}(\rho_A)=\Tr_E[V\rho_A V^\dagger]$, where $V\equiv V_{A\to BE}$ is some isometric extension of $\mathcal{N}$ and $d_E\leq \rank(\Gamma^{\mathcal{N}}_{AB})$. Since we have shown that the fidelity is invariant under isometric channels, it remains to show that the fidelity is non-decreasing under the action of the partial trace. To this end, consider bipartite states $\rho_{AB}$ and $\sigma_{AB}$, and let $\ket{\psi}_{RAB}$ be an arbitrary purification of $\rho_{AB}$ and let $\ket{\phi}_{RAB}$ be an arbitrary purification of $\sigma_{AB}$, where $d_R=d_Ad_B$. Observe that $\ket{\psi}_{RAB}$ and $\ket{\phi}_{RAB}$ are also purifications of $\rho_A=\Tr_B[\rho_{AB}]$ and $\sigma_A=\Tr_B[\sigma_{AB}]$, respectively. Then, by Uhlmann's theorem, we have that
		\begin{equation}
			F(\rho_A,\sigma_A)=\max_{U_{RB}}\abs{\bra{\psi}_{RAB}(U_{RB}\otimes\mathbbm{1}_A)\ket{\phi_{RAB}}}^2.
		\end{equation}
		By restricting the maximization above to unitaries of the form $U_R\otimes\mathbbm{1}_B$, we have that
		\begin{equation}
			F(\rho_A,\sigma_A)\geq \abs{\bra{\psi}_{RAB}(U_R\otimes\mathbbm{1}_{AB})\ket{\phi}_{RAB}}^2
		\end{equation}
		for all unitaries $U_R$. Therefore,
		\begin{equation}
        \max_{U_R}\abs{\bra{\psi}_{RAB}(U_R\otimes\mathbbm{1}_{AB})\ket{\phi}_{RAB}}^2	\leq \max_{U_{RB}}\abs{\bra{\psi}_{RAB}(U_{RB}\otimes\mathbbm{1}_A)\ket{\phi}_{RAB}}^2.
		\end{equation}
		But, by Uhlmann's theorem,
		\begin{equation}
			\max_{U_R}\abs{\bra{\psi}_{RAB}(U_R\otimes\mathbbm{1}_{AB})\ket{\phi}_{RAB}}^2=F(\rho_{AB},\sigma_{AB}).
		\end{equation}
		Therefore,
		\begin{equation}
			F(\rho_{AB},\sigma_{AB})\leq F(\rho_A,\sigma_A)=F(\Tr_B[\rho_{AB}],\Tr_B[\sigma_{AB}]).
		\end{equation}
		The fidelity thus satisfies the data-processing inequality with respect to the partial trace.
		
		Using the data-processing inequality for the fidelity with respect to the partial trace, along with its invariance under isometries, we conclude that
		\begin{align}
			F(\mathcal{N}(\rho),\mathcal{N}(\sigma))&=F\!\left(\Tr_E[V\rho V^\dagger],\Tr_E[V\rho V^\dagger]\right)\\
			&\geq F(V\rho V^\dagger,V\sigma V^\dagger)\\
			&=F(\rho,\sigma),
		\end{align}
		as required.
	\end{Proof}
	
	With Uhlmann's theorem and the data-processing inequality for the fidelity in hand, we can now establish two more properties of the fidelity.
	
	\begin{theorem*}{Concavity of Fidelity}{thm-fidelity_concave}
		The fidelity is concave in either one of its arguments:
		\begin{equation}\label{eq-fidelity_concave}
			F\!\left(\sum_{x\in\mathcal{X}}p(x)\rho^x,\sigma\right)\geq \sum_{x\in\mathcal{X}}p(x)F(\rho^x,\sigma),
		\end{equation}
		where $\mathcal{X}$ is a finite alphabet, $p:\mathcal{X}\to[0,1]$ is a probability distribution, and $\sigma$ and $\{\rho^x\}_{x\in\mathcal{X}}$ are states.
	\end{theorem*}
	
	\begin{Proof}
		By Uhlmann's theorem, we know that the fidelity is given by the maximum overlap between the purifications of the two states under consideration. Based on this, let $\ket{\psi^{\sigma}}_{RA}$ be a purification of $\sigma_A$. Then, for $x\in\mathcal{X}$, let $\ket{\phi^x}_{RA}$ be a purification of $\rho_A^x$ such that $F(\rho_A^x,\sigma)=\abs{\braket{\phi^x}{\psi^{\sigma}}}^2$. Then,
		\begin{align}
			\sum_{x\in\mathcal{X}}p(x)F(\rho_A^x,\sigma_A)&=\sum_{x\in\mathcal{X}}p(x)\abs{\braket{\phi^x}{\psi^{\sigma}}}^2\\
			&=\bra{\psi^{\sigma}}_{RA}\left(\sum_{x\in\mathcal{X}}p(x)\ket{\phi^x}\!\bra{\phi^x}_{RA}\right)\ket{\psi^{\sigma}}_{RA}\\
			&=F\!\left(\sum_{x\in\mathcal{X}}p(x)\ket{\phi^x}\!\bra{\phi^x}_{RA},\ket{\psi^{\sigma}}\!\bra{\psi^{\sigma}}_{RA}\right),
		\end{align}
		where  the last line follows from the formula in \eqref{eq-fidelity_pure_mixed} for the fidelity between a pure state and a mixed state. Then, using the data-processing inequality for the fidelity with respect to the partial trace, we obtain
		\begin{align}
			\sum_{x\in\mathcal{X}}p(x)F(\rho_A^x,\sigma_A)&=F\!\left(\sum_{x\in\mathcal{X}}p(x)\ket{\phi^x}\!\bra{\phi^x}_{RA},\ket{\psi^{\sigma}}\!\bra{\psi^{\sigma}}_{RA}\right)\\
			&\leq F\!\left(\sum_{x\in\mathcal{X}}p(x)\Tr_R[\ket{\phi^x}\!\bra{\phi^x}_{RA}],\Tr_R[\ket{\psi^{\sigma}}\!\bra{\psi^{\sigma}}_{RA}]\right)\\
			&=F\!\left(\sum_{x\in\mathcal{X}}p(x)\rho_A^x,\sigma_A\right),
		\end{align}
		which is the required result.
	\end{Proof}
	
	A more general result than the concavity result proved above, namely \textit{joint concavity}, can be obtained if we consider instead the square root of the fidelity, which we call the ``root fidelity'' and denote by
	\begin{equation}
		\sqrt{F}(\rho,\sigma)\coloneqq\sqrt{F(\rho,\sigma)}=\norm{\sqrt{\rho}\sqrt{\sigma}}_1.
	\end{equation}
	
	\begin{theorem*}{Joint Concavity of Root  Fidelity}{thm-joint_concave_sqrt_fid}
		The root fidelity is jointly concave:
		\begin{equation}
			\sqrt{F}\!\left(\sum_{x\in\mathcal{X}}p(x)\rho^x,\sum_{x\in\mathcal{X}}p(x)\sigma^x\right)\geq\sum_{x\in\mathcal{X}}p(x)\sqrt{F}(\rho^x,\sigma^x),
			\label{eq-joint-concave-root-fidelity}
		\end{equation}
		where $\mathcal{X}$ is a finite alphabet, $p:\mathcal{X}\to [0,1]$ is a probability distribution, and $\{\rho^x\}_{x\in\mathcal{X}}$ and $\{\sigma^x\}_{x\in\mathcal{X}}$ are sets of states.
	\end{theorem*}
	
	\begin{Proof}
		This result follows by defining the classical--quantum states
		\begin{align}
		\rho_{XA} & \coloneqq \sum_{x \in \mathcal{X}} p(x) \ket{x}\!\bra{x}_X \otimes \rho^x_A ,\\
		\sigma_{XA} & \coloneqq \sum_{x \in \mathcal{X}} p(x) \ket{x}\!\bra{x}_X \otimes \sigma^x_A ,
		\end{align}
		and observing that
		\begin{align}
		& \sqrt{F}(\rho_{XA},\sigma_{XA}) \nonumber \\
		& = \norm{\sqrt{\rho_{XA}} \sqrt{\sigma_{XA}} }_1 \label{eq-root_fid_joint_concave_pf1}\\
		& = \norm{\left(\sum_{x \in \mathcal{X}}  \ket{x}\!\bra{x}_X \otimes \sqrt{p(x)\rho^x_A}\right)\left(\sum_{x' \in \mathcal{X}}  \ket{x'}\!\bra{x'}_X \otimes \sqrt{p(x')\sigma^{x'}_A}\right) }_1 \label{eq-root_fid_joint_concave_pf2} \\
		& = \norm{\sum_{x \in \mathcal{X}}  \ket{x}\!\bra{x}_X \otimes p(x) \sqrt{\rho^x_A} \sqrt{\sigma^{x}_A} }_1 \label{eq-root_fid_joint_concave_pf3}\\
		& = \sum_{x \in \mathcal{X}}\norm{   p(x) \sqrt{\rho^x_A} \sqrt{\sigma^{x}_A} }_1 \label{eq-root_fid_joint_concave_pf4}\\
		& = \sum_{x \in \mathcal{X}}p(x)\norm{    \sqrt{\rho^x_A} \sqrt{\sigma^{x}_A} }_1 \label{eq-root_fid_joint_concave_pf5}\\
		 & = \sum_{x \in \mathcal{X}}p(x)\sqrt{F}(\rho^x_A, \sigma^{x}_A ).\label{eq-root_fid_joint_concave_pf5}
		\end{align}
		From the above and the data-processing inequality for the fidelity under partial trace (Theorem~\ref{thm-fidelity_monotone}), we conclude that
		\begin{equation}
		\sum_{x \in \mathcal{X}}p(x)\sqrt{F}(\rho^x_A, \sigma^{x}_A ) =
		\sqrt{F}(\rho_{XA},\sigma_{XA}) \leq \sqrt{F}(\rho_{A},\sigma_{A}),
		\end{equation}
		which is equivalent to \eqref{eq-joint-concave-root-fidelity}.
	\end{Proof}
	
	The steps in \eqref{eq-root_fid_joint_concave_pf1}--\eqref{eq-root_fid_joint_concave_pf5} demonstrate that the root fidelity satisfies the direct-sum property: for every finite alphabet $\mathcal{X}$, probability distributions $p,q:\mathcal{X}\to[0,1]$, and sets $\{\rho_A^x\}_{x\in\mathcal{X}}$, $\{\sigma_A^x\}_{x\in\mathcal{X}}$ of states, we have
	\begin{multline}\label{eq-direct_sum_root_fid}
		\sqrt{F}\left(\sum_{x\in\mathcal{X}}p(x)\ket{x}\!\bra{x}_X\otimes\rho_A^x,\sum_{x\in\mathcal{X}}q(x)\ket{x}\!\bra{x}_X\otimes\sigma_A^x\right)\\ =\sum_{x\in\mathcal{X}}\sqrt{p(x)q(x)}\sqrt{F}(\rho_A^x,\sigma_A^x).
	\end{multline}
	
	Just as the trace distance can be achieved with a measurement, so it holds that the fidelity can also be achieved with a measurement, as we now show.
	
	\begin{theorem*}{Fidelity via Measurement}{thm-fidelity_meas}
		For two states $\rho$ and $\sigma$, the following equality holds
		\begin{equation}
			F(\rho,\sigma)=\min_{\{\Lambda_x\}_x}\left(\sum_{x\in\mathcal{X}}\sqrt{\Tr[\Lambda_x\rho]}\sqrt{\Tr[\Lambda_x\sigma]}\right)^2,
		\end{equation}
		where the optimization is with respect to all POVMs $\{\Lambda_x\}_{x \in \mathcal{X}}$ defined with respect to a finite alphabet $\mathcal{X}$.
	\end{theorem*}
	
	\begin{Proof}
		Let $\mathcal{M}$ be a measurement channel defined as
		\begin{equation}
			\mathcal{M}(\rho)=\sum_{x\in\mathcal{X}}\Tr[\Lambda_x\rho]\ket{x}\!\bra{x},
		\end{equation}
		where $\{\Lambda_x\}_{x\in\mathcal{X}}$ is a POVM and $\mathcal{X}$ is a finite alphabet. Then, by the data-processing inequality for the fidelity with respect to the channel $\mathcal{M}$, and since the action of $\mathcal{M}$ leads to a state that is diagonal in the orthonormal basis $\{\ket{x}\}_{x\in\mathcal{X}}$, we obtain
		\begin{align}
			F(\rho,\sigma)&\leq F(\mathcal{M}(\rho),\mathcal{M}(\sigma))\\
			&=\norm{\sqrt{\mathcal{M}(\rho)}\sqrt{\mathcal{M}(\sigma)}}_1^2\\
			&=\norm{\sqrt{\sum_{x\in\mathcal{X}}\Tr[\Lambda_x\rho]\ket{x}\!\bra{x}}\sqrt{\sum_{x\in\mathcal{X}}\Tr[\Lambda_x\sigma]\ket{x}\!\bra{x}}}_1^2\\
			&=\norm{\left(\sum_{x\in\mathcal{X}}\sqrt{\Tr[\Lambda_x\rho]}\ket{x}\!\bra{x}\right)\left(\sum_{x\in\mathcal{X}}\sqrt{\Tr[\Lambda_x\sigma]}\ket{x}\!\bra{x}\right)}_1^2\\
			&=\norm{\sum_{x\in\mathcal{X}}\sqrt{\Tr[\Lambda_x\rho]}\sqrt{\Tr[\Lambda_x\sigma]}\ket{x}\!\bra{x}}_1^2\\
			&=\left(\sum_{x\in\mathcal{X}}\sqrt{\Tr[\Lambda_x\rho]}\sqrt{\Tr[\Lambda_x\sigma]}\right)^2.
		\end{align}
		Since the POVM $\{\Lambda_x\}_{x\in\mathcal{X}}$ is arbitrary, we find that
		\begin{equation}
			F(\rho,\sigma)\leq\min_{\{\Lambda_x\}_x}\left(\sum_{x\in\mathcal{X}}\sqrt{\Tr[\Lambda_x\rho]}\sqrt{\Tr[\Lambda_x\sigma]}\right)^2.
		\end{equation}
		
		We now prove the reverse inequality by explicitly constructing a POVM that achieves the fidelity. First, observe that we can write the fidelity $F(\rho,\sigma)$ as
		\begin{equation}
			F(\rho,\sigma)=\norm{\sqrt{\rho}\sqrt{\sigma}}_1^2=\Tr\!\left[\sqrt{\sqrt{\sigma}\rho\sqrt{\sigma}}\right]^2=\Tr[A\sigma]^2,
		\end{equation}
		where
		\begin{equation}
			A\coloneqq \sigma^{-\frac{1}{2}}\left(\sigma^{\frac{1}{2}}\rho\sigma^{\frac{1}{2}}\right)^{\frac{1}{2}}\sigma^{-\frac{1}{2}}.
		\end{equation}
		If $\sigma$ is not invertible, then the inverse is understood to be on the support of $\sigma$, in which case $A$ is supported on the support of $\sigma$. So the fidelity is simply equal to the squared expectation value of the Hermitian operator $A$ with respect to the state $\sigma$. Observe that we can also write
		\begin{align}
			F(\rho,\sigma) & =\left(\Tr\!\left[\sqrt{\sqrt{\sigma}\rho\sqrt{\sigma}}\right]\right)^2 \\
		& =\left(\Tr\!\left[\sqrt{\sqrt{\sigma}\Pi_{\sigma}\rho\Pi_{\sigma}\sqrt{\sigma}}\right]\right)^2\\
		& =F(\Pi_{\sigma}\rho\Pi_{\sigma},\sigma),
		\end{align}
		where $\Pi_{\sigma}$ is the projection onto the support of $\sigma$. This holds because $\sqrt{\sigma}=\Pi_{\sigma}\sqrt{\sigma}=\sqrt{\sigma}\Pi_{\sigma}$.
		
		Now, let us consider a measurement in the eigenbasis of $A$. Let $\{\ket{\psi_i}\}_{i=0}^{r-1}$ be the eigenvectors of $A$, where $r=\rank(A)$. If $\sigma$ is not invertible, then we can always add a set $\{\ket{\psi_i}\}_{i=r}^{d-1}$ of linearly independent pure states orthogonal to the eigenbasis of $A$ in order to obtain a POVM on the full $d$-dimensional space. Therefore, suppose that
		\begin{equation}
			A=\sum_{i=0}^{d-1}\lambda_i\ket{\psi_i}\!\bra{\psi_i},
		\end{equation}
		where we have included the vectors $\{\ket{\psi_i}\}_{i=r}^{d-1}$ that have corresponding eigenvalues equal to zero. Then,
		\begin{align}
			\Tr[A\sigma]&=\Tr\!\left[\sum_{i=0}^{d-1}\lambda_i\ket{\psi_i}\!\bra{\psi_i}\sigma\right]\\
			&=\sum_{i=0}^{d-1}\lambda_i\bra{\psi_i}\sigma\ket{\psi_i}\\
			&=\sum_{i=0}^{d-1}\sqrt{\bra{\psi_i}\lambda_i\sigma\lambda_i\ket{\psi_i}}\sqrt{\bra{\psi_i}\sigma\ket{\psi_i}}\\
			&=\sum_{i=0}^{r-1}\sqrt{\bra{\psi_i}A\sigma A\ket{\psi_i}}\sqrt{\bra{\psi_i}\sigma\ket{\psi_i}},
		\end{align}
		where  the last line follows because $A\ket{\psi_i}=\lambda_i\ket{\psi_i}$ for all $0\leq i\leq r-1$, and we have used the fact that $\lambda_i=0$ for all $r\leq i\leq d-1$. Now, it is straightforward to show that $A\sigma A=\Pi_{\sigma}\rho\Pi_{\sigma}$. Therefore,
		\begin{align}
			F(\rho,\sigma)=\Tr[A\sigma]^2&=\left(\sum_{i=0}^{r-1} \sqrt{\bra{\psi_i}\Pi_{\sigma}\rho\Pi_{\sigma}\ket{\psi_i}}\sqrt{\bra{\psi_i}\sigma\ket{\psi_i}}\right)^2\\
			&=\left(\sum_{i=0}^{r-1}\sqrt{\bra{\psi_i}\rho\ket{\psi_i}}\sqrt{\bra{\psi_i}\sigma\ket{\psi_i}}\right)^2,\label{eq-fidelity_meas_pf}
		\end{align}
		where  the last line follows because $A$ is defined on the support of $\sigma$, which means that $\Pi_{\sigma}\ket{\psi_i}=\ket{\psi_i}$ for all $0\leq i\leq r-1$. We thus have
		\begin{align}
			\min_{\{\Lambda_x\}_x}\left(\sum_{x\in\mathcal{X}}\sqrt{\Tr[\Lambda_x\rho]}\sqrt{\Tr[\Lambda_x\sigma]}\right)^2&\leq\left(\sum_{i=0}^{r-1}\sqrt{\bra{\psi_i}\rho\ket{\psi_i}}\sqrt{\bra{\psi_i}\sigma\ket{\psi_i}}\right)^2\\
			&=F(\rho,\sigma),
		\end{align}
		which is precisely the reverse inequality, as desired.
	\end{Proof}
	
	By employing Theorem~\ref{thm-fidelity_meas}, we conclude the following stronger data-proce\-ssing inequality for the fidelity, which strengthens the statement of Theorem~\ref{thm-fidelity_monotone} considerably:	
	
	\begin{proposition*}{Improved Data Processing for Fidelity}{prop-fidelity-monotone-PTP}
		Let $\rho$ and $\sigma$ be quantum states, and let $\mathcal{N}$ be a positive, trace-preserving map. Then the following inequality holds:
		\begin{equation}
			F(\rho, \sigma) \leq F(\mathcal{N}(\rho), \mathcal{N}(\sigma)).
		\end{equation}
	\end{proposition*}
	
	\begin{Proof}
		The reasoning here follows the reasoning of the proof of Theorem~\ref{thm-trace_dist_monotone} closely. Let $\{\Lambda'_x\}_{x\in\mathcal{X}}$ be a POVM. Then consider that
	\begin{align}
	\sum_{x\in \mathcal{X}} \sqrt{\Tr[\Lambda'_x \mathcal{N}(\rho)]\Tr[\Lambda'_x \mathcal{N}(\sigma)]} & = 
	\sum_{x\in \mathcal{X}} \sqrt{\Tr[\mathcal{N}^\dag(\Lambda'_x) \rho]\Tr[\mathcal{N}^\dag(\Lambda'_x) \sigma]}\\
	& \geq \min_{\{\Lambda_x\}_{x \in \mathcal{X}}}\sum_{x\in \mathcal{X}} \sqrt{\Tr[\Lambda_x \rho]\Tr[\Lambda_x \sigma]} \\
	& = \sqrt{F}(\rho,\sigma).
	\end{align}
	The inequality follows because $\{\mathcal{N}^\dag(\Lambda'_x)\}_{x\in\mathcal{X}}$ is a POVM since $\{\Lambda'_x\}_{x\in\mathcal{X}}$ is and $\mathcal{N}$ is a positive, trace-preserving map, so that $\mathcal{N}^\dag(\Lambda'_x) \geq 0$ for all $x \in \mathcal{X}$ and $\sum_{x\in\mathcal{X}} \mathcal{N}^\dag(\Lambda'_x) = \mathcal{N}^\dag\left(\sum_{x\in\mathcal{X}} \Lambda'_x\right) = \mathcal{N}^\dag\left(\mathbbm{1}\right) = \mathbbm{1}$. The last equality follows from Theorem~\ref{thm-fidelity_meas}. Since the inequality holds for all POVMs $\{\Lambda'_x\}_{x\in\mathcal{X}}$, we conclude that
	\begin{align}
	\sqrt{F}(\mathcal{N}(\rho), \mathcal{N}(\sigma)) & = \min_{\{\Lambda'_x\}_{x\in\mathcal{X}}}\sum_{x\in \mathcal{X}} \sqrt{\Tr[\Lambda'_x \mathcal{N}(\rho)]\Tr[\Lambda'_x \mathcal{N}(\sigma)]} \\
	& \geq \sqrt{F}(\rho,\sigma),
	\end{align}
	where we have again employed Theorem~\ref{thm-fidelity_meas} for the equality.
	\end{Proof}
	
	We now establish a useful relation between trace distance and fidelity.
	
	\begin{theorem*}{Relation Between Trace Distance and Fidelity}{thm-Fuchs_van_de_graaf}
		For  two states $\rho$ and $\sigma$, the following chain of inequalities relates their trace distance with the fidelity between them:
		\begin{equation}\label{eq-Fuchs_van_de_graaf}
			1-\sqrt{F(\rho,\sigma)}\leq\frac{1}{2}\norm{\rho-\sigma}_1\leq\sqrt{1-F(\rho,\sigma)}.
		\end{equation}
	\end{theorem*}
	
	\begin{Proof}
		We first prove the upper bound. To do so, recall the formula in \eqref{eq-trace_dist_pure_states} for the trace distance between two pure states. If we let $\ket{\psi^{\rho}}_{RA}$ and $\ket{\psi^{\sigma}}_{RA}$ be purifications of $\rho_A$ and $\sigma_A$, respectively, such that $F(\rho_A,\sigma_A)=\abs{\braket{\psi^{\rho}}{\psi^{\sigma}}}^2$, and if we use the data-processing inequality for the trace distance with respect to the partial trace channel $\Tr_R$, then we obtain
		\begin{align}
			\frac{1}{2}\norm{\rho_A-\sigma_A}_1&=\frac{1}{2}\norm{\Tr_R[\ket{\psi^{\rho}}\!\bra{\psi^{\rho}}_{RA}-\ket{\psi^{\sigma}}\!\bra{\psi^{\sigma}}_{RA}]}_1\\
			&\leq \frac{1}{2}\norm{\ket{\psi^{\rho}}\!\bra{\psi^{\rho}}_{RA}-\ket{\psi^{\sigma}}\!\bra{\psi^{\sigma}}_{RA}}_1\\
			&=\sqrt{1-\abs{\braket{\psi^{\rho}}{\psi^{\sigma}}}^2}\\
			&=\sqrt{1-F(\rho_A,\sigma_A)},
		\end{align}
		as required.
		
		For the lower bound, we use the results of Theorems~\ref{thm-fidelity_meas} and \ref{thm-trace_dist_ach_by_meas_channel}. Theorem \ref{thm-fidelity_meas} tells us that there exists a POVM $\{\Lambda_x\}_{x\in\mathcal{X}}$ such that
		\begin{align}
			F(\rho,\sigma)&=\left(\sum_{x\in\mathcal{X}}\sqrt{\Tr[\Lambda_x\rho]}\sqrt{\Tr[\Lambda_x\sigma]}\right)^2\\
			&\equiv\left(\sum_{x\in\mathcal{X}}\sqrt{p(x)q(x)}\right)^2,
		\end{align}
		where we have let $p(x)\coloneqq\Tr[\Lambda_x\rho]$ and $q(x)\coloneqq\Tr[\Lambda_x\sigma]$. Using this, observe that
		\begin{align}
			\sum_{x\in\mathcal{X}}\left(\sqrt{\smash[b]{p(x)}}-\sqrt{\smash[b]{q(x)}}\right)^2&=\sum_{x\in\mathcal{X}}\left(p(x)-2\sqrt{\smash[b]{p(x)q(x)}}+q(x)\right)\\
			&=2-2\sum_{x\in\mathcal{X}}\sqrt{\smash[b]{p(x)q(x)}}\\
			&=2-2\sqrt{F(\rho,\sigma)}.
		\end{align}
		
		Now, Theorem \ref{thm-trace_dist_ach_by_meas_channel} tells us that
		\begin{equation}
			\norm{\rho-\sigma}_1=\max_{\{\Omega_y\}_{y}}\sum_{x\in\mathcal{X}}|r(y)-s(y)|,
		\end{equation}
		where $r(y)\coloneqq\Tr[\Omega_y\rho]$ and $s(y)\coloneqq\Tr[\Omega_y\sigma]$. In particular, for the POVM $\{\Lambda_x\}_{x\in\mathcal{X}}$ that achieves the fidelity, we have
		\begin{equation}
			\sum_{x\in\mathcal{X}}|p(x)-q(x)|\leq\norm{\rho-\sigma}_1.
		\end{equation}
		Using this, and the fact that $|\sqrt{p(x)}-\sqrt{q(x)}|\leq|\sqrt{p(x)}+\sqrt{q(x)}|$, we obtain
		\begin{align}
			\sum_{x\in\mathcal{X}}\left(\sqrt{\smash[b]{p(x)}}-\sqrt{\smash[b]{q(x)}}\right)^2&\leq \sum_{x\in\mathcal{X}}\abs{\sqrt{\smash[b]{p(x)}}-\sqrt{\smash[b]{q(x)}}}\abs{\sqrt{\smash[b]{p(x)}}+\sqrt{\smash[b]{q(x)}}}\\
			&=\sum_{x\in\mathcal{X}}|p(x)-q(x)|\\
			&\leq \norm{\rho-\sigma}_1.
		\end{align}
		So we have
		\begin{equation}
			2-2\sqrt{F(\rho,\sigma)}=\sum_{x\in\mathcal{X}}\left(\sqrt{\smash[b]{p(x)}}-\sqrt{\smash[b]{q(x)}}\right)^2\leq\norm{\rho-\sigma}_1,
		\end{equation}
		which is the required lower bound.
	\end{Proof}

\begin{Lemma*}
{Gentle Measurement}{lem-dm:gentle-measurement}
Let $\rho$ be a density
operator  and $\Lambda$ a measurement operator, satisfying $0\leq\Lambda\leq
I$ and $\operatorname{Tr}[  \Lambda\rho]  \geq 1-\varepsilon$, for $\varepsilon\in[0,1]$.
 Then the post-measurement state
\begin{equation}
\rho^{\prime}\coloneqq \frac{\sqrt{\Lambda}\rho\sqrt{\Lambda}}{\operatorname{Tr}%
[  \Lambda\rho]  }%
\end{equation}
satisfies
\begin{align}
F(\rho,\rho') & \geq 1-\varepsilon , \\
\frac{1}{2} \left\Vert \rho-\rho^{\prime}\right\Vert _{1} & \leq\sqrt{\varepsilon}.
\end{align}
\end{Lemma*}

\begin{Proof}
Suppose first that $\rho$ is a pure state $|\psi\rangle\!\langle\psi|$. The
post-measurement state is then%
\begin{equation}
\frac{\sqrt{\Lambda}|\psi\rangle\!\langle\psi|\sqrt{\Lambda}}{\langle
\psi|\Lambda|\psi\rangle}.
\end{equation}
The fidelity between the original state $|\psi\rangle$ and the
post-measurement state above is as follows:%
\begin{align}
\langle\psi|\left(  \frac{\sqrt{\Lambda}|\psi\rangle\!\langle\psi|\sqrt{\Lambda
}}{\langle\psi|\Lambda|\psi\rangle}\right)  |\psi\rangle &  =\frac{\left\vert
\langle\psi|\sqrt{\Lambda}|\psi\rangle\right\vert ^{2}}{\langle\psi
|\Lambda|\psi\rangle} \geq\frac{\left\vert \langle\psi|\Lambda|\psi
\rangle\right\vert ^{2}}{\langle\psi|\Lambda|\psi\rangle}\\
&  =\langle\psi|\Lambda|\psi\rangle\geq1-\varepsilon.
\end{align}
The first inequality follows because $\sqrt{\Lambda}\geq\Lambda$ when
$\Lambda\leq I$. The second inequality follows from the hypothesis of the
lemma. Now let us consider when we have mixed states $\rho_{A}$ and $\rho
_{A}^{\prime}$. Suppose $|\psi\rangle_{RA}$ and $\left\vert \psi^{\prime
}\right\rangle _{RA}$ are respective purifications of $\rho_{A}$ and $\rho
_{A}^{\prime}$, where%
\begin{equation}
\left\vert \psi^{\prime}\right\rangle _{RA}\equiv\frac{I_{R}\otimes
\sqrt{\Lambda_{A}}|\psi\rangle_{RA}}{\sqrt{\langle\psi|I_{R}\otimes\Lambda
_{A}|\psi\rangle_{RA}}}.
\end{equation}
Then we can apply the data-processing inequality for fidelity
(Proposition~\ref{prop-fidelity-monotone-PTP}) and the result above  for pure states
to conclude that
\begin{equation}
F(\rho_{A},\rho_{A}^{\prime})\geq F(\psi_{RA},\psi_{RA}^{\prime}%
)\geq1-\varepsilon.
\end{equation}
We obtain the bound on the normalized trace distance $\frac{1}{2} \left\Vert \rho_{A}-\rho
_{A}^{\prime}\right\Vert _{1}$ by exploiting
Theorem~\ref{thm-Fuchs_van_de_graaf}.
\end{Proof}
	
	\subsubsection{Sine Distance}
	
	Unlike the trace distance, the fidelity is not a distance measure in the mathematical sense because it does not satisfy the triangle inequality. The following distance measure based on the fidelity, however, does satisfy the triangle inequality, along with the other properties that define a distance measure.

	
	\begin{definition}{Sine Distance}{def-purified_distance}
		For  two states $\rho$ and $\sigma$, we define the \textit{sine distance} between $\rho$ and $\sigma$ as
		\begin{equation}\label{eq-purified_distance}
			P(\rho,\sigma)\coloneqq \sqrt{1-F(\rho,\sigma)}.
		\end{equation}
	\end{definition}
	
	The measure $P(\rho,\sigma)$ is known as the sine distance due to the fact that $F(\rho,\sigma)$ has the interpretation as the largest value of the squared cosine of the angle between two arbitrary purifications of $\rho$ and $\sigma$ (see Theorem~\ref{thm-Uhlmann_fidelity}), which means that $\sqrt{1-F(\rho,\sigma)}$ has the interpretation as the sine of the same angle. Related to this interpretation, the measure $P(\rho,\sigma)$ is equal to the minimum trace distance between purifications of $\rho$ and $\sigma$:
	\begin{multline}
		\inf_{\ket{\psi^\rho}_{RA}, \ket{\psi^\sigma}_{RA}} \frac{1}{2}\norm{\ket{\psi^\rho}\!\bra{\psi^\rho}_{RA}- \ket{\psi^\sigma}\!\bra{\psi^\sigma}_{RA}}_1 \\= \inf_{\ket{\psi^\rho}_{RA}, \ket{\psi^\sigma}_{RA}} \sqrt{1-\vert\! \braket{\psi^\rho} {\psi^\sigma}_{RA} \vert^2} = P(\rho,\sigma),
	\end{multline}
	where the optimization is over all purifications $\ket{\psi^\rho}_{RA}$ and $\ket{\psi^\sigma}_{RA}$ of $\rho$ and $\sigma$, respectively. This follows by applying \eqref{eq-trace_dist_pure_states}, as well as Uhlmann's theorem (Theorem~\ref{thm-Uhlmann_fidelity}).
	
	Since the fidelity satisfies the data-processing inequality with respect to positive, trace-preserving maps (Proposition~\ref{prop-fidelity-monotone-PTP}), so does the sine distance: for  two states $\rho$ and $\sigma$ and a positive, trace-preserving map $\mathcal{N}$, we have that
	\begin{equation}\label{eq-sine_dist_data_proc}
		P(\rho,\sigma)\geq P(\mathcal{N}(\rho),\mathcal{N}(\sigma)).
	\end{equation}
	
	\begin{Lemma*}{Triangle Inequality for Sine Distance}{lem-sine-distance-triangle}
		Let $\rho$, $\sigma$, and $\omega$ be quantum states. Then the triangle inequality holds for the sine distance:
		\begin{equation}
		P(\rho,\sigma) \leq P(\rho,\omega) + P(\omega,\sigma).
		\end{equation}
	\end{Lemma*}

	\begin{Proof}	
		Define the canonical purifications as%
		\begin{align}
			\ket{\psi^{\rho}}_{RA}&=(\mathbbm{1}_{R}\otimes\sqrt{\rho_{A}})\ket{\Gamma}_{RA},\\
			\ket{\psi^{\sigma}}_{RA}&=(\mathbbm{1}_{R}\otimes\sqrt{\sigma_{A}})\ket{\Gamma}_{RA},\\
			\ket{\psi^{\omega}}_{RA}&=(\mathbbm{1}_{R}\otimes\sqrt{\omega_{A}})\ket{\Gamma}_{RA},
		\end{align}
		where $\ket{\Gamma}_{RA}$ is the maximally entangled vector from \eqref{eq-max_ent_vector}. Recalling \eqref{eq-trace_dist_pure_states}, for pure states
$|\phi\rangle$ and $|\varphi\rangle$, we have that%
\begin{equation}
\frac{1}{2}\left\Vert |\phi\rangle\!\langle\phi|-|\varphi\rangle\!\langle
\varphi|\right\Vert _{1}=\sqrt{1-F(\phi,\varphi)}=\sqrt{1-|\langle\phi
|\varphi\rangle|^{2}}.
\end{equation}
Let $U_{R}$ and $V_{R}$ be arbitrary unitaries acting on the reference system
$R$. From the fact that trace distance obeys the triangle inequality and the
equality given above, we find that%
\begin{multline}
\sqrt{1-|\langle\psi^{\sigma}|_{RA}(W_R\otimes \mathbbm{1}_{A})|\psi^{\rho
}\rangle_{RA}|^{2}}\leq\sqrt{1-|\langle\psi^{\sigma}|_{RA}(U_{R}^{\dag}\otimes
\mathbbm{1}_{A})|\psi^{\omega}\rangle_{RA}|^{2}}\\
+\sqrt{1-|\langle\psi^{\omega}|_{RA}(V_{R}\otimes \mathbbm{1}_{A})|\psi^{\rho}\rangle
_{RA}|^{2}},
\end{multline}
where $W_R\coloneqq U_R^\dagger V_R$. By minimizing the left-hand side with respect to all unitaries $W_R$, and applying
Uhlmann's theorem, we find that%
\begin{multline}
\sqrt{1-F(\sigma_{A},\rho_{A})}\leq\sqrt{1-|\langle\psi^{\sigma}|_{RA}(U_{R}^{\dag}\otimes \mathbbm{1}_{A})|\psi^{\omega}\rangle_{RA}|^{2}}\\+\sqrt{1-|\langle
\psi^{\omega}|_{RA}(V_{R}\otimes \mathbbm{1}_{A})|\psi^{\rho}\rangle_{RA}|^{2}}.
\end{multline}
Since the inequality holds for arbitrary unitaries $U$ and $V$, it holds for
the minimum of each term on the right, and so this, combined with Uhlmann's
theorem (Theorem~\ref{thm-Uhlmann_fidelity}), implies the desired result:%
\begin{equation}
\sqrt{1-F(\sigma_{A},\rho_{A})}\leq\sqrt{1-F(\sigma_{A},\omega_{A})}%
+\sqrt{1-F(\omega_{A},\rho_{A})},
\end{equation}
concluding the proof.
\end{Proof}
	
	
\subsection{Diamond Norm and Diamond Distance}
	
	Just as there are measures of distinguishability for quantum states, it is important to develop measures of distinguishability for quantum channels, in order to assess the performance of quantum information-processing protocols that attempt to simulate an ideal process. The measures that we introduce in this section are again motivated by operational concerns, stemming from the ability of an experimenter to distinguish one quantum channel from another when given access to a single use of the channel. In what follows, our discussion mirrors and generalizes the discussion in Section~\ref{sec-QM-trace-distance} that motivated trace distance as a measure of distinguishability for quantum states.
	
	How should we measure the distance between two quantum channels $\mathcal{N}_{A\to B}$ and $\mathcal{M}_{A\to B}$? Related, how should we assess the performance of a quantum inform\-ation-processing protocol in which the ideal channel to be simulated is $\mathcal{N}_{A\to B}$ but the channel realized in practice is $\mathcal{M}_{A\to B}$? Suppose that a third party is trying to assess how distinguishable the actual channel $\mathcal{M}_{A\to B}$ is from the ideal channel $\mathcal{N}_{A\to B}$. Such an individual has access to both the input and output ports of the channel, and so the most general strategy for the distinguisher to employ is to prepare a state $\rho_{RA}$ of a reference system $R$ and the channel input system $A$. The distinguisher transmits the $A$ system of $\rho_{RA}$ into the unknown channel. After that, the distinguisher receives the channel output system $B$ and then performs a measurement described by the POVM $\{\Lambda^x_{RB}\}_x$ on the reference system $R$ and the channel output system~$B$. The probability of obtaining a particular outcome $\Lambda^x_{RB}$ is given by the Born rule. In the case that the unknown channel is $\mathcal{N}_{A\to B}$,  this probability is $\Tr[\Lambda^x_{RB}\mathcal{N}_{A\to B}(\rho_{RA})]$, and in the case that the unknown channel is $\mathcal{M}_{A\to B}$,  this probability is $\Tr[\Lambda^x_{RB}\mathcal{M}_{A\to B}(\rho_{RA})]$. What we demand is that the absolute deviation between the two probabilities $\Tr[\Lambda^x_{RB}\mathcal{N}_{A\to B}(\rho_{RA})]$ and $\Tr[\Lambda^x_{RB}\mathcal{M}_{A\to B}(\rho_{RA})]$ is no larger than some tolerance $\varepsilon$. Since this should be the case for all possible input states and measurement outcomes, what we demand mathematically is that 
	\begin{equation}
	\sup_{\rho_{RA},\, 0\leq \Lambda_{RB} \leq \mathbbm{1}_{RB}} |\Tr[\Lambda_{RB}\mathcal{N}_{A\to B}(\rho_{RA})] - 
	\Tr[\Lambda_{RB}\mathcal{M}_{A\to B}(\rho_{RA})]| \leq \varepsilon.
	\end{equation}
	As a consequence of the characterization of trace distance from Theorem~\ref{thm-trace_dist_meas} we have
	\begin{multline}\label{eq-diamond_dist_meas}
	\sup_{\rho_{RA},0\leq \Lambda_{RB} \leq \mathbbm{1}_{RB}} |\Tr[\Lambda_{RB}(\mathcal{N}_{A\to B} - 
	\mathcal{M}_{A\to B})(\rho_{RA})]|\\=\sup_{\rho_{RA}}\frac{1}{2}\norm{\mathcal{N}_{A\to B}(\rho_{RA})-\mathcal{M}_{A\to B}(\rho_{RA})}_1\eqqcolon\frac{1}{2}\norm{\mathcal{N}-\mathcal{M}}_{\diamond},
	\end{multline}
	where $\frac{1}{2}\norm{\mathcal{N} - \mathcal{M}}_{\diamond}$ is defined to be the \textit{normalized diamond distance} between $\mathcal{N}$ and $\mathcal{M}$. This indicates that if $\frac{1}{2}\norm{\mathcal{N} - \mathcal{M}}_{\diamond} \leq \varepsilon$, then the absolute deviation between probabilities for every possible input state and measurement operator never exceeds $\varepsilon$, so that the approximation between quantum channels $\mathcal{N}_{A\to B}$ and $\mathcal{M}_{A\to B}$ is naturally quantified by the normalized diamond distance $\frac{1}{2}\norm{\mathcal{N} - \mathcal{M}}_{\diamond}$. 
	
	With the above in mind, we now define the diamond norm for Hermiticity-preserving maps, from which the diamond distance measure for channels arises.
	
	\begin{definition}{Diamond Norm}{def-diamond_norm}
		The \textit{diamond norm} of a Hermiticity-preserving map $\mathcal{P}_{A\to B}$ is defined  as
		\begin{equation}\label{eq-diamond_norm}
			\norm{\mathcal{P}}_{\diamond}\coloneqq\sup_{\rho_{RA}}\norm{\mathcal{P}_{A\to B}(\rho_{RA})}_1,
		\end{equation}
		where the optimization is over all states $\rho_{RA}$, with the dimension of $R$ unbounded.
	\end{definition}

%	\begin{remark}
%		A more general definition of the diamond norm, and the corresponding diamond distance, holds for arbitrary linear maps acting on the space of linear operators. Specifically, for every such map $\mathcal{T}_{A\to B}$, we have
%		\begin{equation}
%			\norm{\mathcal{T}}_{\diamond}\coloneqq\sup_{\substack{X_{AA'},\\\norm{X_{AA'}}_1\leq 1}}\norm{\mathcal{T}_{A'\to B}(X_{AA'})}_1.
%		\end{equation}
%		Then, if $\mathcal{T}$ is a hermiticity-preserving map, it can be shown that this expression for the diamond norm is equal to the one in \eqref{eq-diamond_norm}.
%	\end{remark}
	
	For two quantum channels $\mathcal{N}$ and $\mathcal{M}$, note that the difference $\mathcal{N}-\mathcal{M}$ is a Hermiticity-preserving map. An important simplification of the diamond norm of a Hermiticity-preserving map is given by the following proposition:
	
	\begin{proposition}{prop-diamond_norm_herm_pres}
		The diamond norm of a Hermiticity-preserving map $\mathcal{P}_{A\to B}$ can be calculated as
		\begin{equation}\label{eq-diamond_norm_alt}
			\norm{\mathcal{P}}_{\diamond}=\sup_{\psi_{RA}}\norm{\mathcal{P}_{A\to B}(\psi_{RA})}_1,
		\end{equation}
		where the optimization is over all pure states $\psi_{RA}$, such that the dimension of $R$ is equal to the dimension of the system $A$.
	\end{proposition}

\begin{Proof}
Let $\rho_{RA}$ be an arbitrary state. It has a spectral decomposition as follows:
\begin{equation}
\rho_{RA} = \sum_x p(x) \psi^x_{RA} ,
\end{equation}
where $\{p(x)\}_x$ is a probability distribution and $\{\psi^x_{RA}\}_x$ is a set of pure states. From the convexity of the trace norm (see Section~\ref{sec:math-tools:norms}), it follows that
\begin{align}
\norm{\mathcal{P}_{A\to B}(\rho_{RA})}_1 &
\leq \sum_x p(x) \norm{\mathcal{P}_{A\to B}(\psi^x_{RA})}_1 \\
& \leq \sup_x  \norm{\mathcal{P}_{A\to B}(\psi^x_{RA})}_1 \\
& \leq \sup_{\psi_{RA}}\norm{\mathcal{P}_{A\to B}(\psi_{RA})}_1 
\end{align}
From the Schmidt decomposition (Theorem~\ref{thm-Schmidt}), it follows that the rank of the reduced state $\psi_{R}$ is no larger than the dimension of system $A$. So then it suffices to optimize with respect to all pure states $\psi_{RA}$, such that the dimension of $R$ is equal to the dimension of the system $A$.
\end{Proof}
	
%	We note that if $\mathcal{N}$ is a quantum channel, then $\norm{\mathcal{N}}_{\diamond}=1$ (see Bibliographic Notes). 
	
		The normalized diamond distance between two quantum channels can be computed via a semi-definite program (SDP). The following proposition states this fact formally and also states the dual optimization problem. Appendix~\ref{app-trace_dist_fidelity_SDP} provides a proof.
		
		\begin{proposition*}{SDPs for Normalized Diamond Distance}{prop-diamond_dist_SDP}
		The diamond distance between two quantum channels $\mathcal{N}_{A\to B}$ and $\mathcal{M}_{A\to B}$ can be written as the following semi-definite programs:
		\begin{align}
			&\frac{1}{2}\norm{\mathcal{N}-\mathcal{M}}_{\diamond}\nonumber\\
			& =\sup_{\substack{\rho_R\geq 0,\\\Omega_{RB}\geq 0}}\{\Tr[\Omega_{RB}(\Gamma_{RB}^{\mathcal{N}}-\Gamma_{RB}^{\mathcal{M}})]:\Omega_{RB}\leq\rho_R\otimes\mathbbm{1}_B, \Tr[\rho_R]=1 \}\label{eq-diamond_dist_SDP_primal}\\[0.2cm]
			&=\inf_{\substack{\mu\geq 0,\\Z_{RB}\geq 0}}\{ \mu : Z_{RB}\geq \Gamma_{RB}^{\mathcal{N}}-\Gamma_{RB}^{\mathcal{M}},\mu\mathbbm{1}_R\geq \Tr_B[Z_{RB}]\}.\label{eq-diamond_dist_SDP_dual}
		\end{align}
		The latter expression is equal to
		\begin{equation}
			\inf_{Z_{RB}\geq 0}\{\norm{\Tr_B[Z_{RB}]}_{\infty}:Z_{RB}\geq \Gamma_{RB}^{\mathcal{N}}-\Gamma_{RB}^{\mathcal{M}}\}.
		\end{equation}
	\end{proposition*}


	
	As described at the beginning of this section, the diamond distance has an operational meaning in terms of the task of \textit{channel discrimination}, which is a generalization of state discrimination (see Section \ref{subsec-state_discrimination}). Let us now analyze the task of channel discrimination in more detail.
	
	Suppose that Alice gives Bob a device that implements either the channel $\mathcal{N}$ or the channel $\mathcal{M}$, but she does not tell him which channel it implements. Bob's task is to decide which channel the device implements. Suppose that the channels $\mathcal{N}$ and $\mathcal{M}$ have prior probabilities $\lambda$ and $1-\lambda$ of being selected, respectively. The only way for Bob to determine which channel the device implements (without guessing randomly) is to pass a quantum system, say in the state $\rho$, through it. He can then perform a measurement on the resulting output state and make a guess as to which channel was implemented. Therefore, in addition to having the freedom to choose any binary measurement (which is the case in state discrimination), in channel discrimination Bob also has the freedom to prepare a system $A$ and a reference system $R$ in any state $\rho_{RA}$ of his choosing, with the system $A$ being passed through the device. 
	
	\begin{figure}
		\centering
		\includegraphics[scale=0.8]{Figures/chan_discrimination.pdf}
		\caption{Schematic depiction of a general strategy for the task of discriminating between the quantum channels $\mathcal{N}$ and $\mathcal{M}$. Starting with the state $\rho_{RA}$, the system $A$ is passed through the device that implements either $\mathcal{N}$ or $\mathcal{M}$. Then, both systems $R$ and $A$ are measured according to the POVM $\{\Lambda,\mathbbm{1}-\Lambda\}$, the result of which is used to form a guess for which channel the device implements.}\label{fig-chan_discrimination}
	\end{figure}
	
	
	
	For every fixed input state $\rho_{RA}$, there are two possible output states, depending on which channel was implemented. This means that, for every fixed input state, the task of channel discrimination reduces to the task of state discrimination. Using the result of Theorem~\ref{thm-Holevo_Helstrom}, for the input state $\rho_{RA}$ the corresponding optimal error probability (i.e., the error probability obtained by optimizing over all measurements) is
	\begin{equation}
		p_{\text{err}}^*(\rho_{RA})=\frac{1}{2}\left(1-\norm{\lambda\mathcal{N}_{A\to B}(\rho_{RA})-(1-\lambda)\mathcal{M}_{A\to B}(\rho_{RA})}_1\right).
	\end{equation}
	Then, optimizing over all input states $\rho_{RA}$ in order to minimize the error probability, we find that
	\begin{align}
		\inf_{\rho_{RA}}p_{\text{err}}^*(\rho_{RA})&=\frac{1}{2}\left(1-\sup_{\rho_{RA}}\norm{(\lambda\mathcal{N}_{A\to B}-(1-\lambda)\mathcal{M}_{A\to B})(\rho_{RA})}_1\right)\\
		&=\frac{1}{2}\left(1-\norm{\lambda\mathcal{N}-(1-\lambda)\mathcal{M}}_{\diamond}\right),
	\end{align}
	where  the last line follows from the definition of the diamond norm. The optimal error probability for the task of channel discrimination is thus a simple function of the diamond norm.
	
	
\subsection{Fidelity Measures for Channels}

	The diamond distance is a distance measure for channels that is based on the trace distance for states. We now define a fidelity-based quantity for channels that can be used to assess its ability to preserve entanglement. 
		
	\begin{definition}{Entanglement Fidelity of a Channel}{def-ent_fid_chan}
		For a quantum channel $\mathcal{N}_{A}$ with input and output systems of equal dimension $d$, we define its \textit{entanglement fidelity} as
		\begin{equation}
			F_e(\mathcal{N})\coloneqq \bra{\Phi}_{RA} (\id_R\otimes \mathcal{N}_{A})(\Phi_{RA})\ket{\Phi}_{RA},
		\end{equation}
		where
		\begin{equation}
			\ket{\Phi}_{RA}=\frac{1}{\sqrt{d}}\sum_{i=0}^{d-1}\ket{i,i}_{RA}.
		\end{equation}
	\end{definition}

	Notice that the entanglement fidelity of a channel is the fidelity of the maximally entangled state with the Choi state of the channel. Intuitively, then, the entanglement fidelity quantifies how good a channel is at preserving the entanglement between two systems when it acts on one of the two systems.
	
	It turns out that the entanglement fidelity is very closely related to another fidelity-based measure on quantum channels called the \textit{average fidelity}:
	\begin{equation}\label{eq-chan_avg_fid}
		\overline{F}(\mathcal{N})\coloneqq \int_{\psi} \bra{\psi}\mathcal{N}(\psi)\ket{\psi}~\text{d}\psi,
	\end{equation}
	where we integrate over all pure states acting on the input Hilbert space of $\mathcal{N}$ with respect to the Haar measure. The Haar measure is the uniform probability measure on pure quantum states (see the remark after \eqref{eq-sym_proj_integral}). For a quantum channel $\mathcal{N}$ with input system dimension $d$, the following identity holds
	\begin{equation}
		\overline{F}(\mathcal{N})=\frac{dF_e(\mathcal{N})+1}{d+1}.
		\label{eq:QM-over:average-fid-to-ent-fid}
	\end{equation}
	
	Instead of taking the average as in \eqref{eq-chan_avg_fid}, we can take the minimum over all input states to obtain the \textit{minimum fidelity}:
	\begin{equation}\label{eq-minimum_fidelity_chan}
		F_{\min}(\mathcal{N})\coloneqq\inf_{\psi} \bra{\psi}\mathcal{N}(\psi)\ket{\psi},
	\end{equation}
	where the optimization is over all pure states $\psi$ acting on the input Hilbert space of the channel $\mathcal{N}$. By introducing a reference system $R$ and optimizing over all joint states $\ket{\psi}_{RA}$ of $R$ and the input system $A$ of the channel $\mathcal{N}$, we obtain a fidelity measure that generalizes the entanglement fidelity.
	
	\begin{definition}{Fidelity of a Quantum Channel}{eq-worse_case_fid_chan}
		For a quantum channel $\mathcal{N}_A$ with equal input and output system dimension, we define the \textit{fidelity of $\mathcal{N}$} as
		\begin{equation}\label{eq-worst_case_fidelity_chan}
			F(\mathcal{N})\coloneqq \inf_{\psi_{RA}}\bra{\psi}_{RA}(\id_R \otimes \mathcal{N}_{A})(\psi_{RA})\ket{\psi}_{RA},
		\end{equation}
		where we take the infimum over all pure states $\ket{\psi}_{RA}$, with the dimension of $R$ equal to the dimension of $A$.
	\end{definition}
	
	Note that the state $\ket{\psi}_{RA}=\ket{\Phi}_{RA}$ is a special case in the optimization in \eqref{eq-worst_case_fidelity_chan}. This implies that, for a channel $\mathcal{N}$, $F(\mathcal{N})\leq F_e(\mathcal{N})$.
	
	More generally, we define the fidelity between  two quantum channels $\mathcal{N}_{A\to B}$ and $\mathcal{M}_{A\to B}$ as follows:
	\begin{definition}{Fidelity of Quantum Channels}{def:QM-over:fid-channels}
	Let $\mathcal{N}_{A\to B}$ and $\mathcal{M}_{A\to B}$ be quantum channels. Their channel fidelity is defined as
	\begin{equation}\label{eq-fidelity_chan_distance}
		F(\mathcal{N},\mathcal{M})=\inf_{\rho_{RA}}F(\mathcal{N}_{A\to B}(\rho_{RA}),\mathcal{M}_{A\to B}(\rho_{RA})),
	\end{equation}
	where the infimum is taken over all bipartite states $\rho_{RA}$, with the dimension of $R$ arbitrarily large.
	\end{definition}
	
	
	\begin{remark}
	
	Similar to the diamond distance, we define the channel fidelity as above in order to indicate its operational meaning with an infimum over all possible input states, but it is not necessary to take the infimum over all bipartite states. One can instead restrict the infimum to be over pure bipartite states where the reference system $R$ is isomorphic to the channel input system $A$, so that
	\begin{equation}
	F(\mathcal{N},\mathcal{M})=\inf_{\psi_{RA}}F(\mathcal{N}_{A\to B}(\psi_{RA}),\mathcal{M}_{A\to B}(\psi_{RA})),
	\end{equation}
	where $\psi_{RA}$ is a pure bipartite state with system $R$ is isomorphic to  system $A$. The same statement thus applies to \eqref{eq-worst_case_fidelity_chan}.
	An argument for this is similar to that given in the proof of Proposition~\ref{prop-diamond_norm_herm_pres}, except using the joint concavity of root fidelity rather than  convexity of the trace norm.
	
	Here, we provide a different argument for this fact. First, we have that
		\begin{align}
			\inf_{\rho_{RA}}F(\mathcal{N}_{A\to B}(\rho_{RA}),\mathcal{M}_{A\to B}(\rho_{RA}))\leq \inf_{\psi_{RA}}F(\mathcal{N}_{A\to B}(\psi_{RA}),\mathcal{M}_{A\to B}(\psi_{RA}))
		\end{align}
		which holds simply by restricting the optimization on the left-hand side to pure states.
		
		Next, given a state $\rho_{RA}$, with the dimension of $R$ not necessarily equal to the dimension of $A$, we can purify it to a state $\psi_{R'RA}$. Then, using the data-processing inequality for the fidelity with respect to the partial trace channel $\Tr_{R'}$ (Proposition~\ref{prop-fidelity-monotone-PTP}), we find that
		\begin{align}
			F(\mathcal{N}_{A\to B}(\rho_{RA}),\mathcal{M}_{A\to B}(\rho_{RA}))&=F\left(\mathcal{N}_{A\to B}(\Tr_{R'}[\psi_{R'RA}]),\mathcal{M}_{A\to B}(\Tr_{R'}[\psi_{R'RA}])\right)\\
			&=F\left(\Tr_{R'}[\mathcal{N}_{A\to B}(\psi_{R'RA})],\Tr_{R'}[\mathcal{M}_{A\to B}(\psi_{R'RA})]\right)\\
			&\geq F(\mathcal{N}_{A\to B}(\psi_{R'RA}),\mathcal{M}_{A\to B}(\psi_{R'RA}))\\
			&\geq \inf_{\psi_{R'RA}}F(\mathcal{N}_{A\to B}(\psi_{R'RA}),\mathcal{M}_{A\to B}(\psi_{R'RA})).
		\end{align}
		Since the state $\rho_{RA}$ is arbitrary, we obtain
		\begin{equation}
			\inf_{\rho_{RA}}F(\mathcal{N}_{A\to B}(\rho_{RA}),\mathcal{M}_{A\to B}(\rho_{RA}))\geq \inf_{\psi_{RA}}F(\mathcal{N}_{A\to B}(\psi_{RA}),\mathcal{M}_{A\to B}(\psi_{RA})).
		\end{equation}
		
		Finally, by the Schmidt decomposition theorem (Theorem~\ref{thm-Schmidt}), for every pure state $\psi_{RA}$, the rank of the reduced state $\psi_R$ need not exceed the dimension of $A$, implying that it suffices to optimize over pure states for which the system $R$ has the same dimension as the system $A$. We thus obtain
		\begin{align}
			\inf_{\rho_{RA}}F(\mathcal{N}_{A\to B}(\rho_{RA}),\mathcal{M}_{A\to B}(\rho_{RA}))&=\inf_{\psi_{RA}}F(\mathcal{N}_{A\to B}(\psi_{RA}),\mathcal{M}_{A\to B}(\psi_{RA})\\
			&=F(\mathcal{N},\mathcal{M}).
		\end{align}
	\end{remark}
	
	We then have that $F(\mathcal{N})=F(\mathcal{N},\id)$. In other words, the fidelity $F(\mathcal{N})$ of a quantum channel $\mathcal{N}$ can be viewed as the fidelity between $\mathcal{N}$ and the identity channel $\id$.
	
	Similar to the diamond distance, the fidelity of quantum channels can be computed by means of primal and dual semi-definite programs:
	
%	\begin{proposition*}{SDP for Root Fidelity of Channels}{prop:QM-over:SDP-fidelity-channels}
%	For quantum channels $\mathcal{N}_{A\to B}$ and $\mathcal{M}_{A\to B}$, their root fidelity $\sqrt{F}(\mathcal{N}_{A\to B}
%,\mathcal{M}_{A\to B})$ is characterized by the following primal and dual
%semi-definite programs:%
%\begin{align}
%\sqrt{F}(\rho,\sigma)  & =\frac{1}{2}\sup_{X\in\mathcal{L}(\mathcal{H}%
%)}\left\{  \operatorname{Tr}[X]+\operatorname{Tr}[X^{\dag}]:%
%\begin{pmatrix}
%\rho & X\\
%X^{\dag} & \sigma
%\end{pmatrix}
%\geq0\right\}  \label{eq:QM-over:fidelity-channels-primal-SDP}\\
%& =\frac{1}{2}\inf_{Y,Z\geq 0}\left\{  \operatorname{Tr}[Y\rho]+\operatorname{Tr}%
%[Z\sigma]:%
%\begin{pmatrix}
%Y & \mathbbm{1}\\
%\mathbbm{1} & Z
%\end{pmatrix}
%\geq0\right\}  \label{eq:QM-over:fidelity-channels-dual-SDP}%
%\end{align}
%	\end{proposition*}
%	
%	Using this semi-definite program, we then find the following for the root
%fidelity of quantum channels:

\begin{proposition*}{SDP for Root Fidelity of Channels}
{prop:QM-over:SDP-fidelity-channels}
Let $\mathcal{N}_{A\rightarrow B}$ and $\mathcal{M}
_{A\rightarrow B}$ be quantum channels with respective Choi operators
$\Gamma_{RB}^{\mathcal{N}}$ and $\Gamma_{RB}^{\mathcal{M}}$. Then their root
channel fidelity
\begin{equation}
\sqrt{F}(\mathcal{N}_{A\rightarrow B},\mathcal{M}_{A\rightarrow B}
)\coloneqq \inf_{\psi_{RA}}\sqrt{F}(\mathcal{N}_{A\rightarrow B}(\psi_{RA}
),\mathcal{M}_{A\rightarrow B}(\psi_{RA}))
\end{equation}
can be calculated by means of the following semi-definite program:
\begin{align}
& \sqrt{F}(\mathcal{N}_{A\rightarrow B},\mathcal{M}_{A\rightarrow B}
) \notag \\
& = \sup_{\lambda\geq0,Q_{RB}}\left\{  \lambda:\lambda I_{R}\leq\operatorname{Re}
[\operatorname{Tr}_{B}[Q_{RB}]],\quad
\begin{pmatrix}
\Gamma_{RB}^{\mathcal{N}} & Q_{RB}^{\dag}\\
Q_{RB} & \Gamma_{RB}^{\mathcal{M}}
\end{pmatrix}
\geq0\right\}   \label{eq:SDP-root-fid-ch}\\
& = \frac{1}{2}\inf_{\rho_{R}\geq 0,W_{RB},Z_{RB}}
\Bigg\{\operatorname{Tr}[\Gamma
_{RB}^{\mathcal{N}}W_{RB}]+\operatorname{Tr}[\Gamma_{RB}^{\mathcal{M}}Z_{RB}] : 
\operatorname{Tr}[\rho_{R}]=1,\notag \\
& \qquad\qquad\qquad\qquad\qquad\qquad
\begin{pmatrix}
W_{RB} & \rho_{R}\otimes I_{B}\\
\rho_{R}\otimes I_{B} & Z_{RB}
\end{pmatrix}
\geq 0\Bigg\}.
\end{align}
The expression in \eqref{eq:SDP-root-fid-ch}\ is equal to
\begin{equation}
\sup_{Q_{RB}}\left\{  \lambda_{\min}\left(  \operatorname{Re}
[\operatorname{Tr}_{B}[Q_{RB}]]\right)  :
\begin{pmatrix}
\Gamma_{RB}^{\mathcal{N}} & Q_{RB}^{\dag}\\
Q_{RB} & \Gamma_{RB}^{\mathcal{M}}
\end{pmatrix}
\geq0\right\}  ,
\end{equation}
where $\lambda_{\min}$ denotes the minimum eigenvalue of its argument.
\end{proposition*}
	
	\begin{Proof}
	See Appendix \ref{app:QM-over:SDP-fid-chs}.
	\end{Proof}
	
	
	The inequality in \eqref{eq-Fuchs_van_de_graaf} relating the fidelity between two states $\rho$ and $\sigma$ and their trace distance can be used to relate the fidelity-based distance measure $F(\mathcal{N},\mathcal{M})$ on channels and the diamond distance $\frac{1}{2}\norm{\mathcal{N}-\mathcal{M}}_{\diamond}$. It is straightfoward to show that
	\begin{equation}
		1-\sqrt{F(\mathcal{N},\mathcal{M})}\leq\frac{1}{2}\norm{\mathcal{N}-\mathcal{M}}_{\diamond}\leq\sqrt{1-F(\mathcal{N},\mathcal{M})}.
	\end{equation}
	
	The following proposition relates the fidelity $F(\mathcal{N})$ of a channel $\mathcal{N}$ to its minimum fidelity $F_{\min}(\mathcal{N})$ in \eqref{eq-minimum_fidelity_chan}, telling us that if $F_{\min}(\mathcal{N})$ is large then so is $F(\mathcal{N})$.
	
	\begin{proposition}{prop:min-fid-to-min-ent-fid}
		Let $\mathcal{N}$ be a quantum channel. For all $\varepsilon\in[0,1]$, if $F_{\min}(\mathcal{N})\geq 1-\varepsilon$, then $F(\mathcal{N})\geq 1-2\sqrt{\varepsilon}$.
	\end{proposition}
	
	\begin{Proof}
		The inequality in $F_{\min}(\mathcal{N})\geq 1-\varepsilon$ implies that the following inequality holds for all state vectors $\ket{\phi}\in\mathcal{H}$:%
		\begin{equation}
			\bra{\phi}\left[\ket{\phi}\!\bra{\phi}-\mathcal{N}(\ket{\phi}\!\bra{\phi})\right]\ket{\phi}\leq\varepsilon.
		\end{equation}
		By \eqref{eq-Fuchs_van_de_graaf}, this implies that
		\begin{equation}\label{eq:min-to-ent-t-norm-bnd}
			\norm{\ket{\phi}\!\bra{\phi}-\mathcal{N}(\ket{\phi}\!\bra{\phi})}_{1}\leq 2\sqrt{\varepsilon},
		\end{equation}
		for all state vectors $\ket{\phi}\in\mathcal{H}$. We will show that
		\begin{equation}\label{eq:ortho-pairs-fid-bnd}
			\left| \bra{\phi}\left[\ket{\phi}\!\bra{\phi^{\bot}}-\mathcal{N}(\ket{\phi}\!\bra{\phi^{\bot}})\right]\ket{\phi^{\bot}}\right| \leq 2\sqrt{\varepsilon},
		\end{equation}
		for every orthonormal pair $\left\{\ket{\phi},\ket{\phi^{\bot}}\right\}$ of state vectors in $\mathcal{H}$. Set%
		\begin{equation}
			\ket{w_{k}}\coloneqq\frac{\ket{\phi}+\I^{k}\ket{\phi^{\bot}}}{\sqrt{2}},
		\end{equation}
		for $k\in\{0,1,2,3\}$. Then, it follows that%
		\begin{equation}\label{eq:ortho-pairs-char}
			\ket{\phi}\!\bra{\phi^{\bot}}=\frac{1}{2}\sum_{k=0}^{3}\I^{k}\ket{w_{k}}\!\bra{w_{k}}.
		\end{equation}
		Consider now that%
		\begin{align}
			&\left|\bra{\phi}\left[\ket{\phi}\!\bra{\phi^{\bot}}-\mathcal{N}(\ket{\phi}\!\bra{\phi^{\bot}})\right]\ket{\phi^{\bot}}\right| \nonumber\\
			&\leq \norm{\ket{\phi}\!\bra{\phi^{\bot}}-\mathcal{N}(\ket{\phi}\!\bra{\phi^{\bot}})}_{\infty}\\
			&\leq\frac{1}{2}\sum_{k=0}^{3}\norm{\ket{w_{k}}\!\bra{w_{k}}-\mathcal{N}(\ket{w_{k}}\!\bra{w_{k}})}_{\infty}\\
			&\leq\frac{1}{4}\sum_{k=0}^{3}\norm{\ket{w_{k}}\!\bra{w_{k}}-\mathcal{N}(\ket{w_{k}}\!\bra{w_{k}})}_{1}\\
			&  \leq 2\sqrt{\varepsilon}.
		\end{align}
		The first inequality follows from the characterization of the operator norm in \eqref{eq-inf_norm_matrix_sing_decomp} as $\norm{X}_{\infty}=\sup_{|\phi\rangle,|\psi\rangle}\abs{\bra{\psi}X\ket{\phi}}$, where the optimization is with respect to pure states. The second inequality follows from substituting \eqref{eq:ortho-pairs-char} and applying the triangle inequality and homogeneity of the $\infty$-norm. The third inequality follows because the $\infty$-norm of a traceless Hermitian operator is bounded from above by half of its trace norm (see Lemma~\ref{lem-QCAP:traceless-Hermitian} below). The final inequality follows from applying \eqref{eq:min-to-ent-t-norm-bnd}. Let $\ket{\psi}\in\mathcal{H}^{\prime}\otimes\mathcal{H}$ be an arbitrary state. All such states have a Schmidt decomposition of the following form:
		\begin{equation}
			\ket{\psi}=\sum_{x}\sqrt{p(x)}|\zeta_{x}\rangle\otimes|\varphi_{x}\rangle,
		\end{equation}
		where $\{p(x)\}_{x}$ is a probability distribution and $\{\ket{\zeta_{x}}\}_{x}$ and $\{\ket{\varphi_{x}}\}_{x}$ are sets of states. Then, consider that%
		\begin{align}
			&  1-\bra{\psi}(\id_{\mathcal{H}^{\prime}}\otimes \mathcal{N})(\ket{\psi}\!\bra{\psi})\ket{\psi}\nonumber\\
			&  =\bra{\psi}(\id_{\mathcal{H}^{\prime}}\otimes\id_{\mathcal{H}}-\id_{\mathcal{H}^{\prime}}\otimes\mathcal{N})(\ket{\psi}\!\bra{\psi})\ket{\psi}\\
			&  =\bra{\psi}(\id_{\mathcal{H}^{\prime}}\otimes\left[\id_{\mathcal{H}}-\mathcal{N}\right])(\ket{\psi}\!\bra{\psi})\ket{\psi}\\
			&  =\sum_{x,y}p(x)p(y)\bra{\varphi_{x}}\left[\ket{\varphi_{x}}\!\bra{\varphi_{y}}-\mathcal{N}(\ket{\varphi_{x}}\!\bra{\varphi_{y}})\right]\ket{\varphi_{y}}.
		\end{align}
		Now, applying the triangle inequality and \eqref{eq:ortho-pairs-fid-bnd}, we find that the following holds for all $\ket{\psi}\in\mathcal{H}^{\prime}\otimes\mathcal{H}$:
		\begin{align}
			&  1-\bra{\psi}(\id_{\mathcal{H}^{\prime}}\otimes\mathcal{N})(\ket{\psi}\!\bra{\psi})\ket{\psi}\nonumber\\
			&  =\left|\sum_{x,y}p(x)p(y)\bra{\varphi_{x}}\left[\ket{\varphi_{x}}\!\bra{\varphi_{y}}-\mathcal{N}(\ket{\varphi_{x}}\!\bra{\varphi_{y}})\right]\ket{\varphi_{y}}\right| \\
			&  \leq\sum_{x,y}p(x)p(y)\left|\bra{\varphi_{x}}\left[\ket{\varphi_{x}}\!\bra{\varphi_{y}}-\mathcal{N}(\ket{\varphi_{x}}\!\bra{\varphi_{y}})\right]\ket{\varphi_{y}}\right| \\
			&  \leq 2\sqrt{\varepsilon}.
		\end{align}
		This concludes the proof.
	\end{Proof}
	
	

\section{Bibliographic Notes}\label{sec:qm:bib-notes}




	More details on many of the concepts that have been presented in this chapter can be found in the  books of \citet{NC00}, \citet{H13book}, \citet{H17}, \citet{Wbook17}, and \citet{Wat18}. For a treatment of these concepts in infinite-dimensional Hilbert spaces, see the books by \citet{H13book} and \citet{HZ12}. A more mathematically oriented exposition of completely positive maps is available in \citet{paulsen_2003}.
	
	The mathematical theory of quantum mechanics was developed by \citet{Neu1927,Neu32} and \citet{Lan27}. The book by \citet{Hel76} also contains early developments in the theory of quantum measurements. 
	
	We have used quantum-optical modes as a concrete example of qubit encodings throughout this chapter. For a detailed reference on this topic, see the review by \citet{KMNRDM07}.
	
	Lemma~\ref{lem-symm_purif}, regarding purifications of permutation-invariant states, is due to \citet{RennerThesis}. Separable and entangled states were defined by \citet{Wer89}. The relevance of the partial transpose for characterizing entanglement in quantum information was given by \citet{Per96,HHH96}, and the set of positive-partial-tranpose states was discussed by \citet{PH97,HHH98}. In particular, the existence of PPT entangled states was found by \citet{PH97}.
	
	
	The problem of state discrimination as described in Section \ref{subsec-state_discrimination} was considered by \citet{Hel67} (see also \citet{H69}) and \citet{Hol72}, who determined the optimal success probability in the case of projective measurements and general POVMs, respectively. The proof of the optimal measurement operators in Theorem~\ref{thm-Holevo_Helstrom} is due to \citet{Jen10}. Lemma~\ref{lemma:spectral-ineq} is due to \citet{ACMBMAV07}, with the simple proof presented here attributed by \citet{JOPS12} and \citet{A14} as being due to N.~Ozawa. The Chernoff bound for probability distributions was given by \citet{Cher52}. The corresponding bound for quantum states in Theorem~\ref{thm-quantum_Chernoff} was established in two works: \citet{ACMBMAV07} determined the upper bound on the optimal error exponent, while \citet{nussbaum2009chernoff} established the lower bound. The semi-definite program and complementary slackness conditions for multiple state discrimination in Section~\ref{sec:QM-over:multiple-state-disc} are due to \citet{YKL75}.
	
	The Choi representation of a linear map is named after \citet{C75}, with his paper establishing the equivalence between complete positivity of a map and positivity of its Choi representation. Naimark's dilation theorem for positive operator-valued measures was established by \citet{N40} (see also \citet{GN43}). Stinespring's dilation theorem for completely positive maps was established by \citet{Sti55}. An early exposition of the theory of quantum channels was presented by \citet{K83}. \citet{Leifer07} proposed the concept of conditional states (see also \citep{LS13}). Proposition~\ref{prop-extension_purif} was found by \citet{CW04}. The channel in \eqref{eq-isometry_recover} for reversing the action of an isometric channel was presented by \citet{Wbook17}. The notions of a complementary channel and a degradable channel were defined by \citet{DS05}. Anti-degradable channels were defined by \citet{CG06}. The quantum erasure channel was defined by \citet{GBP97}. The connection of the amplitude damping channel to the bosonic pure-loss channel was realized by \citet{GF05}. The quantum instrument formalism was developed by \citet{DL70} and further developed by \citet{Ozawa1984}. Entanglement-breaking channels were defined by \citet{HSR03} and several of their properties were established therein. Hadamard channels were defined by \citet{KMNR07}. 

	The Petz recovery map was established by \citet{Petz1986} and \citet{Petz1988} in the context of proving the conditions under which equality holds in the monotonicty of the quantum relative entropy.  The results therein are stated for von Neumann algebras. A more accessible exposition that considers operators acting only on finite-dimensional Hilbert spaces can be found in \citet{Petz2001} and \citet{MP04} (see also \citet{HJPW04}). 
	
	The paradigm of local operations and classical communication was defined by \citet{BDSW96}, and its mathematical properties were explored in more detail by \citet{CLM+14}. See Section 4.3 of \citet{CLM+14} for a justification of the example provided in Section \ref{subsec-LOCC_channels} of a separable channel that is not an LOCC channel. Separable channels were defined by \citet{VPRK97,BNS98}. The existence of a separable channel that is not LOCC was found by \citet{PhysRevA.59.1070}. Completely PPT-preserving channels were defined by \citet{R99} and further developed by \citet{CVGG17}. Non-signaling channels were introduced and studied by \citet{BGNP01,ESW02} and further considered by \citet{PHHH06}.
	
	The quantum teleportation protocol for qubits and qudits presented in Section~\ref{sec-teleportation} was devised by \citet{BBC+93}. The generalization to groups that act irreducibly on the input state was presented by \citet{BDMS00,Werner01}. Covariant channels were considered by \citet{Hol02}. For an overview of group- and representation-theoretic concepts for finite groups, see \citet{group_theory_book}. The notion of teleportation simulation of a quantum channel was presented by \citet{BDSW96} (see Section~V therein). The LOCC simulation of a quantum channel was given by \citet{HHH99} (see Eq.~(10) therein), and the related PPT simulation of a quantum channel was given by \citet{KW17}.  The generalized teleportation simulation of a quantum channel was developed for groups that act irreducibly on the channel input space by \citet{CDP09} (see Section~VII therein). \citet{PLOB15} played a role in developing the tool of LOCC/teleportation simulation in more recent years. The fact that the channel twirl can be realized by generalized teleportation simulation was observed by \citet{KW17} (see Appendix~B therein). The teleportation protocol was extended to states of bosonic systems by \citet{prl1998braunstein}.  Teleportation simulation of bosonic Gaussian channels was given by \citet{GI02,NFC09}, and a detailed analysis of convergence in this scenario was presented by \citet{PhysRevA.97.062305}.
	
	The quantum super-dense coding protocol was given by \citet{PhysRevLett.69.2881}.
	 
	The quantum fidelity was defined by \citet{Uhl76}, and Theorem~\ref{thm-Uhlmann_fidelity} is due to \citet{Uhl76}. The semi-definite program for root fidelity in Proposition~\ref{prop:QM-over:SDP-fidelity-states} was established by \citet{Wat13}, and we have followed the proof therein. The fact that the fidelity is achieved by a quantum measurement was realized by \citet{FC95}. The relation between trace distance and fidelity presented in Theorem~\ref{thm-Fuchs_van_de_graaf} was proved by \citet{FG98}. For very closely related inequalities, with the fidelity replaced by the ``Holevo fidelity'' $(\Tr[\sqrt{\rho}\sqrt{\sigma}])^2$, see \citet{Kholevo1972}. The sine distance was defined by \citet{R02,R03,GLN04,R06}, and its interpretation in terms of the minimal trace distance of purifications was given by \citet{R06}. The sine distance was generalized to subnormalized states by \citet{TCR10}, where it was given the name ``purified distance.''
	
	The diamond norm was presented and studied by \citet{Kit97}, who applied it to problems in quantum information theory and quantum computation. The operational interpretation of the diamond distance in terms of hypothesis testing of quantum channels was given by \citet{KWerner04,RW05,GLN04}. More properties of the diamond norm can be found in \citet{Wat18}. The SDP in Proposition~\ref{prop-diamond_dist_SDP} for the normalized diamond distance of quantum channels was given by \citet{Wat09}.

\citet{Sch96} introduced the entanglement fidelity of a quantum channel, and \citet{BKN98} made further observations regarding it. \citet{Nielsen2002249} provided a simple proof for the relation between entanglement fidelity and average fidelity in \eqref{eq:QM-over:average-fid-to-ent-fid}. The fidelity of quantum channels was introduced by \citet{GLN04}, and it can be understood as a special case of the generalized channel divergence \citep{LKDW18}. A semi-definite program for the root fidelity of channels was given by \citet{Yuan2017}. The particular semi-definite program in Proposition~\ref{prop:QM-over:SDP-fidelity-channels}, for the root fidelity of channels, was presented by \citet{KW20}. Proposition~\ref{prop:min-fid-to-min-ent-fid} was established by \citet{BKN98} and reviewed by \citet{KWerner04}. Here we followed the proof given by \citet[Theorem~3.56]{Wat18}, which
therein established a relation between trace distance and
diamond distance between an arbitrary channel and the
identity channel.

\begin{subappendices}


\section{The Quantum Chernoff Bound}\label{app-Chernoff}
	
%	Before getting to the proof of the quantum Chernoff bound, let us first show that the error probability $p_{\text{err}}^*(\lambda\rho^{\otimes n},\bar{\lambda}\sigma^{\otimes n})$ decays exponentially with $n$.
%	
%	Letting $\lambda$ be the probability of having the state $\rho^{\otimes n}$ in the state discrimination task, and applying Lemma~\ref{lemma:spectral-ineq} with $A=\lambda\rho^{\otimes n}$, $B=(1-\lambda)\sigma^{\otimes n}$, and $s=1/2$, we find that
%	\begin{align}
%		p_{\text{err}}^*(\{\rho,\sigma\})&=\frac{1}{2}\left(1-\norm{\lambda\rho^{\otimes n}-(1-\lambda)\sigma^{\otimes n}}_1\right)\\
%		&\leq
%		\Tr\!\left[ \sqrt{\lambda\rho^{\otimes n}}\sqrt{(1-\lambda)\sigma^{\otimes n}}\right]\\
%				&=
%		\sqrt{\lambda(1-\lambda)} \Tr\!\left[ \sqrt{\rho^{\otimes n}}\sqrt{\sigma^{\otimes n}}\right]\\
%		&\leq
%		\sqrt{\lambda(1-\lambda)} F(\rho^{\otimes n},\sigma^{\otimes n})^{\frac{1}{2}}
%		\\
%		&\leq F(\rho,\sigma)^{\frac{n}{2}},
%	\end{align}
%	where to obtain the second-to-last inequality, we employed Proposition~\ref{prop:math-tools:var-char-t-norm} and Definition~\ref{def-fidelity}, and to obtain the last inequality, we used the fact that $\lambda(1-\lambda)\leq 1$ and the multiplicativity of the fidelity (see \eqref{eq-fidelity_multiplicative}). Then, because the fidelity between two quantum states is always between zero and one, it follows that the optimal error probability $p_{\text{err}}^*(\lambda\rho^{\otimes n},\bar{\lambda}\sigma^{\otimes n})$ decays monotonically with $n$, i.e.,
%	\begin{equation}
%		p_{\text{err}}^*(\lambda\rho^{\otimes n},\bar{\lambda}\sigma^{\otimes n})\to 0\quad\text{as}\quad n\to\infty.
%	\end{equation}
%	In particular, the optimal error probability decreases at an exponential rate:
%	\begin{equation}
%		p_{\text{err}}^*(\lambda\rho^{\otimes n},\bar{\lambda}\sigma^{\otimes n})\leq 2^{-n\xi(\rho,\sigma)},
%	\end{equation}
%	where $\xi(\rho,\sigma)\coloneqq -\frac{1}{2}\log_2F(\rho,\sigma)\geq 0$. The inequality above can be written as
%	\begin{equation}\label{eq-state_disc_err_prob_decay}
%		-\frac{1}{n}\log_2 p_{\text{err}}^*(\lambda\rho^{\otimes n},\bar{\lambda}\sigma^{\otimes n}) \geq  \xi(\rho,\sigma).
%	\end{equation}
%	The rate of the exponential decay is at least $\xi(\rho,\sigma)$, and it is thus one possible error exponent.
%%	The inequality in \eqref{eq-state_disc_err_prob_decay} implies that
%%	\begin{align}
%%		r_{\text{err}}^*(\{\rho,\sigma\})&\coloneqq\inf_{n\geq 1}\frac{1}{n}\log_2 p_{\text{err}}^*(\lambda\rho^{\otimes n},\bar{\lambda}\sigma^{\otimes n})\\
%%		&=\lim_{n\to\infty} \frac{1}{n}\log_2 p_{\text{err}}^*(\lambda\rho^{\otimes n},\bar{\lambda}\sigma^{\otimes n}).
%%	\end{align}

	The quantities $\underline{\xi}(\rho,\sigma)$ and $ \overline{\xi}(\rho,\sigma)$ are by definition the optimal error exponents, and the quantum Chernoff bound (Theorem~\ref{thm-quantum_Chernoff}) establishes that they are equal to the Chernoff divergence in \eqref{eq:qm:chern-divergence}. It is an important quantity to consider because it tells us how fast the error probability converges to zero as $n$ increases. 
	
	We now proceed to the proof of the quantum Chernoff bound, which is the following statement: For quantum states $\rho$ and $\sigma$, the optimal error exponents of discrimination, as defined in \eqref{eq:qm-over:chernoff-def-lower} and \eqref{eq:qm-over:chernoff-def-upper},  are given by
	\begin{equation}
		\underline{\xi}(\rho,\sigma)= \overline{\xi}(\rho,\sigma)= \sup_{s\in(0,1)} \left(-\log_2\Tr[\rho^s\sigma^{1-s}]\right).
	\end{equation}
	
\subsection{Proof of Theorem~\ref{thm-quantum_Chernoff}}
	
	If $\lambda$ is the probability with which $\rho$ is chosen, and $1-\lambda$ the probability with which $\sigma$ is chosen, then an application of Lemma~\ref{lemma:spectral-ineq}, with $A=\lambda\rho^{\otimes n}$, $B=(1-\lambda)\sigma^{\otimes n}$, and $s\in(0,1)$, gives the following:
	\begin{align}
		p_{\text{err}}^*(\lambda\rho^{\otimes n},\bar{\lambda}\sigma^{\otimes n})&=\frac{1}{2}\left(1-\norm{\lambda\rho^{\otimes n}-(1-\lambda)\sigma^{\otimes n}}_1\right)\\
		&\leq \Tr\!\left[\lambda^s(\rho^{\otimes n})^s(1-\lambda)^{1-s}(\sigma^{\otimes n})^{1-s}\right]\\
		&=\lambda^s(1-\lambda)^{1-s}\Tr[(\rho^s)^{\otimes n}(\sigma^{1-s})^{\otimes n}]\\
		&=\lambda^s(1-\lambda)^{1-s}\left(\Tr[\rho^s\sigma^{1-s}]\right)^n\\
		&\leq \left(\Tr[\rho^s\sigma^{1-s}]\right)^n,
	\end{align}
	where  the last line follows from the fact that $\lambda^s(1-\lambda)^{1-s}\leq 1$. Since the bound above holds for all $s\in(0,1)$, we obtain the following bound:
	\begin{equation}\label{eq-quantum_Chernoff_pf}
		\underline{\xi}(\rho,\sigma)=\liminf_{n\to\infty}-\frac{1}{n}\log_2 p_{\text{err}}^*(\lambda\rho^{\otimes n},\bar{\lambda}\sigma^{\otimes n})\geq \sup_{s\in(0,1)}- \log_2\Tr[\rho^s\sigma^{1-s}].
	\end{equation}
	
	For the reverse inequality, we start by observing that it suffices to optimize over projectors when determining the optimal error probability $p_{\text{err}}^*(\lambda\rho^{\otimes n},\bar{\lambda}\sigma^{\otimes n})$. (This holds because one choice of an optimal measurement is a projective measurement, as shown in the proof of Theorem~\ref{thm-Holevo_Helstrom}, where we can set $\Lambda_0 = 0$.) Next, let $\rho$ and $\sigma$ have the following spectral decompositions:
	\begin{equation}
		\rho=\sum_{i=0}^{d-1} \lambda_i \ket{\psi_i}\!\bra{\psi_i},\quad \sigma=\sum_{j=0}^{d-1} \mu_j \ket{\phi_j}\!\bra{\phi_j},
	\end{equation}
	where $d$ is the dimension of the underlying Hilbert space. Then, for every projection $\Pi$,
	\begin{align}
		\Tr[(\mathbbm{1}-\Pi)\rho]&=\sum_{i=0}^{d-1} \lambda_i\Tr[(\mathbbm{1}-\Pi)\ket{\psi_i}\!\bra{\psi_i}]\\
		&=\sum_{i=0}^{d-1} \lambda_i\Tr[(\mathbbm{1}-\Pi)\ket{\psi_i}\!\bra{\psi_i}(\mathbbm{1}-\Pi)]\\
		&=\sum_{i,j=0}^{d-1}\lambda_i\Tr[\ket{\phi_j}\!\bra{\phi_j}(\mathbbm{1}-\Pi)\ket{\psi_i}\!\bra{\psi_i}(\mathbbm{1}-\Pi)]\\
		&=\sum_{i,j=0}^{d-1} \lambda_i\abs{\bra{\psi_i}(\mathbbm{1}-\Pi)\ket{\phi_j}}^2,
	\end{align}
	where we have used the fact that $\mathbbm{1}=\sum_{j=0}^{d-1}\ket{\phi_j}\!\bra{\phi_j}$. Similarly, using the fact that $\mathbbm{1}=\sum_{i=0}^{d-1}\ket{\psi_i}\!\bra{\psi_i}$, we have
	\begin{align}
		\Tr[\Pi\sigma]&=\sum_{j=0}^{d-1} \mu_j\Tr[\Pi\ket{\phi_j}\!\bra{\phi_j}]\\
		&=\sum_{j=0}^{d-1}\mu_j\Tr[\Pi\ket{\phi_j}\!\bra{\phi_j}\Pi]\\
		&=\sum_{i,j=0}^{d-1}\mu_j\Tr[\ket{\psi_i}\!\bra{\psi_i}\Pi\ket{\phi_j}\!\bra{\phi_j}\Pi]\\
		&=\sum_{i,j=0}^{d-1}\mu_j\abs{\bra{\psi_i}\Pi\ket{\phi_j}}^2.
	\end{align}
	Then, using the fact that $\lambda_i\geq\min\{\lambda_i,\mu_j\}$ and $\mu_j\geq\min\{\lambda_i,\mu_j\}$ for all $0\leq i,j\leq d-1$, the error probability under the measurement given by $\Pi$ is
	\begin{align}
		&p_{\text{err}}(\{\Pi,\mathbbm{1}-\Pi\};\{\rho,\sigma\})\nonumber\\
		&\quad =\Tr[(\mathbbm{1}-\Pi)(\lambda\rho)]+\Tr[\Pi(1-\lambda)\sigma]\\
		&\quad=\sum_{i,j=0}^{d-1} \left(\lambda\lambda_i\abs{\bra{\psi_i}(\mathbbm{1}-\Pi)\ket{\phi_j}}^2+(1-\lambda)\mu_j\abs{\bra{\psi_i}\Pi\ket{\phi_j}}^2\right)\\
		&\quad \geq \frac{1}{2}\min\{\lambda\lambda_i,(1-\lambda)\mu_j\}(\abs{x_{i,j}}^2+\abs{y_{i,j}}^2),
	\end{align}
	where in the last line we have defined $x_{i,j}\coloneqq\bra{\psi_i}(\mathbbm{1}-\Pi)\ket{\phi_j}$ and $y_{i,j}\coloneqq\bra{\psi_i}\Pi\ket{\phi_j}$.  Using the identity $\abs{a}^2+\abs{b}^2\geq\frac{1}{2}\abs{a+b}^2$, which holds for all $a,b\in\mathbb{C}$, we obtain
	\begin{equation}
		p_{\text{err}}(\{\Pi,\mathbbm{1}-\Pi\};\{\rho,\sigma\})\geq \frac{1}{2}\sum_{i,j=0}^{d-1} \min\{\lambda\lambda_i,(1-\lambda)\mu_j\}\abs{\braket{\psi_i}{\phi_j}}^2.
	\end{equation}
	Now, let us define two probability distributions, $p,q:\{0,1,\dotsc,d-1\}^2\to[0,1]$ as follows:
	\begin{equation}
		p(i,j)\coloneqq \lambda_i\abs{\braket{\psi_i}{\phi_j}}^2,\quad q(i,j)\coloneqq \mu_j\abs{\braket{\psi_i}{\phi_j}}^2,\quad\forall~0\leq i,j\leq d-1.
	\end{equation}
	It is straightforward to verify that $p$ and $q$ are indeed probability distributions. Then, since the projector $\Pi$ is arbitrary, and it suffices to optimize over projective measurements, as explained above, the following inequality holds
	\begin{equation}
		p_{\text{err}}^*(\{\rho,\sigma\})\geq \frac{1}{2}\sum_{i,j=0}^{d-1}\min\{\lambda p(i,j),(1-\lambda)q(i,j)\}.
	\end{equation}
	The expression on the right-hand side of the above inequality is precisely half the optimal error probability for discriminating the two probability distributions $p$ and $q$, with a prior probability of $\lambda$. Indeed, we can see this by an application of Theorem~\ref{thm-Holevo_Helstrom} to the case of commutative $A$ and $B$. To this end, letting $A = \sum_{i=0}^{d-1} a_i \ket{i}\!\bra{i}$ and $B = \sum_{i=0}^{d-1} b_i \ket{i}\!\bra{i}$ where $a_i,b_i\geq 0$ for all $i\in \{0,\dotsc,d-1\}$, it follows that an optimal measurement operator $\Pi_+ = \sum_{i:a_i \geq b_i} \ket{i}\!\bra{i}$ and its complement $\Pi_- = \sum_{i:a_i < b_i} \ket{i}\!\bra{i}$, so that
	\begin{align}
	\inf_{M:0\leq M\leq\mathbbm{1}}\left\{\Tr[(\mathbbm{1}-M)A]+\Tr[MB]\right\} & =
	\Tr[\Pi_- A]+\Tr[\Pi_+ B] \\
	& = \sum_{i : a_i < b_i} a_i + \sum_{i : a_i \geq b_i} b_i \\
	& = \sum_{i=0}^{d-1} \min\{a_i,b_i\}.
	\end{align}
	
	We denote this optimal error probability by $p_{\text{err}}(\{p,q\})$. Therefore,
	\begin{equation}
		p_{\text{err}}^*(\{\rho,\sigma\})\geq \frac{1}{2} p_{\text{err}}^*(\{p,q\}).
	\end{equation}
	Now, for $n\geq 2$, by following the same arguments as above, we obtain
	\begin{equation}
		p_{\text{err}}^*(\lambda\rho^{\otimes n},\bar{\lambda}\sigma^{\otimes n})\geq \frac{1}{2} p_{\text{err}}^*(\{p^{(n)},q^{(n)}\}),
		\label{eq:qm-c-to-q-chernoff-asymp}
	\end{equation}
	where $p^{(n)},q^{(n)}$ are the $n$-fold i.i.d probability distributions corresponding to $p$ and $q$, respectively. Then, by the classical Chernoff bound (please consult the Bibliographic Notes in Section~\ref{sec:qm:bib-notes}), we find that
	\begin{align}
		\overline{\xi}(\rho,\sigma)&=\limsup_{n\to\infty}-\frac{1}{n}\log_2 p_{\text{err}}^*(\lambda\rho^{\otimes n},\bar{\lambda}\sigma^{\otimes n})\\
		&\leq\limsup_{n\to\infty}-\frac{1}{n}\log_2 p_{\text{err}}^*(\{p^{(n)},q^{(n)}\})\\
		&=\sup_{s\in(0,1)}-\log_2\sum_{i,j=0}^{d-1} p(i,j)^sq(i,j)^{1-s},
	\end{align}
	where the factor of $\tfrac{1}{2}$ in \eqref{eq:qm-c-to-q-chernoff-asymp} vanishes in the asymptotic limit. 
	Finally, observe that
	\begin{align}
		\sum_{i,j=0}^{d-1} p(i,j)^s q(i,j)^{1-s}&=\sum_{i,j=0}^{d-1} \lambda_i^s\left(\abs{\braket{\psi_i}{\phi_j}}^2\right)^s\mu_j^{1-s}\left(\abs{\braket{\psi_i}{\phi_j}}^2\right)^{1-s}\\
		&=\sum_{i,j=0}^{d-1} \lambda_i^s\mu_j^{1-s}\abs{\braket{\psi_i}{\phi_j}}^2\\
		&=\sum_{i,j=0}^{d-1} \lambda_i^s\mu_j^{1-s}\Tr[\ket{\psi_i}\langle \psi_i| \phi_j \rangle \!\bra{\phi_j}]\\
		&=\Tr\!\left[\left(\sum_{i=0}^{d-1}\lambda_i^s \ket{\psi_i}\!\bra{\psi_i}\right)\left(\sum_{j=0}^{d-1} \mu_j^{1-s}\ket{\phi_j}\!\bra{\phi_j}\right)\right]\\
		&=\Tr[\rho^s\sigma^{1-s}].
	\end{align}
	Therefore,
	\begin{equation}
		\overline{\xi}(\rho,\sigma)\leq \sup_{s\in(0,1)} - \log_2\Tr[\rho^s\sigma^{1-s}],
	\end{equation}
	which, combined with \eqref{eq-quantum_Chernoff_pf}, implies that
	\begin{equation}
		\underline{\xi}(\rho,\sigma) = \overline{\xi}(\rho,\sigma)=\sup_{s\in(0,1)} -\log_2\Tr[\rho^s\sigma^{1-s}],
	\end{equation}
	which is what we set out to prove.
	
\section{Support Containment Lemmas}\label{app:QM-over:support-lemmas}

This appendix contains useful technical lemmas about containments of supports of operators.

\begin{Lemma}{lem-app:support-1}Let $X_{AB}\in\mathcal{L}(\mathcal{H}_{A}%
\otimes\mathcal{H}_{B})$ be positive semi-definite, and let $X_{A}
\coloneqq \operatorname{Tr}_{B}[X_{AB}]$ and $X_{B}\coloneqq \operatorname{Tr}
_{A}[X_{AB}]$. Then $\operatorname{supp}(X_{AB})\subseteq\operatorname{supp}%
(X_{A})\otimes\operatorname{supp}(X_{B})$.
\end{Lemma}

\begin{proof}
First suppose that $X_{AB}$ is rank one, so that $X_{AB}=|\Psi\rangle
\langle\Psi|_{AB}$ for some vector $|\Psi\rangle_{AB}\in\mathcal{H}_{A}
\otimes\mathcal{H}_{B}$. Due to the Schmidt decomposition theorem
(Theorem~\ref{thm-Schmidt}), we have that%
\begin{equation}
|\Psi\rangle_{AB}=\sum_{z\in\mathcal{Z}}\gamma_{z}|\theta_{z}\rangle
_{A}\otimes|\xi_{z}\rangle_{B},
\end{equation}
where $\left\vert \mathcal{Z}\right\vert \leq\min\{\dim(\mathcal{H}_{A}
),\dim(\mathcal{H}_{B})\}$, the set $\{\gamma_{z}\}_z$ is a set of strictly positive
numbers, and $\{|\theta_{z}\rangle_{A}\}_z$ and $\{|\xi_{z}\rangle_{B}\}_z$ are
orthonormal bases. Then
\begin{align}
\operatorname{supp}(X_{AB})  &  =\operatorname{span}\{|\Psi\rangle_{AB}\}\\
&  \subseteq\operatorname{span}\{|\theta_{z}\rangle_{A}:z\in\mathcal{Z}
\}\otimes\operatorname{span}\{|\xi_{z}\rangle_{B}:z\in\mathcal{Z}\}.
\end{align}
The statement then follows for this case because $\operatorname{supp}%
(X_{A})=\operatorname{span}\{|\theta_{z}\rangle_{A}:z\in\mathcal{Z}\}$ and
$\operatorname{supp}(X_{B})=\operatorname{span}\{|\xi_{z}\rangle_{B}
:z\in\mathcal{Z}\}$.

Now suppose that $X_{AB}$ is not rank one. It admits a decomposition into
rank-one vectors of the following form:%
\begin{equation}
X_{AB}=\sum_{x\in\mathcal{X}}|\Psi^{x}\rangle\!\langle\Psi^{x}|_{AB},
\end{equation}
where $|\Psi^{x}\rangle_{AB}\in\mathcal{H}_{A}\otimes\mathcal{H}_{B}$ for all
$x\in\mathcal{X}$. Set $\Psi_{AB}^{x}=|\Psi^{x}\rangle\!\langle\Psi^{x}|_{AB}$,
and let $\Psi_{A}^{x}\coloneqq \operatorname{Tr}_{B}[\Psi_{AB}^{x}]$ and
$\Psi_{B}^{x}\coloneqq \operatorname{Tr}_{A}[\Psi_{AB}^{x}]$. Then
\begin{align}
\operatorname{supp}(X_{AB})  &  =\operatorname{span}\{|\Psi^{x}\rangle
_{AB}:x\in\mathcal{X}\}\\
&  \subseteq\operatorname{span}\left[  \bigcup\limits_{x\in\mathcal{X}}\left[
\operatorname{supp}(\Psi_{A}^{x})\otimes\operatorname{supp}(\Psi_{B}
^{x})\right]  \right] \\
&  \subseteq\operatorname{span}\left[  \bigcup\limits_{x\in\mathcal{X}
}\operatorname{supp}(\Psi_{A}^{x})\right]  \otimes\operatorname{span}\left[
\bigcup\limits_{x\in\mathcal{X}}\operatorname{supp}(\Psi_{B}^{x})\right] \\
&  =\operatorname{supp}(X_{A})\otimes\operatorname{supp}(X_{B}),
\end{align}
concluding the proof.
\end{proof}

\begin{Lemma}{lem-app:support-2}Let $X_{AB},Y_{AB}\in\mathcal{L}(\mathcal{H}
_{A}\otimes\mathcal{H}_{B})$ be positive semi-definite, and suppose that
$\operatorname{supp}(X_{AB})\subseteq\operatorname{supp}(Y_{AB})$. Then
$\operatorname{supp}(X_{A})\subseteq\operatorname{supp}(Y_{A})$, where
$X_{A}\coloneqq \operatorname{Tr}_{B}[X_{AB}]$ and $Y_{A}\coloneqq \operatorname{Tr}
_{B}[Y_{AB}]$.
\end{Lemma}

\begin{proof}
First suppose that $X_{AB}$ is rank one, as in the first part of the proof of
the previous lemma, and let us use the same notation as given there. Applying
the same lemma gives that%
\begin{equation}
\operatorname{supp}(X_{AB})\subseteq\operatorname{supp}(Y_{AB})\subseteq
\operatorname{supp}(Y_{A})\otimes\operatorname{supp}(Y_{B}),
\end{equation}
which in turn implies that $\operatorname{supp}(X_{AB})=\operatorname{span}
\{|\Psi\rangle_{AB}\}\subseteq\operatorname{supp}(Y_{A})\otimes
\operatorname{supp}(Y_{B})$. This implies that $|\theta_{z}\rangle_{A}%
\in\operatorname{supp}(Y_{A})$ for all $z\in\mathcal{Z}$, and thus that
$\operatorname{span}\{|\theta_{z}\rangle_{A}\}\in\operatorname{supp}(Y_{A})$.
We can then conclude the statement in this case because $\operatorname{span}
\{|\theta_{z}\rangle_{A}\}=\operatorname{supp}(X_{A})$.

Now suppose that $X_{AB}$ is not rank one. Then it admits a decomposition as
given in the proof of the previous lemma. Using the same notation, we have
that $\operatorname{supp}(\Psi_{AB}^{x})\subseteq\operatorname{supp}(Y_{AB}
)$\ holds for all $x\in\mathcal{X}$. Since we have proven the lemma for
rank-one operators, we can conclude that $\operatorname{supp}(\Psi_{A}
^{x})\subseteq\operatorname{supp}(Y_{A})$\ holds for all $x\in\mathcal{X}$. As
a consequence, we find that
\begin{equation}
\operatorname{supp}(X_{A})=\operatorname{span}\left[  \bigcup\limits_{x\in
\mathcal{X}}\operatorname{supp}(\Psi_{A}^{x})\right]  \subseteq
\operatorname{supp}(Y_{A}),
\end{equation}
concluding the proof.
\end{proof}

\section{SDPs for Normalized Trace and Diamond Distance}

\label{app-trace_dist_fidelity_SDP}


	In this section, we prove that the normalized trace distance between two states and the normalized diamond distance between  two quantum channels can be computed via SDPs. We start with the normalized trace distance, providing a proof of Proposition~\ref{prop-trace_dist_SDP}.
	

\subsection{Proof of Proposition~\ref{prop-trace_dist_SDP}}

	%\begin{Proof}[Proof of Proposition~\ref{prop-trace_dist_SDP}]
		The first expression follows immediately from Theorem \ref{thm-trace_dist_meas} and \eqref{eq-trace_dist_meas}. In particular, \eqref{eq-trace_dist_SDP_primal} is in the standard form of \eqref{eq-primal_SDP_def}, namely,
		\begin{equation}
			\sup\{\Tr[D Y]:\Phi(Y)\leq C,Y\geq 0\},
		\end{equation}
		with $D=\rho-\sigma$, $C=\mathbbm{1}$, and $\Phi=\id$. Then, since $\Phi^\dagger=\id$, the standard form of the dual problem in \eqref{eq-dual_SDP_def} is
		\begin{equation}\label{eq-trace_dist_SDP_dual_2}
			\inf\{\Tr[C Z]:\Phi^\dagger(Z)\geq D,Z\geq 0\},
		\end{equation}
		which is precisely \eqref{eq-trace_dist_SDP_dual}. Note that strong duality holds because $Z=\rho-\sigma+\delta\mathbbm{1}$ is a strictly feasible point in \eqref{eq-trace_dist_SDP_dual_2} for all $\delta>0$.
	%\end{Proof}
	
	We now derive the primal and dual SDPs for the diamond distance between quantum channels, thus providing a proof of Proposition~\ref{prop-diamond_dist_SDP}.
	

\subsection{Proof of Proposition~\ref{prop-diamond_dist_SDP}}
	%\begin{Proof}[Proof of Proposition~\ref{prop-diamond_dist_SDP}]
		Employing \eqref{eq-diamond_dist_meas}, consider that
		\begin{align}
			&\frac{1}{2}\norm{\mathcal{N}-\mathcal{M}}_{\diamond}\nonumber\\
			&\quad =\sup_{\substack{\psi_{RA}\geq 0,\\\Lambda_{RB}\geq 0}}\left\{\begin{array}{c}\Tr[\Lambda_{RB}(\mathcal{N}_{A\to B}-\mathcal{M}_{A\to B})(\psi_{RA})]:\Lambda_{RB}\leq\mathbbm{1}_{RB},\\\Tr[\psi_{RA}]=1,\Tr[\psi_{RA}^2]=1\end{array}\right\},
		\end{align}
		where the constraints $\psi_{RA}\geq 0$, $\Tr[\psi_{RA}]=1$, and $\Tr[\psi_{RA}^2]=1$ correspond to $\psi_{RA}$ being a pure bipartite state. Note that the above is equal to
		\begin{equation}\label{eq-diamond_dist_SDP_pf_1}
			\sup_{\substack{\psi_{RA}\geq 0,\\\Lambda_{RB}\geq 0}}\left\{\begin{array}{c}\Tr[\Lambda_{RB}(\mathcal{N}_{A\to B}-\mathcal{M}_{A\to B})(\psi_{RA})]:\Lambda_{RB}\leq\mathbbm{1}_{RB},\psi_R>0,\\\Tr[\psi_{RA}]=1,\Tr[\psi_{RA}^2]=1\end{array}\right\},
		\end{equation}
		due to the fact that the set of pure states with reduced state $\psi_R$ positive definite is dense in the set of all pure states. Now, recall from \eqref{eq-pure_state_vec} that any such pure state can be written as $\psi_{RA}=X_R\Gamma_{RA}X_R^\dagger$ for some linear operator $X_R$ such that $\Tr[X_R^\dagger X_R]=1$ and $|X_R|>0$, where $\Gamma_{RA}$ defined in \eqref{eq-max_ent_vector}. Using this, we find that the objective function can be rewritten as
		\begin{align}
			&\Tr[\Lambda_{RB}(\mathcal{N}_{A\to B}-\mathcal{M}_{A\to B})(X_R\Gamma_{RA}X_R^\dagger)]\\
			&\quad =\Tr[X_R^\dagger\Lambda_{RB}X_R(\mathcal{N}_{A\to B}-\mathcal{M}_{A\to B})(\Gamma_{RA})]\\
			&=\Tr[X_R^\dagger\Lambda_{RB}X_R(\Gamma_{RB}^{\mathcal{N}}-\Gamma_{RB}^{\mathcal{M}})].
		\end{align}
		Now, observe the following equivalence:
		\begin{equation}
			0\leq\Lambda_{RB}\leq\mathbbm{1}_{RB}\Leftrightarrow 0\leq X_R^\dagger\Lambda_{RB}X_R\leq X_R^\dagger X_R\otimes\mathbbm{1}_B.
		\end{equation}
		Thus, defining $\Omega_{RB}\coloneqq X_R^\dagger\Lambda_{RB}X_R$ and $\rho_R\coloneqq X_R^\dagger X_R$, the optimization in \eqref{eq-diamond_dist_SDP_pf_1} is equivalent to the following one:
		\begin{equation}
			\sup_{\substack{\rho_R,\\\Omega_{RB}\geq 0}}\{\Tr[\Omega_{RB}(\Gamma_{RB}^{\mathcal{N}}-\Gamma_{RB}^{\mathcal{M}})]: \Omega_{RB}\leq\rho_R\otimes\mathbbm{1}_B,\rho_R>0,\Tr[\rho_R]=1\},
		\end{equation}
		giving the equality in \eqref{eq-diamond_dist_SDP_primal}. Finally, setting 
		\begin{align}
			Y&\coloneqq \begin{pmatrix} \Omega_{RB} & 0 \\ 0 & \rho_R \end{pmatrix},\\
			D&\coloneqq \begin{pmatrix} \Gamma_{RB}^{\mathcal{N}}-\Gamma^{\mathcal{M}}_{RB} & 0 \\ 0 & 0 \end{pmatrix},\\
			\Phi(Y)&\coloneqq \begin{pmatrix} \Omega_{RB}-\rho_R\otimes\mathbbm{1}_B & 0 & 0 \\ 0 & \Tr[\rho_R] & 0 \\ 0 & 0 & -\Tr[\rho_R]\end{pmatrix},\\
			C&\coloneqq \begin{pmatrix} 0 & 0 & 0\\ 0 & 1 & 0 \\ 0 & 0 & -1\end{pmatrix}
		\end{align}
		we find that \eqref{eq-diamond_dist_SDP_primal} is now in the standard form from \eqref{eq-primal_SDP_def}, namely,
		\begin{equation}
		\sup_{Y\geq 0}\{\Tr[DY]:\Phi(Y)\leq C\}.
		\end{equation}
		
		Now, to establish the dual SDP in \eqref{eq-diamond_dist_SDP_dual}, we first determine the adjoint $\Phi^\dagger$ of $\Phi$ using
		\begin{equation}
			\Tr[\Phi(Y)Z]=\Tr[Y\Phi^\dagger(Z)],
		\end{equation}
		where without loss of generality we can take $Z$ to be
		\begin{equation}
			Z\coloneqq\begin{pmatrix} Z_{RB} & 0 & 0 \\ 0 & \mu_1 & 0 \\ 0 & 0 & \mu_2\end{pmatrix}.
		\end{equation}
		Then, we find that
		\begin{align}
			\Tr[\Phi(Y)Z]&=\Tr[(\Omega_{RB}-\rho_R\otimes\mathbbm{1}_B)Z_{RB}]+\Tr[\rho_R]\mu_1-\Tr[\rho_R]\mu_2\\
			&=\Tr[\Omega_{RB}Z_{RB}]+\Tr[\rho_R((\mu_1-\mu_2)\mathbbm{1}_R-\Tr_B[Z_{RB}])],
		\end{align}
		from which we conclude that
		\begin{equation}
			\Phi^\dagger(Z)=\begin{pmatrix} Z_{RB} & 0 \\ 0 & (\mu_1-\mu_2)\mathbbm{1}_R-\Tr_B[Z_{RB}] \end{pmatrix}.
		\end{equation}
		The standard form of the dual SDP from \eqref{eq-dual_SDP_def}, which is
		\begin{equation}
		\inf_{Z\geq 0}\{\Tr[CZ]:\Phi^\dagger(Z)\geq D\},
		\end{equation}
		then becomes
		\begin{equation}\label{eq-diamond_dist_SDP_pf_2}
			\inf_{\substack{\mu_1\geq 0,\\\mu_2\geq 0,\\ Z_{RB}\geq 0}}\{\mu_1-\mu_2:Z_{RB}\geq \Gamma_{RB}^{\mathcal{N}}-\Gamma_{RB}^{\mathcal{M}}, (\mu_1-\mu_2)\mathbbm{1}_R\geq \Tr_B[Z_{RB}]\}.
		\end{equation}
		Now, observe that the variables $\mu_1$ and $\mu_2$ always appear together in the above optimization as $\mu_1-\mu_2$, and so can be reduced to the a single real variable $\mu\in\mathbb{R}$. Then, the condition $\mu\mathbbm{1}_R\geq \Tr_B[Z_{RB}]$ implies that $\mu\geq 0$. Thus, the optimization in \eqref{eq-diamond_dist_SDP_pf_2} can be simplified to
		\begin{equation}
			\inf_{\substack{\mu\geq 0,\\ Z_{RB}\geq 0}}\{\mu: Z_{RB}\geq \Gamma_{RB}^{\mathcal{N}}-\Gamma_{RB}^{\mathcal{M}},\mu\mathbbm{1}_R\geq \Tr_B[Z_{RB}]\},
		\end{equation}
		which is precisely \eqref{eq-diamond_dist_SDP_dual}. Equality of the primal and dual SDPs is due to strong duality, which holds for the SDP in \eqref{eq-diamond_dist_SDP_dual} because $Z_{RB}=\Gamma_{RB}^{\mathcal{N}}-\Gamma_{RB}^{\mathcal{M}}+\delta\mathbbm{1}_{RB}$ and $\mu = \Tr_B[Z_{RB}]+\delta\mathbbm{1}_R$ together form a strictly feasible point for all $\delta>0$ and a feasible point for the primal is $\rho_R = \pi_R$ and $\Omega_{RB} = \pi_R \otimes \mathbbm{1}_B$.
		
		Finally, the equality
		\begin{multline}
			\inf_{\substack{\mu\geq 0,\\ Z_{RB}\geq 0}}\{\mu:Z_{RB}\geq \Gamma_{RB}^{\mathcal{N}}-\Gamma_{RB}^{\mathcal{M}},\mu\mathbbm{1}_R\geq \Tr_B[Z_{RB}]\}\\=\inf_{Z_{RB}\geq 0}\{\norm{\Tr_B[Z_{RB}]}_{\infty}:Z_{RB}\geq \Gamma_{RB}^{\mathcal{N}}-\Gamma_{RB}^{\mathcal{M}}\}
		\end{multline}
		holds by the expression in \eqref{eq-PSD_largest_eig_SDP} for the Schatten $\infty$-norm for positive semi-definite operators.
	%\end{Proof}

\section{SDPs for Fidelity of States and Channels}

\label{app:QM-over:SDPs-fidelity}

\subsection{Proof of Proposition~\ref{prop:QM-over:SDP-fidelity-states}}

\label{app:QM-over:SDP-fid-states}

First, let us verify that strong duality holds for the primal and dual
semi-definite programs in \eqref{eq:QM-over:fidelity-primal-SDP} and
\eqref{eq:QM-over:fidelity-dual-SDP}, respectively. Consider that $X=0$ is a
feasible choice for the primal program, while $Y=Z=2\mathbbm{1}$ is strictly feasible
for the dual program. Thus, strong duality holds according to Theorem~\ref{thm:math-tools:slater-cond}.

In order to prove the equality in \eqref{eq:QM-over:fidelity-primal-SDP}, we
start with the following lemma:

\begin{Lemma}{lem:QM-over:Bhatia-lemma-1}
Let $P$ and $Q$ be positive semi-definite
operators in $\mathcal{L}(\mathcal{H})$, and let $X\in\mathcal{L}%
(\mathcal{H})$. Then the operator
\begin{equation}%
\begin{pmatrix}
P & X\\
X^{\dag} & Q
\end{pmatrix}
\end{equation}
is positive semi-definite if and only if there exists $K\in\mathcal{L}%
(\mathcal{H})$ satisfying $\left\Vert K\right\Vert _{\infty}\leq1$ and
$X=\sqrt{P}K\sqrt{Q}$.
\end{Lemma}

\begin{Proof}
See Theorem~IX.5.9 of \citet{Bha97}.
\end{Proof}

It follows from this lemma that the operators $X$ in the primal optimization
in \eqref{eq:QM-over:fidelity-primal-SDP} can range over $X=\sqrt{P}K\sqrt{Q}$
such that $K\in\mathcal{L}(\mathcal{H})$ and $\left\Vert K\right\Vert
_{\infty}\leq1$, so that the optimization over $X$ is reduced to an
optimization over $K$. We then find that the primal optimal value is given by%
\begin{align}
& \frac{1}{2}\sup_{X\in\mathcal{L}(\mathcal{H})}\left\{  \operatorname{Tr}%
[X]+\operatorname{Tr}[X^{\dag}]:%
\begin{pmatrix}
\rho & X\\
X^{\dag} & \sigma
\end{pmatrix}
\geq0\right\}  \nonumber\\
& =\frac{1}{2}\sup_{K:\left\Vert K\right\Vert _{\infty}\leq1}\operatorname{Tr}%
[\sqrt{\rho}K\sqrt{\sigma}]+\operatorname{Tr}[\sqrt{\sigma}K^{\dag}\sqrt{\rho
}]\\
& =\sup_{K:\left\Vert K\right\Vert _{\infty}\leq1}\operatorname{Re}%
[\operatorname{Tr}[\sqrt{\rho}K\sqrt{\sigma}]]\\
& =\sup_{K:\left\Vert K\right\Vert _{\infty}\leq1}\left\vert \operatorname{Tr}%
[\sqrt{\rho}K\sqrt{\sigma}]\right\vert \\
& =\left\Vert \sqrt{\rho}\sqrt{\sigma}\right\Vert _{1}=\sqrt{F}(\rho,\sigma).
\end{align}
The first equality follows from Lemma~\ref{lem:QM-over:Bhatia-lemma-1}. The
third equality follows because we can use the optimization over $K$ to adjust
a global phase such that the real part is equal to the absolute value (here,
one should think of the fact that $\operatorname{Re}[z]=r\cos(\theta)$ for
$z=re^{i\theta}$, and then one can optimize the value of $\theta$ so that
$\operatorname{Re}[z]=r$). The final equality follows by a generalization of
Proposition~\ref{prop:math-tools:var-char-t-norm} (in fact the same proof given there implies that the optimization can
be with respect to $U$ satisfying $\left\Vert U\right\Vert _{\infty}\leq1$,
rather than just with respect to isometries).

We now prove that \eqref{eq:QM-over:fidelity-dual-SDP} is the dual program of
\eqref{eq:QM-over:fidelity-primal-SDP}. We can rewrite the primal SDP\ as%
\begin{equation}
\frac{1}{2}\sup\operatorname{Tr}[X]+\operatorname{Tr}[X^{\dag}]
\end{equation}
subject to%
\begin{equation}%
\begin{pmatrix}
\rho & 0\\
0 & \sigma
\end{pmatrix}
\geq%
\begin{pmatrix}
0 & X\\
X^{\dag} & 0
\end{pmatrix}
,\qquad%
\begin{pmatrix}
R & X\\
X^{\dag} & S
\end{pmatrix}
\geq0
\end{equation}
because $R$ and $S$ are not involved in the objective function and can always
be chosen so that the second operator is PSD. Also, the following equivalences
hold%
\begin{align}%
\begin{pmatrix}
\rho & X\\
X^{\dag} & \sigma
\end{pmatrix}
\geq0\quad &  \Longleftrightarrow\quad%
\begin{pmatrix}
\rho & -X\\
-X^{\dag} & \sigma
\end{pmatrix}
\geq0\\
&  \Longleftrightarrow\quad%
\begin{pmatrix}
\rho & 0\\
0 & \sigma
\end{pmatrix}
\geq%
\begin{pmatrix}
0 & X\\
X^{\dag} & 0
\end{pmatrix}
.
\end{align}


As given in \eqref{eq-primal_SDP_def} and \eqref{eq-dual_SDP_def}, the standard forms of primal and dual SDPs for Hermitian $A$ and $B$ and
Hermiticity-preserving map $\Phi$ are as follows:%
\begin{align}
&  \sup_{G\geq0}\left\{  \operatorname{Tr}[AG]:\Phi(G)\leq B\right\}  ,\\
&  \inf_{Y\geq0}\left\{  \operatorname{Tr}[BY]:\Phi^{\dag}(Y)\geq A\right\}  .
\end{align}


So the SDP\ above is in standard form with%
\begin{align}
G &  =%
\begin{pmatrix}
R & X\\
X^{\dag} & S
\end{pmatrix}
,\quad A=%
\begin{pmatrix}
0 & \mathbbm{1}\\
\mathbbm{1} & 0
\end{pmatrix}
,\\
\Phi(G) &  =%
\begin{pmatrix}
0 & X\\
X^{\dag} & 0
\end{pmatrix}
,\quad B=%
\begin{pmatrix}
\rho & 0\\
0 & \sigma
\end{pmatrix}
.
\end{align}
Setting%
\begin{equation}
Y=%
\begin{pmatrix}
W & V\\
V^{\dag} & Z
\end{pmatrix}
,
\end{equation}
the adjoint of $\Phi$ is given by%
\begin{align}
\operatorname{Tr}[Y\Phi(X)] &  =\operatorname{Tr}\left[
\begin{pmatrix}
W & V\\
V^{\dag} & Z
\end{pmatrix}%
\begin{pmatrix}
0 & X\\
X^{\dag} & 0
\end{pmatrix}
\right]  \\
&  =\operatorname{Tr}\left[
\begin{pmatrix}
VX^{\dag} & WX\\
ZX^{\dag} & V^{\dag}X
\end{pmatrix}
\right]  \\
&  =\operatorname{Tr}[VX^{\dag}]+\operatorname{Tr}[XV^{\dag}]\\
&  =\operatorname{Tr}\left[
\begin{pmatrix}
0 & V\\
V^{\dag} & 0
\end{pmatrix}%
\begin{pmatrix}
R & X\\
X^{\dag} & S
\end{pmatrix}
\right]  ,
\end{align}
so that%
\begin{equation}
\Phi^{\dag}(Y)=%
\begin{pmatrix}
0 & V\\
V^{\dag} & 0
\end{pmatrix}
.
\end{equation}
Then the dual is given by%
\begin{equation}
\frac{1}{2}\inf\operatorname{Tr}\left[
\begin{pmatrix}
\rho & 0\\
0 & \sigma
\end{pmatrix}%
\begin{pmatrix}
W & V\\
V^{\dag} & Z
\end{pmatrix}
\right]
\end{equation}
subject to%
\begin{equation}%
\begin{pmatrix}
0 & V\\
V^{\dag} & 0
\end{pmatrix}
\geq%
\begin{pmatrix}
0 & \mathbbm{1}\\
\mathbbm{1} & 0
\end{pmatrix}
,\qquad%
\begin{pmatrix}
W & V\\
V^{\dag} & Z
\end{pmatrix}
\geq0.
\end{equation}
This simplifies to%
\begin{equation}
\frac{1}{2}\inf\operatorname{Tr}[\rho W]+\operatorname{Tr}[\sigma Z],
\end{equation}
subject to%
\begin{equation}%
\begin{pmatrix}
0 & V\\
V^{\dag} & 0
\end{pmatrix}
\geq%
\begin{pmatrix}
0 & \mathbbm{1}\\
\mathbbm{1} & 0
\end{pmatrix}
,\qquad%
\begin{pmatrix}
W & V\\
V^{\dag} & Z
\end{pmatrix}
\geq0
\end{equation}
Since%
\begin{align}%
\begin{pmatrix}
W & V\\
V^{\dag} & Z
\end{pmatrix}
\geq0\quad &  \Longleftrightarrow\quad%
\begin{pmatrix}
W & -V\\
-V^{\dag} & Z
\end{pmatrix}
\geq0\\
&  \Longleftrightarrow\quad%
\begin{pmatrix}
W & 0\\
0 & Z
\end{pmatrix}
\geq%
\begin{pmatrix}
0 & V\\
V^{\dag} & 0
\end{pmatrix}
,
\end{align}
we find that there is a single condition%
\begin{equation}%
\begin{pmatrix}
W & 0\\
0 & Z
\end{pmatrix}
\geq%
\begin{pmatrix}
0 & V\\
V^{\dag} & 0
\end{pmatrix}
\geq%
\begin{pmatrix}
0 & \mathbbm{1}\\
\mathbbm{1} & 0
\end{pmatrix}
,
\end{equation}
and since $V$ plays no role in the objective function, we can set $V=\mathbbm{1}$. So
the final SDP\ simplifies as follows:%
\begin{equation}
\frac{1}{2}\inf_{W,Z}\operatorname{Tr}[\rho W]+\operatorname{Tr}[\sigma Z]
\end{equation}
subject to%
\begin{equation}%
\begin{pmatrix}
W & -\mathbbm{1}\\
-\mathbbm{1} & Z
\end{pmatrix}
\geq0.
\end{equation}
Using the fact that%
\begin{equation}%
\begin{pmatrix}
W & -\mathbbm{1}\\
-\mathbbm{1} & Z
\end{pmatrix}
\geq0\quad\Longleftrightarrow\quad%
\begin{pmatrix}
W & \mathbbm{1}\\
\mathbbm{1} & Z
\end{pmatrix}
\geq0
\end{equation}
we can do one final rewriting as follows:%
\begin{equation}
\frac{1}{2}\inf_{W,Z}\operatorname{Tr}[\rho W]+\operatorname{Tr}[\sigma Z]
\end{equation}
subject to%
\begin{equation}%
\begin{pmatrix}
W & \mathbbm{1}\\
\mathbbm{1} & Z
\end{pmatrix}
\geq0.
\end{equation}

\subsection{Proof of Proposition~\ref{prop:QM-over:SDP-fidelity-channels}}

\label{app:QM-over:SDP-fid-chs}

First, strong duality holds, according to Theorem~\ref{thm:math-tools:slater-cond}, because $Q_{RB} = 0$ and $\lambda = 0$ is feasible for the primal program, while $\rho_R = \mathbbm{1}/|R|$ and $W_{RB} = Z_{RB} = 2 \mathbbm{1}_{RB}$ is strictly feasible for the dual.

For a pure bipartite state
$\psi_{RA}$, we use \eqref{eq-pure_state_vec} to conclude that
\begin{equation}
\psi_{RA}=X_{R}\Gamma_{RA}X_{R}^{\dag},
\end{equation}
where $\operatorname{Tr}[X_{R}^{\dag}X_{R}]=1$ to see that
\begin{equation}
\mathcal{N}_{A\rightarrow B}(\psi_{RA})=X_{R}\Gamma_{RB}^{\mathcal{N}}
X_{R}^{\dag},\quad\mathcal{M}_{A\rightarrow B}(\psi_{RA})=X_{R}\Gamma
_{RB}^{\mathcal{M}}X_{R}^{\dag},
\end{equation}
and then plug in to \eqref{eq:QM-over:fidelity-dual-SDP}\ to get that
\begin{equation}
\sqrt{F}(\mathcal{N}_{A\rightarrow B},\mathcal{M}_{A\rightarrow B})=\frac
{1}{2}\inf_{W_{RB},Z_{RB}}\operatorname{Tr}[X_{R}\Gamma_{RB}^{\mathcal{N}
}X_{R}^{\dag}W_{RB}]+\operatorname{Tr}[X_{R}\Gamma_{RB}^{\mathcal{M}}
X_{R}^{\dag}Z_{RB}]
\end{equation}
subject to
\begin{equation}
\begin{pmatrix}
W_{RB} & \mathbbm{1}_{RB}\\
\mathbbm{1}_{RB} & Z_{RB}
\end{pmatrix}
\geq0. \label{eq:QM-over:ineq-const-dual-fid-states-SDP}
\end{equation}
Consider that the objective function can be written as
\begin{equation}
\operatorname{Tr}[\Gamma_{RB}^{\mathcal{N}}W_{RB}^{\prime}]+\operatorname{Tr}
[\Gamma_{RB}^{\mathcal{M}}Z_{RB}^{\prime}],
\end{equation}
with
\begin{equation}
W_{RB}^{\prime}\coloneqq X_{R}^{\dag}W_{RB}X_{R},\quad Z_{RB}^{\prime}\coloneqq X_{R}^{\dag
}Z_{RB}X_{R}
\end{equation}
Now consider that the inequality in
\eqref{eq:QM-over:ineq-const-dual-fid-states-SDP}\ is equivalent to
\begin{equation}
\begin{pmatrix}
X_{R} & 0\\
0 & X_{R}
\end{pmatrix}
^{\dag}
\begin{pmatrix}
W_{RB} & \mathbbm{1}_{RB}\\
\mathbbm{1}_{RB} & Z_{RB}
\end{pmatrix}
\begin{pmatrix}
X_{R} & 0\\
0 & X_{R}
\end{pmatrix}
\geq0 .
\end{equation}
(Here we have assumed that $X_R$ is invertible, but it suffices to do so for this optimization because the set of invertible $X_R$ is dense in the set of all possible~$X_R$.)
Multiplying out the last matrix we find that
\begin{align}
&
\begin{pmatrix}
X_{R} & 0\\
0 & X_{R}
\end{pmatrix}
^{\dag}
\begin{pmatrix}
W_{RB} & \mathbbm{1}_{RB}\\
\mathbbm{1}_{RB} & Z_{RB}
\end{pmatrix}
\begin{pmatrix}
X_{R} & 0\\
0 & X_{R}
\end{pmatrix}
\nonumber\\
&  =
\begin{pmatrix}
X_{R}^{\dag}W_{RB}X_{R} & X_{R}^{\dag}X_{R}\otimes \mathbbm{1}_{B}\\
X_{R}^{\dag}X_{R}\otimes \mathbbm{1}_{B} & X_{R}^{\dag}Z_{RB}X_{R}
\end{pmatrix}
\\
&  =
\begin{pmatrix}
W_{RB}^{\prime} & \rho_{R}\otimes \mathbbm{1}_{B}\\
\rho_{R}\otimes \mathbbm{1}_{B} & Z_{RB}^{\prime}
\end{pmatrix}
,
\end{align}
where we defined $\rho_{R}=X_{R}^{\dag}X_{R}$. Observing that $\rho_{R}\geq0$
and $\operatorname{Tr}[\rho_{R}]=1$, we can write the final SDP\ as follows:
\begin{equation}
\sqrt{F}(\mathcal{N}_{A\rightarrow B},\mathcal{M}_{A\rightarrow B})=\frac
{1}{2}\inf_{\rho_{R},W_{RB},Z_{RB}}\operatorname{Tr}[\Gamma_{RB}^{\mathcal{N}
}W_{RB}]+\operatorname{Tr}[\Gamma_{RB}^{\mathcal{M}}Z_{RB}],
\end{equation}
subject to
\begin{equation}
\rho_{R}\geq0,\quad\operatorname{Tr}[\rho_{R}]=1,\quad
\begin{pmatrix}
W_{RB} & \rho_{R}\otimes \mathbbm{1}_{B}\\
\rho_{R}\otimes \mathbbm{1}_{B} & Z_{RB}
\end{pmatrix}
\geq0. \label{eq:QM-over:ch-fid-SDP-constr}
\end{equation}


Now let us calculate the dual SDP\ to this, using the following standard forms
for primal and dual SDPs, with Hermitian operators $A$ and $B$ and a
Hermiticity-preserving map $\Phi$ (as given in \eqref{eq-primal_SDP_def} and \eqref{eq-dual_SDP_def}):
\begin{equation}
\sup_{X\geq0}\left\{  \operatorname{Tr}[AX]:\Phi(X)\leq B\right\}  ,\qquad
\inf_{Y\geq0}\left\{  \operatorname{Tr}[BY]:\Phi^{\dag}(Y)\geq A\right\}  .
\end{equation}
Consider that the constraint in \eqref{eq:QM-over:ch-fid-SDP-constr} implies
$W_{RB}\geq0$ and $Z_{RB}\geq0$, so that we can set
\begin{align}
Y  &  =
\begin{pmatrix}
W_{RB} & 0 & 0\\
0 & Z_{RB} & 0\\
0 & 0 & \rho_{R}
\end{pmatrix}
,\quad B=
\begin{pmatrix}
\Gamma_{RB}^{\mathcal{N}} & 0 & 0\\
0 & \Gamma_{RB}^{\mathcal{M}} & 0\\
0 & 0 & 0
\end{pmatrix}
,\\
\Phi^{\dag}(Y)  &  =
\begin{pmatrix}
W_{RB} & \rho_{R}\otimes \mathbbm{1}_{B} & 0 & 0\\
\rho_{R}\otimes \mathbbm{1}_{B} & Z_{RB} & 0 & 0\\
0 & 0 & \operatorname{Tr}[\rho_{R}] & 0\\
0 & 0 & 0 & -\operatorname{Tr}[\rho_{R}]
\end{pmatrix}
,\\
A  &  =
\begin{pmatrix}
0 & 0 & 0 & 0\\
0 & 0 & 0 & 0\\
0 & 0 & 1 & 0\\
0 & 0 & 0 & -1
\end{pmatrix}
.
\end{align}
Then with
\begin{equation}
X=
\begin{pmatrix}
P_{RB} & Q_{RB}^{\dag} & 0 & 0\\
Q_{RB} & S_{RB} & 0 & 0\\
0 & 0 & \lambda & 0\\
0 & 0 & 0 & \mu
\end{pmatrix}
\end{equation}
the map $\Phi$ is given by
\begin{align}
&  \operatorname{Tr}[X\Phi^{\dag}(Y)]\nonumber\\
&  =\operatorname{Tr}\left[
\begin{pmatrix}
P_{RB} & Q_{RB}^{\dag} & 0 & 0\\
Q_{RB} & S_{RB} & 0 & 0\\
0 & 0 & \lambda & 0\\
0 & 0 & 0 & \mu
\end{pmatrix}
\begin{pmatrix}
W_{RB} & \rho_{R}\otimes \mathbbm{1}_{B} & 0 & 0\\
\rho_{R}\otimes \mathbbm{1}_{B} & Z_{RB} & 0 & 0\\
0 & 0 & \operatorname{Tr}[\rho_{R}] & 0\\
0 & 0 & 0 & -\operatorname{Tr}[\rho_{R}]
\end{pmatrix}
\right] \nonumber\\
&  =\operatorname{Tr}[P_{RB}W_{RB}]+\operatorname{Tr}[Q_{RB}^{\dag}\left(
\rho_{R}\otimes \mathbbm{1}_{B}\right)  ]+\operatorname{Tr}[Q_{RB}(\rho_{R}\otimes
\mathbbm{1}_{B})]\nonumber\\
&  \qquad+\operatorname{Tr}[S_{RB}Z_{RB}]+\left(  \lambda-\mu\right)
\operatorname{Tr}[\rho_{R}]\nonumber\\
&  =\operatorname{Tr}[P_{RB}W_{RB}]+\operatorname{Tr}[S_{RB}Z_{RB}
]+\operatorname{Tr}[(\operatorname{Tr}_{B}[Q_{RB}+Q_{RB}^{\dag}]+\left(
\lambda-\mu\right)  \mathbbm{1}_{R})\rho_{R}]\nonumber\\
&  =\operatorname{Tr}\left[
\begin{pmatrix}
P_{RB} & 0 & 0\\
0 & S_{RB} & 0\\
0 & 0 & \operatorname{Tr}_{B}[Q_{RB}+Q_{RB}^{\dag}]+\left(  \lambda
-\mu\right)  \mathbbm{1}_{R}
\end{pmatrix}
\begin{pmatrix}
W_{RB} & 0 & 0\\
0 & Z_{RB} & 0\\
0 & 0 & \rho_{R}
\end{pmatrix}
\right]  .
\end{align}
So then
\begin{equation}
\Phi(X)=
\begin{pmatrix}
P_{RB} & 0 & 0\\
0 & S_{RB} & 0\\
0 & 0 & \operatorname{Tr}_{B}[Q_{RB}+Q_{RB}^{\dag}]+\left(  \lambda
-\mu\right)  \mathbbm{1}_{R}
\end{pmatrix}
.
\end{equation}
The primal is then given by
\begin{equation}
\frac{1}{2}\sup\operatorname{Tr}\left[
\begin{pmatrix}
0 & 0 & 0 & 0\\
0 & 0 & 0 & 0\\
0 & 0 & 1 & 0\\
0 & 0 & 0 & -1
\end{pmatrix}
\begin{pmatrix}
P_{RB} & Q_{RB}^{\dag} & 0 & 0\\
Q_{RB} & S_{RB} & 0 & 0\\
0 & 0 & \lambda & 0\\
0 & 0 & 0 & \mu
\end{pmatrix}
\right]  ,
\end{equation}
subject to
\begin{align}
\begin{pmatrix}
P_{RB} & 0 & 0\\
0 & S_{RB} & 0\\
0 & 0 & \operatorname{Tr}_{B}[Q_{RB}+Q_{RB}^{\dag}]+\left(  \lambda
-\mu\right)  \mathbbm{1}_{R}
\end{pmatrix}
&  \leq
\begin{pmatrix}
\Gamma_{RB}^{\mathcal{N}} & 0 & 0\\
0 & \Gamma_{RB}^{\mathcal{M}} & 0\\
0 & 0 & 0
\end{pmatrix}
,\\
\begin{pmatrix}
P_{RB} & Q_{RB}^{\dag} & 0 & 0\\
Q_{RB} & S_{RB} & 0 & 0\\
0 & 0 & \lambda & 0\\
0 & 0 & 0 & \mu
\end{pmatrix}
&  \geq0,
\end{align}
which simplifies to
\begin{equation}
\frac{1}{2}\sup\left(  \lambda-\mu\right)
\end{equation}
subject to
\begin{align}
P_{RB}  &  \leq\Gamma_{RB}^{\mathcal{N}},\\
S_{RB}  &  \leq\Gamma_{RB}^{\mathcal{M}},\\
\operatorname{Tr}_{B}[Q_{RB}+Q_{RB}^{\dag}]+\left(  \lambda-\mu\right)  \mathbbm{1}_{R}
&  \leq0,\\
\begin{pmatrix}
P_{RB} & Q_{RB}^{\dag}\\
Q_{RB} & S_{RB}
\end{pmatrix}
&  \geq0,\\
\lambda,\mu &  \geq0.
\end{align}
We can simplify this even more. We can set $\lambda^{\prime}=\lambda-\mu
\in\mathbb{R}$, and we can substitute $Q_{RB}$ with $-Q_{RB}$ without changing
the value, so then it becomes
\begin{equation}
\frac{1}{2}\sup\lambda^{\prime}
\end{equation}
subject to
\begin{align}
P_{RB}  &  \leq\Gamma_{RB}^{\mathcal{N}},\\
S_{RB}  &  \leq\Gamma_{RB}^{\mathcal{M}},\\
\lambda^{\prime}\mathbbm{1}_{R}  &  \leq\operatorname{Tr}_{B}[Q_{RB}+Q_{RB}^{\dag}],\\
\begin{pmatrix}
P_{RB} & -Q_{RB}^{\dag}\\
-Q_{RB} & S_{RB}
\end{pmatrix}
&  \geq0,\\
\lambda^{\prime}  &  \in\mathbb{R}.
\end{align}
We can rewrite
\begin{align}
\begin{pmatrix}
P_{RB} & -Q_{RB}^{\dag}\\
-Q_{RB} & S_{RB}
\end{pmatrix}
\geq0\quad &  \Longleftrightarrow\quad
\begin{pmatrix}
P_{RB} & Q_{RB}^{\dag}\\
Q_{RB} & S_{RB}
\end{pmatrix}
\geq0\\
&  \Longleftrightarrow\quad
\begin{pmatrix}
P_{RB} & 0\\
0 & S_{RB}
\end{pmatrix}
\geq
\begin{pmatrix}
0 & -Q_{RB}^{\dag}\\
-Q_{RB} & 0
\end{pmatrix}
\end{align}
We then have the simplified condition
\begin{equation}
\begin{pmatrix}
0 & -Q_{RB}^{\dag}\\
-Q_{RB} & 0
\end{pmatrix}
\leq
\begin{pmatrix}
P_{RB} & 0\\
0 & S_{RB}
\end{pmatrix}
\leq
\begin{pmatrix}
\Gamma_{RB}^{\mathcal{N}} & 0\\
0 & \Gamma_{RB}^{\mathcal{M}}
\end{pmatrix}
.
\end{equation}
Since $P_{RB}$ and $S_{RB}$ do not appear in the objective function, we can
set them to their largest value and obtain the following simplification
\begin{equation}
\frac{1}{2}\sup\lambda^{\prime}
\end{equation}
subject to
\begin{equation}
\lambda^{\prime}\mathbbm{1}_{R}\leq\operatorname{Tr}_{B}[Q_{RB}+Q_{RB}^{\dag}],\quad
\begin{pmatrix}
\Gamma_{RB}^{\mathcal{N}} & Q_{RB}^{\dag}\\
Q_{RB} & \Gamma_{RB}^{\mathcal{M}}
\end{pmatrix}
\geq0,\quad\lambda^{\prime}\in\mathbb{R}
\end{equation}
Since a feasible solution is $\lambda^{\prime}=0$ and $Q_{RB}=0$, it is clear
that we can restrict to $\lambda^{\prime}\geq0$. After a relabeling, this
becomes
\begin{multline}
\frac{1}{2}\sup_{\lambda\geq0,Q_{RB}}\left\{  \lambda:\lambda \mathbbm{1}_{R}
\leq\operatorname{Tr}_{B}[Q_{RB}+Q_{RB}^{\dag}],\quad
\begin{pmatrix}
\Gamma_{RB}^{\mathcal{N}} & Q_{RB}^{\dag}\\
Q_{RB} & \Gamma_{RB}^{\mathcal{M}}
\end{pmatrix}
\geq0\right\} \\
=\sup_{\lambda\geq0,Q_{RB}}\left\{  \lambda:\lambda \mathbbm{1}_{R}\leq\operatorname{Re}
[\operatorname{Tr}_{B}[Q_{RB}]],\quad
\begin{pmatrix}
\Gamma_{RB}^{\mathcal{N}} & Q_{RB}^{\dag}\\
Q_{RB} & \Gamma_{RB}^{\mathcal{M}}
\end{pmatrix}
\geq0\right\}  .
\end{multline}
This is equivalent to
\begin{equation}
\sup_{Q_{RB}}\left\{  \lambda_{\min}\left(  \operatorname{Re}
[\operatorname{Tr}_{B}[Q_{RB}]]\right)  :
\begin{pmatrix}
\Gamma_{RB}^{\mathcal{N}} & Q_{RB}^{\dag}\\
Q_{RB} & \Gamma_{RB}^{\mathcal{M}}
\end{pmatrix}
\geq0\right\}  .
\end{equation}
This concludes the proof.




\end{subappendices}





